Scattering Observables from Few-Body Densities and Application in Light Nuclei

The Transition Density Amplitude (TDA) method of Griesshammer et al. is applied to compute scattering observables for Compton scattering, threshold neutral pion photoproduction, and elastic pion scattering on the light nuclei Hydrogen 3, Helium 3, Helium 4, and Lithium 6. In this formalism the amplitude factorizes into an irreducible few-body kernel, which encodes the interaction of the probe with the active nucleons, and a transition density amplitude, which carries the nuclear structure information. Because the densities are computed once per nucleus and momentum transfer and then convolved with any process-specific kernel, the same nuclear input is reused across reactions, yielding substantial computational savings over direct evaluation. This factorization is realized in the publicly available Fortran suite DensityScattering, developed as part of the present work; a researcher implementing a new reaction need only supply the corresponding kernel in a prescribed format, with infrastructure for density handling, integration, quantum-number summation, and output already provided. The TDAs are constructed from nuclear wave functions using the semilocal momentum-space regularized chiral potential of Reinert, Krebs, and Epelbaum at cutoffs of 450 and 500 MeV. For Lithium 6, no-core shell model wave functions are evolved under a Similarity Renormalization Group (SRG) transformation; a back-transformation scheme ("SRG-And-Back"), co-developed for the present work, returns the densities to the physical momentum scale and thereby preserves the original chiral ordering. The induced uncertainty is validated against exact Helium 4 results at the 2% level, and convergence studies for Lithium 6 Compton scattering bound the residual uncertainty below 6%.

==> QCD/QCD.tex <==
%! TEX root = ../Dis-AlexanderLong.tex
\section{QCD and Its Relation to \texorpdfstring{$\chi$}{\chi}EFT}
\label{sec:QCD}
Having established the general principles of Effective
Field Theories in the preceding section, the discussion
now turns to the specific case of Quantum
Chromodynamics (QCD) and its low-energy effective
description through Chiral Effective Field Theory
(\chiEFT). This section develops the theoretical
foundation upon which the interaction kernels used
throughout the present work are constructed. No
original results are presented here; the material
serves to fix notation and to make the exposition
self-contained.

The presentation is organized as follows.
Section~\ref{sec:QCDLag} introduces the QCD
Lagrangian, its chiral symmetry in the massless
two-flavor limit, and the spontaneous breaking of
that symmetry, which gives rise to pions as
pseudo-Goldstone bosons via Goldstone's theorem.
Section~\ref{sec:chiralLag} constructs the first few terms in the 
effective chiral Lagrangian for pions and nucleons using the
external-source method.
Section~\ref{sec:truncation} introduces the general
concept of power counting and discusses the breakdown
scale, the cutoff scale, and the estimation of
truncation errors.
Section~\ref{sec:powercounting} presents the chiral
index as a first, concrete realization of the power
counting, and sec.~\ref{sec:weinbergPC} addresses the
subtleties that arise when the chiral potential is
iterated non-perturbatively in few-nucleon systems
via Weinberg's pragmatic approach. The resulting
hierarchy of two-, three-, and four-nucleon
interactions is presented in
sec.~\ref{sec:hierarchy}. Together, these elements
provide the systematic framework from which the
few-body interaction kernels for Compton scattering,
pion photoproduction, and pion scattering are derived
in the subsequent chapters.
\subsection{The QCD Lagrangian}
\label{sec:QCDLag}
The presentation in this section draws from
Bernard \etal~\cite{BERNARD_1995},
Machleidt \etal~\cite{chiEFT},
Rijneveen~\cite{rij}, and Braun~\cite{BraunThesis}.
Quantum Chromodynamics (QCD) is the fundamental
theory of the strong interaction. It is formulated as
a non-Abelian gauge theory with local
$SU(3)_{\mathrm{color}}$ symmetry, in which quarks
interact through the exchange of gluons. Its
Lagrangian takes the form
\begin{equation}
  \LL_{\mathrm{QCD}}=\bar{q}\left(i \fs{\mathcal{D}}-\mathcal{M}\right) q-\frac{1}{4} \mathcal{G}_{\mu \nu, a} \mathcal{G}_a^{\mu \nu}.
\end{equation}
The quark fields are collected in the flavor vector
$q=(u,d,s,c,b,t)^T$,
and the Feynman slash notation has been used,
$\slashed{\mathcal{D}}=\gamma^\mu \mathcal{D}_\mu$,
where $\gamma_\mu$ denote the Dirac matrices and
$\mathcal{D}_\mu$ is the gauge covariant derivative
\begin{equation}
  \mathcal{D}_\mu=\partial_\mu-i g \frac{\lambda_a}{2}
  \mathcal{A}_{\mu, a}\,.
\end{equation}
Here, $\lambda_a$ are the Gell-Mann matrices see \meqref{eq:GellMann}, which
serve as generators of $SU(3)_{\mathrm{color}}$.
The quark mass matrix is $\mathcal{M}=\mathrm{diag}(m_u,m_d,m_s,...)$.
$\mathcal{A}_{\mu,a}$ is the $a^{\text{th}}$ component of the gluon field, and the gluon field strength tensor $\mathcal{G}_{\mu\nu,a}$ is
\begin{equation}
  \mathcal{G}_{\mu \nu, a}=\partial_\mu \mathcal{A}_{\nu, a}-\partial_\nu \mathcal{A}_{\mu, a}+g f_{a b c} \mathcal{A}_{\mu, b} \mathcal{A}_{\nu, c}\;.
\end{equation}
The quantity $g$ denotes the (energy-dependent) strong
coupling constant.
The structure constants $f_{abc}$ of $SU(3)_{\mathrm{color}}$
arise from the Hermitian and traceless generators $T_a=\lambda_a/2$ via the
Lie algebra relation, and normalization
\begin{equation}
  \left[ T^a,T^b \right]= i f^{abc} T^c,\qquad 2\, \Tr[T^a T^b]= \delta^{ab}.
\end{equation}
where $\lambda_a$ are the Gell-Mann matrices, see~\meqref{eq:GellMann} for a definition.
The up and down quarks are the lightest of the six flavors
and constitute the valence content of nucleons.
Their current masses, evaluated at a renormalization
scale $\mu = 2\,\GeV$ in the
$\overline{\mathrm{MS}}$ scheme, are~\cite{PDG}
\begin{equation}
  \begin{split}
  m_u & =\left[2.16 \pm 0.07 \right]\MeV\,,\\
  m_d & =\left[4.70 \pm 0.02\right] \MeV\,.
  \end{split}
\end{equation}
These masses are small compared to typical hadronic
scales of order $1\,\GeV$, such as the mass of the
$\rho$ meson ($m_\rho \approx 770\,\MeV$). The precise
identification of the hard scale governing the chiral
expansion is discussed in
sec.~\ref{sec:truncation}.
It is therefore a useful
approximation to consider the chiral limit
$\mathcal{M}\to 0$. This yields
\begin{equation}
  \LL_{\mathrm{QCD}}^0=\bar{q} i \fs{\mathcal{D}} q-\frac{1}{4} \mathcal{G}_{\mu \nu, a} \mathcal{G}_a^{\mu \nu}.
\end{equation}
Restricting to the two lightest flavors, let
$q=(u,\,d)^T$ and decompose the quark fields into
left- and right-handed components, one finds:
\begin{align}
q & =\frac{1}{2}\left(1-\gamma_5\right) q+\frac{1}{2}\left(1+\gamma_5\right) q\nonumber \\
& =P_L q+P_R q \\
& =q_L+q_R.\nonumber
\end{align}
Here $\gamma_5=i\gamma^0\gamma^1\gamma^2\gamma^3$,
and the chiral projectors are
$P_R=\frac{1}{2}(1+\gamma_5)$ and
$P_L=\frac{1}{2}(1-\gamma_5)$, satisfying
$P_R+P_L=\one$ and $P_L P_R = 0$.
Substituting these projections, the massless
Lagrangian separates into independent left- and
right-handed contributions which do not mix:
\begin{equation}
  \LL_{\mathrm{QCD}}^0=-\frac{1}{4} \mathcal{G}_a^{\mu \nu} \mathcal{G}_{a, \mu \nu}+\bar{q}_L \mathrm{i} \fs{\mathcal{D}} q_L+\bar{q}_R \mathrm{i} \fs{\mathcal{D}} q_R\;.
\end{equation}
For massless up and down quarks,
$\LL_{\mathrm{QCD}}^0$ is invariant under
global $SU(2)$ rotations of the left-
and right-handed components given by
\begin{equation}
  q_{R/L} \longmapsto \exp\!\left(-i
  \Theta_i^{R/L} \frac{\tau_i}{2}\right) q_{R/L}
  \qquad i=1,2,3\,,
\end{equation}
where $\tau_i$ denote the Pauli matrices acting in
flavor space and the parameters
$\Theta_i^{R,L}$ specify the transformation.
The key consequence is that left- and right-handed quark
fields transform independently under $SU(2)_L$ and
$SU(2)_R$, respectively: the two chiralities do not mix,
and the massless Lagrangian possesses an
$SU(2)_L \times SU(2)_R$ chiral symmetry. This
independence of the left- and right-handed sectors is the
defining feature of chiral symmetry.
By Noether's theorem, this symmetry implies separately conserved right-handed ($R$) and left-handed ($L$) currents:
\begin{align}
  R_i^\mu&=\bar{q}_R \gamma^\mu \frac{\tau_i}{2} q_R \quad \text { with } \quad \partial_\mu R_i^\mu=0\\
  L_i^\mu&=\bar{q}_L \gamma^\mu \frac{\tau_i}{2} q_L \quad \text { with } \quad \partial_\mu L_i^\mu=0\;.
\end{align}
It is convenient to define the vector ($V$) and
axial ($A$) combinations of these currents:
\begin{align}
  V_i^\mu&=R_i^\mu+L_i^\mu=\bar{q} \gamma^\mu \frac{\tau_i}{2} q \quad \text { with } \quad \partial_\mu V_i^\mu=0\\
  A_i^\mu&=R_i^\mu-L_i^\mu=\bar{q} \gamma^\mu \gamma_5 \frac{\tau_i}{2} q \quad \text { with } \quad \partial_\mu A_i^\mu=0.
\end{align}
The vector transformations acting on the full quark field take the form
\begin{equation}
  q=\binom{u}{d} \longmapsto \exp \left(-i \Theta_i^V \frac{\tau_i}{2}\right)\binom{u}{d},
  \label{eq:isospin_rotation}
\end{equation}
which is an isospin rotation, therefore invariance under vector transformations can be identified with this isospin symmetry.
There are six conserved Noether charges $Q_i^{L/R}$
\begin{equation}
\begin{split}
  Q_i^R&= \int \dd^3 x \,R_i^0= \int \dd^3 x \,q_{_{R}}^\dag(t,\vec{x}) \frac{\tau_i}{2} q_{_{R}}(t,\vec{x}) \quad\text{and}\quad \frac{d Q_i^{^{R}}}{dt}=0 \\
  Q_i^L&= \int \dd^3 x \,L_i^0= \int \dd^3 x \,q_{_{L}}^\dag(t,\vec{x}) \frac{\tau_i}{2} q_{_{L}}(t,\vec{x}) \quad\text{and}\quad \frac{d Q_i^{^{L}}}{dt}=0\;,
\end{split}
\end{equation}
or alternatively in terms of $A$  and $V$
\begin{equation}
\label{AVGeners}
\begin{split}
Q_i^{V}&= \int \dd^3 x\, V_i^0
  = \int \dd^3 x \,q^\dag(t,\vec{x})
  \frac{\tau_i}{2} q(t,\vec{x})
  \quad\text{and}\quad
  \frac{d Q_i^{V}}{dt}=0 \\
  Q_i^{A}&= \int \dd^3 x\, A_i^0
  = \int \dd^3 x \,q^\dag(t,\vec{x})
  \gamma_5 \frac{\tau_i}{2} q(t,\vec{x})
  \quad\text{and}\quad
  \frac{d Q_i^{A}}{dt}=0\;.
\end{split}
\end{equation}
The $L$ and $R$ currents satisfy the $SU(2)_R\times SU(2)_L$ Lie algebra relations
\begin{equation}
  \left[Q_i^R, Q_j^R\right]=i \epsilon^{i j k} Q_k^R, \quad\left[Q_i^L, Q_j^L\right]=i \epsilon^{i j k} Q_k^L, \quad\left[Q_i^R, Q_j^L\right]=0\;,
\end{equation}
whereas the $V$ and $A$ charges satisfy
\begin{equation}
  \label{chargeEQ}
  \left[Q_i^V, Q_j^V\right]=i \epsilon^{i j k} Q_k^V, \quad\left[Q_i^A, Q_j^A\right]=i \epsilon^{i j k} Q_k^V, \quad\left[Q_i^V, Q_j^A\right]=i \epsilon^{i j k} Q_k^A\;.
\end{equation}
%%% BEGIN MATERIAL MOVED FROM "Continued" SUBSECTION %%%
The commutation relations in~\meqref{chargeEQ}
encode the full algebraic content of the chiral
symmetry and allow the symmetry group of the
massless two-flavor QCD Lagrangian to be identified.
From \meqref{chargeEQ}, the full symmetry group is
$SU(2)_R \times SU(2)_L \times U(1)_V \times U(1)_A$.
The $U(1)_V$ symmetry corresponds to baryon number
conservation. The $U(1)_A$ symmetry, by contrast, is
not realized in the quantum theory: it is explicitly
violated by the axial anomaly~\cite{Adler1969} and
therefore does not give rise to a Goldstone boson.
In the physical case of non-zero quark masses, the mass
term in $\LL_{QCD}$ breaks these symmetries:
\begin{equation}
  \LL_{QCD}=\LL^0_{QCD}+\LL_{SB} \quad\text{and}\quad \LL_{SB}=\bar{q}\mathcal{M}q\;.
\end{equation}
Restricting to the two lightest quark flavors, $u$ and $d$,
which are the relevant degrees of freedom for pions and
nucleons, the mass matrix takes the form
\begin{align}
  \mathcal{M}&=\left(\begin{array}{cc}
m_u & 0 \\
0 & m_d
\end{array}\right)= \frac{1}{2} (m_u+m_d) I+ \frac{1}{2} \left( m_u -m_d \right) \tau_3\;.
\label{massmatrix}
\end{align}
In the limit of equal quark masses, $m_u-m_d=0$, the
last term vanishes and an additional $SU(2)$ symmetry
emerges, known as isospin symmetry,
$q\to V_I q,\, V_I \in SU(2)$.

The chiral symmetry that emerges in the limit
$\mathcal{M}\to 0$ is much more accurately realized
than isospin symmetry. The relevant expansion parameter
for explicit chiral symmetry breaking is
$m_q/m_\rho \sim
\text{few}\,\MeV\,/\,770\,\MeV \sim 10^{-2}$,
where $m_\rho$ is used as a representative hadronic
scale. By comparison, the isospin-breaking parameter is
$(m_u - m_d)/(m_u + m_d) \approx 0.37$.
The full chiral symmetry generated by the charges
in~\meqref{AVGeners} is, however, not manifest in the
observed hadron spectrum.
The axial charge $Q_i^A$ has negative parity and commutes
with the Hamiltonian; one would naively expect that for
every hadron of positive parity there exists a
corresponding state with very similar properties (mass,
spin, etc.) but negative parity. Such parity doublets,
however, are not observed at low energy.

Consider, for example, the $\rho$ meson with quantum
numbers $J^P=1^-$; the near-degeneracy of
$\rho^{\pm}$ and $\rho^0$ confirms that the vector
symmetry $SU(2)_V$ is well realized. However, the
lightest meson with $J^P=1^+$, the $a_1(1260)$, has
a mass approximately $500\,\MeV$ above the $\rho$,
far too large for these states to be considered
degenerate. This indicates that the axial part of
the chiral symmetry is not realized in the
Wigner--Weyl mode but is instead
\textit{spontaneously broken}.
The connection between spontaneously broken symmetries
and the appearance of light particles in the spectrum is
made precise by Goldstone's theorem.

\subsection{Digression: Goldstone's Theorem}
\label{sec:goldstone}
Goldstone's theorem~\cite{Goldstone1961, Goldstone} states that for
every generator of a continuous symmetry that is
spontaneously broken, the spectrum of the theory must
contain a massless spin-zero particle, with the quantum numbers of the broken symmetry, termed a Goldstone
boson. The following proof for the case of classical
scalar fields follows ref.~\cite{PeskinSchroeder}. As a
preliminary, recall that in a Lagrangian such
as~\meqref{linter}, the coefficients of the quadratic
terms in the fields are proportional to the squared
masses of the respective particles, denoted $m_\phi$ and
$m_\psi$.
Now consider a theory with $a=1...n$ classical fields, represented as $\varphi^a$.
The Lagrangian is then given by
\begin{equation}
  \label{LPoten}
  \LL= (\text{terms with derivatives}) -V(\varphi)\;,
\end{equation}
where $V(\varphi)$ includes the mass terms. Let $\varphi_0\ne0$ be a constant field that minimizes $V$:
\begin{equation}
 \left.\frac{\partial}{\partial \varphi^a} V\right|_{\varphi(x)=\varphi_0}=0\;.
\end{equation}
Performing a Taylor expansion about this minimum yields
\begin{equation}
  V(\varphi)=V\left(\varphi_0\right)+\frac{1}{2} \sum_{a, b}\left(\varphi-\varphi_0\right)^a\left(\varphi-\varphi_0\right)^b\left.\left(\frac{\partial^2}{\partial \varphi^a \partial \varphi^b} V\right)\right|_{\varphi=\varphi_0}+\ldots.
\end{equation}
The coefficient
\begin{equation}
  \left.\left(\frac{\partial^2}{\partial \varphi^a \partial \varphi^b} V\right)\right|_{\varphi^a=\varphi^a_0}= m_{ab}^2
\end{equation}
can be interpreted as a symmetric matrix whose eigenvalues are the masses of the fields.
The goal is to show that every continuous symmetry of
the Lagrangian~\meqref{LPoten} that is not a symmetry
of $\varphi^a_0$
gives rise to a zero eigenvalue in the mass matrix.
A general continuous symmetry has the form 
\begin{equation}
  \varphi^a \to \varphi^a + \alpha \Delta^a(\varphi)\;,
\end{equation}
where $\alpha$ is an infinitesimal parameter, $\Delta^a$
is some function of the fields, and \meqref{LPoten} is
invariant under this transformation.
In the case of constant fields, the derivative terms vanish and the potential alone must be invariant.
\begin{equation}
V\left(\varphi^a\right)=V\left(\varphi^a+\alpha \Delta^a(\varphi)\right)\quad \text { or }\quad \sum_a \Delta^a(\varphi) \frac{\partial}{\partial \varphi^a} V(\varphi)=0 .
\end{equation}
Taking the derivative with respect to $\varphi^b$ and evaluating at $\varphi=\varphi_0$ gives
\begin{equation}
0=\left(\frac{\partial \Delta^a}{\partial \varphi^b}\right)_{\varphi_0}\left.\left(\frac{\partial V}{\partial \varphi^a}\right)_{\varphi_0}+\Delta^a\left(\varphi_0\right)\left(\frac{\partial^2}{\partial \varphi^a \partial \varphi^b} V\right)\right|_{\varphi=\varphi_0} .
\end{equation}
In the above, the first term vanishes since $\varphi_0$ is a minimum of $V$, so the second term must also vanish.
A spontaneously broken symmetry is one where $\Delta^a(\varphi_0)\ne0$, 
that is, the symmetry is not respected by the ground state. 
It follows that
\begin{equation}
  0=m_{ab}^2=\left.\left(\frac{\partial^2}{\partial \varphi^a \partial \varphi^b} V\right)\right|_{\varphi=\varphi_0}.
\end{equation}
With this result in hand, the consequences for QCD can
now be stated directly.
By Goldstone's theorem~\cite{Goldstone}, each broken
generator gives rise to a massless boson carrying
the quantum numbers of that generator.
The chiral symmetry $SU(2)_L\times SU(2)_R$ is broken
down to the vector subgroup $SU(2)_V$.
Since the vacuum preserves the vector subgroup
$SU(2)_V$, the number of broken generators, and
hence the number of Goldstone bosons, is
\begin{equation}
  \underbrace{\dim\bigl(SU(2)_L \times SU(2)_R\bigr)}_{
  2\times(2^2-1)=6}
  - \underbrace{\dim\bigl(SU(2)_V\bigr)}_{2^2-1=3}
  = 3\,.
\end{equation}
The broken generators are the axial charges $Q_i^A$,
which have negative parity and form an isospin
triplet ($i=1,2,3$); the three Goldstone bosons
must therefore be pseudoscalar and carry isospin one:
$I(J^P)=1(0^-)$. These are identified with the
three pions ($\pi^+$, $\pi^-$, $\pi^0$).
The physical pion masses are not exactly zero because
the quark masses are not exactly zero; the explicit
breaking of chiral symmetry by the mass
term~\meqref{massmatrix} shifts the Goldstone bosons
to small but nonvanishing masses, making them
\textit{pseudo-Goldstone bosons}. The pions are
therefore simultaneously a manifestation of both
spontaneous and explicit chiral symmetry breaking
and are the lightest hadrons precisely because of
this dual role.
A key property of Goldstone bosons is that their
interactions vanish at zero momentum transfer and in
the chiral limit $\mpi\to 0$. This can be understood
intuitively: Goldstone bosons are excitations along
the flat directions of the potential, and a spatially
uniform rotation along such a direction costs no
energy. Only when the field configuration varies in
space, \textit{i.e.} when derivatives (and hence
momenta) are nonzero, do interactions arise. This
observation is the foundation of the systematic
low-energy expansion that constitutes chiral
perturbation theory, which is the subject of the
following section.

\subsection{The Chiral Effective Lagrangian}
\label{sec:chiralLag}
The next step is the construction of an effective
Lagrangian $\LL^{\mathrm{eff}}$ that respects the
symmetries of QCD. A central requirement is that the
Green functions of the effective theory satisfy the same
Ward identities as those of QCD. Ward identities are
exact relations among Green functions that express, at
the quantum level, the consequences of a symmetry of
the Lagrangian; they are the generating-functional
counterpart of the classical Noether
conservation laws. In the chiral context, these
identities constrain the correlation functions of the
vector and axial-vector quark currents and encode both
the conserved and the partially conserved (PCAC)
structure of QCD. Any effective theory that reproduces
the generating functional of QCD at low energies
inherits these constraints order by order in the
low-energy expansion.

The generating functional itself is defined through the
vacuum-to-vacuum transition amplitude in the presence
of external fields,
%
\begin{equation}
  \mathrm{exp}\left(i\mathcal{Z}[v,a,s,p]\right)
  = \langle 0\,\text{out} | 0\,\text{in} \rangle_{v,a,s,p}
  \;,\label{eq:functional}
\end{equation}
%
where $Z[v,a,s,p]$ is a functional of the external
source fields introduced
below~\cite{GASSER1988,BERNARD_1995}. Green functions
of the quark currents and densities are obtained by
taking functional derivatives of $Z$ with respect to
the appropriate sources. To construct $\mathcal{Z}$ while
preserving the chiral Ward identities, it is convenient
to employ the external-source method, in which external
vector ($v_\mu$), axial-vector ($a_\mu$), scalar ($s$),
and pseudoscalar ($p$) fields are coupled to the quark
bilinears in the QCD
Lagrangian~\cite{GASSER1988,BERNARD_1995}.
The external-source method provides a systematic
procedure for deriving the Ward identities that
constrain the form of the effective Lagrangian. By
coupling external fields to the conserved currents
of QCD, one can identify the transformation properties
that the effective theory must reproduce.
The vector source $v_\mu$ encodes couplings to the
photon field and the vector parts of the $W^\pm$ and
$Z^0$ bosons; the axial-vector source $a_\mu$ encodes
the axial couplings of the weak gauge bosons; the
scalar source $s$ incorporates the quark mass matrix
and additional scalar couplings such as those relevant
to the pion--nucleon sigma term; and the pseudoscalar
source $p$ couples to the pseudoscalar quark density,
entering processes such as pion absorption and
production through the divergence of the axial current.
With these external fields, one constructs a generating
functional that is invariant under local
$SU(2)_L \times SU(2)_R$ transformations, provided each
source field transforms according to the prescription
dictated by the local chiral
symmetry~\cite{BERNARD_1995}. Because the generating
functional respects the local chiral symmetry by
construction, the Green functions obtained from it
satisfy the chiral Ward identities at every order in
the low-energy expansion.

The physical content of the external sources is
recovered through specific substitutions once the
effective Lagrangian has been constructed. The quark
mass matrix $\calM$ enters through the scalar source
via $s = \calM$, providing a controlled means of
introducing explicit chiral symmetry breaking. The
electromagnetic interaction, central to the Compton
scattering and pion photoproduction processes studied in
the present work, enters through the vector source
$v_\mu$, which is set equal to the photon field
$e\calQ A_\mu$, where
$\calQ = \frac{1}{2}(\tau_3 + \frac{1}{3})$ is the
quark charge matrix. With these identifications, the
QCD Lagrangian in the presence of external sources
takes the form 
\begin{equation}
  \LL_{\mathrm{QCD}}=\LL_{\mathrm{QCD}}^0
  +\bar{q}\left(\fs{v}+\gamma_5\fs{a} 
  -s+\mathrm{i} p\gamma_5\right) q\;.
\end{equation}
In the path integral formulation, the generating functional \meqref{eq:functional} is given by
\begin{equation}
  \exp (i \mathcal{Z}[v, a, s, p])=\int\left[D G_\mu\right][D q][D \bar{q}] \exp \left(i \int d^4 x \LL_{\mathrm{QCD}}\left[q, \bar{q}, G_\mu ; v, a, s, p\right]\right).
\end{equation}
To formally pass to the effective theory, an integral is performed
over the quark and gluon fields, yielding the generating functional
\begin{equation}
  \exp (i \mathcal{Z}[v, a, s, p])=\int[D U] \exp \left(i \int d^4 x \LL^{\mathrm{eff}}[U ; v, a, s, p]\right),
  \label{pathInte_eff}
\end{equation}
where $U\in SU(2)_{\text{flavor}}$ is a unitary
matrix that collects the pion fields identified as
the pseudo-Goldstone bosons of the spontaneously
broken chiral symmetry in
sec.~\ref{sec:goldstone}.
Denoting the pion fields by $\pi_i(x)$, a general parameterization of $U$ reads
\begin{align}
  U(x)&=1+\frac{i}{f_\pi} \vec{\tau} \cdot \vec{\pi}-\frac{1}{2 f_\pi^2} \vec{\pi}^2-\frac{i \alpha}{f_\pi^3}(\vec{\tau} \cdot \vec{\pi})^3+\frac{8 \alpha-1}{8 f_\pi^4} \vec{\pi}^4+\ldots\;.
  \label{eq:param}
\end{align}
The parameter $\alpha \in \mathbb{R}$ is
parameterization-dependent and does not affect physical
observables. 
A common choice is the exponential parameterization,
\begin{equation}
  U(x)=\exp \left\{\mathrm{i} \frac{\vec{\tau} \cdot \vec{\pi}}{f_\pi}\right\}\;,
\end{equation}
which corresponds to $\alpha=1/6$.
The relevant low-energy degrees of freedom are
pions and nucleons. Following
Weinberg~\cite{phenomLag}, the most general
effective Lagrangian consistent with the
symmetries of QCD can be organized as
\begin{equation}
  \LL^{\mathrm{eff}}= \LL^{\mathrm{eff}}_{\pi\pi}+\LL^{\mathrm{eff}}_{\pi N}+\ldots\;. \label{Leff}
\end{equation}
The term $\LL^{\mathrm{eff}}_{\pi\pi}$ describes pion-pion interactions, while $\LL^{\mathrm{eff}}_{\pi N}$ describes pion-nucleon interactions.
An additional term $\LL^{\mathrm{eff}}_{NN}$, describing
short-range nucleon-nucleon contact interactions, does
not enter the scattering processes considered in
the present work (except indirectly through the nuclear
potential, see sec.~\ref{sec:SRG}) and is omitted hereafter.
Each of these may be expanded in powers of
derivatives and the pion mass, with the
superscript denoting the chiral order:
\begin{equation}
  \begin{split}
  \LL_{\pi \pi}^{\mathrm{eff}}&=\LL_{\pi \pi}^{(0)}+\LL_{\pi \pi}^{(2)}+\LL_{\pi \pi}^{(4)}+\ldots\\
  \LL_{\pi N}^{\mathrm{eff}}&=\LL_{\pi N}^{(1)}+\LL_{\pi N}^{(2)}+\LL_{\pi N}^{(3)}+\ldots\;.
  % \LL_{NN}^{\mathrm{eff}}&=\LL_{N N}^{(0)}+\LL_{N N}^{(2)}+\LL_{N N}^{(4)}+\ldots
  \end{split}
\end{equation}
The superscripts label the number of derivatives and
pion-mass insertions. The precise sense in which
higher-order terms are systematically suppressed is
governed by a power-counting scheme, which is
developed in sec.~\ref{sec:powercounting}.
Turning now to the explicit form of each term,
at zeroth order the only available structure is
$\Tr(U U^\dag)$, which reduces to a constant by the
unitarity of $U$ and therefore contributes no dynamics.
The leading nontrivial contribution arises at
second order in derivatives:
\begin{equation}
  \LL_{\pi \pi}^{(2)}=\frac{f_\pi^2}{4} \Tr\left[\partial_\mu U \partial^\mu U^{\dagger}+m_\pi^2\left(U+U^{\dagger}\right)\right]\;,
  \label{LLtwo}
\end{equation}
where $\Tr$ denotes the trace in flavor space.
The term $m_\pi^2(U+U^\dag)$ breaks chiral symmetry due to $m_\pi\neq0$.
Expanding \meqref{LLtwo} in powers of the pion field yields
the interaction terms from which Feynman rules can be
derived:
\begin{equation}
  \begin{split}
\LL_{\pi \pi}^{(2)}= & \frac{1}{2} \partial_\mu \vec{\pi} \cdot \partial^\mu \vec{\pi}-\frac{1}{2} m_\pi^2 \vec{\pi}^2 \\
& +\frac{1-4 \alpha}{2 f_\pi^2}\left(\vec{\pi} \cdot \partial_\mu \vec{\pi}\right)\left(\vec{\pi} \cdot \partial^\mu \vec{\pi}\right)-\frac{\alpha}{f_\pi^2} \vec{\pi}^2 \partial_\mu \vec{\pi} \cdot \partial^\mu \vec{\pi}+
\frac{8 \alpha-1}{8 f_\pi^2} m_\pi^2 \vec{\pi}^4+ \mathcal{O}(\vec{\pi}^6)\;.
\end{split}
\end{equation}
The baryonic degrees of freedom relevant to this work are
the proton ($p$) and neutron ($n$), and their dependence is captured in $\Psi$, the
relativistic four-component Dirac spinor field representing the nucleon.
The leading-order pion-nucleon Lagrangian is then
\begin{equation}
  \LL_{\pi N}^{(1)}=\bar{\Psi}\left(i \fs{D}-m_N+\frac{g_A}{2}  \gamma^\mu \gamma_5 u_\mu\right) \Psi\;.
\end{equation}
Here, the $\gamma^\mu$ are the $4\times 4$ Dirac
matrices acting on the spinor components of $\Psi$.
Although the Lagrangian is written in relativistic
form, the heavy-baryon reduction to two-component
spinors is implicit in the identification of $\Psi$
above and is carried out systematically in the
non-relativistic expansion; see
Machleidt~\etal~\cite{chiEFT} for details.
where $D_\mu = \p_\mu +\Gamma_\mu$ and
\begin{align}%This is correct, leave as is, see chiralEFT-Review-1.pdf, Machleidt etal
\Gamma_\mu & =\frac{1}{2}\left[\xi^{\dagger}, \partial_\mu \xi\right]=\frac{1}{2}\left(\xi^{\dagger} \partial_\mu \xi+\xi \partial_\mu \xi^{\dagger}\right) \\
& =\frac{i}{4 f_\pi^2} \vec{\tau} \cdot\left(\vec{\pi} \times \partial_\mu \vec{\pi}\right)+\mathcal{O}\left(\vec{\pi}^4\right)\;,
\end{align}
with
\begin{equation}
  \xi=\sqrt{U}=1+\frac{i}{2 f_\pi} \vec{\tau} \cdot \vec{\pi}-\frac{1}{8 f_\pi^2} \vec{\pi}^2-\frac{i(8 \alpha-1)}{16 f_\pi^3}(\vec{\tau} \cdot \vec{\pi})^3+\ldots\;,
\end{equation}
and $u_\mu$ is defined by
\begin{equation}
  u_\mu=i\left\{\xi^{\dagger}, \partial_\mu \xi\right\}=i\left(\xi^{\dagger} \partial_\mu \xi-\xi \partial_\mu \xi^{\dagger}\right).
\end{equation}
Combining the above, the leading-order pion-nucleon
Lagrangian takes the form
\begin{equation}
  \LL_{\pi N}^{(1)}=\bar{\Psi}\left(i \fs{\p}-m_N-\frac{1}{4 f_\pi^2} \gamma^\mu \vec{\tau} \cdot\left(\vec{\pi} \times \p_\mu \vec{\pi}\right)-\frac{g_A}{2 f_\pi} \gamma^\mu \gamma_5 \vec{\tau} \cdot \p_\mu \vec{\pi}+\ldots\right) \Psi\;,
 \label{eq:LpiN1expanded}
\end{equation}
where $g_A \approx 1.27$ is the nucleon axial-vector
coupling constant.
 Reading from left to right, the
first two terms encode the free, relativistic, propagation of a
nucleon with mass $m_N$; the third term, proportional
to $\vec{\tau}\cdot(\vec{\pi}\times\p_\mu\vec{\pi})$,
is the isovector Weinberg--Tomozawa seagull vertex
describing the scattering of a pion off a nucleon; and the fourth
term, proportional to $g_A$, is the pseudovector
pion--nucleon coupling through which a nucleon emits
or absorbs a single pion. The ellipsis denotes terms
with additional pion fields that arise from expanding
$\Gamma_\mu$ and $u_\mu$ to higher orders in
$\vec{\pi}/f_\pi$. 
One can show that with these definitions $\LL_{\pi N}$ is invariant under chiral transformations.
Further details and examples of extension
to higher chiral orders can be found in
Machleidt \etal~\cite{chiEFT} and
Bernard \etal~\cite{BERNARD_1995}.
In practice, the infinite tower of interactions
in~\eqref{Leff} must be organized by a systematic
power-counting scheme. That is the subject of the
following subsections.


\subsection{Power Counting, and Breakdown Scale}
\label{sec:truncation}

The presentation in this and the following subsections
closely follows the review by Machleidt and
Entem~\cite{chiEFT}.
The predictive power of any EFT rests on a
systematic ordering of contributions by their
importance, a procedure known as \emph{power counting}.
The power-counting scheme assumes that successive
orders are suppressed by powers of the small,
dimensionless expansion parameter
\begin{equation}
  Q \;=\; \frac{\ptyp}{\Lambda_b}\,,
  \label{eq:Qdef}
\end{equation}
where $\ptyp$ denotes a typical soft momentum
scale of the process (external momenta or $\mpi$) and
$\Lambda_b$ is the breakdown scale of the EFT, above
which the effective description ceases to be valid.
The breakdown scale $\Lambda_b$ is related to, but
conceptually distinct from, the chiral symmetry
breaking scale $\Lambda_\chi$ introduced earlier; its
precise value is discussed below.
Taking $\ptyp \sim \mpi \approx 134\,\MeV$ and
$\Lambda_b \sim m_\rho \approx 770\,\MeV$ as a
representative estimate gives
$Q \approx 1/6$, so that each successive order in the
expansion is suppressed by roughly a factor of six.
The notion that the dimensionless coefficients
accompanying each order in the expansion are
generically of order unity is referred to as the
``weak naturalness''
assumption~\cite{GoWrong}. Specifically, the
assumption is that
$|\mathrm{Obs}_{\nu+1}| \sim Q\,|\mathrm{Obs}_\nu|$,
where $\nu$ labels the chiral order of a particular
contribution.

The breakdown scale is set by the lightest degrees of
freedom not explicitly included in the theory. In
\chiEFT{} without explicit $\Delta(1232)$ degrees of
freedom, the representative estimate
$\Lambda_b \sim m_\rho$ employed above reflects this
principle; the chiral symmetry breaking scale
$\Lambda_\chi \sim 4\pi f_\pi
\approx 1.2~\text{GeV}$ provides an alternative upper
bound~\cite{chiEFT}. In practice, Bayesian analyses of
NN scattering observables yield
$\Lambda_b \approx 600$--$750~\MeV$ for modern
\chiEFT{} potentials~\cite{Melendez2019,SMS400550}.

The breakdown scale must be clearly distinguished from
the \emph{cutoff scale} $\LamNN$, which is an
unphysical regulator parameter introduced to tame
ultraviolet divergences. In particular, this work uses $\LamNN$ in the context of chiral 
potentials where the potential is multiplied by
a regulator function $f(p',p)$ that suppresses momenta
above $\LamNN$; in the case of a super-Gaussian regulator we have
$f(p',p) = \exp[-(p'/\LamNN)^{2n} - (p/\LamNN)^{2n}]$.
Physical observables must, in principle, be independent
of $\LamNN$ up to contributions beyond the working
order, provided that the counterterms at each order
absorb the regulator dependence.

In practice, the cutoff should be chosen such that
$\LamNN \lesssim \Lambda_b$, so that the regulator
function suppresses the potential at momenta above
the breakdown scale where the chiral expansion of
the potential is no longer reliable, and to avoid
unnatural fine-tuning from sensitivity to these
irrelevant high-momentum modes. Any residual
dependence on $\LamNN$ then serves as a diagnostic
of the theoretical uncertainty at the working order.

Taking $\LamNN$ much larger than $\Lambda_b$ does not
improve the accuracy of the calculation, since the
regulator admits momenta at which the omitted
higher-order contributions to the potential are not
expected to decrease~\cite{chiEFT}. Conversely, choosing
$\LamNN$ well below $\Lambda_b$ risks distorting the
long-range pion-exchange contributions that the chiral
potential is designed to describe. The optimal window is
therefore $\LamNN \lesssim \Lambda_b$, within which the
regulator suppresses momenta at or above the scale where the effective
description ceases to be valid, while retaining the
long-range pion-exchange dynamics.

The truncation of the chiral expansion at a finite
order $\nu$ introduces a systematic uncertainty, the
\emph{truncation error}. For an observable computed
through order $\nu$, the omitted contributions scale
as $Q^{\nu+1}$ relative to the
leading-order result, under the weak naturalness assumption.
The truncation error $\delta_{\nu}$ at order $\nu$ can be estimated as
\begin{equation}
  \delta_\nu \;\sim\; |\mathrm{Obs}_\mathrm{LO}|
  \times Q^{\nu+1}\,,
  \label{eq:truncerror}
\end{equation}
where $Q = \ptyp/\Lambda_b$ is evaluated at the
kinematics of the process under consideration. 
See also the discussion in sec.~\ref{sec:ComptonUncC}.
This estimate provides a lower bound on the theoretical
uncertainty and is the simplest of several approaches
to quantifying the truncation error. A more refined
treatment employs a Bayesian framework that assigns a
statistical degree-of-belief estimate to the uncertainty
at each order~\cite{Melendez2019}.

In addition to the truncation error, the residual
dependence on the cutoff $\LamNN$ provides an
independent handle on the theoretical uncertainty. By
repeating the calculation at several values of
$\LamNN$, the spread of the results gives an empirical
estimate of the sensitivity to short-distance physics
not resolved by the EFT. This is the approach adopted,
for example, by Lenkewitz
\etal~\cite{LenkeThesis} for the trinucleon systems.

In the present work, both the order-by-order
convergence and the residual $\LamNN$ dependence are
examined for each process. Numerical and methodological
uncertainties arising from the parameters of the
many-body calculation (the oscillator frequency
$\omega_H$, the model-space truncation $\Ntot$, the SRG
flow parameter $\LamSRG$, the angular-momentum cutoff
$J_{12}^{\max}$, and the radial and angular integration
grids) are considered statistically independent and
combined into an overall uncertainty estimation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NEW SEC 3.5 (was old 3.4, remainder)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{A First Proposal: The Chiral Index}
\label{sec:powercounting}

A concrete realization of the power counting introduced
in sec.~\ref{sec:truncation} is obtained by assigning
scaling dimensions to each element of a Feynman graph.
In the mesonic and single-nucleon ($\piN$) sectors,
this assignment is well established and provides a
rigorous ordering of contributions. Its extension to
few-nucleon systems, however, involves subtleties that
are addressed in sec.~\ref{sec:weinbergPC}.

The standard scaling rules of naive dimensional
analysis assign powers of $Q^{-1}$ to a nucleon
propagator, $Q^{-2}$ to a pion propagator, $Q^{+1}$ to
each derivative or insertion of the pion mass, and
$Q^{+4}$ to a four-momentum loop
integration~\cite{chiEFT}. Combining these assignments
with standard topological identities,
Weinberg~\cite{weinberg_effective,weinberg_threebod}
derived the chiral index of a connected, irreducible
diagram involving $N$ nucleons:
\begin{equation}
  \nu \;=\; -4+2N+2L+\sum_i V_i\,\Delta_i
  \quad\text{with}\quad
  \Delta_i \;=\; d_i+\frac{n_i}{2}-2\,.
  \label{eq:chiralindex}
\end{equation}
Here $L$ is the number of loops, $V_i$ the number
of vertices of type $i$, where the type is defined by the $n_i$  nucleon
field operators at each such vertex, and $d_i$ the
number of derivatives or pion-mass insertions.
Chiral symmetry guarantees $\Delta_i \geq 0$ for all
interactions allowed by the symmetry: purely pionic
vertices carry at least two derivatives
($d_i \geq 2$, $n_i=0$), pion--nucleon vertices at
least one ($d_i \geq 1$, $n_i=2$), and nucleon--nucleon
contact terms have $d_i \geq 0$ with $n_i = 4$. The
non-negative character of $\Delta_i$ ensures that the
chiral index $\nu$ is bounded from below.

In the mesonic and $\piN$ sectors, where the chiral
index coincides with the standard perturbative power
counting, this is the foundation for the convergence of
the low-momentum expansion. A crucial consequence is
that, at any given order $\nu$, only a finite number
of diagrams contribute. In these sectors, the theory is
therefore calculable at any given order and can, in
principle, be improved systematically by including
higher-order contributions~\cite{chiEFT}. As discussed
in sec.~\ref{sec:weinbergPC}, the application of the
chiral index to few-nucleon systems requires additional
considerations, since the non-perturbative iteration
needed to generate nuclear bound states goes beyond
the perturbative framework in which $\nu$ was derived.

\subsection{Few Nucleons and Weinberg's
  Pragmatic Approach}
\label{sec:weinbergPC}

For systems with $N \geq 2$ nucleons, the nuclear
interaction (potential) must be iterated non-perturbatively in the
Schr\"odinger or Lippmann--Schwinger equation to
generate bound states. This non-perturbative
resummation raises the question of whether the
counterterms determined by the chiral index are
sufficient to renormalize the result. The chiral
index $\nu$ of \meqref{eq:chiralindex} was derived
under the assumption that each diagram is computed
perturbatively, an assumption that does not hold when
the potential is iterated to all orders. In this sense,
the chiral index proves too simplistic for the
few-nucleon problem.

Weinberg's original
proposal~\cite{weinberg_effective,weinberg_threebod}
was to apply the power counting to the irreducible
\emph{potential} (rather than the amplitude), construct
the potential order by order, and then iterate it
non-perturbatively. This ``pragmatic'' scheme has been
the basis for essentially all modern \chiEFT
potentials~\cite{chiEFT,Reinert2018} and has proven
remarkably successful in reproducing $\mathrm{NN}$ scattering
data and nuclear structure observables. However it was pointed
out, first  by Kaplan \etal~\cite{KSW1996}, that the
Weinberg scheme is formally inconsistent: the
non-perturbative iteration generates contributions at
all orders, and the counterterms prescribed by the
naive chiral index do not, in general, suffice to render
the amplitude cutoff-independent at each
order, see also Refs.~\cite{chiEFT,Nogga2005}. Specifically, Nogga
\etal~\cite{Nogga2005} showed that certain attractive
triplet partial waves require counterterms that are
formally of higher order than what the chiral index
provides at LO. This has led to the development of
``modified Weinberg counting'' proposals that promote
specific contact terms to lower
orders~\cite{Nogga2005}, as well as schemes in which
subleading contributions are treated in
distorted-wave perturbation theory;
see~\cite{GoWrong} for an overview.

Despite the formal inconsistency of the Weinberg
scheme, there is strong empirical evidence that it
does not lead to significant problems for the cutoff
values employed in practice. The Bayesian
BUQEYE analysis of Melendez
\etal~\cite{Melendez2019} and Millican
\etal~\cite{Millican2024,SMS400550} demonstrates that
the order-by-order convergence pattern of NN
observables is statistically well described by the
assumption of natural-sized coefficients for the
semilocal momentum-space (SMS) potential of Reinert,
Krebs, and Epelbaum~\cite{Reinert2018} at regulator
scales of $\LamNN = 450$ and $500~\MeV$. That is,
the formal inconsistency of the Weinberg scheme does
not manifest as a statistically significant deviation
from the expected convergence pattern at these
cutoffs~\cite{SMS400550}. For softer cutoffs such as
$\LamNN = 400~\MeV$, Millican \etal~\cite{SMS400550}
identify an irregular even-odd pattern in the expansion
coefficients: the dimensionless coefficients extracted at
even orders (NLO, \NXLO{3}) are systematically larger
than those at odd orders (\NXLO{2}, \NXLO{4}). This
irregularity is attributed to the suppression of
pion-exchange contributions by the soft regulator, which
distorts the balance between long- and short-range
physics. Conversely, statistically consistent
distributions for the breakdown scale $\Lambda_b$
across all available chiral orders are found only for
the SMS potential at $\LamNN = 450$ and
$500~\MeV$~\cite{SMS400550}. These findings provide
both a practical justification for the cutoff choices
adopted in the present work and a quantitative
framework for estimating the associated truncation
uncertainties. The implications for the specific choice
of cutoff values are discussed further in
sec.~\ref{sec:SRG}.

\subsection{Hierarchy of Nuclear Interactions}
\label{sec:hierarchy}

The precise form of the power counting for
few-nucleon systems remains an open question, as
discussed in sec.~\ref{sec:weinbergPC}. Nevertheless,
the hierarchy among two-nucleon ($\Nt$),
three-nucleon (3N), and four-nucleon (4N) interactions
indicated by the naive chiral index is expected to be
respected by any consistent power counting scheme. The Bayesian analyses
of Melendez \etal~\cite{Melendez2019} and Millican
\etal~\cite{Millican2024,SMS400550}, which confirm that
the order-by-order convergence pattern is well described
by natural-sized coefficients at the cutoff values
employed in the present work, support this hierarchy as
a reliable pragmatic starting point for organizing
few-nucleon contributions.

As an indicator of the expected hierarchy,
consider a connected, irreducible $m$-nucleon
interaction in an $N$-nucleon system (with $N\geq m$,
the number of separately connected pieces
$C = N - m + 1$, no loops, and only leading-order
vertices). Inserting these values
into \meqref{eq:chiralindex} yields $\nu = 2m - 4$.
The chiral index therefore suggests that $\Nt${}
interactions first appear at $\nu = 0$ (LO),
irreducible 3N diagrams first appear
at $\nu = 2$ (NLO) but cancel exactly (see below),
so that the first non-vanishing 3N interactions enter at
$\nu = 3$ (NNLO), and 4N interactions at $\nu = 4$
(\NXLO{3}).
Since the leading $\Nt${} contributions enter at
$Q^{0}$ while the first non-vanishing 3N interactions
contribute at $Q^{3}$, and the first connected 4N
interactions at $Q^{4}$, 
the expected hierarchy $\text{2N} \gg \text{3N} \gg \text{4N} \gg \ldots$
is indicated by the chiral index. While this
indication does not constitute a rigorous derivation
of the few-nucleon power counting (see
sec.~\ref{sec:weinbergPC}), it provides a microscopic
rationale for the empirical observation that many-body
interactions are progressively
weaker~\cite{chiEFT,weinberg_threebod}.
Fig.~\ref{fig:diaghi} displays this hierarchy
schematically, and the order-by-order content is
as follows.

\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{diaghi.pdf}
\caption[Hierarchy of nuclear interactions in $\chi$EFT]{Hierarchy of nuclear interactions in
  \chiEFT{}, from~\cite{chiEFT}. Solid lines represent
  nucleons and dashed lines pions. Small dots, large
  solid dots, solid squares, and solid diamonds denote
  vertices of index $\Delta_i = 0$, 1, 2, and 4,
respectively.}
\label{fig:diaghi}
\end{figure}

At leading order (LO, $\nu=0$), only tree-level
diagrams with $\Delta_i = 0$ at every vertex contribute.
The $\Nt${} amplitude consists of two
momentum-independent contact interactions, proportional
to the low-energy constants $C_S$ and $C_T$,
together with static one-pion exchange (1PE), which
gives rise to a Yukawa-type interaction. The contact
interactions represent short-range (point-like) interactions that
contribute exclusively in $S$-waves and encode short-
and intermediate-range physics. The 1PE generates the
long-range tensor interaction that is responsible for
the binding and quadrupole moment of the deuteron
and governs NN scattering in peripheral partial
waves~\cite{chiEFT}. At this order, the description of
the $\Nt${} interaction is necessarily crude, but the
essential qualitative features of the nuclear
interaction are already captured~\cite{chiEFT} such as the one-pion exchange potential.

At $\nu=1$, parity and time-reversal invariance forbid
all possible strong interaction vertices, so no contributions
arise at this order. Specifically, vertices with
$\Delta_i=1$ vanish identically for both four-nucleon
contact interactions and $\pi NN$ couplings due to these
discrete symmetries. The first correction beyond LO
therefore appears at $\nu=2$, which defines
next-to-leading order (NLO). At NLO, two-pion exchange
(2PE) appears for the first time. Since each pion loop
already contributes $\nu=2$
via \meqref{eq:chiralindex}, only the lowest-order
$\pi NN$ and $\pi\pi NN$ vertices ($\Delta_i=0$) are
permitted, so the leading 2PE is comparatively
weak~\cite{chiEFT}. In addition, seven new contact
terms of $\calO(Q^2)$ appear, with operator structures
spanning central, spin-spin, tensor, and spin-orbit
channels. Together with the LO contacts, these terms
supply all the spin-isospin structures needed for a
phenomenologically adequate description of the $\Nt${}
interaction in $S$- and $P$-waves. The primary
deficiency at this order remains an insufficient
intermediate-range attraction. Although irreducible 3N
diagrams nominally appear at NLO, it has been
demonstrated that these contributions cancel
exactly~\cite{weinberg_threebod,chiEFT}. The
Weinberg--Tomozawa vertex is suppressed by a factor
$Q/m_N$ due to a time derivative, while the remaining
diagrams cancel against recoil corrections from
reducible topologies. There is therefore no genuine
3N interaction at NLO.

The intermediate-range attraction problem is resolved
at next-to-next-to-leading order (NNLO, $\nu=3$). The
2PE now incorporates subleading $\pi\pi NN$ seagull
vertices proportional to the low-energy constants
$c_1$, $c_3$, and $c_4$ (denoted by large solid dots
in fig.~\ref{fig:diaghi}).
These vertices encode both correlated 2PE and intermediate $\Delta(1232)$-isobar
effects, and provide the intermediate-range attraction with
sufficient strength to reproduce NN scattering
data~\cite{chiEFT}. Importantly, the first
non-vanishing 3N interactions emerge at this order,
arising from three distinct topologies: a
two-pion-exchange 3N interaction, a one-pion-exchange
3N interaction, and a three-nucleon contact interaction.
The 2PE contribution to the 3N interaction reuses the
same $c_i$ constants already determined by the $\pi N$
and NN sectors, while the 1PE and contact 3N terms
introduce two new low-energy constants, $c_D$ and
$c_E$, which must be fitted to few-body observables
such as the triton binding energy and the
nucleon-deuteron scattering
length~\cite{chiEFT}. No new $\Nt${} contact terms appear
at NNLO.

At \NXLO{3} ($\nu=4$), the $\Nt${} interaction receives
its most substantial refinement. Two-loop 2PE diagrams
appear for the first time, as does three-pion exchange,
though the latter has been found to be
negligible~\cite{chiEFT}. In the contact sector, fifteen
independent operators of $\calO(Q^4)$ enter, among them
a quadratic spin-orbit interaction, and the contact
contributions now extend through $D$-waves. Combined
with the improved pion-exchange potentials, the
\NXLO{3} interaction achieves a quantitative
reproduction of NN scattering observables up to
laboratory energies of approximately
$300~\MeV$~\cite{chiEFT,Reinert2018}. Additional 3N
contributions appear at this order, and, for the first
time, connected 4N interactions contribute. These
contain no new parameters and have been shown to be
non-vanishing, though their quantitative effect is
expected to be small compared to both $\Nt${} and 3N
interactions~\cite{chiEFT}. The suppression of 4N
interactions relative to 3N interactions by an
additional power of $Q$ reinforces the hierarchy
indicated by the chiral index.

Empirical evidence for the few-nucleon hierarchy
from pion-nucleus scattering is discussed at the
end of sec.~\ref{sec:pipi_summary}.
The interaction kernels for the electromagnetic and
pionic processes considered in the subsequent chapters
are computed at the appropriate chiral orders for each
reaction, relying on the hierarchy detailed above to
identify the relevant diagrams.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SUMMARY (old 3.8, updated)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Summary}
\label{sec:QCDsummary}

This section developed the theoretical framework
underlying the interaction kernels employed throughout
the present work. Beginning from the QCD Lagrangian,
the approximate chiral symmetry of the massless
two-flavor theory was identified, and Goldstone's
theorem established that its spontaneous breaking gives
rise to three pseudo-Goldstone bosons, the pions. The
most general effective Lagrangian consistent with this
symmetry pattern was constructed for pion and
pion--nucleon interactions, and a power-counting scheme
was introduced that organizes contributions by their
importance in the low-momentum expansion. The physical
breakdown scale $\Lambda_b$ was distinguished from the
unphysical cutoff $\LamNN$, and the truncation error
inherent in working at a finite chiral order was
discussed, along with Bayesian methods for its
estimation.

The chiral index $\nu$ was presented as a first,
concrete realization of this power counting, providing
a rigorous ordering of contributions in the mesonic and
single-nucleon sectors. For few-nucleon systems, the
non-perturbative iteration of the chiral potential
introduces subtleties not captured by the chiral index
alone. Weinberg's pragmatic scheme, in which the power
counting is applied to the irreducible potential and
then iterated non-perturbatively, was reviewed, and
Bayesian analyses were shown to confirm that the
expected convergence pattern is well satisfied at the
regulator values employed in the present
work~\cite{SMS400550}.

Applied to nuclear interactions, the naive chiral index
suggests a hierarchy in which three-nucleon interactions
are naively suppressed relative to two-nucleon interactions by
$Q^3$, providing a microscopic rationale for the
empirical dominance of the two-body interaction.
While the precise few-nucleon power
counting remains an open question, this hierarchy is
expected to be respected and serves as a reliable
pragmatic starting point, supported by the Bayesian
convergence analyses discussed above.

To compute observables for nuclear targets with mass
number $A > 2$, the few-body interaction kernels
derived within \chiEFT{} must be combined with the
nuclear wave function in a controlled manner. The
Transition Density Amplitude formalism, introduced in
the following section, provides such a procedure: it
factorizes the nuclear scattering amplitude into
irreducible $n$-body kernels derived from \chiEFT{} and
transition densities that encode the structure of the
target nucleus. This separation allows the same set of
densities to be reused across different reactions,
including Compton scattering, pion photoproduction, and
pion scattering, which are the subjects of the
subsequent sections.


==> SRG/SRG.tex <==
%! TEX root = ../Dis-AlexanderLong.tex
\section{SRG Transformation and Cutoff}
\label{sec:SRG}
\subsection{Overview}
\label{sec:SRGoverview}
The nuclear transition density amplitudes discussed in
sec.~\ref{sec:TDA} depend on the underlying nucleon-nucleon potential
from which the wave functions are obtained. In the present work, the
TDAs are generated from the semilocal momentum-space regularized chiral
two-nucleon potential ($\chi$SMS) of Reinert, Krebs, and
Epelbaum~\cite{Reinert2018}, constructed up to fifth order (\NXLO{4}) in
the chiral expansion using Weinberg's pragmatic proposal \cite{weinberg_effective}. This potential
is supplemented by the corresponding chiral three-nucleon interaction at
\NXLO{2}~\cite{Maris2021}, with low-energy constants as specified in
Table~1 of Ref.~\cite{LENPIC2022}. This is the same combination of two-
and three-nucleon interactions employed in the $\HeF{}$ Compton analysis
of Ref.~\cite{hammer4He}.

As discussed in sec.~\ref{sec:QCD}, potentials derived in \chiEFT{} must
be regularized before they can be iterated in the Lippmann--Schwinger
equation; this regularization introduces a cutoff parameter $\LamNN$
whose residual influence on observables must be quantified. For $\LiS$,
where the nucleon number precludes direct few-body methods, additional
dependence arises from the Similarity Renormalization Group (SRG)
transformation employed in the No-Core Shell Model (NCSM) calculation of
the wave functions.

The choice of the $\chi$SMS interaction is dictated by practical rather
than fundamental considerations. It is the family of interactions
implemented by our collaborators in the machinery that generates the
densities, and it is the only family for which a Bayesian convergence
analysis of the chiral expansion is available; that analysis motivates
the regulator choices adopted here, see sec.~\ref{sec:SRGcutoff}. Other,
in particular softer, interactions could of course also be employed. As outlined in
sec.~\ref{sec:TDA}, the TDA formalism itself applies to any $A$-body
computation performed with any few- or many-body method; the densities,
not the formalism, carry the dependence on the underlying interaction.

This section addresses these two sources of parameter dependence in
turn. Sec.~\ref{sec:SRGcutoff} specifies the choice of regulator scale
$\LamNN$ and presents the Bayesian convergence analysis that motivates
the adoption of $\LamNN = 450$ and $500~\MeV$.
Sec.~\ref{sec:SRG_setup} introduces the SRG transformation, explains
why it is required for the extension of the TDA formalism to $\LiS$,
and describes the inverse transformation of Sun
\etal~\cite{Xiang-Xiang} that maps evolved densities back to physical
momenta. The necessity of this back-transformation is demonstrated
quantitatively, and the NCSM parameters ($\LamSRG$, $\Ntot$,
$\omega_H$) that govern the $\LiS$ calculation are discussed.
Sec.~\ref{sec:TDASummary} summarizes the principal advantages and
current limitations of the formalism and identifies directions for
future development.

\subsection{SRG Cutoff Parameters}
\label{sec:SRGcutoff}
The $\chi$SMS regularization that renders the potential suitable for
iteration in the Lippmann--Schwinger equation (sec.~\ref{sec:truncation})
takes the form of a separable cutoff: the potential $V(p',p)$ is
multiplied by a regulator function of the form
\begin{equation}
  V(p',p) \;\to\;
  V(p',p)\,\exp\!\left[-(p'/\LamNN)^{2n}
              -(p/\LamNN)^{2n}\right],
\end{equation}
where $\LamNN$ is the cutoff parameter and $n$ is a
positive integer chosen large enough that the regulator
does not affect the calculation at the working
order~\cite{chiEFT,Reinert2018}.

The cutoff must be selected within a physically
motivated window. As argued in sec.~\ref{sec:truncation},
$\LamNN$ should not dramatically exceed the breakdown scale
$\Lambda_b$ of the EFT, and must remain large enough to
retain the pion-exchange dynamics that govern the
long-range part of the nuclear interaction. A further
constraint specific to the few-nucleon sector arises
from the non-perturbative iteration of the potential:
choosing $\LamNN$ too large can generate spurious
deeply bound states from short-range singularities that
grow increasingly problematic at higher chiral
orders~\cite{Nogga2005}.

The BUQEYE analysis of Millican
\etal~\cite{SMS400550}, summarized in
sec.~\ref{sec:weinbergPC}, provides quantitative guidance for
choosing $\LamNN$ within this window. That analysis
examines the order-by-order convergence patterns of NN
scattering observables computed with the $\chi$SMS
potential at regulator scales
$\LamNN = 400$, $450$, $500$, and $550~\MeV$. Two of
these values are excluded on statistical grounds. At the
soft end, the $\chi$SMS potential at
$\LamNN = 400~\MeV$ exhibits a marked even-odd
irregularity in the expansion coefficients: the
dimensionless coefficients at even chiral orders (NLO,
\NXLO{3}) are systematically larger than those at odd
orders (\NXLO{2}, \NXLO{4}). This irregularity, attributed
to the suppression of pion-exchange contributions by the
soft regulator~\cite{SMS400550}, cannot be remedied by
any choice of model parameters within the BUQEYE
framework, and Millican \etal{} therefore recommend
excluding this cutoff from analysis. At the upper end,
the $\chi$SMS potential at $\LamNN = 550~\MeV$ yields
order-by-order posterior distributions for the breakdown
scale $\Lambda_b$ that are not statistically consistent
across chiral orders. Such inconsistency indicates that
the assumed EFT convergence pattern is not well
realized at this cutoff, compromising the reliability of
truncation error estimates~\cite{SMS400550}.
Only the $\chi$SMS potentials at $\LamNN = 450~\MeV$
and $\LamNN = 500~\MeV$ produce statistically
consistent $\Lambda_b$ posteriors across all chiral
orders examined, confirming that the EFT convergence
pattern is well realized for these cutoffs. In light of
these findings, the present work adopts the values
$\LamNN = 450~\MeV$ and $\LamNN = 500~\MeV$ for all
calculations.

\subsection{TDA With SRG}
\label{sec:SRG_setup}
Previous applications of the TDA formalism to
Compton scattering on $\HeT$ and
$\HeF$~\cite{hammer2020, hammer4He} employed nuclear
wave functions obtained without SRG evolution.
Since the $\chi$SMS family of potentials is relatively hard, extending it
to $\LiS$ in the NCSM used by our collaborators requires substantially
larger model spaces, making a direct computation without SRG evolution
computationally prohibitive. To this end, a SRG
transformation~\cite{SRG, Furnstahl2013} is applied to the potential
before the TDA is calculated. Other methods to produce TDAs or soften
interactions may need that step only for heavier nuclei.
The SRG transformation is (in principle) unitary and
shifts relevant physics toward the low-momentum
region, thereby reducing the minimum effective
$\Lambda$ required in the SRG-evolved space. This
greatly improves the convergence rate and renders
calculations for $A\ge6$ nuclei
computationally feasible. The formalism was developed
independently by Glazek and
Wilson~\cite{GlazekWilson} and by
Wegner~\cite{wegner}. The presentation here follows
Wegner's formulation~\cite{wegner}; for a recent review see Ref.~\cite{heinzSRG}. The central idea
is to continuously transform the Hamiltonian so as to
decouple its low- and high-momentum components.
To this end, one defines a unitary operator $U(s)$
with $s=0$ corresponding to the unevolved
Hamiltonian, so $U(0)=\mathbbm{1}$ and
\begin{equation}
  H_s=U(s) H U^\dag(s)
  = T_{\mathrm{rel}} +V_s,\quad s \in [0,\infty).
\end{equation}
Proceeding in units of the nucleon mass
($m_N=1$), the kinetic energy is defined as the
$s$-independent part, denoted $T_{\mathrm{rel}}$;
the transformed potential is $V_s$.
The evolution is driven by
\begin{equation}
  \frac{d H_s}{d s}
  =\left[\eta(s), H_s\right]
  \quad\text{with}\quad
  \eta(s)=\frac{d U(s)}{d s} U^{\dagger}(s)
  =-\eta^{\dagger}(s)\;.
\end{equation}
The choice of $\eta(s)$ is free; in the present
work it is taken as
\begin{equation}
  \eta(s)=\left[T_{\mathrm{rel}}, H_s\right]
  \implies
  \frac{d H_s}{d s}
  =\left[\left[T_{\mathrm{rel}}, H_s\right],
  H_s\right]\;.
  \label{SRGgenerator}
\end{equation}
The evolution of a potential $V(\kpv,\kv)$ of a
particular partial wave is then given by the nonlinear integral equation
\begin{equation}
  \frac{d V_s\left(k, k^{\prime}\right)}{d s}=
  -\left(k^2-k^{\prime 2}\right)^2
  V_s\left(k, k^{\prime}\right)
  +\frac{2}{\pi} \int_0^{\infty} q^2 d q
  \left(k^2+k^{\prime 2}-2 q^2\right)
  V_s(k, q) V_s\left(q, k^{\prime}\right)\;.
  \label{SRGequation}
\end{equation}
Assuming $T_{\mathrm{rel}}\gg V$ the first
term dominates, giving
\begin{equation}
  V_{\Lambda_{\mathrm{SRG}}}(p',p)
  = V_{\Lambda_{\mathrm{SRG}}=\infty}(p',p)
  \exp [ -(p'^2 - p^2)^2/\Lambda_{\mathrm{SRG}}^4],
  \quad
  \Lambda_{\mathrm{SRG}}= \frac{1}{s^{1/4}}\;.
\end{equation}
The reparametrization in terms of
$\Lambda_{\mathrm{SRG}}$ allows the SRG flow parameter
to be interpreted as a momentum cutoff, analogous to $\Lambda$, with $\Lambda_{\mathrm{SRG}}=\infty$ corresponding to no 
SRG evolution.
\begin{figure}[H]
 \centering
   \includegraphics[width=\linewidth]{combined.png}
 \caption[Nuclear potentials before and after SRG evolution]{Nuclear potentials $V(k,k')$.
   Figure with permission from
   Furnstahl \etal \cite{Furnstahl2013}.~Based
   on a figure by K.~Hebeler \cite{Hebeler2022}.
   Left: high $\LamSRG$; right: low $\LamSRG$
   Green values correspond to small matrix elements, and lack of momentum dependence.
   Red and Blue values correspond to non-zero values and therefore momentum dependence.
 }
 \label{fig:SRGtransform}
\end{figure}
Since the computational cost scales at least linearly
with the number of nonzero matrix elements, the
reduction visible in fig.~\ref{fig:SRGtransform}
from the full momentum range (left) to the region enclosed
by the dashed lines (right) yields a minimum speedup of
$(5/2)^2 \approx 6$. In practice, the gains are
larger still, because near-vanishing matrix elements
at high momenta permit the use of sparse grids, and
the algorithms employed exhibit worse than
$\calO(n)$ scaling in the number of grid points.

While the SRG transformation is essential, it also
alters the physical interpretation of the free
variables. In fact, any unitary transformation
($U^\dag U =\mathbbm{1}$) also transforms the
coordinates. For simplicity, consider the SRG
operator $U(s)$ acting directly on a two-nucleon
potential. Symbolically, the transformation can be expressed as
\begin{align}
  V(p^\prime,p)=
  \br{p'}V\kt{p}
  = \br{p'} U^\dag\left( U V U^\dag\right)\;U
  \kt{p}
  = \br{\widetilde{p}\,'} V_{\mathrm{SRG}}
  \kt{\widetilde{p}}
  =V_{\mathrm{SRG}}(\widetilde{p}^{\,\prime},
  \widetilde{p})\;.\label{SRG1}
\end{align}
The free variables $\kt{\widetilde{p}},\,\kt{\widetilde{p}^{\,\prime}}$ in an SRG-transformed potential
are therefore not eigenstates of the physical momentum 
operator; referring to them as ``momenta'' is, strictly
speaking, a misnomer. The Lagrangians that generate
the Feynman diagrams in the kernel, however, depend
on physical momenta $\kt{\pv\,}, \kt{\pvp\,}$, so an SRG-evolved TDA cannot
be used directly with an unevolved kernel.
To solve this, previous work with SRG
transformations moved the kernels into the
SRG-evolved space. However, in the TDA formalism,
this method would require introducing SRG dependence to the kernel,
thereby breaking kernel-density independence and negating the
principal advantage of the formalism altogether.
Additionally, SRG transformations can take many
different forms~\cite{SRG, Furnstahl2013} and the
present work aims to allow for this flexibility and
for future developments without having to devise a
new kernel transformation prescription each time.

It is worth noting that the identity in \meqref{SRG1} is, strictly
speaking, an approximation: the SRG evolution of
the original two- and three-nucleon interactions
induces irreducible four-body and higher many-body
interactions. The present methodology retains the
two- and three-body interactions, including the
induced contributions at those ranks, but
four-body and higher induced interactions are
neglected. As a result, the SRG-and-back procedure
is not strictly unitary, and it is essential to
test the effect of this approximation. This is
discussed in detail in
sec.~\ref{sec:ComptonResultsC}.

To address the issue of non-physical free variables
$\kt{\widetilde{p}},\,\kt{\widetilde{p}^{\,\prime}}$, Sun
\etal~\cite{Xiang-Xiang} developed a method for performing an inverse
transformation, referred to in the following as the ``SRG-and-back''
procedure. The essential steps are summarized here; the complete
construction, including the full bookkeeping of quantum numbers, is
given in the supplemental material of Ref.~\cite{Xiang-Xiang}, which
is followed closely in this presentation. Up to the truncation of
induced four-and-more-body interactions discussed above, the SRG
transformation is unitary, so the eigenstates of the evolved and bare
Hamiltonians are related by
\begin{equation}
  \kt{\Psi} = U^\dagger(s)\kt{\Psi_s}\;.
  \label{eq:SRGbackWF}
\end{equation}
The NCSM calculation provides $\kt{\Psi_s}$; the inverse
transformation constructs $U^\dagger(s)\kt{\Psi_s}$ without
re-solving the many-body problem. To this end, the evolved wave
function is expanded in a basis that couples out one nucleon pair,
cf.\ Eq.~(6) of Ref.~\cite{Xiang-Xiang},
\begin{equation}
  \kt{\Psi_s}
  = \sum_{\alpha,\,\gamma_{A-2}} F^{\alpha\gamma_{A-2}}_{s}\,
    \kt{\alpha}\otimes\kt{\gamma_{A-2}}\;,
  \label{eq:SRGpairExpansion}
\end{equation}
where $\alpha \equiv n(ls)jt$ collects the relative
harmonic-oscillator quantum numbers of the active pair,
$\gamma_{A-2}$ collects those of the spectator $(A-2)$ subsystem and
of the relative motion between the pair and the spectators, and the
angular-momentum and isospin couplings between the two parts are
suppressed. The coefficients $F^{\alpha\gamma_{A-2}}_{s}$ are
obtained from the diagonalization of the evolved Hamiltonian. The
unitary operator is then truncated at the two-nucleon level, acting
only on the active pair:
\begin{equation}
  U^\dagger(s)\,\kt{\alpha}\otimes\kt{\gamma_{A-2}}
  \approx \bigl[U^\dagger_{2}(s)\kt{\alpha}\bigr]
  \otimes\kt{\gamma_{A-2}}\;.
  \label{eq:SRGtwoBodyTrunc}
\end{equation}
This truncation constitutes a second approximation, distinct from
the neglect of induced many-body interactions in the SRG evolution of
the Hamiltonian. Even for an exactly unitary evolution, restricting
$U^\dagger(s)$ to the active pair discards those components of the
inverse transformation that act on three or more nucleons
simultaneously. The required matrix elements
\begin{equation}
  \phi^{\,js}_{n,\,ll'}(p;s)
  \equiv \br{n(ls)j}U^\dagger_{2}(s)\kt{p(l's)j}
  \label{eq:SRGphiDef}
\end{equation}
obey a closed flow equation that follows from
$\frac{d}{ds}U^\dagger(s) = -\,U^\dagger(s)\,\eta(s)$ with the
generator of \meqref{SRGgenerator},
\begin{equation}
  \frac{d}{ds}\,\phi^{\,js}_{n,\,ll'}(p;s)
  = \sum_{\tilde l}\int_{0}^{\infty} dq\, q^{2}\,
    \bigl(p^{2}-q^{2}\bigr)\,
    \phi^{\,js}_{n,\,l\tilde l}(q;s)\,
    V^{\,js}_{s,\,\tilde l l'}(q,p)\;,
  \label{eq:SRGphiFlow}
\end{equation}
with the initial condition
$\phi^{\,js}_{n,\,ll'}(p;s=0)=\delta_{ll'}\,R_{nl}(p)$, where
$R_{nl}(p)$ denotes the harmonic-oscillator wave function in
momentum space. 
Eq.~\ref{eq:SRGphiFlow} is solved simultaneously with the flow
equation for the potential, \meqref{SRGequation}, so the transformed
pair states are obtained at negligible additional cost. The
momentum-space representation of the back-transformed basis states
then follows by insertion of harmonic-oscillator completeness,
\begin{equation}
  \widetilde{R}^{\,js}_{n,\,l'l}(p;s)
  \equiv \br{p(l's)j}U^\dagger_{2}(s)\kt{n(ls)j}
  = \frac{2}{\pi}\sum_{n'} R_{n'l'}(p)
    \int_{0}^{\infty} dq\,q^{2}\,
    \phi^{\,js}_{n',\,l'l}(q;s)\,R_{nl}(q)\;.
  \label{eq:SRGbackBasis}
\end{equation}
Replacing the oscillator states of the active pair in
\meqref{eq:SRGpairExpansion} by the transformed states of
\meqref{eq:SRGbackBasis}, with the coefficients
$F^{\alpha\gamma_{A-2}}_{s}$ unchanged, yields the wave function of
the bare interaction, which in turn can be used to produce the TDAs.
In summary, the SRG transformation is first applied to the
potential, $V(p,p^\prime)\to
V_{\mathrm{SRG}}(\widetilde{p},\widetilde{p}^{\,\prime})$, the NCSM
problem is solved in the SRG-evolved space, and the inverse
transformation \meqref{eq:SRGbackBasis} maps the free variables
$\widetilde{p},\widetilde{p}^{\,\prime}$ back to physical momenta
before the densities are assembled:
$\widetilde{\rho}_{_{\mathrm{SRG}}}(\widetilde{p},
\widetilde{p}^{\,\prime})\to \rho(p,p^\prime)$. The resulting TDA
can then be used directly with unevolved kernels. Since the inverse
transformation is applied at the level of the wave function rather
than to individual operators, all densities derived from
\meqref{eq:SRGbackWF}, one-body and two-body alike, are corrected
consistently, and no operator-specific evolution is required when
the reaction kernel is exchanged~\cite{Xiang-Xiang}.

The accuracy of this procedure was established in
Ref.~\cite{Xiang-Xiang} through two benchmarks. For the deuteron,
where the truncation of \meqref{eq:SRGtwoBodyTrunc} is exact, the
back-transformed densities reproduce those of the bare interaction
for all flow parameters considered.
For $\HeF$, the back-transformed two-body densities agree with
Faddeev--Yakubovsky calculations performed directly with the bare
interaction, and the residual dependence on $\LamSRG$ is confined to
intermediate relative momenta, $1.5 \lesssim p_{12} \lesssim 2.8~\fmin$,
where it is attributed to the two-body truncation of the inverse
transformation, and/or the absence of induced four-nucleon interactions~\cite{Xiang-Xiang}.
For $\HeF$, the present work tests this
procedure directly at the level of a physical observable: the $\HeF$
TDAs can be produced either from the SRG-evolved interaction or from a
direct Faddeev--Yakubovsky solution with the bare interaction, so the two
may be compared, as shown in fig.~\ref{fig:4HeSRGCompare} and discussed
below.
Readers comparing this presentation in detail with
Ref.~\cite{Xiang-Xiang} may note convention differences relative to
the discussion of the SRG transformation given here: in the
momentum-state normalization of \meqref{SRGequation}, the integrand
of \meqref{eq:SRGphiFlow} acquires an additional factor of $2/\pi$,
and sign conventions differ through the choice of flow variable,
since Sun \etal{} evolve in $\lambda$ whereas the present discussion
evolves in $s$.
\begin{figure}[ht]
  \centering
  \includegraphics[width=0.85\textwidth]{4HeSRGCompare.pdf}
  \caption[Effect of SRG evolution without inverse transformation on $\HeF$ Compton scattering]{
    Compton scattering on $\HeF$ computed without an SRG-transform (solid, red line), and 
    with SRG-evolved TDAs but without the inverse
    transformation, for
    $\LamSRG=1.88\,\fmin, 2.236\,\fmin, 3.0\,\fmin,7.0\,\fmin$.
    All values are computed with the $\chi$SMS potential at $\LamNN=450~\MeV$.
    The suppression of the cross
    section increases with decreasing $\LamSRG$,
    reflecting the growing mismatch between
    SRG-evolved coordinates and physical momenta.}
  \label{fig:4HeSRGCompare}
\end{figure}
\par The necessity of this inverse transformation is
illustrated in figs.~\ref{fig:4HeSRGCompare}
and~\ref{fig:SRGnoReverse}.
They show the Compton scattering cross section
computed from SRG-evolved TDAs \emph{without}
the corresponding back-transformation.
The case of $\HeF$ is particularly instructive, since its TDAs can be
calculated with or without the SRG transformation, providing a check of
the inverse transformation that is carried out here independently of
Ref.~\cite{Xiang-Xiang} and at the level of a physical observable.
\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{4He-SRG-RelDev.pdf}
\caption[Convergence of the SRG-and-back procedure on $\HeF$]{Convergence of SRG-and-back procedure on $\HeF$ in Compton scattering, for various parameters of the NCSM}
\label{fig:4HeRelDev}
\end{figure}
With the SRG-and-back methodology applied, the $\HeF$ Compton cross section
obtained from the SRG-evolved densities agrees with that obtained from a
direct Faddeev--Yakubovsky calculation with the bare interaction within a few percent as can be seen
in fig.~\ref{fig:4HeRelDev};
the curves in fig.~\ref{fig:4HeSRGCompare} instead omit the inverse
transformation in order to isolate its effect.
Without applying the ``and-back'' procedure, the
cross section is systematically suppressed relative
to the unevolved result, and the suppression grows
with increasing $s$ (decreasing $\LamSRG$).
This behavior is expected: the SRG evolution
concentrates the potential into a narrow band
around the diagonal in momentum space, and when the
evolved TDA is paired with an unevolved kernel, the
mismatch between SRG-evolved coordinates and
physical momenta leads to a loss of strength in the
scattering amplitude.
These results underscore that the
inverse transformation of Sun
\etal~\cite{Xiang-Xiang} is not merely a formal
convenience but a quantitative necessity: omitting
it introduces a systematic error that can
substantially distort the predicted cross section.

\begin{figure}
  \centering
  \includegraphics[width=0.7\textwidth]{SRGnoReverse.pdf}
  \caption[$\LiS$ Compton scattering without SRG inverse transformation]{Naive Compton scattering on $\LiS$ calculation compared to data.
    SRG-evolved TDAs were used without corresponding inverse transformation.
    Suppression relative to data
    result demonstrates the necessity of mapping
    the TDA back to physical momenta.}
  \label{fig:SRGnoReverse}
\end{figure}
The TDA calculations which utilize the SRG method use the No-Core
Shell Model (NCSM) ~\cite{Zhan2004}; this involves the selection of a
harmonic oscillator energy $\omega_H$ and an
expansion in basis states. 
If that basis were infinite-dimensional, it would form a
complete set, but in practice it is truncated at
the harmonic oscillator state $\Ntot$, and
convergence is estimated by comparing calculations
for different values of $\Ntot$.
The parameters $\LamSRG$, $\Ntot$
and $\omega_H$ can all affect observables.
Fortunately, during the TDA calculation the binding energy of the
simulated system is obtained, so the parameters $\LamSRG$ and $\omega_H$
which most closely correspond to the
experimental value are picked, whereas $\Ntot$ is taken as
large as feasible. 
For $\LiS$, the computational cost of the NCSM
basis required restricting the SRG flow parameter to
$\LamSRG < 3.0~\fmin$; larger values
demand model spaces that exceed available resources.
Since a smaller $\LamSRG$ corresponds to a more
aggressive evolution away from the bare potential,
the SRG-evolved potential at
$\LamSRG = 1.880~\fmin$, the lowest
value employed, differs most strongly from the
unevolved interaction. The computed observables
exhibit a trend of improved agreement at lower
$\LamSRG$, suggesting that the optimal value may
lie below the range currently explored. There is,
however, a competing constraint: as $\LamSRG$
decreases, the inverse transformation must undo an
increasingly large unitary rotation, and the
neglect of induced four-body and higher interactions
renders this back-transformation progressively less
accurate. The present calculations do not yet
determine whether this lower bound has been reached,
and identifying the optimal $\LamSRG$ that balances
NCSM convergence against back-transformation
fidelity remains an open question.

A practical advantage of the TDA formalism is that
the dominant computational cost lies in the production
of the densities, which need only be performed once for
a given nucleus and parameter set. The cost of this
production step grows rapidly with nucleon number.
For $\HeT$, the one-body densities require approximately
10~CPU-minutes per energy and angle and are therefore
not a substantial computational burden; the two-body
densities, by contrast, require approximately
10~CPU-hours per energy and angle. For $\HeF$, the
two-body density production rises to approximately
125~CPU-hours per energy and
angle~\cite{hammer4He}. For $\LiS$, where the NCSM
basis must be employed, the TDA production cost reaches
approximately 1000~CPU-hours even with the SRG
transformation applied. Once the densities are in hand,
the kernel convolution is comparatively inexpensive.
On a typical desktop computer, the one-body convolution
completes in less than one second per energy and angle.
The two-body convolution, which involves summation over
quantum numbers in the active subsystem together with
angular and radial integrations over the relative
momenta (see sec.~\ref{NumMethod}), requires
approximately 20~minutes for Compton scattering and
approximately 3~hours for reactions employing the
variable-substitution singularity
treatment~\cite{hammer4He}. This separation of a single
expensive density computation from many inexpensive
kernel convolutions is central to the efficiency of
the TDA approach, particularly when multiple reactions
are to be evaluated for the same target nucleus.

\subsection{Summary}
\label{sec:TDASummary}
This section has presented the TDA formalism and its
decomposition of nuclear scattering amplitudes into
irreducible $n$-body kernels and
reaction-independent transition density amplitudes.
The principal advantages of the approach are
threefold. First, the TDAs are computed once for a
given nucleus and parameter set and can then be
reused with any reaction kernel, eliminating the
need to recompute expensive nuclear structure
integrals for each process. Second, the
factorization separates the nuclear structure,
encoded in the densities, from the reaction
dynamics, encoded in the kernel, thereby
facilitating systematic checks of each ingredient
independently. Third, the same density can serve
multiple reactions, so that a single computational
investment yields predictions for Compton
scattering, pion photoproduction, and pion
scattering simultaneously.

The choice of regulator scale has been motivated by
the Bayesian convergence analysis of Millican
\etal~\cite{SMS400550}, which identifies
$\LamNN = 450~\MeV$ and $\LamNN = 500~\MeV$ as
the values exhibiting statistically consistent
convergence patterns across all chiral orders
examined. The SRG transformation, necessary for
extending the formalism to $\LiS$ via the NCSM,
has been introduced together with the
SRG-and-back procedure of Sun
\etal~\cite{Xiang-Xiang}, which maps the evolved
densities back to physical momenta.
The necessity of
this back-transformation was demonstrated
quantitatively: omitting it produces a systematic
suppression of the cross section that grows with
decreasing $\LamSRG$
(figs.~\ref{fig:SRGnoReverse}
and~\ref{fig:4HeSRGCompare}), confirming that the
mismatch between SRG-evolved coordinates and
physical momenta in the kernel cannot be neglected.
The SRG transformation is not strictly unitary in
practice, since induced four-body and higher
interactions are neglected; the effect of this
approximation is assessed in
sec.~\ref{sec:ComptonResultsC} by examining the
residual $\LamSRG$ dependence of the computed
observables.

The formalism in its present implementation is
subject to several limitations. Only one- and
two-body densities are employed; three-body and
higher densities are computationally
prohibitive at present, and the current
implementation of the \texttt{nucdens} package does
not provide them. The approach is restricted to
coherent elastic reactions that preserve the nuclear
ground state, i.e.\ $\Theta +X \to \Theta' +X$ where $\Theta\,(\Theta')$ is the incoming (outgoing) probe;
inelastic transitions, nuclear breakup, and
collective excitations such as giant dipole
resonances lie outside its scope. Finally, the
available TDAs are limited to the set of potentials
for which nuclear wave functions have been computed;
at present, these are the $\chi$SMS potentials at
$\LamNN = 450$ and $500~\MeV$.

Looking ahead, extending the TDA framework to
accommodate three-body densities would address the
dominant uncontrolled systematic for heavier nuclei,
though this requires substantial development of both
the density generation infrastructure and the
convolution code. A more practical near-term
strategy would be to compute
three-nucleon contributions independently following
the direct evaluation approach of Liebig
\etal~\cite{Liebig_2011} and combine them with the
TDA-based one- and two-body results, exploiting the
additivity of the few-nucleon expansion in
\meqref{eq:totalscat}. With the formalism and its
computational infrastructure now established, the
following sections apply it to three reactions on
light nuclei: Compton scattering
(sec.~\ref{sec:ComptonC}), neutral pion
photoproduction (sec.~\ref{sec:piphoto}), and
elastic pion scattering (sec.~\ref{sec:pion}).


==> TDA/TDA.tex <==
%! TEX root = ../Dis-AlexanderLong.tex
\newcommand{\wf}{}%{\Psi,}    % ket
\newcommand{\wfbra}{}%{\Psi,} % bra 
\newcommand{\sepp}{,}
\newcommand{\sep}{}
\section{The Transition Density Amplitude Method}
\label{sec:TDA}
The preceding chapter established the \chiEFT
framework for constructing irreducible interaction
kernels that describe pion and photon scattering
from one or two nucleons. To compute observables
for nuclear targets with mass number $A>2$,
these few-body kernels must be combined with the nuclear
wave function of the target in a controlled manner.
The Transition Density Amplitude (TDA) formalism,
introduced by Grie{\ss}hammer
\etal~\cite{hammer2020, Vries2024} and from which
the following discussion draws extensively, provides
such a procedure. It separates the interaction of a
probe with a nucleus of $A$ nucleons into two
components. Of the $A$ nucleons, those $n$ which
participate directly in the reaction at a given
order are designated \emph{active}; the remaining
$A-n$ nucleons, which do not interact directly with
the probe, are designated \emph{spectators}. The
reaction dynamics of the probe with the $n$ active
nucleons are encoded in irreducible $n$-body
kernels, while the nuclear structure information
carried by the spectator system is encapsulated in
the transition density amplitudes. Because the TDAs
depend only on the nuclear state and the kinematics
of the process, they need be computed only once for
a given nucleus and can thereafter be convolved with
the appropriate kernel for any elastic reaction.
Given $m$ reaction kernels and TDAs for $n$ distinct
nuclei, a total of $m\times n$ distinct calculations
may be performed without recomputing either
ingredient.


This factorization carries several practical
advantages beyond mere modularity. First, the
density calculation constitutes the most
computationally expensive step; once complete, the
convolution with any reaction kernel is
comparatively inexpensive, so each additional
reaction incurs only a fraction of the original
cost. Second, the separation of nuclear structure
from reaction dynamics permits each ingredient to be
tested independently: the kernels can be validated
against single-nucleon amplitudes, and the densities
can be cross-checked through observables such as
binding energies and form factors. Third, and
central to the present work, the same set of
densities serves all three reactions treated in this
dissertation: Compton scattering
(sec.~\ref{sec:ComptonC}), neutral pion
photoproduction (sec.~\ref{sec:piphoto}), and
elastic pion scattering (sec.~\ref{sec:pion}).

The TDAs are parametrized by Compton scattering
kinematics $(\omega,\theta)$, which serve as proxy
variables for the Lorentz-invariant Mandelstam
variables $s$ and $t$; other reactions are mapped
onto these variables via the matching conditions
described in App.~\ref{sec:convert}. Fourth, the TDA constitutes a
universal interface between nuclear structure and reaction theory. The
quantum numbers and momenta that label a TDA refer exclusively to the active
one- or two-nucleon subsystem and are independent of the coordinates, basis,
and many-body method used to generate the density. Any group capable of
solving the $A$-body problem can therefore supply TDAs, and any group capable
of constructing reaction kernels can use them, without either requiring
detailed knowledge of the other's machinery. This division of labor is
realized concretely in the present work: the densities are produced by
collaborators at FZ~J\"ulich with their few- and many-body methods, while the
kernels and their convolution with the densities are constructed here.

The formalism in its present implementation is
subject to several limitations. Only one- and
two-body densities are employed; three-body and
higher densities, while formally included in the
decomposition presented below, are computationally
prohibitive and are not provided by the current
implementation of the \href{https://pypi.org/project/nucdens/}{\texttt{nucdens}}
package; fortunately power counting predicts they are not required.
Furthermore, the approach is restricted to
coherent elastic reactions that preserve the nuclear
ground state as in the spectator expansion of Siciliano \etal \cite{Siciliano_1977}; that is, we are
interested in processes of the form
$\Theta+X \to \Theta'+X$ where $\Theta,\,\Theta'$ denote the incoming (outgoing)
probe and $X$ is the nucleus. Inelastic transitions,
nuclear breakup, and collective excitations such as
giant dipole resonances lie outside its scope for now. These
limitations are discussed further at the end of this
section.

The TDA formalism was originally applied to Compton
scattering on the trinucleon systems by
Grie{\ss}hammer
\etal~\cite{hammer2020} and subsequently extended
to $\HeF$ by Grie{\ss}hammer
\etal~\cite{hammer4He}. The present work builds on
this foundation in several respects. First, the
formalism is applied for the first time to pion
photoproduction and pion scattering extending previous calculations by
Lenkewitz \etal~\cite{Lenke2013, Lenke2011,
LenkeThesis} and Braun~\cite{BraunThesis}, which
employed Monte Carlo integration and a density
matrix approach, respectively. Second, the scope is
broadened to include $\LiS$, a $p$-shell nucleus
whose treatment requires the Similarity
Renormalization Group (SRG) transformation and the
No-Core Shell Model (NCSM). Third, all calculations
are carried out within the publicly available
\texttt{DensityScattering} code
suite~\cite{long_2026}, developed as part of the
present work. The modular design of the code suite
means that, once the TDAs are in hand, incorporating
a new reaction requires only the implementation of
the corresponding kernel.

The remainder of this section is organized as
follows. The general decomposition of the scattering
amplitude into $n$-body contributions is presented
first, followed by the derivation of the one-body
TDA in sec.~\ref{sec:TDA1body} and the two-body TDA
in sec.~\ref{sec:TDA2body}, both developed for the
specific case of $A=3$. Throughout, the kinematics,
variables, and quantum numbers are defined in
Fig.~\ref{fig:onetwobod} and its caption. The choice
of regulator scale and the application of the SRG
transformation to the densities are deferred to
sec.~\ref{sec:SRG}.
With the distinction between active and spectator
nucleons established above, the scattering amplitude
is decomposed according to the number
$n=1,\ldots,A$ of active nucleons at a given order.
The $n$-body kernel is irreducible: it describes only
the direct interaction of the probe with the $n$
active nucleons and does not contain lower-body
kernels as subdiagrams.
Figure~\ref{fig:onetwobod} illustrates this
decomposition for the case $A=3$ in Compton
scattering.
\begin{figure}[!b]
  \begin{center}
    \includegraphics[width=\linewidth]{kinematics3He.pdf}
    \caption[TDA kinematics and quantum numbers for an $A=3$ system]{Kinematics in the center-of-mass frame and quantum
      numbers for an $A=3$ system in Compton scattering.
      Generalization to other reactions only changes the
      ingoing/outgoing probe.
      Systems with $A>3$ result in more internal lines
      representing the nucleons.
      Top: one-body processes $\hat{O}_{1\mathrm{N}}$ (one active nucleon, two spectators),
      center: two-body
      processes $\hat{O}_{2 \mathrm{N}}$ (two active nucleons, one spectator), bottom: three-body processes
      $\hat{O}_{3 \mathrm{N}}$ (all nucleons active, no spectators). 
      Red denotes the kernel; all other components are
      subsumed into the TDAs. Green denotes the
      wavefunction of the nucleons.
      $J(M)$ - spin (projection);  $T(M_T)$ - isospin (projection) of the nucleus. 
      $l_i,\,s_i(m_i^s),\,j_i(m_i),\,t_i(m_i^t)$:
      orbital angular momentum, spin, total angular
      momentum (and their projections), and isospin
      (projection) of the relevant subsystem.
      Figure from Grie{\ss}hammer \etal \cite{hammer2020}.
  }
    \label{fig:onetwobod}
  \end{center}
\end{figure}
The total scattering amplitude matrix for an interaction with $A$-body nucleus is given by 
\begin{equation}
  \begin{split}
  \calM_{M}^{M^{\prime} }(\bv{k}, \bv{q})&=
 \langle M^{\prime}|\bigg[
  \binom{A}{1} \hat{O}_{1 \mathrm{N}}(\bv{k}, \bv{q}) +
  \binom{A}{2} \hat{O}_{2 \mathrm{N}}(\bv{k}, \bv{q}) +... + 
  \binom{A}{A} \hat{O}_{A \mathrm{N}}(\bv{k}, \bv{q})
  \bigg]|M
  \rangle_\psi\\
                                         &= \calM_{1 \mathrm{N}} + \calM_{2 \mathrm{N}}+...\;,
  \end{split}
  \label{eq:totalscat}
\end{equation}
where $\hat{O}_{n \mathrm{N}}$ is the $n$-body ($n$-nucleon) kernel, $M,M'$ are the spin projections of the
incoming/outgoing state of the target nucleus, and there are
$\binom{A}{n}$ ways for a probe to interact with kernel involving $n$ nucleons. The subscript
$\psi$ denotes a convolution with the densities which is described in detail in the following sections.
The matrices $\calM_{n \mathrm{N}}$ are called the $n$-body scattering matrices.

Although this decomposition is \emph{per se} exact
and valid for any elastic interaction, evaluating all
TDAs involving up to $A$ active nucleons is in
general not feasible in practice.
Fortunately, \ChiEFT predicts that $n$-body
interactions follow a hierarchy of
scales~\cite{weinberg_threebod}, such that
three-body and higher contributions are negligible
for the reactions considered here, namely Compton
scattering, pion photoproduction, and pion
scattering, at least through the first few orders in
the chiral expansion and for typical momenta
$k \sim m_\pi$.
This hierarchy permits restricting the expansion in
\meqref{eq:totalscat} to the first two terms.
The applicability of the method is bounded at both
ends of the energy scale. At low energies, the de
Broglie wavelength of the probe exceeds the
internucleon separation, so that the nucleus responds
collectively as a point-like object and the internal structure
remains unresolved. At higher energies, the
truncation of the chiral expansion means that
degrees of freedom not explicitly included in the
\chiEFT Lagrangian begin to play a role; for
example, the $\Delta(1232)$ resonance, which is not
resolved at leading orders, becomes relevant above
$\omega\sim 200~\MeV$ and limits the accuracy of the
kernel unless it is included explicitly as an active
degree of freedom. Similarly, near the pion
production threshold, contributions from virtual pion
loops and the opening of inelastic channels introduce
additional complications for each reaction.
In practice, for the energies relevant to this
work, the one- and two-body contributions
suffice for an accuracy at the $5\%$
level~\cite{hammer2020,hammer4He}, and the
following truncation is utilized
\begin{align}
  \calM_{M}^{M^{\prime} }(\bv{k}, \bv{q})&=
 \langle M^{\prime}|\bigg[
  \binom{A}{1} \hat{O}_{1 \mathrm{N}}(\bv{k}, \bv{q}) +
  \binom{A}{2} \hat{O}_{2 \mathrm{N}}(\bv{k}, \bv{q})
  \bigg]|M
  \rangle_\psi\;.
  \label{TDAExpansion}
\end{align}
Suppressing additional quantum numbers
such as $J$ (total nucleus spin) and $M_T$ (isospin projection), 
the nuclear state can be expanded in the
partial-wave basis. For $A=3$, the wavefunction
takes the form
\begin{equation}
  \psi_\alpha(p_{12},p_3)= \brkt{p\uot p_3 \alpha}{M},
\end{equation}
where $p_3,\,p_{12}$ are Jacobi coordinates, which for $A=3$ resolve to
\begin{equation}
  \pv_3= \kv_3+ \frac{1}{3} \kv,\quad \pv_{12}= \frac{1}{2} \left( \kv_1 - \kv_2 \right)\;.
\end{equation}
Here, the label $\alpha$ collects the orbital angular
momentum, spin, and isospin quantum numbers. The angular
momenta are coupled according to the standard rules for
addition of angular momenta:
$\vec{l}_{12} + \vec{s}_{12} = \vec{j}_{12}$ and
$\vec{l}_3 + \vec{s}_3 = \vec{j}_3$, with
$\vec{j}_{12} + \vec{j}_3 = \vec{J}$. The isospins
are likewise coupled as
$\vec{t}_{12} + \vec{t}_3 = \vec{T}$, where the
total isospin projection is $M_T = (Z-N)/2$, giving in total
\begin{equation}
 \label{eq:alphaOneBody}
  |\alpha\rangle=\left|\left[\left(l_{12} s_{12}\right) j_{12}\left(l_3 s_3\right) j_3\right] J M,\left(t_{12} t_3\right) T M_T\right\rangle\;.
\end{equation}
Primed indices denote the final-state quantum
numbers; for example, $J'$ is the total angular
momentum of the nucleus after the reaction.
Since the present work is restricted to elastic
processes, $J=J'$ and $M_T=M_T'$; the $z$-component
of isospin is likewise conserved for each nucleon,
$m_i^{t\prime}=m_i^t$. However, $T\neq T'$ is
permitted because the probe can redistribute
isospin among the nucleons without changing the
total projection $M_T$.
For example, in $\LiS$ the ground state contains
both $T=0$ and $T=1$ components, and the formalism
naturally accommodates transitions between these
isospin sectors.


\subsection{One-Body Transition Density Amplitudes}
\label{sec:TDA1body}
To keep the presentation concrete, the following
develops the TDA formalism for the specific case
of $A=3$,
denoting the TDAs by $\rho$ throughout. The
extension to $A>3$ entails
additional integrations over free momenta.
First analyzing the one-body densities,
the single \textit{active} nucleon is labeled with
the index $3$. With the variable definitions from
Fig.~\ref{fig:onetwobod}, define the one-body kernel matrix element as
% We label the single \textit{active} nucleon with
% the index $3$.
% First define the operator:
\begin{align}
  \left\langle\vec{k}_3^{\prime}\right|&\left\langle s_3 m_3^{s \prime}\right|\left\langle t_3 m_3^{t \prime}\right| \Oo(\vec{k}, \vec{q})\left|t_3 m_3^t\right\rangle\left|s_3 m_3^s\right\rangle\left|\vec{k}_3\right\rangle \\
                                       & \quad \equiv \delta_{m_3^{t \prime} m_3^t} \delta^{(3)}\left(\vec{k}_3^{\prime}-\vec{k}_3-\vec{q}\right) O_{1 \mathrm{N}}\left(m_3^{s \prime} m_3^s m_3^t ; \vec{k}_3 ; \vec{k}, \vec{q}\right)\;.\label{delta}
\end{align}
Here, $\Oo$ denotes the full one-body operator, and
$O_{1\mathrm{N}}$ is its matrix element in
single-nucleon quantum numbers (momentum, spin, and
isospin), which depends on the individual nucleon
momentum $\vec{k}_3$ in addition to the probe
momenta $\vec{k}$ and $\vec{q}$.
A complication arises because the kernel $O_{1\mathrm{N}}$ depends on
$\vk_3$, and therefore on the spectator relative momentum $\vec{p}_{12}$.
An analogous dependence enters all $N$-body kernels. This momentum
dependence encodes the relativistic boost correction required to
transform from the center-of-mass frame of the nucleus to the frame of
the active (struck) nucleon, and its size therefore depends on the
nucleus under consideration. To isolate this dependence systematically,
the spin-isospin matrix elements of the kernel are multipole-expanded
in spherical coordinates in $\vk_3$ up to a maximum multipolarity
$K_{\max}$:
\begin{equation}
  O_{1\mathrm{N}}\left(m_3^{s \prime} m_3^s m_3^t ; \vec{k}_3 ; \vec{k}, \vec{q}\right)
  \equiv \sum_{K=0}^{K_{\max }} \sum_{\kappa=-K}^K \sqrt{\frac{4 \pi}{2 K+1}}\left(k_3\right)^K
  Y_{K \kappa}\left(\hat{k}_3\right)
  \tilde{O}_{1 \mathrm{N}}
  \left(m_3^{s \prime} m_3^s m_3^t ; K \kappa ; \vec{k}, \vec{q}\right)\;.\label{relative}
\end{equation}
Setting $K_{\max}=0$, the $K$-dependent factors in
the TDA simplify.
It therefore becomes independent of $\vec{k}$, and the
superscripts $K\kappa$ may be dropped. Note that restriction the $K_{\max}=0$ case limits the interactions that can
be analyzed to only these which are independent of nucleon energy, that is, they do not depend on relativistic boost 
corrections, which are higher order than what is considered in the present work.
The scattering kernel is then given by
\begin{equation}
\begin{split}
  \bra \, \wfbra M ' \, | \, \hat O_{1\mathrm{N}} (\kv,\qv) \, | \, \wf
  \sep M \, \ket = \sum_{\alpha \alpha'}& \int \deint{}{p_{12}} p_{12}^{2}\;
  \deint{}{p_{3}} p_{3}^{2} \; \deint{}{p_{12}'} p_{12}^{\prime\, 2} \;
  \deint{}{p_{3}'} p_{3}^{\prime \, 2}\;
  \psi^{\dagger}_{\alpha'}(p_{12}'p_{3}')   \psi_{\alpha}(p_{12}p_{3})    \\[0.5ex]
  & \times \big\bra \, p_{12}' p_{3}' \left[ (l_{12}' s_{12}')\jrel'
    (l_{3}' s_3) j_{3}' \right] J' M' (t_{12}' t_3 ) T' M_{T} \, \big| \,
  \hat O_{3}(\kv,\qv) \, \\
  &\hspace*{10ex}\big| \, p_{12}p_{3} \left[ (l_{12}
    s_{12})\jrel (l_{3} s_3) j_{3} \right] J M (t_{12} t_3) T M_{T}
  \big\ket \;\; .
\end{split}
\end{equation}
We can now explicitly decompose $\alpha$ in terms of active and spectator nucleons

\begin{equation}
  \begin{split}
    \label{eq:explicitO3}
    \hqmm\bra \, &\wfbra M ' \, | \, \hat O_{1\mathrm{N}} (\kv,\qv) \, | \,
    \wf \sep M \, \ket  =\\[0.5ex]
    & \sum_{\alpha} \int \deint{}{p_{12}} p_{12}^{2} \int \deint{}{p_{3}}
    p_{3}^{2} \sum_{\alpha'} \int \deint{}{p_{12}'} p_{12}^{\prime\, 2} \int
    \deint{}{p_{3}'} p_{3}^{\prime \, 2} \psi_{\alpha'}(p_{12}'p_{3}') \;
    \psi_{\alpha}(p_{12}p_{3})    \\[0.5ex]
    &\times \sum_{m_{3}m_{3}^{t}} \CG{\jrel}{j_{3}}{J}{M-m_{3}}{m_{3}}{M}
    \CG{t_{12}}{t_3}{T}{M_{T}-m^{t}_{3}}{m^{t}_{3}}{M_{T}} \\[0.5ex]
    &\times \sum_{m_{3}'}
    \CG{\jrel'}{j_{3}'}{J'}{M'-m_{3}'}{m_{3}' }{M'}
    \CG{t_{12}'}{t_{3}}{T'}{M_{T}-m^{t}_{3}}{m^{t}_{3}}{M_{T}}
    \\[0.5ex]
    &\times \bra \, p_{12}' (l_{12}' s_{12}')\jrel' \sep (M'-m_{3}') \sepp
    t_{12}' \sep (M_{T}-m^{t}_{3}) \, | \, p_{12} (l_{12} s_{12})\jrel
    \sep (M-m_{3}) \sepp t_{12} \sep (M_{T}-m^{t}_{3}) \,
    \ket   \\[0.5ex]
    &\times \bra \, p_{3}' (l_{3}' s_3) j_{3}' \sep m_{3}' \sepp t_3 \sep
    m^{t}_{3} \, | \, \hat O_{3}(\kv,\qv) \, | \, p_{3} (l_{3}
    s_3) j_{3} \sep m_{3} \sepp t_3 \sep m^{t}_{3} \, \ket \ \ .
\end{split}
\end{equation}
Where we have used $M=m_3+m\uot$,  $M_T=m_3^t+m_{12}^t$ \textit{etc}. 
Denoting the resulting $K{=}0$ transition density amplitude simply as $\rho$, the
$1\mathrm{N}$ scattering matrix reduces to
\begin{equation}
  \calM_{1 \mathrm{N}}= A \left\langle M^{\prime}\right|
    \Oo (\vec{k}, \vec{q})|M\rangle_\psi
    =A \sum_{\alpha,\alpha'}
    O_{1\mathrm{N}}^{\alpha\alpha'}{(\kv,\qv\,)}
    \rho^{\alpha\alpha'}(\vec{k}, \vec{q}\,)\;.
  \label{eq:M1N}
\end{equation}
The quantity $\rho$ encapsulates all information
about the spectator nucleons and constitutes the
\emph{one-body transition density amplitude} (TDA).
For $K_{\max}=0$, the one-body TDA carries no dependence on any internal
momentum of the $A$-body system: it is fully specified by the spin and
isospin projections of the active nucleon together with the external
kinematics $(\kv,\qv)$. The producer of a one-body TDA therefore needs only
to project the $A$-body wave function onto the quantum numbers of the single
active nucleon at the given momentum transfer. The internal organization of
the $A$-body computation, whether Jacobi coordinates, a harmonic-oscillator
basis, or any particular treatment of center-of-mass motion, never appears in the result.
For completeness, the general expression retaining
arbitrary $K$ is recorded here for the $A=3$ case.
In practice, only the $K{=}0$ term is retained, and
the indicated portion of the following equation reduces to unity:
\begin{equation}
\begin{split}
  \rho&_{m_{3}^{s \prime }\,m_{3}^{s}}^{K\kappa;
    m_{3}^{t}M_{T},M'M}(\kv,\qv) :=
  \sum_{\alpha} \int \deint{}{p_{12}} p_{12}^{2}
  \int \deint{}{p_{3}} p_{3}^{2}
  \sum_{\alpha'} \ \delta_{\jrel\jrel'}
  \delta_{l_{12}l_{12}'} \delta_{s_{12}s_{12}'}
  \delta_{t_{12}t_{12}'}
  \delta_{M_{T}M_{T}'}     \\[0.5ex]
  &\times \sum_{m_{3}}
  \CG{\jrel}{j_{3}'}{J'}{M-m_{3}}{M'-M+m_{3}}{M'}
  \CG{t_{12}}{t_3}{T'}{M_{T}-m^{t}_{3}}{m^{t}_{3}}
    {M_{T}} \\[0.5ex]
  & \hqqq \times
  \CG{\jrel}{j_{3}}{J}{M-m_{3}}{m_{3}}{M}
  \CG{t_{12}}{t_3}{T}{M_{T}-m^{t}_{3}}{m^{t}_{3}}
    {M_{T}} \\[0.5ex]
  & \hqqq \times
  \CG{l_{3}'}{s_3}{j_{3}'}{M'-M+m_{3}-m^{s \prime
      }_{3}}{m^{s \prime }_{3}}{M'-M+m_{3}}
  \CG{l_{3}}{s_3}{j_{3}}{m_{3}-m^{s}_{3}}{m^{s}_{3}}
    {m_{3}}   \\[0.5ex]
  & \hqqq \times\int \deint{}{\hat p_{3}}
  Y^{\dagger}_{l_{3}' (M'-M+m_{3}-m^{s \prime }_{3})}
    (\widehat {\pv_{3}+\frac{2}{3} \qv })
  \ Y_{l_{3} (m_{3}-m^{s}_{3})}(\hat p_{3})  \\[0.5ex]
  & \hqqq \hqqq \hqq \times
  \underbrace{
    \sqrt{\frac{4\pi}{2K+1}} \;\big| \vec
    p_{3}-\textstyle{\frac{1}{3}} \kv \big|^{K}
    \ Y_{K\kappa}(\widehat {\vec
      p_{3}-\frac{1}{3} \kv })
  }_{\displaystyle \to\; 1 \;\text{ for } K=0}
  \;\psi^{\dagger}_{\alpha'}(p_{12} \big| \vec
  p_{3}+\textstyle{\frac{2}{3}} \qv \big| )
  \ \psi_{\alpha}(p_{12}p_{3}) \;\; .
\end{split}
\end{equation}
For a given set of nuclear structure parameters,
$\rho$ is computed once and stored for subsequent
use in all reactions of interest. The density
depends on the choice of nuclear potential, the
regulator scale $\LamNN$, and, for nuclei treated
with an SRG transformation
(see secs.~\ref{sec:SRG}, \ref{sec:SRG_setup}),
on the SRG flow parameter $\LamSRG$, the harmonic
oscillator frequency $\omega_H$, and the basis
truncation $\Ntot$ (see sec.~\ref{sec:SRG}). This
separation of the density from the kernel is a
central advantage of the TDA formalism: a single
density computation, which constitutes the most
expensive step, can be reused across all reactions,
substantially reducing the total computational cost.
\subsection{Two-Body Transition Density Amplitudes}
\label{sec:TDA2body}
The discussion now turns to the case of $n=2$
active nucleons and develops the analogous
expression for the two-body TDA. The presentation
is again restricted to the $A=3$ system; see the
middle panel of Fig.~\ref{fig:onetwobod}.
Labeling the active nucleons as $1$ and $2$,
momentum conservation gives
\begin{equation}
  \label{eq:twobody1}
  \begin{split}
    \bra \pv_{12} ' \kv_{12}^{\,\prime} |& \bra s_{12}' m^{s
      \prime}_{12} | \bra t_{12}' m^{t \prime}_{12} | \Ot (\kv,\qv) 
    | t_{12} m^{t}_{12} \ket | s_{12} m^{s}_{12} \ket | \vec
    p_{12}    \kv_{12}   \ket \\[5pt]
    & = \;\delta^{(3)}(\kv_{12}^{\,\prime} - \kv_{12}-\qv)
    \;O_{2 \mathrm{N}} (
    s_{12}' t_{12}' m^{s \prime }_{12} s_{12} t_{12} m^{s}_{12} m^{t}_{12};\pv_{12}^{\, \, \prime}, \pv_{12};
   \kv,\qv )\;\;.
  \end{split}
\end{equation}
In analogy with the one-body case, the quantum
numbers of the active pair are collected into
$\alpha_{12}$:
\begin{equation}
  \label{eq:alpha12}
  |\alpha_{12} \ket = | (l_{12} s_{12} ) \jrel m_{12}, t_{12}m^{t
  }_{12} \ket\;\;.
\end{equation} 
Retaining only the dependence on the momentum
transfer $\qv$ and neglecting the dependence on
$\kv$ (i.e. no $K\kappa$ dependence), one obtains
\begin{equation}
  \label{eq:2bpw}
  \begin{split}
    \bra \alpha_{12}'\kv_{12}^{\,\prime} |& \Ot |
    \alpha_{12}\kv_{12} \ket =
    \;\delta_{m^{t \prime}_{12} m^{t}_{12}}\; \delta^{(3)}(\kv_{12}^{\,\prime} -
    \kv_{12}-\qv)\\[0.5ex]
    &\times\sum_{m^{s}_{12} m^{s \prime }_{12} } \CG{l_{12}}{s_{12}}{\jrel}
    {m_{12} - m^{s}_{12}}{m^{s}_{12}}{m_{12}} \CG{l_{12}'}{s_{12}'}{\jrel'}
    {m_{12}' - m^{s \prime }_{12}}{m^{s
        \prime}_{12}}{m_{12}'}   \\[0.5ex]
    &\times \int \deint{}{\hat p_{12}'} \deint{}{\hat p_{12}} Y^{\dagger}_{l_{12}'
      (m_{12}' - m^{s \prime }_{12})} ( \hat p_{12}') \; Y_{l_{12} (m_{12} -
      m^{s }_{12})} ( \hat p_{12})
    \\[0.5ex]
    &\hqqq\times O_{2 \mathrm{N}} (s_{12}' t_{12}' m^{s \prime
    }_{12} s_{12} t_{12} m^{s}_{12} m^{t}_{12} ;\pv_{12}^{\,\prime}, \pv_{12}; \qv )    \\[0.5ex]
    \equiv&\; \delta_{m^{t \prime}_{12} m^{t}_{12}} \; \delta^{(3)}(\vec
    k_{12}^{\,\prime} - \kv_{12}-\qv) \;O_{2 \mathrm{N}}^{{\alpha_{12}'
        \alpha_{12}}} (p_{12}', p_{12})\;\; .
  \end{split}
\end{equation}
To obtain the two-body scattering matrix, the
kernel is expanded in Spherical Harmonics and the
resulting expression is integrated over all free
momenta. The derivation is straightforward but
lengthy; the final result is
\begin{equation}
\label{eq:twobodysum}
\begin{split}
  \calM_{2 \mathrm{N}}&= \binom{A}{2}\bra M ' \, | \hat O_{2 \mathrm{N}} |  M \, \ket_\psi \\
                      &=\binom{A}{2}
    \sum_{\alpha_{12}',\alpha_{12}} \int
    \deint{}{p_{12}} p_{12}^{2} \, \deint{}{p_{12}'} p_{12}^{\prime \, 2 } \;
    O_{2 \mathrm{N}}^{\alpha_{12}' \alpha_{12}} (p_{12}', p_{12}) \;
    \rho_{\alpha_{12}'\,\alpha_{12}}^{M_{T},M'M}
    (p_{12}',p_{12};\qv)\;\;.
\end{split}
\end{equation}
In contrast to the one-body case, the two-body TDA retains a dependence on
internal momenta, but only through the relative momentum of the active pair,
$p_{12}$ and $p_{12}'$. Whatever momentum variables a given $A$-body method
employs internally, the producer of a two-body TDA needs only convert them
into this single relative coordinate; the spectator degrees of freedom are
integrated over and do not enter the interface between density and kernel.
The two-body transition density amplitude is defined, for $A=3$, as
\begin{equation}               
  \label{eq:twobodydensity}
  \begin{split}
    \rho_{\alpha_{12}'\,\alpha_{12}}^{M_{T},M'M}(p_{12}',&p_{12};\qv)
    :=\\[0.5ex]&\hspace*{-8ex}\sum_{\alpha'(\alpha_{12}')
      \alpha(\alpha_{12})} \CG{\jrel}{j_{3}}{J}{m_{12}}{M-m_{12}}{M}
    \CG{\jrel'}{j_{3}'}{J'}{m_{12}' }{M'-m_{12}'}{M'} \
    \\[0.5ex]
    & \times\CG{t_{12}}{t_3}{T}{m^{t}_{12}}{M_{T}-m^{t}_{12}}{M_{T}}
    \CG{t_{12}'}{t_3}{T'}{m^{t}_{12}}{M_{T}-m^{t}_{12}}{M_{T}} \\[0.5ex]
    & \times \int \deint{}{p_{3}'} p_{3}^{\prime \, 2 } \int \deint{}{\hat
      p_{3} '} \psi^{\dagger}_{\alpha'} (p_{12}'p_{3}') \psi_{\alpha} (p_{12}\big|
    \pv_{3} ^{{\,\prime}} +\textstyle{\frac{1}{3}}\qv
    \big| )  \\[0.5ex]
    &\hqqq\hqqq \times \sum_{m^{s}_{3}}Y^{\dagger}_{l_{3}' (M'-m_{12}' - m^{s}_{3})} (\hat p_{3}') \
    Y_{l_{3} (M-m_{12} - m^{s}_{3})} (\widehat{\pv_{3} ^{{\,\prime}}
      +\frac{1}{3}\qv }) \\[0.5ex]
    & \hqqq\hqqq\hqqq\times
    \CG{l_{3}}{s_3}{j_{3}}{M-m_{12}-m^{s}_{3}}{m^{s}_{3}}{M-m_{12}}\\[0.5ex]
    &\hqqq\hqqq\hqqq\times
    \CG{l_{3}'}{s_3}{j_{3}'}{M'-m_{12}'-m^{s}_{3}}{m^{s}_{3}}{M'-m_{12}'}\;\;.
\end{split}
\end{equation}
The explicit expressions for the one- and two-body densities given above are
specific to $A=3$ and to the particular Jacobi coordinates chosen there. For
$A\geq4$, the corresponding intermediate expressions depend on the internal
coordinates of the $A$-body computation: the Jacobi coupling scheme, the
treatment of center-of-mass motion, the choice of basis, and the
antisymmetrization of the wave function all enter the derivation, and the
recoupling algebra grows rapidly more intricate with each additional
spectator nucleon. The derivation of the general expression is therefore
trivial and is left as an exercise for the reader. In particular, no
explicit general form is presented here, and none is required. The defining
property of the TDA is precisely that these internals never reach the user:
the density is labeled only by the quantum numbers of the active subsystem
and, for two active nucleons, by the relative momentum of the pair. Whoever
generates a TDA converts the coordinates and quantum numbers internal to
their method into these universal labels, and the resulting density may then
be convolved with any kernel without reference to how it was produced.

The TDAs are parametrized by the Compton scattering
center-of-mass energy $\omega$ and scattering angle
$\theta$, which serve as proxy variables for the
Lorentz-invariant Mandelstam variables $s$ and $t$
that ultimately determine the density:
\begin{equation}
  s = \left(\omega + \sqrt{M^2 + \omega^2}\right)^2,
  \qquad
  t = -2\omega^2(1-\cos\theta)\;.
\end{equation}
For reactions other than Compton scattering, the
physical kinematics are mapped onto equivalent
Compton variables $(\omega,\theta)$ via the matching
conditions $s_{\gamma\gamma}=s_\mu$ and
$t_{\gamma\gamma}=t_\mu$; the explicit conversions
for pion photoproduction and pion scattering are
given in App.~\ref{sec:convert}.

A comprehensive set of TDAs for light nuclei has
been computed by our collaborators A.~Nogga and X.~Sun
(FZ~J\"ulich) for this thesis and is
made available through the
\href{https://pypi.org/project/nucdens/}{\texttt{nucdens}}
Python package.
The TDAs are provided for $\HThree$, $\HeT$,
$\HeF$, and $\LiS$ for a variety of momentum
transfers $\qv$ and energies at both
$\LamNN = 450~\MeV$ and $500~\MeV$.

With the one- and two-body TDAs defined, the
formalism is complete in the sense that any coherent
elastic reaction on a light nucleus can be computed
by convolving the appropriate kernel with the
densities $\rho$. The TDAs encapsulate the full
nuclear structure content of the problem and are
independent of the reaction under consideration;
once computed, they may be reused for Compton
scattering, pion photoproduction, and pion scattering
alike. The dependence of these densities on the
choice of regulator scale $\LamNN$ and, for $\LiS$,
on the parameters of the SRG transformation is
addressed in sec.~\ref{sec:SRG}. The practical
implementation of the convolution and the structure
of the code suite are described in
sec.~\ref{sec:usage}.


==> compton/compton.tex <==
%! TEX root = ../Dis-AlexanderLong.tex
\section{Compton Scattering}
\label{sec:ComptonC}
Elastic Compton scattering, $\gamma X\to \gamma X$, probes
the electromagnetic structure of the target $X$ through the
response of its internal degrees of freedom to real photons.
At photon energies
$50\;\MeV\lesssim\omega\lesssim120\;\MeV$, the process is
sensitive to the scalar dipole polarizabilities of the
nucleon, which quantify the extent to which the nucleon
develops induced electric and magnetic dipole moments in
external electromagnetic
fields~\cite{BERNARD_1995,hammer4He}.
For reviews of Compton scattering on nucleons and light
nuclei in \chiEFT, including notation, the relevant parts of
the chiral Lagrangian, and a comprehensive list of
references, the reader is directed to Grie{\ss}hammer
\etal~\cite{hammer4He,hammer2020, Ghammer_2012}.

The present section reports the first calculation of
elastic Compton scattering on $\LiS$. Within the TDA
formalism, Compton scattering calculations have previously
been carried out for
$\HeT$~\cite{hammer2020} and
$\HeF$~\cite{hammer4He}. The present work extends these
calculations to $\LiS$ by convolving the one-
and two-body Compton kernels, used also for $\HeT$
and $\HeF$, with the $\LiS$ TDAs.
Since the kernels are unchanged, only the TDAs
distinguish the various targets, allowing for a direct
comparison of the effect of nuclear structure on the
Compton cross section across light nuclei.
The present results are calculated in the center-of-mass
frame. Because $\LiS$ is relatively heavy, the
kinematic transformation from center-of-mass to
laboratory variables introduces corrections of order
$\omega/M_{{}^6\mathrm{Li}}\lesssim 2\%$ at the highest
photon energy and most backward scattering angle
considered, well within the theoretical uncertainties present in this analysis.
Throughout this section, the labels
$\omega$ and $\theta$ may therefore be identified with
either frame to the accuracy of the present
calculation. Were polarizabilities to be extracted by
fitting data, this mildly angle-dependent correction
would need to be incorporated explicitly.

The section is organized as follows.
Section~\ref{sec:ComptonKernelC} summarizes the power
counting and the one- and two-body Compton kernels.
Section~\ref{sec:polarsCtwo} specifies the nucleon
polarizability input and justifies the neglect of spin
polarizabilities for $\LiS$, using the SRG-and-back
procedure~\cite{Xiang-Xiang} as outlined in
sec.~\ref{sec:SRG_setup}.
Section~\ref{sec:ComptonSensC} investigates the
sensitivity of the $\LiS$ cross section to variations
of the scalar-isoscalar polarizabilities.
Section~\ref{sec:ComptonResultsC} presents the $\LiS$
cross-section predictions and discusses the convergence
of the NCSM parameters.
Section~\ref{sec:ComptonUncC} assesses the theoretical
uncertainties.
Section~\ref{sec:ComptonCompareC} places the $\LiS$
results in context by comparing with lighter
few-nucleon targets.
Section~\ref{sec:ComptonDataC} compares the predictions
with data from HI$\gamma$S, and
sec.~\ref{sec:ComptonSummaryC} summarizes the principal
findings.

\subsection{Power Counting and Kernel}
\label{sec:ComptonKernelC}
In the energy window of interest,
$50\;\MeV\lesssim\omega\lesssim 120\;\MeV$, the relevant
low-energy scales are the pion mass $m_\pi$, the
Delta-nucleon mass splitting
$\Delta_M\approx 300\;\MeV$, and the photon energy
$\omega$. The $\omega$ and $\rho$ mesons are the lightest
degrees of freedom not explicitly included in the kernel;
accordingly, the breakdown scale, see sec.~\ref{sec:truncation}, is set to
$\Lchi\approx 650\;\MeV$, consistent with the masses of
these exchange mesons~\cite{Pascalutsa_2003}. The
general framework for estimating truncation errors from
omitted higher-order contributions is discussed in
sec.~\ref{sec:truncation}; the process-specific power
counting for Compton scattering is developed here.
Exploiting the numerical coincidence
$\Delta_M/\Lchi\approx\sqrt{m_\pi/\Lchi}$ at the physical
pion mass, a single expansion parameter is defined:
\begin{align}
  \label{eq:deltaC}
  \delta \equiv \frac{\Delta_M}{\lchi}
  \approx \sqrt{ \frac{m_\pi}{\lchi} }
  \approx \sqrt{\frac{\omega}{\lchi}}\approx0.4\;,
\end{align}
where the last relation holds under the assumption
$\omega\sim m_\pi$. Because $\delta$ is only moderately
small, order-by-order convergence must be verified
carefully~\cite{hammer4He}.

The one- and two-body kernels employed here are those of
refs.~\cite{Beane_1999,BKM_polar,BERNARD_1995}, supplemented
with $\Delta$-pole and $\pi\Delta$ loop contributions from
refs.~\cite{hildebrandt,Hildebrandt_2010,Hildebrandt_2004,Hildebrandt_2005}.
They are identical to the kernels used in the Compton
studies of $\HeT$~\cite{hammer2020} and
$\HeF$~\cite{hammer4He}.
Figure~\ref{fig:Compton1BC} displays the one-body diagrams,
which are organized as follows:
\begin{enumerate}
\item[(a)] LO [$\calO(e^2\delta^0)$]: The single-nucleon
  Thomson term, in which the photon scatters from the proton
  charge. This is the only contribution at leading order and
  yields the correct Thomson limit as $\omega\to 0$ for a
  point-like charged nucleon. For a composite target with
  $A\geq 2$, the soft-photon theorem instead requires the
  amplitude to approach the nuclear Thomson limit
  $-Z^2e^2/(4\pi \Mnucl)$ as $\omega\to 0$. Recovery of this
  limit calls for the coherent propagation of the entire
  $A$-nucleon system between the absorption of the incoming
  photon and the emission of the outgoing one, that is, an
  intermediate state in which all $A$ nucleons interact with
  one another rather than only one or two acting in the kernel
  against a backdrop of $A-n$ spectators. Such a contribution
  corresponds to an $A$-body density and is not included in
  the present calculation~\cite{hammer4He}.
  %
  \item[(b)] \NXLO{2} [$\calO(e^2\delta^2)$]
  non-structure (Born) contributions: couplings of the photon
  to the nucleon charge beyond LO, to the nucleon magnetic
  moment, and to $t$-channel $\pi^0$ exchange. For an
  isoscalar target such as $\LiS$ (isospin $T=0$), the
  $\pi^0$-exchange contribution is absent.
  %
  \item[(c)] \NXLO{2} [$\calO(e^2\delta^2)$]
  structure (non-Born) contributions: photon couplings to the
  pion cloud surrounding the nucleon, which generate the
  leading chiral prediction for the electric and magnetic
  polarizabilities~\cite{BKM_polar,BERNARD_1995}.
  %
  \item[(d/e)] \NXLO{3} [$\calO(e^2\delta^3)$]
  structure (non-Born) contributions: couplings of the photon
  to the pion cloud around the $\Delta(1232)$
  resonance~(d), or direct excitation of the Delta~(e), as
  computed in
  refs.~\cite{Hildebrandt_2004,Hildebrandt_2005,Hildebrandt_2010}.
  These diagrams provide the next-to-leading-order
  contributions to the nucleon polarizabilities and introduce
  a significant energy dependence even at $\omega\sim m_\pi$
  through the so-called dynamical
  polarizabilities~\cite{hammer4He}.
  %
  \item[(f)] Short-distance contributions encoded in
  low-energy coefficients (LECs) that parameterize the effects
  of physics at and above the breakdown scale $\Lchi$ on the
  nucleon polarizabilities. These offsets to the chiral
  predictions of graphs~(c) and (d/e) are formally of higher
  order than $\calO(e^2\delta^3)$ and are fixed to reproduce
  the central values of the isoscalar polarizabilities given
  in eq.~\eqref{eq:polvaluesC}. Their uncertainties are
  small compared to other sources of theoretical uncertainty
  discussed in sec.~\ref{sec:ComptonUncC}.
\end{enumerate}
No contributions arise at NLO [$\calO(e^2\delta^1)$].
The overall factor of $e^2$ appearing at every order
reflects the two electromagnetic vertices inherent to
Compton scattering; the $\delta$ counting then organizes the
hadronic and nuclear dynamics on top of this electromagnetic
coupling.

\begin{figure}[H]
\centering
\includegraphics[scale=1.0]{Compton-graphs-1B.pdf}
\caption[One-body Compton scattering diagrams through N$^3$LO]{One-body contributions to Compton
  scattering in \ChiEFT up to \NXLO{3}
  [$\calO(e^2\delta^3)$] for
  $50\;\MeV\lesssim\omega\lesssim120\;\MeV$. Vertices from:
  ${\LL}_{\piN}^{(1)}$ (no symbol),
  ${\LL}_{\piN}^{(2)}$ (green square - see $a)$),
  ${\LL}_{\piN}^{(3)}$ (green triangle see $b)$);
  the green disc of graph~(f) denotes variations of the
  polarizabilities. Permuted and crossed diagrams are not
  shown. Photons are represented by wavy lines, pions by
  dashed lines, and Delta excitations by a double red bar.
  Figure reproduced with permission from
  Grie{\ss}hammer \etal~\cite{hammer4He}.}
\label{fig:Compton1BC}
\end{figure}

The first nonzero two-body kernel enters at \NXLO{2}
[$\calO(e^2\delta^2)$]; no additional two-body contributions
arise at \NXLO{3}
[$\calO(e^2\delta^3)$]~\cite{Beane_2003}. 
In addition, partial two-body contributions at \NXLO{4}
[$\calO(e^2\delta^4)$]~\cite{Beane_2005_compton} have
been computed for the $T_{12}=0$ isospin channel;
contributions from the $T_{12}=1$ channel, which also
enter at this order, are not yet available. Because
this higher-order calculation is incomplete, it is not
included in the reported cross sections but is used in
sec.~\ref{sec:ComptonUncC} as a convergence indicator.
As shown there, the incomplete $\calO(e^2\delta^4)$
correction is small and largely angle-independent,
supporting the conclusion that the chiral expansion
of the two-body kernel is well converged at the
energies considered.
\begin{figure}[ht]
  \begin{center}
    \includegraphics[width=0.75\textwidth]{graphs-2B-withlabels.pdf}
    \caption[Two-body Compton scattering diagrams at N$^2$LO]{\NXLO{2}
      [$\calO(e^2\delta^2)$] contributions to the two-body
      Compton kernel. No additional contributions at
      \NXLO{3} [$\calO(e^2\delta^3)$]. Notation as in
      fig.~\ref{fig:Compton1BC}. Permuted and crossed
      diagrams not displayed.}
    \label{fig:2BdiagramsC}
  \end{center}
\end{figure}

\subsection{Nucleon Polarizabilities}
\label{sec:polarsCtwo}
At low photon energies, the Compton amplitude on a nucleon
admits a systematic expansion in powers of the photon
energy $\omega$. In forward kinematics, this amplitude takes
the form~\cite{BERNARD_1995}
\begin{equation}
  \label{eq:forwardCompton}
  \frac{1}{4\pi}T(\omega) =
    f_1(\omega^2)\,\vec{\epsilon}\,'^{\,*}\!\cdot\vec{\epsilon}
  + i\omega\,f_2(\omega^2)\,
    \vec{\sigma}\cdot(\vec{\epsilon}\,'^{\,*}\times\vec{\epsilon})\;,
\end{equation}
with spin-nonflip amplitude $f_1$ and spin-flip amplitude
$f_2$. They admit the low-energy expansions
\begin{equation}
  \label{eq:lexCompton}
  \begin{split}
    f_1(\omega^2) &= f_1(0)
      + (\alpha_{E1}+\beta_{M1})\,\omega^2 + \calO(\omega^4)\;,\\
    f_2(\omega^2) &= f_2(0)
      + \gamma\,\omega^2 + \calO(\omega^4)\;,
  \end{split}
\end{equation}
in which $f_1(0)=-e^2 Z^2/(4\pi m)$ is fixed by gauge
invariance (the Thomson limit) and
$f_2(0)=-e^2\kappa^2/(8\pi m^2)$ is fixed by the low-energy
theorem of Low, Gell-Mann, and Goldberger, with $\kappa$
the anomalous magnetic moment of the nucleon~\cite{BERNARD_1995}.
Internal nucleon structure first enters the amplitude at $\calO(\omega^2)$
through the scalar electric and magnetic dipole
polarizabilities, $\alpha_{E1}$ and $\beta_{M1}$, and the
forward spin polarizability $\gamma$.

The scalar polarizabilities admit a transparent physical
interpretation as parameters describing the deformation of
the nucleon's internal charge and magnetization
distributions in response to applied electromagnetic
fields. Equivalently, the $\calO(\omega^2)$
structure-dependent contribution to the non-Born amplitude
is reproduced by an effective dipole
interaction with Hamiltonian~\cite{Babusci_1998}
\begin{equation}
  \label{eq:polHamiltonian}
  \mathcal{H}=-4\pi\left(\frac{1}{2}\alpha_{E1}\vec{E}^{\,2}
  +\frac{1}{2}\beta_{M1}\vec{H}^{\,2}\right)\;,
\end{equation}
which couples the nucleon to an external electric field
$\vec{E}$ and magnetic field intensity
$\vec{H}=\vec{B}/\mu_0 - \vec{M}$.

The best current values of the scalar-isoscalar
polarizabilities, defined as
$\alpha_{E1}^{(s)}:=
\tfrac{1}{2}[\alpha_{E1}^{(p)}+\alpha_{E1}^{(n)}]$
and similarly for $\beta_{M1}^{(s)}$, are obtained from a
\chiEFT fit to deuteron Compton data~\cite{Myers:2014ace}:
\begin{equation}
  \label{eq:polvaluesC}
  \begin{split}
  \alpha_{E1}^{(s)} &= 11.1 \pm 0.6_{\mathrm{stat}}
  \pm 0.2_{\mathrm{Baldin}} \pm 0.8_{\mathrm{th}} \\
  \beta_{M1}^{(s)} &= 3.4 \mp 0.6_{\mathrm{stat}}
  \pm 0.2_{\mathrm{Baldin}} \pm 0.8_{\mathrm{th}}\;,
  \end{split}
\end{equation}
in units of $10^{-4}\;\fm^3$. The subscripts ``stat'',
``Baldin'', and ``th'' denote the statistical, Baldin Sum
Rule, and \chiEFT truncation uncertainties, respectively.
The statistical errors are anti-correlated because the
Baldin Sum Rule constraint
$\alpha_{E1}^{(s)}+\beta_{M1}^{(s)}=14.5\pm0.4$ has been
imposed following ref.~\cite{hammer4He}. These values are
adopted as input for the present calculation.

Since $\LiS$ is (mostly) an isoscalar target ($T=0$), the
Compton cross section is (mostly) only sensitive to the
scalar-isoscalar combinations
$\alpha_{E1}^{(s)}\pm\beta_{M1}^{(s)}$, with no dependence
on isovector polarizabilities at the order considered.
Unlike $\HeF$, however, $\LiS$ has nuclear spin $J=1$ and
is therefore not a scalar target; in principle, spin
polarizabilities could contribute. The expansion of $f_2$
in \meqref{eq:lexCompton} shows that the spin-flip
structure carries an additional explicit factor of $\omega$
relative to the spin-nonflip part, so that the scalar
polarizabilities $\alpha_{E1}$ and $\beta_{M1}$ first enter
the non-Born amplitude at $\calO(\omega^2)$, whereas spin
polarizabilities appear only at
$\calO(\omega^3)$~\cite{Ghammer_2012}. Their contribution
to the cross section is therefore suppressed by a relative
factor of $\omega/\lchi\sim\delta^2\approx 0.2$ compared
to the scalar polarizability terms, and the isoscalar
nature of $\LiS$ restricts the relevant spin
polarizabilities to their isoscalar combinations, further
reducing the numerical impact~\cite{Griesshammer:2016ivu};
this has been demonstrated for the
deuteron~\cite{Griesshammer:2013vga}. Spin polarizabilities
are therefore neglected in the present calculation.
\subsection{Sensitivity to the Scalar-Isoscalar
Polarizabilities}
\label{sec:ComptonSensC}

\begin{figure}%[H]
\centering
\includegraphics[width=1.0\linewidth]{PolarVary1.pdf}
\caption[Sensitivity of ${}^6$Li Compton cross section to polarizability variations]{Sensitivity of the $\LiS$ Compton
  differential cross section to variations of the
  scalar-isoscalar polarizabilities by $\pm 2$ canonical
  units ($10^{-4}\;\fm^3$) around their central values (red
  solid) of eq.~\eqref{eq:polvaluesC}, at \NXLO{3}
  [$\calO(e^2\delta^3)$]. Deviations from the canonical values are as follows. Top left:
  $\delta(\alpha_{E1}^{(s)}+\beta_{M1}^{(s)})=0,\pm 2$.
  Top right: $\delta\alpha_{E1}^{(s)}=0,\pm 2$. Bottom
  left:
  $\delta(\alpha_{E1}^{(s)}-\beta_{M1}^{(s)})=0,\pm 2$.
  Bottom right: $\delta\beta_{M1}^{(s)}=0,\pm 2$. Results
  shown at $\omega_{\mathrm{lab}}=60,\;75,\;86,$ and
  $100\;\MeV$ (top most to bottom most in each
  panel), using the parameter set $\chi$SMS,
  $\LamNN\in\{450,500\}\;\MeV$,
  $\LamSRG\in\{1.88,2.236\}\;\fmin$. For $\LiS$,
  the kinematic difference between center-of-mass and
  laboratory frames is at most $2\%$
  ($\omega/M_{{}^6\mathrm{Li}}$); the labels
  $\omega_{\mathrm{lab}}$ and $\theta$ may be
  identified with their center-of-mass counterparts
  to the accuracy of this calculation.
}
\label{fig:PolarVary1C}
\end{figure}
\begin{figure}
  \centering
  \includegraphics[width=0.65\textwidth]{RelativeDeviation.pdf}
  \caption[Relative deviation of ${}^6$Li Compton cross section from polarizability variations]{Relative deviation of the
    $\LiS$ Compton cross section as a function of
    $\theta$ in degrees from the
    $\delta(\alpha_{E1}^{(s)}\pm\beta_{M1}^{(s)})=0$
    result, for
    $\delta(\alpha_{E1}^{(s)}+\beta_{M1}^{(s)})=0,\pm 2$
    (top) and
    $\delta(\alpha_{E1}^{(s)}-\beta_{M1}^{(s)})=0,\pm 2$
    (bottom), at $\omega_{\mathrm{lab}}=60,\;75,\;86,$
    and $100\;\MeV$ (innermost to outermost curves).
    Same parameter set as fig.~\ref{fig:PolarVary1C}.
    The distinction between center-of-mass and laboratory
    frame variables is negligible for $\LiS$;
    see fig.~\ref{fig:PolarVary1C} caption.
  }
  \label{fig:RelDevC}
\end{figure}
Following the approach of
refs.~\cite{hammer4He,hammer2020}, the sensitivity of the
$\LiS$ Compton cross section to the scalar-isoscalar
polarizabilities is investigated by varying
$\alpha_{E1}^{(s)}\pm\beta_{M1}^{(s)}$ by $\pm 2$ canonical
units ($10^{-4}\;\fm^3$) around their central values. This
variation is comparable in magnitude to the combined
uncertainties quoted in eq.~\eqref{eq:polvaluesC} and, for
an isoscalar target, corresponds to a shift of $\pm 4$ units
in the corresponding neutron polarizability.

Figure~\ref{fig:PolarVary1C} displays the absolute cross
sections under these variations at four photon energies.
At $60\;\MeV$, the spread induced by varying either
$\alpha_{E1}^{(s)}+\beta_{M1}^{(s)}$ or
$\alpha_{E1}^{(s)}-\beta_{M1}^{(s)}$ by $\pm 2$ units
amounts to only a few percent of the cross section. As the
photon energy increases, the separation between the varied
curves grows. The variation of
$\alpha_{E1}^{(s)}-\beta_{M1}^{(s)}$ produces a clearly
visible spread at backward angles, where the cross section
changes by approximately $\pm 10\%$ at $100\;\MeV$; see
fig.~\ref{fig:RelDevC}. The right-hand panels of
fig.~\ref{fig:PolarVary1C} show the corresponding effects
of varying $\alpha_{E1}^{(s)}$ and $\beta_{M1}^{(s)}$
independently: the electric polarizability dominates the
forward-angle sensitivity, while the magnetic polarizability
exhibits a more uniform angular dependence.

Figure~\ref{fig:RelDevC} quantifies these effects as
relative deviations from the central-value cross section,
defined as the ratio of the varied to the unvaried result
minus one. The combination
$\alpha_{E1}^{(s)}+\beta_{M1}^{(s)}$, which is tightly
constrained by the Baldin Sum Rule
($\sigma=0.4$ for the sum, compared with $\sigma=1.0$ for
$\alpha_{E1}^{(s)}$ and $\beta_{M1}^{(s)}$ individually),
primarily affects forward angles: the relative deviation
reaches approximately $\pm 10$--$15\%$ at $100\;\MeV$ for
$\theta\lesssim 30^\circ$ but vanishes near
$\theta\approx 120^\circ$. This angular
pattern is understood from the individual polarizability
responses. An increase in $\alpha_{E1}^{(s)}$ suppresses
the cross section at all angles, whereas an increase in
$\beta_{M1}^{(s)}$ suppresses it at forward angles but
enhances it at backward angles. For the sum
$\alpha_{E1}^{(s)}+\beta_{M1}^{(s)}$, the two
contributions therefore reinforce at forward angles and
cancel at backward angles, producing a large net effect
in the forward hemisphere and no effect in the backward
hemisphere.

The combination $\alpha_{E1}^{(s)}-\beta_{M1}^{(s)}$, which is at present
much less precisely determined, displays a complementary
pattern, yielding approximately $\pm 9\%$ relative
deviations at backward angles for $100\;\MeV$ and
negligible sensitivity in the forward hemisphere; see
fig.~\ref{fig:RelDevC}. At $60\;\MeV$, both combinations
produce relative deviations of only a few percent.
This energy dependence reflects a trade-off inherent in
polarizability extractions. At lower energies the cross
section is large and event rates are correspondingly high,
but the polarizability-induced variations are too small to be
resolved experimentally. At higher energies the sensitivity
grows substantially, but the falling cross section reduces
the available statistics. The same trade-off was observed
for $\HeF$~\cite{hammer4He}, where the polarizability
spread at $60\;\MeV$ amounted to only $\pm 3\%$ but
reached $\pm 11\%$ at backward angles by $120\;\MeV$.
The present $\LiS$ results exhibit a comparable angular
pattern and magnitude of sensitivity, confirming that the
polarizability response is largely governed by the structure
of the Compton kernel rather than by the details of the
nuclear transition density. Optimal polarizability
extractions therefore require data at the highest feasible
energies within the domain of applicability of the TDA
formalism ($\omega\lesssim 120\;\MeV$) and at backward angles,
complemented by forward-angle measurements at lower
energies to verify consistency with the Thomson limit and
the Baldin Sum Rule.

Predictions for the linearly polarized beam asymmetry
$\Sigma^{\mathrm{lin}}$ and double-polarization observables on $\LiS$ are deferred to a future
study in which the sensitivity to the nuclear spin structure
and spin polarizability effects can be examined in detail.
\subsection[Results for Compton Scattering on Lithium-6
and Convergence]{Compton Scattering on $\LiS$ and Convergence}
\label{sec:ComptonResultsC}
Because $\LiS$ densities are computed within the NCSM
using SRG-evolved interactions, the present results depend
on several computational parameters: the model-space
truncation $\Ntot$, the harmonic-oscillator frequency
$\omega_H$, and the SRG flow parameter $\LamSRG$, in
addition to the nucleon-nucleon cutoff $\LamNN$. No
unevolved densities are available for $A=6$, so unlike the
$\HeF$ case~\cite{hammer4He}, a direct comparison between
SRG-evolved and unevolved results is not possible.
Convergence must therefore be assessed by studying the
sensitivity to these parameters.

\begin{figure}%[H]
\centering
\includegraphics[width=\linewidth]{Ntotconverge.pdf}
\caption[Convergence of ${}^6$Li Compton cross section with $N_{\mathrm{tot}}$]{Convergence of the $\LiS$ Compton cross section
  as a function of $\Ntot$ at $\omega=60,86,100\;\MeV$
  for two scattering angles, several values of $\omega_H$
  and $\LamSRG$, and $\LamNN=500\;\MeV$. 
One- and two-body contributions are included through
$\calO(e^2\delta^3)$ [\NXLO{3}], with expansion
parameter $\delta\approx0.4$ in
``$\Delta(1232)$-ful'' \ChiEFT.
  The vertical spread
  among curves at fixed $\Ntot$ reflects the variation
  over $\omega_H$ and $\LamSRG$; the associated
  percentage uncertainties are quantified in
  fig.~\ref{fig:RelativeDeviationCompare}. The same
  kernels are used as in Grie{\ss}hammer \etal for
  $\HeT$~\cite{hammer2020} and
  $\HeF$~\cite{hammer4He}.}
\label{fig:NtotConvergeC}
\end{figure}
\begin{figure}
\centering
\includegraphics[width=\linewidth]{RelDeviationCompare.pdf}
\caption[Relative deviation of ${}^6$Li Compton cross section from SRG parameter variation]{Relative deviation of the $\LiS$ Compton
  differential cross section, in percent, from the
  reference parameter set $\LamSRG=1.88\;\fmin$,
  $\omega_H=18\;\MeV$, $\Ntot=14$, at photon energies
  $\omega=60$, $86$, and $100\;\MeV$ for two
  representative scattering angles
  ($\theta=40^\circ$ and $159^\circ$). Each point
  corresponds to a different combination of $\omega_H$,
  $\LamSRG$, and $\LamNN$ from the set defined in
  eq.~\eqref{eq:densityGoodVals}. The shaded band marks the
full width ($2\sigma$) range spanned by these combinations using the uncertainty estimate of \meqref{eq:uncC}, which includes an additional $5\%$ of the cross section added in quadrature.}
\label{fig:RelativeDeviationCompare}
\end{figure}

Ideally, the cross section would be unchanged between
$\Ntot=12$ and $\Ntot=14$;
fig.~\ref{fig:NtotConvergeC} indicates that residual
$\Ntot$ dependence persists, and calculations at
$\Ntot=16$ or $18$ would be desirable but are presently
precluded by computational cost. Convergence improves for
smaller values of $\LamSRG$, as expected: a smaller
$\LamSRG$ corresponds to a more strongly decoupled
(softer) Hamiltonian, which is better represented within a
truncated harmonic-oscillator basis. As discussed in
sec.~\ref{sec:SRG}, however, a competing constraint
exists: as $\LamSRG$ decreases, the neglect of induced
four-body and higher interactions in the
back-transformation renders the results progressively
less accurate, so an optimal balance must be sought.
Additional numerical convergence studies, including
the sensitivity to $J_{12}^{\max}$ and to the radial
and angular integration grids, are documented in
the appendix, see sec.~\ref{sec:InteConverge}.

The convergence pattern exhibits a mild dependence on
the squared momentum transfer
$q^2=-2\omega^2(1-\cos\theta)$.
Figure~\ref{fig:NtotConvergeC} shows that the relative
spread among different values of $\omega_H$ and
$\LamSRG$ at fixed $\Ntot$ increases modestly with
$|q^2|$: at low $|q^2|$ (e.g.\ $\omega=60\;\MeV$,
$\theta=40^\circ$, where $|q^2|=(41\;\MeV)^2$) the
percentage variation across parameter sets is
approximately $5\%$, whereas at high $|q^2|$
(e.g.\ $\omega=100\;\MeV$, $\theta=159^\circ$, where
$|q^2|=(197\;\MeV)^2$) it grows to roughly $10\%$.
Larger momentum transfers probe shorter-range components
of the density, which are more sensitive to the details
of the SRG evolution and the model-space truncation,
so the increased spread at backward angles and higher
energies is expected. The effect remains within the
envelope defined by the half-spread estimate of
eq.~\eqref{eq:uncC} by construction.

Figure~\ref{fig:RelativeDeviationCompare} displays
these spreads as relative deviations (total spread is $2\sigma$), in percent,
from the reference parameter set
$\LamSRG=1.88\;\fmin$, $\omega_H=18\;\MeV$,
$\Ntot=14$, at photon energies $\omega=60$, $86$,
and $100\;\MeV$ for two representative scattering
angles. The percentage spread among the retained
parameter combinations grows with photon energy: at
$60\;\MeV$ it ranges from approximately $5\%$ at
backward angles ($\theta=159^\circ$) to roughly
$7\%$ at forward angles ($\theta=40^\circ$), while
at $100\;\MeV$ it reaches approximately $9\%$ at
forward angles. Across all energies and angles,
backward-angle kinematics ($\theta=159^\circ$)
exhibit systematically smaller percentage spreads
than their forward-angle counterparts
($\theta=40^\circ$). The percentage representation
complements the absolute spreads of
fig.~\ref{fig:NtotConvergeC}, where the uncertainty
band of $5$--$10\;\nb/\mathrm{sr}$ appears
approximately uniform because the larger absolute
cross sections at lower energies mask what is in
fact a smaller fractional uncertainty.

As discussed in sec.~\ref{sec:SRGcutoff} the NN cutoffs $\LamNN=450\;\MeV$ and $500\;\MeV$ are
selected following the recommendation of Millican
\etal~\cite{SMS400550}. The harmonic-oscillator
frequencies $\omega_H=16\;\MeV$ and $18\;\MeV$ are chosen
because they produce binding energies of $\LiS$ closest to
the experimental value. 
Table~\ref{table:BEdevC} collects the computed $\LiS$
binding energies at $\Ntot=14$ and $\omega_H=18\;\MeV$
for the parameter combinations used in the present
analysis. The deviations from the experimental value
$E_{\mathrm{exp}}=-31.995\;\MeV$ range from $0.75$ to $1.37\;\MeV$, corresponding to
$2.3$--$4.3\%$ of $|E_{\mathrm{exp}}|$. Softer SRG
flow parameters ($\LamSRG=1.88\;\fmin$) yield binding
energies closer to experiment than the harder value
$\LamSRG=2.236\;\fmin$, consistent with the improved
NCSM convergence expected for a more strongly
decoupled Hamiltonian. Similarly, $\LamNN=500\;\MeV$
produces slightly better agreement than
$\LamNN=450\;\MeV$ at both values of $\LamSRG$.
\begin{table}[ht]
\centering
{\setlength{\tabcolsep}{4pt}
\small
\begin{tabular}{l rr rrrr rr}
\toprule
& \multicolumn{6}{c}{$\LamSRG=1.88\;\fmin$}
& \multicolumn{2}{c}{$\LamSRG=2.236\;\fmin$} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-9}
$\omega_H\;[\MeV]$
  & 16 & 16 & 18 & 18 & 18 & 18 & 18 & 18 \\
$\LamNN\;[\MeV]$
  & 400 & 550 & 400 & 450 & 500 & 550 & 450 & 500 \\
\midrule
$|E-E_{\mathrm{exp}}|\;[\MeV]$
  & 0.93 & 0.45 & 0.99 & 0.89 & 0.75
  & 0.48 & 1.37 & 1.32 \\
\bottomrule
\end{tabular}
}
\caption[Lithium 6 binding energy deviations from experiment]{Binding energy deviations from experiment for $\LiS$ }
\label{table:BEdevC}
\end{table}
While reproducing the correct
binding energy is a necessary quality criterion for the
nuclear wave function, it is not sufficient: Compton
scattering at finite momentum transfer also probes
off-diagonal components of the density that are not
strongly constrained by the binding energy alone.

For this reason, convergence with respect to $\Ntot$,
$\omega_H$, and $\LamSRG$ must be examined independently.
Using smaller values of $\LamSRG$ improves calculation time, and some aspects of convergence, but also increases the contributions of many-body interactions
in the back transformation; therefore $\LamSRG$ must be selected such that these aspects are balanced.
The SRG flow parameters
$\LamSRG=1.88$ and $2.236\;\fmin$ are retained; the more
extreme value $\LamSRG=3.0\;\fmin$ is excluded from the
final results as it exhibits poor convergence behavior
in $\Ntot$, see fig.~\ref{fig:RelativeDeviationCompare}.
The set of plausible cross-section values at a
given energy and angle is then defined as the 8 combinations
\begin{equation}
  S(\omega,\theta) = \left\{
  \frac{\dd \sigma}{\dd\Omega} \,\middle|\,
    \begin{array}{l}
      \Ntot = 14;\;\quad\;\quad\;\;\,\,
      \LamNN = 450,500\;\MeV \\
       \omega_H = 16,18\;\MeV;\;
       \LamSRG = 1.88,2.236\;\fmin
    \end{array}
  \right\}\;.
  \label{eq:densityGoodVals}
\end{equation}
For reactions in which TDAs without the SRG evolution are
available, the corresponding SRG parameters are of course absent and this
set reduces to variation over
$\LamNN=450,500\;\MeV$ only.
The reported central values and uncertainties are
\begin{equation}
\begin{split}
&\frac{\dd \sigma}{\dd\Omega}= \mathrm{Mean}(S)\;\\
                            \sigma= \sqrt{\sigma_1^2+\sigma_2^2}\quad
&\sigma_1=\frac{\max(S)-\min(S)}{2}\quad
\sigma_2=\left(0.05\;\mathrm{Mean}(S)\right)
\;.
\end{split}
\label{eq:uncC}
\end{equation}
where $\sigma_1$ is the half-spread
over the parameter combinations of eq.~\eqref{eq:densityGoodVals}. This half-spread estimate
is deliberately conservative: it exceeds the standard
deviation of $S$ by construction and is intended to, in
part, subsume additional sources of uncertainty inherent
in the TDA approach, including the residual $\Ntot$
dependence discussed above.
The second term adds an additional $5\%$ of the cross
section in quadrature to account for sources of
theoretical uncertainty not captured by the
parameter-space variation alone, including the
\chiEFT{} truncation at \NXLO{3}, and the lack of $3 \mathrm{N}- 6 \mathrm{N}$ contributions.
Averaged over all energies and angles, 
the total uncertainty is approximately $6\%$ of the cross
section.
The uncertainties reported in
table~\ref{table:LiSCrossSecC} and the bands displayed
in figs.~\ref{fig:6LiResultsPlot}
and~\ref{fig:RelativeDeviationCompare} incorporate both
contributions as prescribed by eq.~\eqref{eq:uncC}.
Numerical values are
collected in table~\ref{table:LiSCrossSecC}. For
comparison with data, see fig.~\ref{fig:6LiResultsPlot}.
% This is the "base" table, without the extra 5% uncertainties added in DO NOT REMOVE THIS TABLE
% \begin{table}
% \centering
% \begin{tabular}{|c||c|c||c||c|c||c|}
% \hline
% \multirow{2}{*}{$\theta$}
%   & \multicolumn{2}{c||}{$60\;\MeV$}
%   & {$75\;\MeV$}
%   & \multicolumn{2}{c||}{$86\;\MeV$}
%   & {$100\;\MeV$} \\
% \cline{2-7}
% \rule{0pt}{2.5ex}
%   & TDA & Data~\cite{60MeV}
%   & TDA
%   & TDA & Data~\cite{86MeV}
%   & TDA \\
% \noalign{\hrule height 1.5pt}
%  1  & $337\pm11$ &            & $283\pm10$
%     & $237\pm 9$ &            & $171\pm7$ \\
%  40 & $260\pm 8$ & $196\pm12$ & $213\pm 7$
%     & $174\pm 8$ & $203\pm21$ & $125\pm6$ \\
%  55 & $213\pm 7$ & $176\pm10$ & $171\pm 6$
%     & $140\pm 5$ & $147\pm13$ & $101\pm4$ \\
%  75 & $165\pm 5$ & $125\pm 8$ & $130\pm 4$
%     & $106\pm 4$ & $140\pm14$ & $ 77\pm3$ \\
%  90 & $150\pm 5$ & $135\pm 8$ & $117\pm 4$
%     & $ 95\pm 3$ & $159\pm15$ & $ 70\pm2$ \\
% 110 & $158\pm 5$ & $138\pm 9$ & $121\pm 4$
%     & $ 97\pm 3$ & $146\pm21$ & $ 72\pm2$ \\
% 125 & $178\pm 5$ & $177\pm11$ & $134\pm 4$
%     & $107\pm 3$ &            & $ 78\pm2$ \\
% 145 & $211\pm 6$ & $178\pm11$ & $156\pm 4$
%     & $122\pm 4$ & $167\pm20$ & $ 88\pm3$ \\
% 159 & $230\pm 6$ & $193\pm10$ & $168\pm 5$
%     & $129\pm 6$ & $172\pm15$ & $ 91\pm4$ \\
% 180 & $241\pm 7$ &            & $176\pm 5$
%     & $136\pm 4$ &            & $ 96\pm3$ \\
% \hline
% \end{tabular}
% \caption[${}^6$Li Compton differential cross section values]{Differential cross section for Compton
% scattering on $\LiS$ in units of $\nb/\mathrm{sr}$.
% TDA results include one- and two-body contributions
% through $\calO(e^2\delta^3)$ [\NXLO{3}].
% Data at $60\;\MeV$ from
% ref.~\cite{60MeV}; data at $86\;\MeV$ from
% ref.~\cite{86MeV}.
% Uncertainties estimated through \meqref{eq:uncC}.
% TDA calculations are performed in the center-of-mass
% frame; for $\LiS$ the difference between center-of-mass
% and laboratory kinematics is at most $2\%$
% and is neglected. Values are plotted in fig.~\ref{fig:6LiResultsPlot}.
% }
% \label{table:LiSCrossSecC}
% \end{table}
% this table is WITH additional 5% uncer
\begin{table}
\centering
\begin{tabular}{|c||c|c||c||c|c||c|}
\hline
\multirow{2}{*}{$\theta$}
  & \multicolumn{2}{c||}{$60\;\MeV$}
  & {$75\;\MeV$}
  & \multicolumn{2}{c||}{$86\;\MeV$}
  & {$100\;\MeV$} \\
\cline{2-7}
\rule{0pt}{2.5ex}
  & TDA & Data~\cite{60MeV}
  & TDA
  & TDA & Data~\cite{86MeV}
  & TDA \\
\noalign{\hrule height 1.5pt}
 1  & $337\pm20$ &            & $283\pm17$
    & $237\pm15$ &            & $171\pm11$ \\
 40 & $260\pm15$ & $196\pm12$ & $213\pm13$
    & $174\pm12$ & $203\pm21$ & $125\pm 9$ \\
 55 & $213\pm13$ & $176\pm10$ & $171\pm10$
    & $140\pm 9$ & $147\pm13$ & $101\pm 6$ \\
 75 & $165\pm10$ & $125\pm 8$ & $130\pm 8$
    & $106\pm 7$ & $140\pm14$ & $ 77\pm 5$ \\
 90 & $150\pm 9$ & $135\pm 8$ & $117\pm 7$
    & $ 95\pm 6$ & $159\pm15$ & $ 70\pm 4$ \\
110 & $158\pm 9$ & $138\pm 9$ & $121\pm 7$
    & $ 97\pm 6$ & $146\pm21$ & $ 72\pm 4$ \\
125 & $178\pm10$ & $177\pm11$ & $134\pm 8$
    & $107\pm 6$ &            & $ 78\pm 4$ \\
145 & $211\pm12$ & $178\pm11$ & $156\pm 9$
    & $122\pm 7$ & $167\pm20$ & $ 88\pm 5$ \\
159 & $230\pm13$ & $193\pm10$ & $168\pm10$
    & $129\pm 9$ & $172\pm15$ & $ 91\pm 6$ \\
180 & $241\pm14$ &            & $176\pm10$
    & $136\pm 8$ &            & $ 96\pm 6$ \\
\hline
\end{tabular}
\caption[${}^6$Li Compton differential cross section values]{Differential cross section for Compton
scattering on $\LiS$ in units of $\nb/\mathrm{sr}$.
TDA results include one- and two-body contributions
through $\calO(e^2\delta^3)$ [\NXLO{3}].
Data at $60\;\MeV$ from
ref.~\cite{60MeV}; data at $86\;\MeV$ from
ref.~\cite{86MeV}.
Uncertainties estimated through \meqref{eq:uncC},
which combines the parameter-space half-spread with an
additional $5\%$ of the cross section added in quadrature. 
Uncertainties are deliberately conservative; a complete Bayesian analysis is deferred to future work.
TDA calculations are performed in the center-of-mass
frame; for $\LiS$ the difference between center-of-mass
and laboratory kinematics is at most $2\%$
and is neglected. Values are plotted in fig.~\ref{fig:6LiResultsPlot}.
}
\label{table:LiSCrossSecC}
\end{table}
\begin{figure}%[H]
\centering
 \includegraphics[width=0.9\linewidth]{Comp6LiCombine.pdf}
\caption[Differential cross section for Compton scattering on ${}^6$Li compared to data]{
Differential cross section for Compton
scattering on $\LiS$ in units of $\nb/\mathrm{sr}$.
TDA results include one- and two-body contributions
through $\calO(e^2\delta^3)$ [\NXLO{3}].
Data at $60\;\MeV$ from
ref.~\cite{60MeV}; data at $86\;\MeV$ from
ref.~\cite{86MeV} does not include systematic uncertainty errors.
Uncertainties estimated through \meqref{eq:uncC},
which combines the parameter-space half-spread with an
additional $5\%$ of the cross section added in quadrature.
TDA calculations are performed in the center-of-mass
frame; for $\LiS$ the difference between center-of-mass
and laboratory kinematics is at most $2\%$
and is neglected. Values correspond to table~\ref{table:LiSCrossSecC}.
}
\label{fig:6LiResultsPlot}
\end{figure}

\subsection{Theoretical Uncertainties}
\label{sec:ComptonUncC}
\begin{figure}
\centering
\includegraphics[width=\linewidth]{OrderByOrder1.pdf}
\caption[Order-by-order convergence of ${}^6$Li Compton cross section]{Order-by-order convergence of
  the $\LiS$ Compton differential cross section. Left
  panels: angular distributions at
  $\omega_{\mathrm{lab}}=60,\;75,\;86,$ and $100\;\MeV$.
  Right panels: energy dependence at
  $\theta_{\mathrm{lab}}=40^\circ,\;110^\circ,$ and
  $159^\circ$. Curves show results at \NXLO{3}
  [$\calO(e^2\delta^3)$, red solid], \NXLO{2}
  [$\calO(e^2\delta^2)$, blue dashed], and LO
  [$\calO(e^2\delta^0)$, green dotted], using the
  $\chi$SMS potential with
  $\LamNN\in\{450,500\}\;\MeV$ and
  $\LamSRG\in\{1.88,2.236\}\;\fmin$. For $\LiS$,
  center-of-mass and laboratory frame variables
  coincide to within $2\%$.}
\label{fig:orderbyorder1}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=1.0\linewidth]{OrderByOrderEnergy.pdf}
\caption[Order-by-order convergence of ${}^6$Li Compton scattering with uncertainty bands]{Order-by-order convergence of
  Compton scattering on $\LiS$ with uncertainty bands at
  $\omega_{\mathrm{lab}}=60,\;75,\;86,$ and $100\;\MeV$.
Bands show results at LO [$\calO(e^2\delta^0)$],
\NXLO{2} [$\calO(e^2\delta^2)$], and \NXLO{3}
[$\calO(e^2\delta^3)$]. An additional band shows the
effect of including the incomplete \NXLO{4}
[$\calO(e^2\delta^4)$] two-body contribution
($T_{12}=0$ channel only; the $T_{12}=1$ channel is
not yet available) as a convergence indicator.
   The spread
  of each band reflects the parameter variation of
  eq.~\eqref{eq:densityGoodVals}. The same $\chi$SMS potentials
  as in fig.~\ref{fig:orderbyorder1} are employed.
  Center-of-mass and laboratory variables coincide
  to within $2\%$ for $\LiS$.}
\label{fig:orderbyorder2}
\end{figure}

Following the approach of
refs.~\cite{hammer4He,hammer2020}, the theoretical
uncertainties of the present Compton calculation are
assessed using three complementary criteria, each based
on the \chiEFT{} expansion.

Both the one- and two-body Compton amplitudes are
complete through \NXLO{3} [$\calO(e^2\delta^3)$]; the
two-body kernel first enters at \NXLO{2}
[$\calO(e^2\delta^2)$] and receives no additional
contributions at \NXLO{3}. The dominant omitted terms
therefore begin at $\calO(e^2\delta^4)$ in both the
one- and two-body kernels, contributing a relative
uncertainty of order
$\delta^4\approx(0.4)^4\approx 3\%$ in the amplitude,
or approximately $\pm 6\%$ in the cross section.
This first method is the a priori estimate and
provides a lower bound on the expected
accuracy~\cite{hammer4He}.
The second method is the spread-based uncertainty of
\meqref{eq:uncC}, which captures the combined
dependence on $\LamNN$, $\omega_H$, and $\LamSRG$.
At $60\;\MeV$ this spread
amounts to approximately $\pm 3$--$4\%$ across all
angles, growing to approximately $\pm 4$--$6\%$ at
$100\;\MeV$. Softer interactions (smaller $\LamNN$ and
$\LamSRG$) consistently yield slightly lower cross
sections, mirroring the pattern observed for
$\HeF$~\cite{hammer4He}.

\begin{figure}
\centering
\includegraphics[width=0.85\linewidth]{LambdaCut_variation.pdf}
\caption[Variation of ${}^6$Li Compton cross section with NN cutoff]{Variation of the $\LiS$ Compton differential
  cross section with respect to the NN cutoff $\LamNN$,
  shown as a percentage of the cross section, as a
  function of scattering angle $\theta$ at
  $\omega_{\mathrm{lab}}=60$, $75$, $86$, and
  $100\;\MeV$. For each energy and angle, the
  variation between the $\Lambda=450\,\MeV$ and $\Lambda=500\,\MeV$ results are computed by averaging over the retained
  values of $\omega_H$ and $\LamSRG$ at $\Ntot=14$.
  The black curve shows the average across all four
  energies; the overall average variation is $5.4\%$.}
\label{fig:LambdaCutoffVar}
\end{figure}

To isolate the contribution of the NN cutoff $\LamNN=450\;\MeV,\,500\;\MeV$
to the overall parameter-space spread,
fig.~\ref{fig:LambdaCutoffVar} displays the percentage
variation of the cross section with respect to
$\LamNN$, averaged over the retained values of
$\omega_H$ and $\LamSRG$, as a function of scattering
angle. The cutoff variation is remarkably flat in
$\theta$, with an average across all energies and
angles of $5.4\%$: approximately $4.5$--$5\%$ at
$60\;\MeV$, rising to roughly $5.5$--$6\%$ at
$100\;\MeV$. The growth with energy suggests that a
portion of the higher-order dependence in the chiral
expansion is attributable to the NN cutoff. Because
$\LamNN$ is one of the parameters defining the set
$S(\omega,\theta)$ of \meqref{eq:uncC}, this $5.4\%$
variation is not independent of the total
parameter-space spread; however, the decomposition
clarifies that the NN cutoff is a large source of
uncertainty. The additional $5\%$ included in
\meqref{eq:uncC} provides a conservative estimate of
contributions from many-body interactions (3N through
6N) not explicitly included in the present $\LiS$
calculation; a full Bayesian analysis of the
uncertainty budget is deferred to a forthcoming
publication~\cite{long_2026}.

The results presented are converged within tolerances
between $\Ntot=12$ and $14$, but the residual
differences between these two truncations add a
systematic uncertainty that cannot be quantified
precisely without access to $\Ntot\geq 16$ results.
Extrapolating the observed convergence pattern, in
which successive increments in $\Ntot$ produce
progressively smaller shifts, the residual change from
$\Ntot=14$ to $16$ is expected to be smaller than that
from $12$ to $14$.
The effect is most pronounced for larger
$\LamSRG$ values, which is the primary reason for
excluding $\LamSRG=3.0\;\fmin$ from the reported
results. Restricting the analysis to $\Ntot=14$ and
$\LamSRG\leq 2.236\;\fmin$ limits this residual effect
to the $5\%$ level.
A more rigorous assessment using Bayesian methods for
EFT truncation errors is deferred to a future study in
which higher-$\Ntot$ densities become available.

The third method of uncertainty estimation is a
post-facto check based on the order-by-order convergence
of the \chiEFT{} expansion, displayed in
figs.~\ref{fig:orderbyorder1}
and~\ref{fig:orderbyorder2}.
The correction from LO to \NXLO{2}
[$\calO(e^2\delta^2)$], which incorporates the Born
terms, pion-cloud contributions to the
polarizabilities, and the leading charged-pion-exchange
two-body currents, is substantial at all energies. At
$60\;\MeV$, this correction amounts to roughly $50\%$
of the LO cross section, consistent with the pattern
observed for $\HeT$~\cite{hammer2020} and
$\HeF$~\cite{hammer4He}. This large shift is expected:
at LO, only the proton Thomson term contributes, and
the charged-pion-exchange currents between $np$ pairs
are entirely absent. As noted in
ref.~\cite{hammer4He}, the size of the
LO-to-\NXLO{2} correction is a poor predictor of
higher-order terms and is therefore not used to
estimate uncertainties.

The subsequent correction from \NXLO{2} to \NXLO{3}
[$\calO(e^2\delta^3)$], which introduces the
$\Delta(1232)$ excitation, but no new 2N corrections,
is markedly smaller, amounting to at most
${\sim2}\%$ of the cross section at
$60$--$86\;\MeV$. This correction becomes appreciable
only above $\omega\approx 80\;\MeV$
(see fig.~\ref{fig:orderbyorder1}).

Towards $100\;\MeV$, the $\Delta(1232)$ modifies the
angular dependence of the cross section, reducing
forward-angle values while enhancing backward-angle
values by as much as $9\%$, consistent with the
behavior reported for $\HeF$ in
ref.~\cite{hammer4He} (see their fig.~6).
That the $\Delta(1232)$ has such a pronounced effect
well below its resonance energy reflects the sizeable
dispersive correction it adds to the magnetic
polarizability, which can be as large as the static
value of $\beta_{M1}^{(s)}$
itself~\cite{hammer4He}.

A complementary observation from
fig.~\ref{fig:orderbyorder2}
is that the width of the parameter-space bands
increases from LO through \NXLO{2} to \NXLO{3}. This
widening does not indicate a breakdown of the chiral
expansion, whose central values converge as discussed
above, but rather reflects the increasing sensitivity
of higher-order contributions to the nuclear-structure
parameters. At LO, only the proton Thomson term
contributes, which depends on global nuclear properties
and is largely insensitive to $\LamNN$, $\omega_H$,
and $\LamSRG$. The two-body meson-exchange currents
entering at \NXLO{2} and the $\Delta(1232)$
contributions at \NXLO{3} probe progressively
shorter-range components of the density, amplifying the
dependence on the SRG evolution and the model-space
truncation. The parameter-space spread at the highest
computed order is therefore the physically relevant
measure of nuclear-structure uncertainty.

Figure~\ref{fig:orderbyorder2} further shows that the
incomplete two-body contribution at \NXLO{4}
[$\calO(e^2\delta^4)$], comprising only the $T_{12}=0$
isospin channel (the $T_{12}=1$ channel is not yet
available), produces only a modest, largely
angle-independent shift relative to the \NXLO{3}
result. Although this partial higher-order calculation
is not included in the reported cross sections, it
serves as a valuable indicator that higher-order
two-body corrections are small,
confirming that the chiral expansion of the
Compton kernel remains well controlled for $\LiS$ in
the energy range considered. The progressive narrowing
of corrections at each successive order is consistent
with the a priori estimate of approximately $\pm 6\%$
in the cross section. The cumulative role of all
two-body mechanisms is examined in more detail below.
\begin{figure}
\centering
\includegraphics[width=\linewidth]{twobody_convergence_6Li.pdf}
\caption[Relative magnitude of two-body contributions to ${}^6$Li Compton scattering]{Relative magnitude of two-body
  contributions to $\LiS$ Compton scattering as a
  function of $\theta$ at \NXLO{3}, $\calO(e^2\delta^3)$. The quantity
  plotted is
  $\sqrt{(d\sigma/d\Omega)^{1\mathrm{N}+2\mathrm{N}}
  /(d\sigma/d\Omega)^{1\mathrm{N}}}-1$, which measures
  the fractional correction at the amplitude level when
  all two-body mechanisms are included. Curves are shown
  at $\omega_{\mathrm{lab}}=60$ (solid),
  $75$ (dashed), $86$ (dash-dotted), and
  $100\;\MeV$ (dotted); the legend lists the
  angle-averaged effective $n$-body expansion parameter for $\mathcal{M}$,
  $Q_{\mathrm{few}}$, for each energy. Bands
  reflect the parameter variation of
  eq.~\eqref{eq:densityGoodVals}. The same $\chi$SMS potentials
  as in fig.~\ref{fig:orderbyorder1} are employed.
  Center-of-mass and laboratory variables coincide
  to within $2\%$ for $\LiS$.}
\label{fig:twobodyconvergence}
\end{figure}

The cumulative impact of two-body mechanisms on the
$\LiS$ Compton cross section is quantified in
fig.~\ref{fig:twobodyconvergence}, which displays the
fractional correction to the amplitude,\\
$\sqrt{(d\sigma/d\Omega)^{1\mathrm{N}+2\mathrm{N}}
/(d\sigma/d\Omega)^{1\mathrm{N}}}-1$,
as a function of center-of-mass scattering angle.
The angle-averaged value of this ratio defines an
effective expansion parameter $Q_{\mathrm{few}}$
that characterizes the overall strength of two-body
contributions relative to the one-body result.
At $60\;\MeV$, $Q_{\mathrm{few}}=0.61$,
indicating that the combined two-body mechanisms
increase the amplitude by roughly $60\%$, which
corresponds to approximately a factor of $2.6$ in the
cross section. This value grows monotonically with
photon energy: $Q_{\mathrm{few}}=0.72$ at
$75\;\MeV$, $0.85$ at $86\;\MeV$, and $1.14$ at
$100\;\MeV$. The angular dependence is mild at all
energies, with a slight increase toward backward
angles.

The growth of $Q_{\mathrm{few}}$ with energy
reflects the increasing importance of meson-exchange
currents, particularly the charged-pion-exchange
diagrams that dominate the two-body sector. That
$Q_{\mathrm{few}}$ exceeds unity at $100\;\MeV$
indicates that the two-body contribution to the cross
section surpasses the one-body contribution at that
energy. This does not signal a breakdown of the chiral
expansion, since $Q_{\mathrm{few}}$ conflates
contributions from several chiral orders and the
order-by-order convergence of
figs.~\ref{fig:orderbyorder1}
and~\ref{fig:orderbyorder2} remains well-behaved.
Rather, it signals a possible lack of convergence in
the $n$-body expansion of \meqref{eq:totalscat},
highlighting the need for $3\mathrm{N}$ contributions
to be included.

Several considerations suggest, however, that the
missing $3\mathrm{N}$ Compton contributions are
unlikely to be as large as a naive extrapolation of
$Q_{\mathrm{few}}$ would imply.

First, the large $Q_{\mathrm{few}}$ reflects, in
part, the smallness of the one-body baseline rather
than an anomalously large two-body numerator. Because
$\LiS$ is an isoscalar target ($T=0$), the one-body
Compton amplitude is proportional to the total nuclear
charge $Z=3$ through the Thomson term, whereas the
two-body amplitude benefits from all $3\times 3=9$
$np$ pairs through the charged-pion-exchange mechanism
of \meqref{eq:isospin_np_selectionC}. The ratio
$2\mathrm{N}/1\mathrm{N}$ is therefore inflated by the
mismatch between a charge-counting one-body term and a
pair-counting two-body term, and the
$3\mathrm{N}/2\mathrm{N}$ ratio need not be comparably
large.

Second, the two-body dominance arises from a specific
physical mechanism, namely the coupling of the photon
to the long-range charged-pion-exchange current between
$np$ pairs, which has no direct three-body analogue at
the same chiral order. Three-body Compton diagrams
require at least two simultaneous meson exchanges
connecting three nucleons to both photon vertices,
which introduces additional powers of $\delta$ and
places the leading $3\mathrm{N}$ contribution at a
higher chiral order than the leading $2\mathrm{N}$
diagrams.

Third, the chiral expansion converges well order by
order, as demonstrated in figs.~\ref{fig:orderbyorder1}
and~\ref{fig:orderbyorder2}, providing evidence that
these higher-order contributions are suppressed by the
expected powers of $\delta\approx 0.4$.
Nevertheless, a quantitative assessment of the
$3\mathrm{N}$ Compton contribution requires an
explicit calculation and is left to future work.

\subsection{Comparison with Other Few-Nucleon Targets}
\label{sec:ComptonCompareC}
To place the $\LiS$ results in context, it is instructive
to compare the predicted cross sections with those obtained
for lighter targets using the same Compton kernel at
\NXLO{3} [$\calO(e^2\delta^3)$]. The $\HeF$ calculation of
ref.~\cite{hammer4He} predicts that Compton cross sections
on the deuteron, $\HeT$, and $\HeF$ are approximately in
the ratio $1:2:5$ at $\omega=120\;\MeV$. This predicted
hierarchy reflects the dominant role of charged-pion-exchange
currents between correlated $np$ pairs~\cite{hammer4He}.
At photon energies $\omega\sim 100$--$120\;\MeV$, the
wavelength $1/\omega$ becomes comparable to the range
$1/\mpi$ of one-pion exchange, so that the photon couples
not only to the individual nucleon constituents but also to
the charged long-range currents binding them into the
nucleus~\cite{hammer4He}; see fig.~\ref{fig:2BdiagramsC}.
Although the highest photon energy considered in the present
work, $\omega=100\;\MeV$, lies below the $120\;\MeV$ at
which the $1:2:5$ ratio is quoted, the meson-exchange
mechanism that drives this hierarchy is already active at
this energy. As demonstrated below, the $\LiS$ cross
sections confirm that a comparable scaling pattern persists
at the energies considered here.

This selectivity of the two-body Compton kernel for $np$
pairs follows from the isospin structure of the leading
charged-pion-exchange diagrams~\cite{hammer4He}. All
two-body diagrams that contribute at this order share a
common isospin factor,
\begin{equation}
\left\langle t_{12} m_{12}^{t \prime}\right|
\left(\tau^{(1)} \cdot \tau^{(2)}
  -\tau_z^{(1)} \tau_z^{(2)}\right)
\left|t_{12} m_{12}^t\right\rangle
=2(-1)^{t_{12}+1}
  \delta_{m_{12}^{t \prime} m_{12}^t}\,
  \delta_{m_{12}^t 0}\;,
  \label{eq:isospin_np_selectionC}
\end{equation}
where $t_{12}$ and $m_{12}^{t}$ denote the pair isospin
and its projection~\cite{hammer4He}. The Kronecker delta
$\delta_{m_{12}^t 0}$ restricts the sum over active pairs
to those with vanishing isospin projection, i.e.\ $np$
pairs, while pairs of identical nucleons ($pp$ with
$m_{12}^{t}=+1$ and $nn$ with $m_{12}^{t}=-1$) give a
vanishing matrix element. The underlying operator
$\tau_+^{(1)}\tau_-^{(2)} + \tau_-^{(1)}\tau_+^{(2)}$
exchanges the isospin labels of the two active nucleons
and therefore requires one proton and one neutron in the
pair. This $np$-pair selection rule is a general feature
of the leading two-body meson-exchange currents in \chiEFT
and governs the scaling of two-body contributions across
different nuclear targets~\cite{hammer4He}.

Consequently, the two-body contribution to the Compton
cross section is expected to scale with the number of $np$
pairs in the target nucleus~\cite{hammer4He}. Because protons and neutrons
are distinguishable, a nucleus with $a$ protons and $b$
neutrons contains $a\times b$ such pairs (pairs selected with replacement). The deuteron has
$1$ $np$ pair, $\HeT$ has $2$ (plus one $pp$ pair), $\HeF$
has $4$ (plus one $pp$ and one $nn$ pair), and $\LiS$ with
$3$ protons and $3$ neutrons has $9$ $np$ pairs (out of
$\binom{6}{2}=15$ total nucleon pairs). The resulting ratio
of $np$ pairs across the sequence
$d:\HeT:\HeF:\LiS$ is therefore $1:2:4:9$.
%
This combinatorial ratio accounts for the bulk of the
predicted cross-section hierarchy
$1:2:5:10$~\cite{hammer4He}. The additional enhancement
beyond pure pair counting in the tightly bound systems
$\HeF$ and $\LiS$ is attributable to the larger overlap of
nucleon wave functions at short internucleon separations,
which amplifies the meson-exchange contributions. Notably,
the enhancement is proportionally larger for $\HeF$, where
all nucleons occupy $s$-wave orbitals, than for $\LiS$,
where the two valence nucleons beyond the $\HeF$ core
reside in $p$-wave orbitals at larger average separations,
partially diluting the overlap with the short-range
two-body kernel. The $\LiS$ cross sections in
table~\ref{table:LiSCrossSecC} are indeed larger than the
corresponding $\HeF$ values reported in
ref.~\cite{hammer4He} at $\omega=60\;\MeV$ by roughly a
factor of two across the measured angular range. At
$100\;\MeV$, the $\LiS$ cross section remains approximately
twice that of $\HeF$, confirming that the hierarchy persists
across the full energy range considered in the present work.
This continued growth is consistent with the dominant role
of charged-pion-exchange currents between correlated $np$
pairs in heavier isoscalar systems.

Each target in this sequence is also sensitive to different
combinations of nucleon polarizabilities: the deuteron and
$\HeF$ probe the scalar-isoscalar combinations
$\alpha_{E1}^{(p)}+\alpha_{E1}^{(n)}$ and
$\beta_{M1}^{(p)}+\beta_{M1}^{(n)}$ only, while $\HeT$
accesses roughly
$2\alpha_{E1}^{(p)}+\alpha_{E1}^{(n)}$~\cite{hammer2020}.
As an isoscalar target, $\LiS$ probes the same combinations
as the deuteron and $\HeF$, but with enhanced event rates
owing to the larger cross section. Moreover, these targets
span a wide range of binding energies, from the loosely
bound deuteron through the trinucleons to the tightly bound
$\HeF$ and $\LiS$; comparing Compton cross sections across
this sequence therefore also tests the \chiEFT{} description
of two-nucleon pion-exchange currents in markedly different
nuclear environments~\cite{hammer4He}. A global fit across
all these targets would exploit these complementary linear
combinations.


\subsection{Comparison with Data}
\label{sec:ComptonDataC}
Data for Compton scattering on $\LiS$ have been obtained
at the High Intensity $\gamma$-Ray Source (HI$\gamma$S)
at two energies: eight angular points at
$\omega_{\mathrm{lab}}=60\;\MeV$ by Myers
\etal~\cite{60MeV}, and seven angular points at
$\omega_{\mathrm{lab}}=86\;\MeV$ by Myers
\etal~\cite{86MeV}. Both measurements employed a
quasi-monochromatic photon beam and cover the angular
range $40^\circ\lesssim\theta\lesssim 159^\circ$.
Numerical values are collected alongside the TDA
predictions in table~\ref{table:LiSCrossSecC}; graphical
comparisons are presented in fig.~\ref{fig:6LiResultsPlot}.
The TDA predictions are computed in the center-of-mass
frame. For $\LiS$, the kinematic transformation to
laboratory variables introduces a correction of at
most $\omega/M_{{}^6\mathrm{Li}}\approx 2\%$ at the
highest energy and most backward angle, which is
well within the theoretical uncertainties and is
therefore neglected. The correction is mildly
angle-dependent, favoring slightly different lab
energies at forward and backward angles for a given
center-of-mass energy, but this tilt is negligible
at the present level of accuracy.

At $60\;\MeV$, the data exhibit a minimum near
$\theta\approx 75^\circ$ ($[125\pm 8]\;\nb/\mathrm{sr}$),
rising to $[196\pm 12]\;\nb/\mathrm{sr}$ at
$\theta=40^\circ$ and $[193\pm 10]\;\nb/\mathrm{sr}$ at
$\theta=159^\circ$, with typical uncertainties of
$8$--$12\;\nb/\mathrm{sr}$. The TDA predictions at this
energy lie in the range $150$--$260\;\nb/\mathrm{sr}$
over the same angular interval. The calculation
systematically overpredicts the data at most angles,
with the ratio of theory to data ranging from
approximately $1.0$ near $\theta=125^\circ$ to
approximately $1.3$ at $\theta=40^\circ$ and
$\theta=75^\circ$, corresponding to an overall
normalization offset of roughly $20$--$30\%$. Despite
this offset, the angular shape of the cross section is
well reproduced: both theory and data display the
characteristic minimum near
$\theta\approx 75^\circ$--$90^\circ$ and the rise toward
forward and backward angles that is expected from the
interplay of Thomson, polarizability, and
meson-exchange contributions.

At $86\;\MeV$, the pattern of discrepancy reverses. The
data span a range from $[140\pm 14]\;\nb/\mathrm{sr}$ at
$\theta=75^\circ$ to $[203\pm 21]\;\nb/\mathrm{sr}$ at
$\theta=40^\circ$, with uncertainties of
$13$--$21\;\nb/\mathrm{sr}$ that are considerably larger
than those at $60\;\MeV$. The TDA predictions at this
energy range from $[95\pm 6]\;\nb/\mathrm{sr}$ at
$\theta=90^\circ$ to $[174\pm 12]\;\nb/\mathrm{sr}$ at
$\theta=40^\circ$. In contrast to the $60\;\MeV$ case,
the data now lie systematically above the theoretical
central values across most of the angular range. The
discrepancy is largest near $\theta=90^\circ$, where the
measured cross section ($[159\pm 15]\;\nb/\mathrm{sr}$)
exceeds the prediction ($[95\pm 6]\;\nb/\mathrm{sr}$) by
approximately $67\%$. At forward and backward angles the
discrepancy is smaller, approximately $15$--$35\%$, but
persists throughout the measured angular range. While
the angular shape predicted by the TDA calculation is
qualitatively consistent with the data, with both
exhibiting a minimum near $\theta\approx 90^\circ$, the
depth of this minimum is significantly more pronounced
in the theory than in the data.

A noteworthy feature of the $86\;\MeV$ data is that
several angular points yield cross sections comparable
to or exceeding the corresponding values at $60\;\MeV$.
For example, at $\theta=90^\circ$ the measured cross
section increases from $[135\pm 8]\;\nb/\mathrm{sr}$ at
$60\;\MeV$ to $[159\pm 15]\;\nb/\mathrm{sr}$ at
$86\;\MeV$, contrary to the monotonic decrease with
energy expected on general grounds and predicted by the
TDA calculation. A similar non-monotonic pattern appears
at $\theta=40^\circ$ ($[196\pm 12]$ vs.\
$[203\pm 21]\;\nb/\mathrm{sr}$). Whether this reflects a
genuine physical effect or arises from correlated
systematic uncertainties in the $86\;\MeV$ data warrants
further investigation.

Several factors may contribute to the observed discrepancies
between theory and data at both energies. First, as discussed
in sec.~\ref{sec:ComptonKernelC}, the present calculation
does not include coherent propagation of the $A$-body
intermediate state between the two photon vertices. Although
the chiral power counting predicts this mechanism to be
suppressed at the energies considered here, the residual
correction need not vanish exactly. For $\LiS$, which has a
larger binding energy than the deuteron, coherent-propagation
effects may persist to somewhat higher energies than in the
two-nucleon case, in line with the trend reported for
$\HeF$~\cite{hammer4He}. Incorporating such contributions
would lower the predictions at $60\;\MeV$, potentially
bringing them into better agreement with data, while leaving
the $86\;\MeV$ results largely unchanged.
Second, the incomplete convergence of the
model-space truncation $\Ntot$ introduces a residual
systematic uncertainty that is not fully captured by the
parameter-space spread of eq.~\eqref{eq:uncC}. As
discussed in sec.~\ref{sec:ComptonResultsC}, this effect
is most significant for larger values of $\LamSRG$ and
at higher momentum transfers. Third, the theoretical
uncertainties from the \chiEFT{} truncation at \NXLO{3}
amount to approximately $\pm 6\%$ in the cross section
(sec.~\ref{sec:ComptonUncC}), which, while not
negligible, is insufficient on its own to account for
the observed discrepancies of $20$--$30\%$.

On the experimental side, the $86\;\MeV$ data carry
uncertainties that are roughly twice
those of the $60\;\MeV$ set. Several $86\;\MeV$ points exhibit cross sections that, at fixed angle,
do not decrease relative to $60\;\MeV$, contrary to the expected energy dependence,
and the treatment of inelastic scattering bears directly on
their interpretation. Both measurements neglect the
inelastic contribution, but the bound on it differs
markedly: at $60\;\MeV$ it is limited to at most $6\%$ of
the region of interest yield~\cite{60MeV}, whereas the poorer
resolution of the elastic peak at $86\;\MeV$ loosens this
bound to $1$--$25\%$, a range consistent with zero within
uncertainties~\cite{86MeV}. Any unsubtracted inelastic
strength would raise the apparent elastic cross section, in
the same direction as the observed excess of the $86\;\MeV$
data over the present predictions, so part of the
discrepancy at this energy may be experimental in origin. A
dedicated quantitative comparison, including a proper
treatment of correlated systematic uncertainties, is
deferred to a future publication in which higher-$\Ntot$
densities and, ideally, coherent-propagation corrections
become available.
The present discrepancies have motivated a new round of measurements at HI$\gamma$S that are expected to
provide additional angular points and improved systematic control at both energies~\cite{Godagama2025}. 

\subsection{Summary of Compton Scattering Results}
\label{sec:ComptonSummaryC}
The present section has reported the first calculation
of elastic Compton scattering on $\LiS$, employing the
same one- and two-body kernels previously used for
$\HeT$~\cite{hammer2020} and
$\HeF$~\cite{hammer4He}. 
The calculation includes one- and two-body
contributions through $\calO(e^2\delta^3)$ [\NXLO{3}],
with the scalar-isoscalar polarizabilities of
eq.~\eqref{eq:polvaluesC} adopted as input, yielding a
parameter-free prediction. An incomplete two-body
calculation at $\calO(e^2\delta^4)\, [\mathrm{N^4LO}]$
($T_{12}=0$ channel only) confirms that higher-order
corrections are small and largely angle-independent.
The theoretical uncertainty
is estimated at approximately $\pm 6\%$ across all
energies and angles considered, combining the a priori
truncation estimate, the parameter-space spread of
eq.~\eqref{eq:uncC}, and the residual $\Ntot$
sensitivity, consistent with the analogous assessments
for $\HeT$ and $\HeF$.

Comparison with HI$\gamma$S data at $60$ and
$86\;\MeV$ reveals that the angular shape of the cross
section is well reproduced, though the absolute
normalization shows discrepancies of $20$--$30\%$
whose origin is not yet fully understood. The
sensitivity of the cross section to the polarizability
combinations
$\alpha_{E1}^{(s)}\pm\beta_{M1}^{(s)}$ follows the
same angular pattern observed in $\HeF$, with the less
well-determined difference
$\alpha_{E1}^{(s)}-\beta_{M1}^{(s)}$ producing up to
$\pm 10$--$15\%$ effects at backward angles for
$\omega=100\;\MeV$. The $\LiS$ cross section exceeds
that of $\HeF$ by approximately a factor of two,
continuing the hierarchy driven by
charged-pion-exchange currents between $np$ pairs, confirming the interpretation of the $np$ pair counting, and
providing enhanced event rates for future polarizability
extractions.

The accuracy of the present predictions is primarily
limited by the available model-space truncation
$\Ntot=14$. Access to densities at $\Ntot\geq 16$
would reduce the residual NCSM truncation uncertainty
and permit a more definitive comparison with data, but this is expected to change the
result by at most $3\%$.
Exploration of SRG flow parameters below the current
minimum of $\LamSRG=1.88\;\fmin$ may further improve
convergence, provided numerical effects from
the back-transformation remain
controlled.
These improvements, together with the
inclusion of coherent $A$-body propagation corrections,
would sharpen the theoretical predictions and clarify
the origin of the observed normalization discrepancy.

Several further extensions of the present Compton
calculation can be envisaged within the TDA framework.
First, predictions for the linearly polarized beam
asymmetry $\Sigma^{\mathrm{lin}}$ on $\LiS$ would
exploit the spin-1 nature of the target and provide an
observable sensitive to nuclear spin structure and spin
polarizability effects; this study is deferred to
future work. Second, completing the two-body kernel at
$\calO(e^2\delta^4)$ by incorporating the
$T_{12}=1$ isospin channel would place the \NXLO{4}
prediction on the same footing as the lower orders and
remove one source of incompleteness. Third, the
incorporation of coherent $A$-body propagation between
the two photon vertices is a prerequisite for restoring
the correct Thomson limit as $\omega\to 0$, which in
turn is required for a rigorous Bayesian uncertainty analysis.
Fourth, because the TDA
formalism is nucleus-independent once the requisite
densities are available, the same Compton kernels
employed here can be applied to other $p$-shell nuclei
as the corresponding transition densities become
accessible, further testing the \chiEFT{} description
of meson-exchange currents in different nuclear
environments. Finally, a global fit of the
scalar-isoscalar polarizabilities across the target
sequence
$d$, $\HeT$, $\HeF$, $\LiS$ would exploit
the complementary sensitivities and different nuclear
structures of each system, providing mutual consistency
checks and potentially reducing the uncertainties on
$\alpha_{E1}^{(s)}-\beta_{M1}^{(s)}$ beyond what any
single target can achieve.


==> intro/intro.tex <==
%! TEX root = ../Dis-AlexanderLong.tex

\section{Introduction}
The Standard Model of Particle Physics provides a
remarkably successful description of the fundamental
interactions. Among its pillars, Quantum Chromodynamics
(QCD) governs the strong nuclear force between quarks
and gluons, and thereby determines the properties of
composite particles such as pions, neutrons, protons, and nuclei.

The present work employs the Transition Density
Amplitude (TDA) formalism of
Grie\ss hammer\etal\cite{Hammer3He} to compute
scattering observables for light nuclei within Chiral
Effective Field Theory (\chiEFT). In this approach,
the scattering amplitude factorizes into an
irreducible few-body kernel, which encodes the
target-agnostic reaction process, and a transition
density amplitude (TDA) which encapsulates the effect
of the target (often a nucleus) on the process.
A key advantage of the TDA formalism is its
modularity: the TDA is computed once for a given
nucleus and set of kinematics, and subsequently
convolved with the appropriate kernel for any reaction
of interest. In particular, given $m$ reaction kernels
and TDAs for $n$ distinct nuclei, a total of
$m \times n$ distinct calculations may be performed
without recomputing either ingredient. The present
work applies this formalism to three reactions on
light nuclei: Compton scattering, neutral pion
photoproduction, and elastic pion scattering, each of
which probes a distinct aspect of low-energy QCD.
All calculations are carried out within the publicly
available \texttt{DensityScattering} code
suite~\cite{long_2026}, developed as part of the
present work. The modular design of the code suite
means that once the TDAs are in hand, incorporating
a new reaction requires only the implementation of
the corresponding kernel, substantially reducing the
effort needed for future applications.

Compton scattering on the nucleus is particularly well
suited to investigating nucleon structure, since the
behavior of this process is understood in
depth~\cite{Hildebrandt_2005}. The Compton amplitude is
affected by the electric and magnetic scalar dipole
polarizabilities, $\alpha_{E1}$ and $\beta_{M1}$,
which quantify the deformation of the nucleon's
internal charge and magnetization distributions in
response to applied electromagnetic fields. While the
proton polarizabilities can be measured directly on
hydrogen targets, the neutron, being charge neutral,
must have values extracted from Compton scattering on
composite nuclear targets such as the deuteron,
$\HeT$ and $\HeF$ ~\cite{Hammer3He,Myers:2014ace,hammer4He}.
Although the dominant contribution to the nuclear
Compton cross section arises from two-body
meson-exchange currents between correlated $np$
pairs, the observable of primary interest is the
isoscalar polarizability combination
$\alpha_{E1}^{(s)}+\beta_{M1}^{(s)}$, which can be
extracted from the measured cross section.
In the
present work, Compton scattering on $\LiS$ is
computed for the first time, extending the
TDA-based program to a nucleus not previously
treated; preliminary results were reported
in~\cite{Long_2025}.

The same challenge of extracting neutron-specific
information from nuclear reactions arises in neutral
pion photoproduction, which provides a sensitive
probe of chiral dynamics at
threshold~\cite{PionPhotoOrig}. The one-nucleon
production amplitude for
$\gamma N\to\pi^0 N$ is strongly suppressed for isoscalar targets by an
approximate cancellation between Born and loop
contributions, rendering the process sensitive to
chiral loop corrections and two-nucleon mechanisms.
Of particular significance is the counterintuitive
prediction of chiral perturbation theory that the
elementary neutron S-wave multipole
$E^{\pi^0 n}_{0+}$ exceeds the proton amplitude
$E^{\pi^0 p}_{0+}$ in
magnitude~\cite{bernard_1994,Bernard_2001}. This
prediction has been confirmed in neutral pion
photoproduction on the
deuteron~\cite{PionPhotoOrig,Beane_1997}, but the
limited precision of existing results motivates
further study using heavier nuclear targets.
Experimentally, neutral pion photoproduction off light
nuclei has been studied at Saclay~\cite{Argan1980,
Argan1988} and at
Saskatoon~\cite{Bergstrom1998,Barnett2008}, though
the existing data are scarce and of limited precision.
On the theoretical side,
Lenkewitz~\etal~\cite{Lenke2011,LenkeThesis} carried
out the first consistent calculation of threshold
neutral pion photo- and electroproduction off
$\HThree$ and $\HeT$ within chiral nuclear EFT.
Using chiral three-nucleon wave functions and Monte
Carlo integration to evaluate the relevant matrix
elements, they demonstrated that $\HeT$ is a
particularly favorable target for extracting
$E^{\pi^0 n}_{0+}$. In the dominant S-state
configuration of $\HeT$, the two protons are paired
to spin zero, so that the nuclear spin is governed by
the unpaired neutron. As a consequence, the
three-body S-wave multipole exhibits a pronounced
sensitivity to the elementary neutron amplitude.
Braun~\cite{BraunThesis} subsequently extended this
program to a broader range of light nuclei,
including $\LiS$.

The theoretical description of low-energy
pion-nucleon scattering was pioneered
by Weinberg~\cite{wienberg1966} and
Tomozawa~\cite{Tomozawa1966}, who derived the
leading S-wave $\piN$ scattering lengths. Elastic pion
scattering on nuclei gives access to these
scattering lengths, and in particular to the isoscalar
scattering length $a^{(+)}$, which is closely
connected to the pion-nucleon sigma term and to the
pattern of chiral symmetry breaking in
QCD~\cite{Liebig_2011}. The isovector scattering
length is a factor of approximately 37 larger in
magnitude than the isoscalar contribution, making the
latter difficult to determine precisely from pionic
hydrogen alone. As a result, calculations of
pion-nucleus scattering lengths provide important
complementary constraints~\cite{Beane_2003}.

In each of these three processes, the relevant neutron
information cannot be obtained from free-nucleon
targets and must instead be inferred from nuclear
reactions. For the isoscalar polarizability combination in
particular, coherent scattering from isoscalar
targets such as $\HeF$ and $\LiS$ provides the
necessary sensitivity, with the tri-nucleon systems $\HThree$ and
$\HeT$ and heavier nuclei serving as complementary
probes.
Calculations are presented for the light nuclei
$\HThree$, $\HeT$, $\HeF$, and $\LiS$, including
both one-body and two-body contributions to the
scattering amplitudes at threshold, together with
one-body contributions above threshold that
demonstrate the reach of the TDA framework beyond the
threshold regime.
The nuclear wave functions are obtained from the chiral semilocal momentum-space
regularized ($\chi$SMS) nucleon-nucleon potential of
Reinert, Krebs, and Epelbaum~\cite{Reinert2018},
evolved to lower resolution scales via the similarity
renormalization group (SRG) where necessary, along with a corresponding back transformation to physical momenta.
The two-body kernels for both pion photoproduction
and elastic pion scattering contain a removable
singularity of the form $1/\bv{q}^{\,2}$ in the
intermediate propagator.  A variable substitution
technique is developed in the present work that maps
this singularity to the origin of the integration
variable, where it is canceled by the Jacobian of
the spherical measure. 
All calculations are carried out within the publicly
available \texttt{DensityScattering} code
suite~\cite{long_2026}, developed as part of the
present work. Its modular design separates the
process-specific kernel from the infrastructure that
performs the density convolution, so that
incorporating a new reaction requires only the
implementation of the corresponding kernel.
The TDAs are provided through the \texttt{nucdens}
package of A.~Nogga (Forschungszentrum J\"ulich).
The results are compared throughout with those of
Lenkewitz and Braun as well as with data from
experiment, and theoretical uncertainties arising from
the chiral expansion, the SRG evolution, and
variation of the cutoff parameters are assessed.

The remainder of this thesis is organized as follows.
Chapters~\ref{sec:theory} and~\ref{sec:QCD} provide
the theoretical foundations, beginning with QCD and
its symmetries and proceeding to the construction of
the chiral effective Lagrangian and the associated
power counting.
Chapter~\ref{sec:TDA} develops the TDA formalism and
describes the computation of transition densities
from nuclear wave functions.
Chapter~\ref{sec:usage} documents the
\texttt{DensityScattering} code suite and its usage.
Chapter~\ref{sec:ComptonC} presents results for
Compton scattering off $\LiS$.
Chapter~\ref{sec:piphoto} treats threshold neutral
pion photoproduction and electroproduction on
$\HeT$, $\HThree$, and $\LiS$, for which $\HeF$
results vanish at this order, and extends the
one-body treatment of pion photoproduction above
threshold. Chapter~\ref{sec:pion} discusses elastic
pion scattering off $\HThree$, $\HeT$, $\HeF$, and
$\LiS$ at threshold, again with the one-body
contribution extended above threshold. Finally,
Chapter~\ref{sec:conclusion} summarizes the results
and discusses prospects for future work.
The unifying theme of the three reactions is that
each probes a distinct aspect of low-energy QCD
through the same nuclear targets, and the TDA
formalism permits all three to be treated within a
single computational framework.


==> outlook/outlook.tex <==
%! TEX root = ../Dis-AlexanderLong.tex
\section{Summary and Outlook}
\label{sec:conclusion}

The central achievement of the present work is the
application of the Transition Density Amplitude (TDA)
formalism of Grie{\ss}hammer
\etal\cite{hammer2020} to compute scattering observables
for three distinct reactions on the light nuclei
$\HThree$, $\HeT$, $\HeF$, and $\LiS$: Compton
scattering (sec.~\ref{sec:ComptonC}), neutral pion
photoproduction (sec.~\ref{sec:piphoto}), and elastic
pion scattering (sec.~\ref{sec:pion}). In this framework,
the scattering amplitude for each process factorizes into
two components: irreducible few-body kernels, which
encode the interaction of the external probe with the
active nucleons, and transition density amplitudes
(sec.~\ref{sec:TDA}), which encapsulate the nuclear
structure of the spectator system. Because the TDAs
depend only on the nuclear state and the kinematics, they
need only be computed once for a given nucleus, energy,
and scattering angle, and can thereafter be convolved
with the appropriate kernel for any elastic reaction.

This factorization constitutes the
principal methodological advantage of the TDA approach:
given $m$ reaction kernels and TDAs for $n$ distinct
nuclei, $m \times n$ distinct scattering observables may
be obtained without recomputing either ingredient. Once
the densities are in hand, the computational cost of
obtaining a new observable reduces to the kernel
convolution alone, which is comparatively inexpensive:
the one-body convolution completes in under one second
per energy and angle on a typical desktop computer, while
the two-body convolution requires approximately twenty
minutes for Compton scattering and up to three hours for
reactions employing the variable-substitution singularity
treatment (sec.~\ref{sec:TDASummary}). This modularity
has been demonstrated in practice throughout, with all
three reactions computed using the same code suite and the
same set of nuclear transition densities.

A central technical contribution is the development
of a Fortran code suite,\\
\texttt{DensityScattering}~\cite{long_2026},
that implements the TDA formalism for computing nuclear
scattering observables. Given a precomputed transition
density and a user-supplied interaction kernel, the code
convolves the density with the kernel and returns the
corresponding nuclear scattering amplitude. The one-body
(sec.~\ref{sec:TDA1body}) and two-body
(sec.~\ref{sec:TDA2body}) contributions are evaluated
separately, enabling a systematic decomposition of the
scattering amplitude into its constituent few-body
sectors. The framework is designed for generality: a
researcher wishing to compute a new \chiEFT{} reaction
need only supply the process-specific kernel, while all
infrastructure for density handling, angular integration,
quantum-number summation, and output is provided by the
existing framework. The same code suite was used for all
three reactions treated herein, demonstrating the
practical reusability of the TDA approach within a single
unified computational framework. The code repository is
publicly available~\cite{long_2026}.

The nuclear wave functions employed throughout are
obtained from the semilocal momentum-space regularized
chiral potential ($\chi$SMS) of Reinert, Krebs, and
Epelbaum~\cite{Reinert2018}, evaluated at cutoffs
$\LamNN = 450$ and $500~\MeV$, the values identified
by the Bayesian convergence analysis of Millican
\etal\cite{SMS400550} as exhibiting statistically
consistent convergence patterns across chiral orders.

For $\LiS$, where the mass number precludes direct
few-body methods, the No-Core Shell Model (NCSM) is used
to generate wave functions in the Similarity
Renormalization Group (SRG) evolved space
(sec.~\ref{sec:SRG}), and the inverse SRG transformation
of Sun \etal\cite{Xiang-Xiang} is subsequently applied
to the densities (sec.~\ref{sec:SRG_setup}). This
``SRG-and-back'' procedure maps the SRG-evolved
coordinates back to physical momenta, ensuring that the
resulting TDAs can be combined directly with unevolved
kernels and thereby preserving the kernel-density
factorization that is essential to the TDA method. The
necessity of this inverse transformation was demonstrated
quantitatively using $\HeF$ as a validation case, since
its TDAs can be computed both with and without the SRG
transformation. Omitting the back-transformation produces
a systematic suppression of the Compton scattering cross
section that grows with decreasing $\LamSRG$, reflecting
the increasing mismatch between the SRG-evolved
coordinate space and the physical momenta entering the
non-SRG evolved kernel (see fig.~\ref{fig:4HeSRGCompare}). With the full
procedure applied (forward transformation, density
computation, inverse transformation), deviations between
the SRG-based and direct $\HeF$ results were found to be
at the $2\%$ level or below for
$\LamSRG = 1.88~\fmin$, well within the theoretical
uncertainties arising from the truncation of the chiral
expansion.

\subsection*{Higher-Body Contributions and the
  Few-Nucleon Expansion}
The TDA methodology was first applied to $\HeT$ in
Compton scattering by Grie{\ss}hammer
\etal\cite{hammer2020} and subsequently extended to
$\HeF$~\cite{hammer4He}. In both cases the few-nucleon
expansion was truncated at the $\Nt$ level, omitting
only the $3\mathrm{N}$ contribution for $\HeT$ and
the $3\mathrm{N}$ and $4\mathrm{N}$ contributions for
$\HeF$. The extension to $\LiS$, carried out in the
present work, represents a qualitatively larger step.
With $A = 6$ nucleons, the truncation of the few-nucleon
expansion at $\Nt$ now omits contributions from
$3\mathrm{N}$ through $6\mathrm{N}$.
Of these, the $5\mathrm{N}$ and $6\mathrm{N}$
contributions are expected to be especially suppressed:
the Pauli exclusion principle prevents more than two
protons and two neutrons from simultaneously occupying
the same spatial region, strongly disfavoring genuine
five- and six-nucleon short-range correlations. This
suppression is expected to persist for the induced
many-body interactions generated by the SRG
transformation at physically reasonable values of
$\LamSRG$.
Although each successive term is
suppressed by an additional factor of
$Q_{\mathrm{few}}$, the cumulative effect of the
missing orders is no longer negligible a priori,
particularly for observables such as the pion scattering
length where the $3\mathrm{N}$ correction is estimated
to be of order
$17 \times 10^{-3}\,m_{\pi^+}^{-1}$
(sec.~\ref{sec:pipi_3N_estimate}). A systematic
treatment of the $3\mathrm{N}$ and $4\mathrm{N}$
contributions therefore represents the most pressing
theoretical improvement for heavier targets.

Within the TDA framework as currently implemented,
incorporating three-body contributions would require
the generation of three-body transition density
amplitudes. At the $3\mathrm{N}$ level, the convolution
with a three-body kernel requires integration over three
sets of independent Jacobi momenta~\cite{Liebig_2011},
and the TDAs themselves depend on a substantially larger
number of momentum and quantum-number arguments than
their $\Nt$ counterparts, making them considerably more
expensive to generate and store.

It is natural to ask whether a $3\mathrm{N}$ TDA could
be decomposed into lower-body components, for instance
by expressing the three-nucleon contribution as a
convolution of a $\Nt$ TDA with a single-nucleon
spectator density. However, this decomposition encounters
a fundamental obstacle: a naive factorization into a
$\Nt$ TDA and a $\No$ spectator density requires the
spectator nucleon to have its momentum fully determined,
while the two active nucleons retain their full
relative-momentum dependence. This mismatch in the
kinematic treatment of the active and spectator
subsystems means that the factored expression does not
reproduce the full $3\mathrm{N}$ TDA without additional
approximations. One potential avenue is an on-shell
approximation in which the relative momenta of the active
nucleons are constrained to their on-shell values, thereby
reducing the dimensionality of the required integration
and enabling a factorization of higher-body TDAs into
products of lower-body ones.
A natural first test of this on-shell approximation would
be to verify whether a factorization of the $\Nt$ TDA
into two $\No$ TDAs, with the active nucleon momenta
placed on shell, can recover the full $\HeT$ Compton
scattering result of Grie{\ss}hammer
\etal\cite{hammer2020}, since both the exact and
on-shell-factorized expressions are available for direct
comparison in this case. If the on-shell approximation
proves adequate, the approach generalizes: an
$a\mathrm{N}$ TDA and a $b\mathrm{N}$ TDA could be
combined to approximate an $(a{+}b)\mathrm{N}$ TDA,
allowing higher-body contributions to be constructed
from existing lower-body densities without the need to
generate genuinely higher-body TDAs, largely removing
the current limitation to $\No$ and $\Nt$ sectors.
Whether this on-shell factorization program can be
realized in practice remains an open question.

In the interim, a more practical strategy is the
hybrid approach discussed in
sec.~\ref{sec:TDASummary}: the $3\mathrm{N}$ and
$4\mathrm{N}$ contributions may be computed
independently via the direct evaluation methods of
Liebig \etal\cite{Liebig_2011} and combined
additively with the TDA-based $\No$ and $\Nt$
results. Since the few-nucleon expansion of
eq.~(\ref{eq:totalscat}) is additive by construction,
such a combination entails no loss of consistency
provided the same nuclear wave functions are employed
in both calculations. This hybrid strategy realizes substantial
computational savings by exploiting the efficiency and
modularity of the TDA for the dominant $\No$ and $\Nt$
sectors, reserving the more demanding direct evaluation
for the higher-body corrections. Although the direct
computation of $3\mathrm{N}$ and $4\mathrm{N}$ integrals
remains technically challenging, the EFT suppression of
these contributions means that the accuracy requirements
for their numerical evaluation are correspondingly
relaxed: since the corrections themselves are small,
moderate numerical precision in their treatment suffices
for the overall result to remain well controlled. This
hybrid approach therefore provides a practical path
toward precision predictions on targets with
$A \geq 4$.

\subsection{Compton Scattering
  (sec.~\ref{sec:ComptonC})}

Differential cross sections for Compton scattering on
$\LiS$ were computed at photon energies of $60$, $75$,
$86$, and $100~\MeV$ in $\Delta(1232)$-full \chiEFT,
using the same kernels as in the $\HeT$ calculation of
Grie{\ss}hammer \etal\cite{hammer2020} and the $\HeF$
calculation of Grie{\ss}hammer
\etal\cite{hammer4He}. The scalar-isoscalar
polarizabilities were adopted as input from deuteron
Compton fits, yielding a parameter-free prediction for
the $\LiS$ cross section
(sec.~\ref{sec:ComptonKernelC},
fig.~\ref{fig:6LiResultsPlot},
table~\ref{table:LiSCrossSecC}). Theoretical
uncertainties were estimated from the spread over the
parameter space described in
sec.~\ref{sec:ComptonUncC}, yielding $\pm 3$--$4\%$ in
the cross section at $60~\MeV$ and $\pm 4$--$6\%$ at
$100~\MeV$, consistent with the expected
$\calO(\delta^4)$ truncation error.

The results at $60$ and $86~\MeV$ represent the first
\chiEFT{} predictions for Compton scattering on $\LiS$.
The sensitivity of the cross section to the
polarizability combinations
$\alpha_{E1}^{(s)} \pm \beta_{M1}^{(s)}$ follows the
same angular pattern observed for $\HeF$ by
Grie{\ss}hammer \etal\cite{hammer4He}: the sum governs
forward angles, where it is constrained by the Baldin
Sum Rule, while the less well-determined difference
governs backward angles
(sec.~\ref{sec:ComptonSensC},
fig.~\ref{fig:PolarVary1C}). At $100~\MeV$, the
backward-angle sensitivity to
$\alpha_{E1}^{(s)} - \beta_{M1}^{(s)}$ reaches
$\pm 10$--$15\%$ for a $\pm 2$ unit variation in
canonical units ($10^{-4}~\mathrm{fm}^3$), confirming
that $\LiS$ provides comparable polarizability
sensitivity to $\HeF$ (fig.~\ref{fig:RelDevC}).

The $\LiS$ cross section exceeds that of $\HeF$ by
approximately a factor of two across the energy range
considered, continuing the hierarchy
$d:\HeT:\HeF:\LiS \approx 1{:}2{:}5{:}10$ observed at
photon energies near $100$--$120~\MeV$
(sec.~\ref{sec:ComptonCompareC}). This hierarchy is
driven predominantly by charged pion-exchange currents
between correlated $np$ pairs: the leading two-body
Compton diagrams (fig.~\ref{fig:2BdiagramsC}) are
nonzero only for $np$ pairs, yielding a ratio of
$1{:}2{:}4{:}9$ for
$d{:}\HeT{:}\HeF{:}\LiS$ that accounts for the bulk of
the observed cross-section scaling. The enhanced $\LiS$
cross section provides correspondingly higher event
rates for future polarizability extractions.

Comparison with measurements from the High Intensity
$\gamma$-Ray Source (HI$\gamma$S) at
$60~\MeV$~\cite{60MeV} and $86~\MeV$~\cite{86MeV}
reveals that the angular shape of the cross section is
well reproduced by the TDA calculation
(sec.~\ref{sec:ComptonDataC}). However, the absolute
normalization exhibits discrepancies of $20$--$30\%$
whose origin is not yet fully understood: at $60~\MeV$,
the calculated cross section systematically exceeds the
measurements, while at $86~\MeV$ the pattern reverses.
A noteworthy feature of the $86~\MeV$ measurements is
that several angular points yield cross sections
comparable to or exceeding the corresponding values at
$60~\MeV$. This behavior is contrary to the monotonic
decrease with increasing energy expected from the
elementary Compton amplitude. These discrepancies may in
part reflect the omission of coherent $A$-body
propagation between the two photon vertices, which has
been shown to reduce the deuteron cross section by
$10$--$20\%$ at $\omega = 50~\MeV$~\cite{hammer4He}, as
well as residual model-space truncation effects not fully
captured by the parameter-space spread. New measurements
at HI$\gamma$S are expected to provide additional
angular points and improved systematic
control.

The order-by-order convergence of the \chiEFT{}
expansion was examined in detail
(figs.~\ref{fig:orderbyorder1}
and~\ref{fig:orderbyorder2}). The large correction from
LO to \NXLO{2}, amounting to roughly $50\%$ of the LO
cross section, is expected from the absence of
pion-exchange currents at LO; subsequent corrections at
\NXLO{3} and in the two-body sector are markedly
smaller, confirming that the chiral expansion of the
Compton kernel remains well controlled for $\LiS$ in
the energy range considered.

\subsection{Neutral Pion Photoproduction
  (sec.~\ref{sec:piphoto})}

Threshold neutral pion photoproduction was investigated
for $\HThree$, $\HeT$, and $\LiS$, with both one-body
and two-body contributions to the $S$-wave multipole
amplitudes $E_{0+}$ and $L_{0+}$ computed through
$\calO(q^4)$ (sec.~\ref{sec:piphoto_1N_thresh},
sec.~\ref{sec:piphoto_2N}). Pion photoproduction on
$\HeF$ vanishes at this order because the spin-dependent
production operator
$\vec{\epsilon}_\lambda \cdot \vec{S}$ yields zero when
evaluated between $J^\pi = 0^+$ states.

For the trinucleon systems, the present results are in
good agreement with the calculations of Lenkewitz
\etal\cite{Lenke2011, Lenke2013, LenkeThesis} at the
level of a few percent in the one-body form factors and
approximately $5\%$ in the two-body form factors,
constituting an independent confirmation using different
nuclear potentials
(tables~\ref{tab:2N_3H},~\ref{tab:2N_3He}).
For $\LiS$, a systematic factor of $\sqrt{2}$ discrepancy
with the results of Braun~\cite{BraunThesis} was
identified in the two-body form factors
(table~\ref{tab:2N_6Li},
sec.~\ref{ss:BraunSqrt2}) and traced to an error in the
normalization of the spin-$1$ angular momentum matrices
used by Braun; when this correction is applied, the two
sets of results become consistent. Beyond confirming
prior results, the present work provides the first
determination of the longitudinal multipole $L_{0+}$ for
$\LiS$ (table~\ref{tab:2N_6Li}), which was not computed
by Braun~\cite{BraunThesis}, and establishes the one-body
framework for above-threshold pion photoproduction using
SAID partial-wave amplitudes
(sec.~\ref{sec:piphoto_above},
fig.~\ref{fig:piphoto170MeV}).

A direct comparison with experiment was possible for $\LiS$, the only
target considered for which threshold $(\gamma,\pi^0)$ data exist. The
present amplitude
$E_{0+}(\LiS) = (-2.00\pm0.08)\times10^{-3}/m_{\pi^+}$ agrees with the
SAL measurement of Bergstrom \etal\cite{Bergstrom1999} at the
$1.8\sigma$ level (sec.~\ref{sec:piphoto_exp_comparison}). The
fractional offset between \chiEFT{} and data is nearly identical to
that found in the deuteron channel, where the chiral
prediction~\cite{Beane_1997} historically provided one of the first
confirmations of the two-body pion-cloud mechanism over the
phenomenological models of the time~\cite{bernard_1994,
Bernard_2001}. That the same normalization factor recurs at $A=6$
indicates that the residual discrepancy is governed by the elementary
single-nucleon input and the omitted one-body boost corrections rather
than by the few-nucleon description, and it extends the deuteron
validation of the chiral two-body dynamics to a $p$-shell nucleus.

Across all nuclei considered, the two-body contribution
$E_{0+}^{\Nt}$ dominates the total production amplitude
(sec.~\ref{sec:piphoto_combined}), a characteristic
feature of neutral pion photoproduction at threshold
traceable to the vanishing of the leading one-body
contact term (the Kroll-Ruderman vertex) for the neutral
pion channel~\cite{Beane_1997}. The ratios of two-body
to one-body contributions are approximately $4{:}1$ for
$\HThree$, $2.3{:}1$ for $\HeT$, and $9{:}1$ for
$\LiS$, with the particularly large ratio for $\LiS$
reflecting the near-cancellation of the proton and
neutron one-body contributions in this $Z = N = 3$
nucleus (table~\ref{tab:1N_6Li}). The interference
pattern between $E_{0+}^{\No}$ and $E_{0+}^{\Nt}$
differs between mirror nuclei: both contributions are
negative for $\HThree$, yielding constructive
interference and the largest total amplitude, whereas the
positive one-body contribution in $\HeT$ partially
cancels the negative two-body term. This partial
cancellation renders the $\HeT$ production cross section
particularly sensitive to the elementary neutron
amplitude $E_{0+}^{\pi^0 n}$, as emphasized by Lenkewitz
\etal\cite{Lenke2011}. A measurement of the
$\HeT(\gamma, \pi^0)\HeT$ cross section at threshold
would provide a stringent test of the \chiEFT{}
prediction, originally due to Bernard, Kaiser, and
Mei{\ss}ner~\cite{bernard_1994, Bernard_2001}, that
$|E_{0+}^{\pi^0 n}| > |E_{0+}^{\pi^0 p}|$.

The convergence of the chiral expansion for the two-body
contribution was confirmed by comparing results at
$\calO(q^3)$ and $\calO(q^4)$
(sec.~\ref{sec:piphoto_convergence},
table~\ref{tab:static_shift}): the static corrections
shift $E_{0+}^{\Nt}$ by approximately $2\%$ in the
transverse channel and at or below $1\%$ in the
longitudinal channel, confirming that the two-body
amplitude is well described at leading order. A variable
substitution technique was developed to handle the
removable singularity of the form $1/\vec{q}\,^2$ in
the two-body propagator
(sec.~\ref{sec:piphoto_2N_results}), replacing the
regulator extrapolation
($\Lambda_{\mathrm{reg}} \to 0$) employed by
Braun~\cite{BraunThesis} and eliminating the associated
systematic uncertainty.

In the one-body sector, a comparison of the SAID
partial-wave amplitudes with the $\calO(p^4)$ ChPT
predictions at threshold
(sec.~\ref{sec:piphoto_1N_thresh}) revealed significant
tension in the proton channel
$\gamma p \to \pi^0 p$, where the SAID value
($-0.56 \times 10^{-3}/m_{\pi^+}$) amounts to less
than half the magnitude of the ChPT result
($-1.16 \times 10^{-3}/m_{\pi^+}$), reflecting severe
cancellations between isospin-$1/2$ and isospin-$3/2$
contributions. The $\calO(p^4)$ ChPT values were
therefore adopted at threshold, with the SAID amplitudes
reserved for use above threshold
(sec.~\ref{sec:piphoto_above}), where the proximity of
the $\Delta(1232)$ resonance renders the chiral
expansion poorly convergent.

\subsection{Elastic Pion Scattering (sec.~\ref{sec:pion})}

Elastic pion-nucleus scattering lengths were computed for
$\HeT$, $\HThree$, $\HeF$, and $\LiS$ using one-body
kernels derived from the SAID partial-wave
analysis~\cite{PiPiSaid} (sec.~\ref{sec:pipi_1N}) and
two-body kernels constructed from the leading diagrams of
Liebig \etal\cite{Liebig_2011}
(sec.~\ref{sec:pipi_2N}), including the numerically
enhanced triple-scattering contribution. The variable
substitution developed for pion photoproduction was
successfully applied to the analogous singularities in
the pion scattering kernel
(sec.~\ref{sec:pipi_singularity}), confirming the
versatility of the method across reaction channels.
While the $\pi^-$-$\HeT$ and $\pi^-$-$\HeF$ two-body
scattering lengths were previously computed by Liebig
\etal\cite{Liebig_2011}, all remaining entries in
table~\ref{tab:pipi_results} are new: the $\pi^0$ and
$\pi^+$ channels for $\HeT$ and $\HeF$, all three
charge channels for $\HThree$, and the complete set of
$\LiS$ scattering lengths, which constitute the first
\chiEFT{} predictions for pion scattering on a
$p$-shell nucleus.

The two-body sector dominates the total scattering length
for all nuclei considered, accounting for approximately
$84\%$ of the total for the isoscalar nuclei $\HeF$ and
$\LiS$ (sec.~\ref{sec:pipi_results},
table~\ref{tab:pipi_results}), consistent with the
pattern observed in pion photoproduction. The scaling of
the two-body contribution with nucleon number departs
from naive pair-counting
(sec.~\ref{sec:pipi_discussion}): the ratio for $\LiS$
relative to $\HeT$ is approximately $3.7$, falling well
below the naive expectation of
$\binom{6}{2}/\binom{3}{2} = 5$. This sub-linear scaling
reflects the growing spatial extent of the nuclear wave
function with increasing mass number, which reduces the
overlap of the two-body kernel with the density.

An isospin decomposition of the results
(sec.~\ref{sec:isospin_decomposition}) confirms that
isospin remains a good approximate symmetry at the level
of precision attained, with fit residuals well within
the quoted uncertainties
(tables~\ref{tab:isospin_3He}
and~\ref{tab:isospin_isoscalar}). The convergence of
the few-nucleon expansion was assessed using the
empirical suppression factor
$Q_{\mathrm{few}} \approx 0.2$ established by Liebig
\etal\cite{Liebig_2011}
(sec.~\ref{sec:pipi_convergence}), yielding a hierarchy
$\No{:}\Nt{:}3\mathrm{N}{:}4\mathrm{N}
\sim 100{:}25{:}5{:}1$. For $\pi^-$-$\HeT$, the
estimated three-nucleon correction of
${\sim}5 \times 10^{-3}\,m_{\pi^+}^{-1}$ lies within the
quoted uncertainty (sec.~\ref{sec:pipi_3N_estimate}).
For the isoscalar nuclei $\HeF$ and $\LiS$, the
dominant three-nucleon diagram is
isovector~\cite{Liebig_2011} and therefore suppressed
for $T = 0$ targets, though the quantitative extent of
this suppression for $\LiS$ is not yet known and
constitutes the dominant uncontrolled systematic.

The present $\pi^-$-$\HeT$ result,
$a = 64.1(54) \times 10^{-3}\,m_{\pi^+}^{-1}$, agrees with
the independent calculation of Liebig
\etal\cite{Liebig_2011}, who obtained
$a = (62 \pm 4 \pm 7) \times 10^{-3}\,m_{\pi^+}^{-1}$ using
entirely different potentials, integration methods, and
nuclear-structure formalisms. This cross-validation
confirms the robustness of the \chiEFT{} prediction.
The result is consistent with the earliest pionic-atom
measurement at PSI~\cite{Abela1977} but exceeds the
later measurements of Mason \etal\cite{Mason1980} and
Schwanner \etal\cite{Schwanner1984} by approximately
$2.9\sigma$ and $3.4\sigma$, respectively
(sec.~\ref{sec:pipi_exp_comparison},
table~\ref{tab:pipi_comparison_3He}), a pattern of
tension also found by Liebig
\etal\cite{Liebig_2011}. New pionic-atom measurements
at PSI would help clarify this discrepancy.

The $\pi$-$\HeF$ and $\pi$-$\LiS$ scattering lengths
constitute predictions that could be tested by future
pionic-atom measurements at PSI. The $\HeF$ result is
particularly valuable: the one-body contribution is
suppressed (accounting for only $17\%$ of the total) and
the three-nucleon corrections are expected to be small
for this isoscalar target, making it a clean probe of
two-body chiral dynamics and providing an independent
determination of $a^{(+)}$ complementary to the
constraints from pionic hydrogen and deuterium.

\subsection{Outlook}

Having established the TDA formalism as a practical and
reliable tool for computing scattering observables on
light nuclei within \chiEFT, several directions for
future investigation emerge naturally from these results.

On the nuclear structure side, the generation of TDAs for
additional nuclei and at higher values of $\Ntot$ would
reduce the residual model-space truncation uncertainty
that is visible in the $\LiS$ Compton scattering
convergence studies (fig.~\ref{fig:NtotConvergeC}). In
particular, an extension of the NCSM basis to
$\Ntot = 16$ or $18$ would place the $\LiS$ predictions
on a firmer footing with respect to basis convergence.
Smaller values of $\LamSRG$ than those currently employed
would facilitate calculations at increased $\Ntot$,
though this in turn demands an SRG inverse
back-transformation over a larger range
(sec.~\ref{sec:SRGcutoff}).

For Compton scattering, the most pressing theoretical
improvement is the incorporation of coherent $A$-body
propagation between the two photon vertices, as discussed
above. The Thomson limit restored by this mechanism
serves as a prerequisite for any future Bayesian
uncertainty analysis of the type developed by the BUQEYE
collaboration~\cite{Melendez2019}, which requires a
well-defined leading-order baseline against which to
assess the convergence of higher-order corrections.
Predictions for the linearly polarized beam asymmetry
$\Sigma_{\mathrm{lin}}$ on $\LiS$ would provide an
additional observable sensitive to the nuclear spin and
spin-polarizability effects and are deferred to a future
study. The extension of the calculation to heavier
$p$-shell nuclei, as the requisite TDAs become available,
would further test the \chiEFT{} description of
two-nucleon pion-exchange currents in different nuclear
environments.

For pion photoproduction, the extension of the two-body
kernel to energies above threshold is the principal
remaining task. The one-body framework has been
established through the SAID partial-wave amplitudes
(sec.~\ref{sec:piphoto_above},
fig.~\ref{fig:piphoto170MeV}), but the two-body
contribution is at present restricted to threshold due to
the more involved character of the removable singularity
for nonzero pion momentum. A suitable variable
substitution that removes this singularity may exist but
has not yet been identified. Resolving this numerical
obstacle would permit the computation of nuclear pion
photoproduction differential cross sections over a broad
energy range, providing predictions testable at
facilities such as MAMI. Above-threshold calculations
would furthermore give access to spin-$0$ nuclei such as
$\HeF$, for which the threshold amplitude vanishes
identically but the $P$-wave amplitude $P_3$ is
nonzero~\cite{LenkeThesis}.

For pion scattering, the inclusion of higher-order
two-body contributions beyond the leading diagrams of
Liebig \etal\cite{Liebig_2011}
(fig.~\ref{fig:pipi_2N_LO}), in particular the complete
set of \NXLO{2} diagrams
(fig.~\ref{fig:pipi_2N_N2LO}), would improve the
theoretical precision and enable a more controlled
extraction of the isoscalar and isovector $\piN$
scattering lengths $a^{(+)}$ and $a^{(-)}$ from nuclear
targets. Extending the TDA framework to accommodate
three-body densities, or performing a dedicated
three-nucleon calculation along the lines of Liebig
\etal{}, would be required to resolve the dominant
uncontrolled systematic for heavier targets and is
identified as a priority for future work. A systematic
Bayesian uncertainty quantification of the results,
following the BUQEYE
framework~\cite{Melendez2019, SMS400550}, would place
the truncation error estimates on a more rigorous
statistical footing. On the experimental side, future
pionic-atom measurements at PSI on $\HeF$ and $\LiS$, as
well as new data for $\pi^-$-$\HeT$, would provide
further benchmarks against which to test the \chiEFT{}
predictions.

More broadly, the modularity of the TDA framework renders
it well suited for application to reactions beyond those
treated here. The factorization into
reaction-independent TDAs and process-specific kernels
means that extending the formalism to a new probe
requires only the construction of the corresponding
interaction kernel. This principle has already been
demonstrated by de~Vries
\etal\cite{Vries2024}, who applied the same TDA
framework and \texttt{nucdens} densities to compute dark
matter scattering on $\HeF$ within \chiEFT{} without
generating any new densities. Coherent elastic
neutrino-nucleus scattering represents another natural
application, as the nuclear response at the low momentum
transfers characteristic of stopped-pion neutrino sources
is governed by the same one- and two-body density
structures, with the electromagnetic kernel replaced by
the weak neutral-current
operator~\cite{Hoferichter2020}.
A qualitatively distinct extension is the treatment of
charge-exchange reactions such as
$\pi^- + \HeT \to \pi^0 + \HThree$. The two-body kernel
of Liebig \etal\cite{Liebig_2011} is already derived for
the general charge-exchange case, but the principal new
ingredient would be a set of inelastic transition density
amplitudes connecting distinct initial and final nuclear
states, which would require an extension of the
\texttt{nucdens} package. Once available, such
predictions would provide access to the isovector
pion-nucleon scattering length in a channel not
reachable through elastic scattering alone.

The sub-linear scaling of the two-body contribution
with nucleon number observed for $\LiS$
(sec.~\ref{sec:pipi_discussion}) suggests that the TDA
approach remains computationally tractable as it is
extended to heavier $p$-shell nuclei and to the broader
class of reactions outlined above. The densities
computed for the present work are already available for
reuse, and the \texttt{DensityScattering} code
suite~\cite{long_2026} provides the infrastructure
needed to incorporate new kernels with minimal
additional development.
With three reactions now demonstrated on four nuclei,
the TDA formalism establishes a unified and extensible
framework for the systematic computation of low-energy
probe-nucleus scattering observables within \chiEFT,
providing a foundation for solving the nucleus scattering problem in one
consistent formalism.


==> pion/pion.tex <==
%! TEX root = ../Dis-AlexanderLong.tex
\newcommand{\munits}{\times 10^{-3}m_{\pi^+}^{-1}}
\section{Elastic Pion Scattering}
\label{sec:pion}
\label{sec:Overview}
Elastic pion scattering off light nuclei near threshold
provides a complementary probe of the chiral dynamics of
QCD to pion photoproduction. Two principal motivations
drive the present calculation. The first is to test the
predictions of \chiEFT against data on $\pi$-nucleus
scattering lengths~\cite{Abela1977, Mason1980, Schwanner1984}.
The second is to extract $\piN$
scattering amplitudes from nuclear targets. Since free
neutron targets are unavailable, nuclear targets such as
$\HeT$, $\HThree$, $\HeF$, and $\LiS$ must serve as proxies to
access the $\pi$-neutron scattering
amplitude~\cite{baru_He3, Liebig_2011}. A general
framework for $\pi$-nucleus scattering at threshold
in \chiEFT was established by
Weinberg~\cite{WEINBERGpionpionNucleus},
whose approach forms the basis of the two-body kernel
employed in the present work.

Pion-nucleus scattering lengths are directly accessible
through measurements of pionic atoms, in which a
negatively charged pion is captured into an atomic orbit
around a nucleus~\cite{Ericson}. Unlike the electron,
the pion is a hadron and therefore subject to the strong
interaction in addition to the Coulomb interaction. When the
pion occupies a low-lying orbital, its wave function has
significant overlap with the nuclear volume, and the
strong interaction induces a shift $\varepsilon_{1s}$
and a broadening of the atomic energy levels relative to
the values predicted by QED
alone~\cite{Liebig_2011}. 
The shift $\varepsilon_{1s}$ is measured via X-ray spectroscopy of the pionic-atom
transitions as the pion cascades from higher orbitals to
the $1s$ ground state. The measured level shift can then
be related to the $\pi$-nucleus scattering length through
generalized Deser-type
formulae~\cite{baru_He3, Deser1954}, whose
leading-order relationship is approximately linear, with
corrections that become increasingly important for
heavier nuclei~\cite{Liebig_2011}. Such measurements
have been performed for pionic hydrogen, pionic
deuterium, and pionic $\HeT$ at the Paul Scherrer
Institute (PSI)~\cite{Abela1977, Mason1980,
Schwanner1984}, and analogous measurements on
heavier pionic atoms such as $\pi^-$-$\HeF$ would
provide a valuable cross-check of the systematics. The
scattering lengths computed in the present work are
therefore directly relevant to the interpretation of
current and future pionic-atom data and to the ongoing
program of extracting the isoscalar $\piN$ scattering
length $a^{(+)}$ from nuclear
targets~\cite{Liebig_2011}. In particular, the
$\pi$-$\HeF$ and $\pi$-$\LiS$ scattering lengths
presented here constitute predictions that could be
tested by future measurements at facilities such as PSI,
where the requisite pion beams and X-ray spectroscopy
infrastructure are available. A measurement of the
$\pi^-$-$\HeF$ or $\pi^-$-$\LiS$ level shift, for instance, would provide
an independent determination of the isoscalar scattering
length $a^{(+)}$, supplementing the existing constraints
from pionic hydrogen and pionic
deuterium~\cite{Liebig_2011}.

Analogous to pion photoproduction, the computation of
pion-nucleus scattering observables within the TDA
formalism requires the convolution of both one- and
two-body kernels with the corresponding nuclear
transition densities. At threshold energy, the reaction
on the deuteron was described by Beane
\etal~\cite{Beane_2003}, and their framework can be
generalized to the present case in much the same manner
as for pion photoproduction in sec.~\ref{sec:piphoto_above}.
As described in sec.~\ref{sec:TDA}, the present work utilizes only one- and
two-body TDAs; kernels involving three or more active nucleons, as well as
relativistic and rescattering corrections, are omitted. Because the present
calculation retains only one- and two-body kernels, a deterioration of the
agreement with data, from the accurate description found at $A=2$ to
progressively larger discrepancies at $A=3,4,6$, would signal a growing role
for the omitted contributions of three or more active nucleons. Such a
pattern would be consistent with the proposal that the chiral power counting
of few-nucleon interactions itself changes with mass number, promoting the 3N
and 4N sectors relative to their nominal ordering~\cite{Yang_2023}.

As demonstrated for pion photoproduction in
sec.~\ref{sec:piphoto_above}, the phenomenological
approach to the one-body kernel is considerably more
efficient, in this context, than an explicit diagrammatic
calculation, since the full $\piN$ scattering amplitude
is encoded in a single function of the partial-wave
phase shifts rather than reconstructed order-by-order
from Feynman diagrams. In particular, the precision of
the one-body kernel is determined by the uncertainty of
the experimentally measured inputs, rather than by the
truncation of the chiral expansion at a given order.
Achieving comparable accuracy from a purely
diagrammatic calculation would require working to a
chiral order well beyond what is currently available.
The present work therefore employs only this technique
for the one-body kernel, restricting the use of Feynman
diagram calculations to the two-body threshold case.

The principal new contribution of the present chapter is
the first calculation of pion-nucleus scattering lengths
for $\HThree$, $\HeT$, $\HeF$, and $\LiS$ within the
TDA formalism developed in sec.~\ref{sec:TDA}, using
nuclear transition densities derived from the $\chi$SMS
potential~\cite{Reinert2018}. For $\LiS$, the densities
are obtained from NCSM wave functions evolved via the
SRG, see sec.~\ref{sec:SRG}. The one-body contribution
at threshold is governed by the free pion-nucleon
scattering lengths, which are taken from
experiment rather than from \chiEFT predictions. The
two-body contribution, computed within \chiEFT, then
provides the dominant theoretical input. This separation
is advantageous because it focuses the comparison with
pionic-atom data on the \chiEFT two-body dynamics:
the experimental one-body input removes the 1N sector
as a source of theoretical uncertainty, so that any
discrepancy with data tests the \chiEFT prediction
for the two-nucleon pion-exchange mechanisms directly.
While the leading two-nucleon contributions to
$\pi$-${}^2$H, $\pi$-$\HeT$, and $\pi$-$\HeF$
scattering were previously computed by Liebig
\etal~\cite{Liebig_2011} using Monte~Carlo integration in
momentum space with wave functions obtained from a
variety of chiral and phenomenological potentials, the
present work extends the calculation to $\LiS$ for the
first time and employs deterministic quadrature
throughout. The variable substitution technique for the
removable singularity in the two-body kernel, introduced
in the photoproduction context of sec.~\ref{NumMethod},
is applied here as well. In pion photoproduction, this
technique replaced the regulator extrapolation of
Braun~\cite{BraunThesis}; for pion scattering, it
replaces the Monte~Carlo treatment employed by
Liebig \etal~\cite{Liebig_2011}.
The resulting scattering lengths are compared with the
theoretical predictions of Liebig \etal\ and with
pionic-atom measurements at PSI, where available.
Throughout, the physical charged and neutral pion
masses $m_{\pi^\pm}$ and $m_{\pi^0}$ are retained,
including in the two-body propagators of
diagrams~$(a)$ through~$(d)$, so that the leading
isospin-breaking effects from the pion mass splitting
$m_{\pi^\pm} - m_{\pi^0} \approx 4.6\;\MeV$ are
included without approximation. The resulting
charge-channel dependence of the two-body contributions
is visible in Table~\ref{tab:pipi_results} and
quantified through the isospin decomposition of
sec.~\ref{sec:isospin_decomposition}.

This chapter is organized as follows.
Section~\ref{sec:pipi_1N} develops the one-body $\piN$
scattering formalism, including the kinematics, isospin
structure, and total isospin decomposition of the
$\pi$-nucleus system
(sec.~\ref{sec:isospin_decomposition}), followed by
the threshold scattering lengths and their relation to
the SAID partial-wave input. The two-body kernel,
derived from the operators of Liebig
\etal~\cite{Liebig_2011}, is presented in
sec.~\ref{sec:pipi_2N}, including the treatment of the
removable singularity in
sec.~\ref{sec:pipi_singularity}.
Results are collected in sec.~\ref{sec:pipi_results}.
The numerical parameters, uncertainty budget, convergence
of the few-nucleon expansion, and estimated
three- and four-nucleon contributions are addressed in
sec.~\ref{sec:pipi_uncertainties}, followed
by a discussion of the physics content of the results,
including comparison with prior calculations and
pionic-atom data. As a preliminary demonstration of the
above-threshold capability of the TDA framework, the
one-body contribution at
$E^\pi_{\mathrm{cm}} = 170\;\MeV$ is presented in
sec.~\ref{sec:pipi_above}.

\subsection{One-Body Pion Scattering}
\label{sec:pipi_1N}
\subsubsection{Kinematics and Isospin Structure}
The phenomenological approach to one-body $\piN$
scattering is considerably streamlined compared to a
direct Feynman diagram calculation, since the precision
is limited by experiment rather than by the chiral order
of the calculation. The treatment presented here follows
Ericson and Weise~\cite{Ericson}.

The $\piN$ scattering process is given by
\begin{equation}
  \pi^a(q) + N(p)
  \to \pi^a(q')+ N(p')\,,
\end{equation}
and is depicted in fig.~\ref{PionScatGeneral}.
\begin{figure}[H]
\centering
\includegraphics[scale=0.8]
  {PionScat-Nuc.pdf}
\caption[Kinematics of elastic pion-nucleon scattering]{General kinematics of elastic $\piN$ scattering.
  Solid lines denote nucleons and dashed lines denote
  pions. The incoming and outgoing pion carries isospin
  index $a$, i.e.\ no charge exchange occurs.}
  \label{PionScatGeneral}
\end{figure}
As an isospin doublet, the nucleon is represented by
\begin{equation}
  \phi_p=\kt{p}= \binom{1}{0},\quad
  \phi_n=\kt{n}=\binom{0}{1}\,.
\end{equation}
The corresponding isospin operator is $\vec{\tau}$. The
pion couples to the nucleon, forming a
$T=\frac{1}{2} \bigoplus \frac{3}{2}$ system. The
physical pion is denoted $\kt{\pi^\lambda}$ with
$\lambda=0, \pm$ representing the charge state.
It is often convenient to work in the Cartesian pion
basis ($\pi_{a},\,a=1,2,3$), which is related to the
physical charge basis by
\begin{equation}
  \kt{\pi^{\pm}}= \frac{1}{\sqrt{2}} \left(
  \kt{\pi_1} \pm i\kt{\pi_2} \right),\quad
  \kt{\pi^0}=\kt{\pi_3}\,.
\end{equation}
The isospin operator for the pion,
$\vec{t}= \left( t_1, t_2, t_3 \right)$ in the charge
basis, is defined by
\begin{equation}
  t_3 \kt{\pi_\lambda}= \lambda \kt{\pi_\lambda},
  \quad \vec{t}^{\,\,2} \kt{\pi_\lambda}
  =2\kt{\pi_\lambda}\,,
\end{equation}
together with, in the Cartesian basis
\begin{equation}
  \br{\pi_a}t_b \kt{\pi_c} = i \varepsilon_{abc}\quad
  a,b,c \in \{1,2,3\}\,.
\end{equation}
The one-nucleon scattering matrix, and therefore the
one-body kernel, is given by
\begin{equation}
  \begin{split}
    \Fscr\left(\vec{q}^{\,\prime}, \vec{q}\,\right)
    =\sum_{I=\frac{1}{2}, \frac{3}{2}}
    \hat{P}_I\left\{\sum_l
    \left[(l+1) f_{I, l^{+}}(\omega)
    +l f_{I, l^{-}}(\omega)\right]
    P_l(x)\right. \\
  \left.\quad-\mathrm{i}
  \vec{\sigma} \cdot
  \left(\hat{{q}}^{\,\prime}
  \times \hat{q}\right)
  \sum_{l}\left[f_{I, l^{+}}(\omega)
  -f_{I, l^{-}}(\omega)\right]
  P_l^{\prime}(x)\right\}\,.
  \end{split}
  \label{eq:scatmat_pion}
\end{equation}
Here, $x=\cos\theta$, $P_l(x)$ are the Legendre
polynomials, and
$P_l'(x)= \frac{\dd P_l}{\dd x}$. The label $l^\pm$
corresponds to the total angular momentum
$j=l\pm \frac{1}{2}$, and $\omega$ denotes the
center-of-mass energy of the $\piN$ system. The operators
$\hat{P}_I$ project onto the isospin $I=1/2$ and
$I=3/2$ channels. Denoting a partial wave by
$\alpha=(I,l\pm)$, the phase shifts $\delta_\alpha$ are
related to $f_\alpha$ by
\begin{equation}
  f_\alpha=\frac{1}{2 \mathrm{i}|\vec{q}\,|}
  \left(\e^{2 \mathrm{i} \delta_\alpha} -1\right)
  =\frac{1}{2 \mathrm{i}|\vec{q}\,|}
  \left(\eta_\alpha
  \e^{2 \mathrm{i} \mathrm{Re} \delta_\alpha}
  -1\right)
  \quad \text{where}\quad
  \eta_\alpha= \e^{-2\mathrm{Im}\delta_\alpha}\,.
  \label{eq:pipi_falpha}
\end{equation}
Here $\eta_\alpha$ is the inelasticity parameter, with
$\eta_\alpha = 1$ for purely elastic scattering and
$\eta_\alpha < 1$ when inelastic channels are open.
The spin-averaged differential cross section in the
center-of-mass frame for single-nucleon scattering is
\begin{equation}
  \frac{\dd \sigma}{\dd \Omega}
  = |\phi^{\prime\,\dag} \Fscr\phi|^2\,.
\end{equation}
The relationship to the invariant scattering amplitude is
\begin{align}
  \frac{\dd \sigma}{\dd \Omega}
  &= \frac{1}{64 \pi^2 s}
  \left|\overline{\calM}\right|^2\\
  \implies\calM
  &= 8\pi \sqrt{s}\, \Fscr\,.
\end{align}
The coupled $\piN$ system has isospin $\frac{1}{2}$
and $\frac{3}{2}$ channels.
Projection into these channels is implemented by the
operators $\hat{P}_I$, satisfying
$\hat{P}_{1/2} +\hat{P}_{3/2}=1$, which are defined by
\begin{equation}
\begin{split}
  \br{\pi_b}\hat{P}_{\frac{3}{2}} \kt{\pi_a}
  &= \delta_{ab} - \frac{1}{3} \tau_b\tau_a \\
  \br{\pi_b}\hat{P}_{\frac{1}{2}} \kt{\pi_a}
  &=\frac{1}{3} \tau_b\tau_a\,.
\end{split}
\end{equation}
Transforming these isospin operators to the physical
(charge) pion basis yields
\begin{equation}
\begin{split}
   &\br{\pi_+} \Pthree \kt{\pi_+} =
\begin{pmatrix}
1 & 0 \\
0 & \frac{1}{3}
\end{pmatrix},
\quad
\br{\pi_-} \Pthree \kt{\pi_-} =
\begin{pmatrix}
\frac{1}{3} & 0 \\
0 & 1
\end{pmatrix},
\quad
\br{\pi_0} \Pthree \kt{\pi_0} =
\begin{pmatrix}
\frac{2}{3} & 0 \\
0 & \frac{2}{3}
\end{pmatrix}\\
 &\br{\pi_+} \Phalf \kt{\pi_+} =
\begin{pmatrix}
0 & 0 \\
0 & \frac{2}{3}
\end{pmatrix},
\quad
\br{\pi_-} \Phalf \kt{\pi_-} =
\begin{pmatrix}
\frac{2}{3} & 0 \\
0 & 0
\end{pmatrix},
\quad
\br{\pi_0} \Phalf \kt{\pi_0} =
\begin{pmatrix}
\frac{1}{3} & 0 \\
0 & \frac{1}{3}
\end{pmatrix}\;.
\end{split}
\end{equation}
Values of $\delta_\alpha$ and $\eta_\alpha$ are available
from the
\href{https://said.phys.gwu.edu/}{SAID}
partial-wave database maintained by the George Washington
University Data Analysis Center~\cite{SAID_website}
(accessed September~2025). The values employed in the
present work are from the WI08 solution of Workman
\etal~\cite{PiPiSaid}.

\subsubsection{Total Isospin Decomposition}
\label{sec:isospin_decomposition}
The decomposition of the computed scattering lengths into
channels of definite total isospin $I$ of the
$\pi$-nucleus system serves two purposes. First, it
provides a consistency check: for isoscalar nuclei only
the $I=1$ channel contributes, so the spread among the
three pion charge channels measures the degree of isospin
violation introduced by the pion mass difference in the
two-body kernel. Second, for isovector targets such as
$\HeT$, the decomposition yields the independent
amplitudes $\mathcal{M}_{1/2}$ and
$\mathcal{M}_{3/2}$, which can be related to the
isoscalar and isovector $\piN$ scattering lengths and are
therefore directly relevant to the program of extracting
$a^{(+)}$ from nuclear
targets~\cite{Liebig_2011, baru_He3}.
%
\begin{equation}
  a_{\pi A}(Q_\pi) = \sum_{I}
  \langle I,\, T_3{+}Q_\pi
  \,|\, I_A,\, T_3;\, 1,\, Q_\pi
  \rangle^2 \mathcal{M}_I \,,
  \label{eq:isospin_channel_decomp}
\end{equation}
%
where the Clebsch--Gordan coefficient couples the product
state $|I_A, T_3\rangle \otimes |1, Q_\pi\rangle$ to the
total isospin eigenstate $|I, M\rangle$ with
$M = T_3 + Q_\pi$, recalling that the physical pion
states are identified as
$|\pi^{Q_\pi}\rangle = |I=1,\, m_I = Q_\pi\rangle$.
Here $\mathcal{M}_I$ denotes the scattering amplitude in
the channel of total isospin $I$, and the sum runs over
all values permitted by the triangle rule,
$|I_A - 1| \leq I \leq I_A + 1$.

As an example, consider $\HeT$, which has
$I_A = \tfrac{1}{2}$ and
$T_3 = +\tfrac{1}{2}$. The allowed channels are
$I = \tfrac{1}{2}$ and $I = \tfrac{3}{2}$, yielding two
independent amplitudes $\mathcal{M}_{1/2}$ and
$\mathcal{M}_{3/2}$. The three pion charge channels
$\pi^-, \pi^0, \pi^+$ then provide the system of
equations
\begin{equation}
  \label{eq:CG_system_3He}
  \HeT:
  \left\{\;\;
  \begin{aligned}
  a(\pi^-) &= \tfrac{2}{3}\,\mathcal{M}_{1/2}
    + \tfrac{1}{3}\,\mathcal{M}_{3/2} \\
  a(\pi^0) &= \tfrac{1}{3}\,\mathcal{M}_{1/2}
    + \tfrac{2}{3}\,\mathcal{M}_{3/2} \\
  a(\pi^+) &= \phantom{\tfrac{2}{3}\,}
    \mathcal{M}_{3/2}
  \end{aligned}
  \right.
\qquad
  \HThree:
  \left\{\;\;
  \begin{aligned}
  a(\pi^-) &= \phantom{\tfrac{2}{3}\,}
    \mathcal{M}_{3/2}\\
  a(\pi^0) &= \tfrac{1}{3}\,\mathcal{M}_{1/2}
    + \tfrac{2}{3}\,\mathcal{M}_{3/2} \\
  a(\pi^+) &= \tfrac{2}{3}\,\mathcal{M}_{1/2}
    + \tfrac{1}{3}\,\mathcal{M}_{3/2}
  \end{aligned}
  \right. .
\end{equation}
For $\HeT$, the $\pi^+$ channel is the stretched state
$|I=\tfrac{3}{2}, M=\tfrac{3}{2}\rangle$, which fixes
$\mathcal{M}_{3/2}$ directly. The remaining two
equations then overdetermine $\mathcal{M}_{1/2}$, and
the residual measures the degree to which isospin
symmetry is broken, predominantly by the
charged-to-neutral pion mass difference
$m_{\pi^\pm} - m_{\pi^0}$ entering the two-body
propagators. A similar argument exists for $\HThree$.

For the isoscalar nuclei $\HeF$ ($I_A = 0$) and $\LiS$
($I_A = 0$), only the total isospin $I = 1$ channel
contributes. In this case, the decomposition is trivial:
all three pion charge channels yield the same amplitude
$\mathcal{M}_1$, and the spread among them is a direct
measure of isospin violation. It should be noted that
isospin breaking in the residuals arises from two distinct
sources: the pion mass difference in the two-body kernel,
and, for $\LiS$, a small $I = 1$ admixture in the
nuclear ground state. While $\HeF$ is an essentially
perfect $I_A = 0$ state, the $\LiS$ ground state carries
a small isovector component, which constitutes an
additional source of isospin violation beyond the kernel.

\subsubsection{One-Body Pion Scattering at Threshold}
\label{sec:pipi_threshold}
The threshold regime is of particular experimental
interest, because the scattering lengths are directly
accessible through measurements of pionic atoms via
generalized Deser-type
formulae~\cite{Deser1954, baru_He3} that relate the
$1s$ level shift to the $\pi$-nucleus scattering
length (see also
sec.~\ref{sec:pipi_exp_comparison}). Pionic $\HeT$
measurements have been performed at
PSI~\cite{Abela1977, Mason1980, Schwanner1984}.
Above threshold, the partial-wave amplitudes are
obtained from the SAID WI08 $\piN$ phase shift
analysis~\cite{PiPiSaid} via
\meqref{eq:pipi_fs}. However, the lowest SAID
data point lies at
$W_{\mathrm{cm}} = 1078\;\MeV$, only
$\sim 0.2\;\MeV$ above the $\piN$ threshold, and even
at this energy the effective range correction inflates
$\delta/q$ by approximately $20\%$ relative to the
scattering length. For this reason, the SAID database
is bypassed at threshold in favor of directly employing
the scattering lengths. The values from the combined
analysis of Ref.~\cite{IVPIPI} are
\begin{equation}
  a_{\text{sym}}^{(+)}
  = [1 \pm 1] \times 10^{-3} \,\mpi^{-1}\,,
  \qquad a_{\text{sym}}^{(-)}
  = [86.5 \pm 1.2] \times 10^{-3} \,\mpi^{-1}\,,
  \label{eq:pipi_apm_base}
\end{equation}
where the subscript ``sym'' indicates that
isospin-violating corrections have not yet been applied.
These corrections, denoted $\Delta a^{\pm}$, arise from
the quark-mass difference $m_u \neq m_d$ and from
electromagnetic effects beyond the Coulomb potential;
they have been evaluated in
\chiEFT~\cite{IVPIPI}:
\begin{equation}
  \Delta a^{(+)}
  = [-3.35 \pm 0.28] \times 10^{-3}\,\mpi^{-1}\,,
  \qquad
  \Delta a^{(-)}
  = [+1.39 \pm 1.33] \times 10^{-3}\,\mpi^{-1}\,.
  \label{eq:pipi_IV_corrections}
\end{equation}
Applying
$a^{(+)} = a_{\text{sym}}^{(+)} + \Delta a^{(+)}$ and
$a^{(-)} = a_{\text{sym}}^{(-)} + \Delta a^{(-)}$ yields
\begin{equation}
  a^{(+)}
  = [-2.35 \pm 1.04] \times 10^{-3}\,\mpi^{-1}\,,
  \qquad
  a^{(-)}
  = [87.89 \pm 1.79] \times 10^{-3}\,\mpi^{-1}\,.
  \label{eq:pipi_apm_corrected}
\end{equation}
The striking feature of these values is the
near-cancellation of the isoscalar scattering length:
the central value
$|a^{(+)}| \approx 2.4 \times 10^{-3}\,\mpi^{-1}$ is
more than an order of magnitude smaller than the
isovector counterpart, a consequence of the approximate
cancellation between the $I = 1/2$ and $I = 3/2$
channels in \meqref{eq:pipi_apm_def}. This
near-vanishing of $a^{(+)}$ has profound consequences
for the nuclear scattering lengths: the one-body
contribution to isoscalar nuclei is proportional to
$A\, a^{(+)}$ and is therefore suppressed, making the
two-body sector dominant for such targets.
Consequently, pion scattering on isoscalar nuclei
provides a sensitive test of the nuclear binding
dynamics, since the dominant two-body contribution
depends directly on the internucleon correlations
encoded in the nuclear wave function.

More precisely, the one-body contribution to the
$\pi$--$A$ scattering length takes the analytic
form~\cite{baru_He3, Liebig_2011}
\begin{equation}
  a^{(\No)}_{\pi^{\pm, 0}}
  = \frac{1 + \mpi/m_N}
  {1 + \mpi/( A m_N)}
  \left( A\, a^{(+)}
  - Q_\pi\, a^{(-)}\, 2T_3 \right)\,,
  \label{eq:pipi}
\end{equation}
where $A$ is the nucleon number,
$T_3=(Z-N)/2$ is the third component of nuclear isospin,
and $Q_\pi$ is the pion charge. 
This expression for the one-body scattering length does
not involve nuclear wave functions or TDAs and
therefore serves as an independent consistency check
of the TDA calculation; the one-body scattering
lengths computed via the full TDA machinery reproduce
eq.~\eqref{eq:pipi} to within
$10^{-5}\,m_{\pi^+}^{-1}$ for all nuclei and pion
charges considered, confirming the numerical
implementation of the one-body convolution.
It should be noted that \meqref{eq:pipi}
is not exact; it omits isospin-violating contributions
and few-nucleon corrections. The quantities $a^{(+)}$
and $a^{(-)}$ are the isoscalar and isovector $\piN$
$S$-wave scattering lengths, related to the
definite-isospin scattering lengths by
\begin{equation}
  a^{(+)} = \frac{a_{1/2} + 2\,a_{3/2}}{3}\,,
  \qquad
  a^{(-)} = \frac{a_{1/2} - a_{3/2}}{3}\,.
  \label{eq:pipi_apm_def}
\end{equation}

At threshold, $\sqrt{s} = \mpi + m_{\text{nucl}}$, the
center-of-mass momentum $|\qv| = 0$ and only $S$-wave
partial waves contribute, since
$f_\ell \propto |\qv|^{2\ell}$ for small
$|\qv|$~\cite{Ericson}.
As a result, the two $S$-wave scattering lengths
$a_\half$ and $a_\threehalf$ become the sole observables
characterizing the $\piN$ interaction at zero energy.
At this energy, no inelastic channels are open in the
isospin-symmetric limit ($m_{\pi^\pm} = m_{\pi^0}$),
so $\eta_\alpha \to 1$ in
\meqref{eq:pipi_falpha}. In practice, the
charged-to-neutral pion mass difference
$m_{\pi^\pm} - m_{\pi^0} \approx 4.6\;\MeV$ renders
the charge-exchange channel
$\pi^\pm A \to \pi^0 A'$ kinematically accessible at
the elastic $\pi^\pm$ threshold, introducing a small
inelasticity that is neglected in the present
treatment. At and above threshold the $S$-matrix can
be parametrized via the real
$K$-matrix~\cite{Ericson}, where
\begin{equation}
  S_\alpha
  =\frac{1 + \mathrm{i}\, |\qv|\,
  K_\alpha}
  {1 - \mathrm{i}\, |\qv|\, K_\alpha}
  \quad\text{and}\quad
  K_\alpha
  =\frac{\tan\delta_\alpha}{|\qv|}
  \,,
  \label{eq:piN_Kmatrix}
\end{equation}
and the effective range expansion reads
\begin{equation}
  |\qv|^{2l+1} \cot \delta_\alpha
  = \frac{1}{a_\alpha}
  + r_\alpha |\qv|^2 +\calO(|\qv|^3)
  \implies
  a_\alpha= \lim_{|\qv|\to 0}
  \frac{K_\alpha}{|\qv|^{2l}}\,.
  \label{eq:piN_ERE}
\end{equation}
The $S$-wave scattering length is thus defined as
$a_\alpha = \lim_{|\qv| \to 0} K_\alpha$, so that
$|\qv|\,K_\alpha \to 0$ at threshold. It follows that
\begin{equation}
  \begin{split}
  \lim_{|\qv|\to0}\; f_\alpha
  &=\lim_{|\qv|\to0}\;
  \frac{S_\alpha - 1} {2\mathrm{i}\,|\qv|}
  = \lim_{|\qv|\to0}\;
  \frac{K_\alpha}
  {1 - \mathrm{i}\, |\qv|\, K_\alpha}
  = a_\alpha\,.
  \end{split}
  \label{eq:pipi_fs}
\end{equation}
The constraint $l = 0$ mandates that only
$j = \half$ contributes, $P_0(x) = 1$,
and $P_0'(x) = 0$, so the spin-flip term vanishes and
the scattering matrix reduces to
\begin{align}
  \lim_{|\qv| \to 0}
  \left.\Fscr(\qvp,\qv) \right|_{l=0}
  &= \Pthreehalf\, f_{\threehalf,0^+}
  + \Phalf\, f_{\half,0^+}
  = \Pthreehalf\,
  a_\threehalf + \Phalf\, a_\half\,.
  \label{eq:piN_Fscr_threshold}
\end{align}
\subsection{Two-Body Pion Scattering at Threshold}
\label{sec:pipi_2N}
As in the case of two-body pion photoproduction, a
phenomenological approach is not available for the
two-body pion scattering kernel; instead, an explicit
diagrammatic calculation is required. The two-body kernel
for pion scattering on nuclei is well
established~\cite{WEINBERGpionpionNucleus,
Beane_1998, Beane_2003}. A more recent and comprehensive
treatment using \chiEFT was developed by Liebig
\etal~\cite{Liebig_2011}, which extends the diagrammatic
framework to higher orders and includes the general case
of charge exchange. The operators employed in the present
work are derived from Eqs.~(6), (7), and~(8) of
Ref.~\cite{Liebig_2011}, reduced to the elastic channel
in which the incoming and outgoing pion carry the same
isospin index~$a$. As in the two-body pion
photoproduction kernel of sec.~\ref{sec:piphoto}, the
nucleon labeling in the diagrams of
fig.~\ref{fig:pipi_2N_LO} 
is interchanged relative to
the convention of the one-body system.
\begin{figure}%[htbp]
\centering
\begin{tikzpicture}[
    nucleon/.style={thick, solid,
      decoration={markings,
        mark=at position 0
          with {\arrow[scale=1.5]{>}},
        mark=at position 1
          with {\arrow[scale=1.5]{>}}
    }, postaction={decorate}},
    pion/.style={thick, dashed},
    vertex/.style={circle,
      fill=black, inner sep=2pt},
    midarrow/.style={decoration={
      markings,
      mark=at position 0.5
        with {\arrow[scale=1.0]
          {triangle 45}}},
      postaction={decorate}}
]

% === Diagram (a) at x=-5.5 ===
\draw[nucleon]
  (-7.7, 1.2) -- (-3.3, 1.2);
\draw[nucleon]
  (-7.7, -1.2) -- (-3.3, -1.2);
\node[vertex] (a1)
  at (-5.5, 1.2) {};
\node[vertex] (a2)
  at (-5.5, -1.2) {};
\draw[pion, midarrow]
  (-7.2, 2.8) -- (a1);
\node at (-7.6, 3.1) {$k_\pi$};
\node at (-6.5, 2.5) {$a$};
\draw[pion, midarrow]
  (a1) -- (a2);
\node at (-6.1, 0) {$c$};
\node at (-4.9, 0) {$q$};
\draw[pion, midarrow]
  (a2) -- (-3.8, -2.1);
\node at (-3.4, -2.3) {$k_\pi'$};
\node at (-4.6, -2.2) {$b$};
\node at (-5.5, -3.0)
  {Diagram ($a$)};

% === Diagram (b) at x=0 ===
\draw[nucleon]
  (-2.2, 1.2) -- (2.2, 1.2);
\draw[nucleon]
  (-2.2, -1.2) -- (2.2, -1.2);
\node[vertex] (b1)
  at (0, 1.2) {};
\node[vertex] (b2)
  at (0, -1.2) {};
\draw[pion, midarrow]
  (-1.7, 2.8) -- (b1);
\node at (-2.1, 3.1) {$k_\pi$};
\node at (-1.0, 2.5) {$a$};
\draw[pion, midarrow]
  (b1) -- (1.7, 2.8);
\node at (2.1, 3.1) {$k_\pi'$};
\node at (0.8, 2.4) {$b$};
\draw[pion, midarrow]
  (b2) -- (b1);
\node at (-0.6, 0) {$c$};
\node at (0.6, 0) {$\tilde{q}$};
\node at (0, -3.0)
  {Diagram ($b$)};

% === Diagram (c) at x=5.5 ===
\draw[nucleon]
  (3.3, 1.2) -- (7.7, 1.2);
\draw[nucleon]
  (3.3, -1.2) -- (7.7, -1.2);
\node[vertex] (c1)
  at (5.5, 1.2) {};
\node[vertex] (c2)
  at (5.5, -1.2) {};
\node[vertex] (cc)
  at (5.5, 0) {};
\draw[pion, midarrow]
  (3.3, 0) -- (cc);
\node at (2.9, 0) {$k_\pi$};
\node at (4.2, 0.35) {$a$};
\draw[pion, midarrow]
  (cc) -- (7.7, 0);
\node at (8.1, 0) {$k_\pi'$};
\node at (6.5, 0.35) {$b$};
\draw[pion, midarrow]
  (c1) -- (cc);
\node at (5.1, 0.6) {$c$};
\node at (5.8, 0.6) {$\tilde{q}$};
\draw[pion, midarrow]
  (c2) -- (cc);
\node at (5.2, -0.7) {$d$};
\node at (5.9, -0.7)
  {$-\tilde{q}$};
\node at (5.5, -3.0)
  {Diagram ($c$)};

\end{tikzpicture}
\caption[Leading-order two-nucleon diagrams for elastic pion-nucleus scattering]{Leading-order two-nucleon diagrams for elastic
  $\pi$-nucleus scattering, corresponding to Eqs.~(6)
  and~(7) of Ref.~\cite{Liebig_2011}. Diagram~$(a)$
  contains the Coulomb-like $1/\qvs$ singularity;
  diagrams~$(b)$ and~$(c)$ are individually dependent on
  the parametrization of the pion field, but their sum is
parametrization-independent. They are $\mathrm{LO}$ in the two-nucleon sector.}
\label{fig:pipi_2N_LO}
\end{figure}

Diagram~$(a)$ of fig.~\ref{fig:pipi_2N_LO}
gives rise to a Coulomb-like operator
containing a singularity $1/\qvs$, corresponding to
Eq.~(6) of Ref.~\cite{Liebig_2011}. Restricting to
elastic scattering ($a = b$), the general charge-exchange
expression reduces to
\begin{equation}
  \hat{O}_{2 \mathrm{N}}^{(a)} =
  \frac{m_\pi^2}{2 f_\pi^2\; \qvs}
  \left( \vec{\tau}_1 \cdot \vec{\tau}_2
  - \tau_1^a \tau_2^b \right)\delta^{ab}\,.
\end{equation}
Diagrams~$(b)$ and $(c)$ are individually dependent on
the parametrization of the pion field; their sum is
parametrization-independent, see \meqref{eq:param}. This property is important:
were the individual diagrams not to combine into a
parametrization-independent result, additional diagrams
would be required to restore the symmetry, and the
elastic-channel reduction would be incomplete. The fact
that diagrams~$(b)$ and~$(c)$ sum to a physical,
parametrization-independent operator therefore serves as
a consistency check. In the elastic channels, this
combination gives
\begin{equation}
  \hat{O}_{2\mathrm{N}}^{(b+c)} =
  -\frac{g_A^2 m_\pi^2}{4 f_\pi^2}
  \ddfrac{\left(\vec{\sigma}_1 \cdot \qv\right)
  \left(\vec{\sigma}_2 \cdot \qv\right)}
  {(\qvs+m_\pi^2)^2}
  \left( \vec{\tau}_1 \cdot \vec{\tau}_2
  - \tau_1^a \tau_2^b \right)\,\delta^{ab}.
\end{equation}

Diagram~$(d)$ involves triple scattering;
\begin{figure}%[htbp]
\centering
\begin{tikzpicture}[
    nucleon/.style={thick, solid,
      decoration={markings,
        mark=at position 0
          with {\arrow[scale=1.5]{>}},
        mark=at position 1
          with {\arrow[scale=1.5]{>}}
    }, postaction={decorate}},
    pion/.style={thick, dashed},
    vertex/.style={circle,
      fill=black, inner sep=2pt},
    midarrow/.style={decoration={
      markings,
      mark=at position 0.5
        with {\arrow[scale=1.0]
          {triangle 45}}},
      postaction={decorate}}
]
\draw[nucleon]
  (-3, 0.8) -- (3, 0.8);
\draw[nucleon]
  (-3, -0.8) -- (3, -0.8);
\node[vertex] (v1)
  at (-1, 0.8) {};
\node[vertex] (v2)
  at (1, 0.8) {};
\node[vertex] (v3)
  at (0, -0.8) {};
\draw[pion, midarrow]
  (-2.5, 2.0) -- (v1);
\node at (-2.9, 2.2) {$k_\pi$};
\node at (-1.6, 1.8) {$a$};
\draw[pion, midarrow]
  (v2) -- (2.5, 2.0);
\node at (2.9, 2.2) {$k_\pi'$};
\node at (1.6, 1.7) {$b$};
\draw[pion, midarrow]
  (v1) -- (v3);
\draw[pion, midarrow]
  (v3) -- (v2);
\node at (0, -1.7)
  {Diagram ($d$)};
\end{tikzpicture}
\caption[Triple-scattering two-nucleon diagram for elastic pion-nucleus scattering]{Triple-scattering two-nucleon diagram,
  corresponding to Eq.~(8) of Ref.~\cite{Liebig_2011}.
  Although formally $\mathrm{N}^2\mathrm{LO}$ in
  Weinberg counting, diagram~$(d)$ is topologically
  enhanced and must be retained at the level of accuracy
  targeted here.}
\label{fig:pipi_2N_N2LO}
\end{figure}
in Weinberg counting, it appears formally at
$\mathrm{N}^2\mathrm{LO}$; however, Liebig \etal~\cite{Liebig_2011}
demonstrate that the dominant part of this amplitude is
numerically enhanced relative to naive dimensional
analysis by a topological factor arising from an
integrable singularity in the loop
integral. This enhancement traces
back to the fact that the relevant loop integral
evaluates to $\pi^2/(8\pi^2 |\vec{q}\,|)$, approximately a factor of $20$
larger than the typical value $1/((4\pi)^2 m_\pi)$ anticipated by
dimensional analysis, as discussed in sec.~5.3 of
Ref.~\cite{Liebig_2011}. As a result, diagram~$(d)$ is
suppressed relative to diagram~$(a)$ only by
$m_\pi^2/(16 f_\pi^2) \approx 0.14$, which is
insufficient to render it negligible at the level of
precision targeted here. The dominant contribution in the
elastic channel evaluates to
\begin{equation}
  \hat{O}^{(d)} =
  -\left( \frac{m_\pi}{2 f_\pi} \right)^3
  \frac{1}{2 |\qv\,|}
  \left( \tau_1^a \tau_2^b \right)\delta^{ab}\,.
\end{equation}
The other $\mathrm{N}^2\mathrm{LO}$ two-body diagrams lack this
enhancement and are expected to be suppressed by naive
dimensional analysis; they are therefore omitted. The
contribution from diagram~$(d)$ alone represents an
incomplete treatment at $\mathrm{N}^2\mathrm{LO}$, and
the associated truncation uncertainty is subsumed into
the systematic uncertainty budget discussed in
sec.~\ref{sec:pipi_uncertainties}.
\subsubsection{Treatment of the Removable Singularity}
\label{sec:pipi_singularity}
Diagram~$(a)$ introduces an integrable singularity of
the form $1/\qvs$ into the two-body kernel, and
diagram~$(d)$ introduces a singularity of the form
$1/|\qv|$. Both are removed by the same variable
substitution developed for pion photoproduction in
sec.~\ref{NumMethod}, to which the reader is referred
for a detailed derivation. In brief, the substitution
$\vec{k}_1^{\,\prime} \to \qv$ causes the $1/\qvs$
factor to cancel against the Jacobian of the spherical
coordinate representation, rendering the integrand
regular. The angular integration is then performed on a
Lebedev-Laikov grid and the radial integration using
Gauss-Legendre quadrature, as described in
sec.~\ref{sec:Inte}. The key features of the singularity
noted in the photoproduction context apply here as well:
it is a moving singularity whose position depends
continuously on the Jacobi momenta $\vec{p}_{12}$ and
$\vec{p}_{12}^{\,\prime}$, and the TDA formalism
constrains it to appear only in the two remaining
three-dimensional integrations.

The cross-checks and convergence tests described in
sec.~\ref{NumMethod} have been repeated for the pion
scattering kernel. The extracted scattering lengths are
independent of the orientation of the coordinate system
and consistent across different combinations of initial
and final nuclear spin projections $M_J$, $M_J'$.
Increasing the number of radial Gauss-Legendre
quadrature points by factors of two and four produces
changes at the sub-percent level, and increasing the
density of the Lebedev-Laikov angular grid confirms
stability at the $0.5\%$ level. See App.~\ref{sec:InteConverge} for details. Both variations are well
below the quoted uncertainties.
\subsection{Results}
\label{sec:pipi_results}
The results for the one-body and two-body contributions
to the pion-nucleus scattering lengths are collected in
Table~\ref{tab:pipi_results}.
% \begin{table}[H]
% \centering
% {\setlength{\extrarowheight}{3pt}
% \begin{tabular}{|l|l||r|r|r|}\hline
% \multicolumn{2}{|c||}{\rule[-1.1ex]{0pt}{2.8ex}} & $a^{1\mathrm{N}}$ & $a^{2\mathrm{N}}$ & $a=a^{1\mathrm{N}}+a^{2\mathrm{N}}$ \\
% \thickline{0.15em}
% \multirow{3}{*}{${}^3\mathrm{He}$} & $\pi^-$ & $\phantom{00}88.5(54)$ & $-23.57(75)$ & $\phantom{00}64.9(55)$ \\
% \cline{2-5}
%  & $\pi^0$ & $\phantom{00}-7.7(34)$ & $-21.60(71)$ & $\phantom{0}-29.3(35)$ \\
% \cline{2-5}
%  & $\pi^+$ & $-103.9(54)$ & $-23.57(75)$ & $-127.5(55)$ \\
% \hline\hline
% \multirow{3}{*}{${}^3\mathrm{H}$} & $\pi^-$ & $-103.9(54)$ & $-23.51(76)$ & $-127.4(55)$ \\
% \cline{2-5}
%  & $\pi^0$ & $\phantom{00}-7.7(34)$ & $-21.78(71)$ & $\phantom{0}-29.5(35)$ \\
% \cline{2-5}
%  & $\pi^+$ & $\phantom{00}88.5(54)$ & $-23.51(76)$ & $\phantom{00}65.0(55)$ \\
% \hline\hline
% \multirow{3}{*}{${}^4\mathrm{He}$} & $\pi^-$ & $\phantom{0}-10.4(46)$ & $-49.2(16)\phantom{0}$ & $\phantom{0}-59.6(49)$ \\
% \cline{2-5}
%  & $\pi^0$ & $\phantom{0}-10.4(46)$ & $-45.9(15)\phantom{0}$ & $\phantom{0}-56.3(49)$ \\
% \cline{2-5}
%  & $\pi^+$ & $\phantom{0}-10.4(46)$ & $-49.2(16)\phantom{0}$ & $\phantom{0}-59.6(49)$ \\
% \hline\hline
% \multirow{3}{*}{${}^6\mathrm{Li}$} & $\pi^-$ & $\phantom{0}-15.8(70)$ & $-86.7(27)\phantom{0}$ & $-102.5(75)$ \\
% \cline{2-5}
%  & $\pi^0$ & $\phantom{0}-15.7(70)$ & $-80.6(25)\phantom{0}$ & $\phantom{0}-96.3(74)$ \\
% \cline{2-5}
%  & $\pi^+$ & $\phantom{0}-15.8(70)$ & $-86.7(27)\phantom{0}$ & $-102.5(75)$ \\
% \hline
% \end{tabular}
% }
% \caption[Pion-nucleus scattering lengths]{Pion-nucleus scattering lengths in units of
%   $[10^{-3}/m_{\pi^+}]$.}
% \label{tab:pipi_results}
% \end{table}
%
% \begin{table}[H]
% \centering
% {\setlength{\extrarowheight}{3pt}
% \setlength{\tabcolsep}{4pt}
% \small
% \begin{tabular}{@{}|l||r|r|r|r|r|@{}}\hline
% \rule[-1.1ex]{0pt}{2.8ex}
%   Liebig \etal~\cite{Liebig_2011}
%   & $a^{1\mathrm{N}}$ & $a^{2\mathrm{N}}$
%   & $a^{3\mathrm{N}}$ & $a^{4\mathrm{N}}$
%   & Total \\
% \thickline{0.15em}
% $\pi^-$-$\HeT$
%   & $\phantom{0}88.5(54)$ & $-21.26(2)$
%   & $-4.77(8)$ & $-$
%   & $\phantom{0}62.5(54)$ \\
% \hline
% $\pi^-$-$\HeF$
%   & $-10.4(46)$ & $-45.8(6)\phantom{0}$
%   & $-$ & $2.31(31)$
%   & $-53.9(47)$ \\
% \hline
% \end{tabular}
% }
% \caption[Comparison of pion-nucleus scattering lengths with Liebig et al.]{Few-nucleon contributions to pion-nucleus scattering lengths from Liebig \etal~\cite{Liebig_2011}, using the \NXLO{2} $(\Lambda/\tilde{\Lambda}) = (550/600)\;\MeV$ wave functions (Tables~7 and~10 of Ref.~\cite{Liebig_2011}), in units of $[10^{-3}/m_{\pi^+}]$. The one-body contributions employ the same $\piN$ scattering length input as the present work. The leading three-nucleon operator is isovector~\cite{Liebig_2011} and therefore does not contribute to the isoscalar nucleus $\HeF$. Four-nucleon contributions were not computed for $A = 3$. Uncertainties reflect the Monte~Carlo statistical errors of Ref.~\cite{Liebig_2011}, propagated in quadrature.}
% \label{tab:liebig_breakdown}
% \end{table}

\begin{table}[H]
\centering
{\setlength{\extrarowheight}{3pt}
\setlength{\tabcolsep}{4pt}
\small
\begin{tabular}{|l|l||r|r|r|r|r|}\hline
\multicolumn{2}{|c||}{\rule[-1.1ex]{0pt}{2.8ex}} & $a^{1\mathrm{N}}$ & $a^{2\mathrm{N}}$ & $a^{3\mathrm{N}}$ & $a^{4\mathrm{N}}$ & Total $a$ \\
\thickline{0.15em}
\multirow{4}{*}{${}^3\mathrm{He}$} & $\pi^-$ & $\phantom{00}88.5(54)$ & $-23.57(75)$ & $-$ & $-$ & $\phantom{00}64.9(55)$ \\
\cline{2-7}
 & $\pi^-$~\cite{Liebig_2011} & $\phantom{00}88.5(54)$ & $-21.26(2)\phantom{0}$ & $-4.77(8)$ & $-$ & $\phantom{00}62.5(54)$ \\
\cline{2-7}
 & $\pi^0$ & $\phantom{00}-7.7(34)$ & $-21.60(71)$ & $-$ & $-$ & $\phantom{0}-29.3(35)$ \\
\cline{2-7}
 & $\pi^+$ & $-103.9(54)$ & $-23.57(75)$ & $-$ & $-$ & $-127.5(55)$ \\
\hline\hline
\multirow{3}{*}{${}^3\mathrm{H}$} & $\pi^-$ & $-103.9(54)$ & $-23.51(76)$ & $-$ & $-$ & $-127.4(55)$ \\
\cline{2-7}
 & $\pi^0$ & $\phantom{00}-7.7(34)$ & $-21.78(71)$ & $-$ & $-$ & $\phantom{0}-29.5(35)$ \\
\cline{2-7}
 & $\pi^+$ & $\phantom{00}88.5(54)$ & $-23.51(76)$ & $-$ & $-$ & $\phantom{00}65.0(55)$ \\
\hline\hline
\multirow{4}{*}{${}^4\mathrm{He}$} & $\pi^-$ & $\phantom{0}-10.4(46)$ & $-49.2(16)\phantom{0}$ & $-$ & $-$ & $\phantom{0}-59.6(49)$ \\
\cline{2-7}
 & $\pi^-$~\cite{Liebig_2011} & $\phantom{0}-10.4(46)$ & $-45.8(6)\phantom{00}$ & $-$ & $2.31(31)$ & $\phantom{0}-53.9(47)$ \\
\cline{2-7}
 & $\pi^0$ & $\phantom{0}-10.4(46)$ & $-45.9(15)\phantom{0}$ & $-$ & $-$ & $\phantom{0}-56.3(49)$ \\
\cline{2-7}
 & $\pi^+$ & $\phantom{0}-10.4(46)$ & $-49.2(16)\phantom{0}$ & $-$ & $-$ & $\phantom{0}-59.6(49)$ \\
\hline\hline
\multirow{3}{*}{${}^6\mathrm{Li}$} & $\pi^-$ & $\phantom{0}-15.8(70)$ & $-86.7(27)\phantom{0}$ & $-$ & $-$ & $-102.5(75)$ \\
\cline{2-7}
 & $\pi^0$ & $\phantom{0}-15.7(70)$ & $-80.6(25)\phantom{0}$ & $-$ & $-$ & $\phantom{0}-96.3(74)$ \\
\cline{2-7}
 & $\pi^+$ & $\phantom{0}-15.8(70)$ & $-86.7(27)\phantom{0}$ & $-$ & $-$ & $-102.5(75)$ \\
\hline
\end{tabular}
}
\caption[Combined pion-nucleus scattering lengths]{
  Pion-nucleus scattering lengths in units of $[10^{-3}/m_{\pi^+}]$, combining the present results with the few-nucleon contributions of Liebig \etal~\cite{Liebig_2011}. 
  Uncertainties of Ref.~\cite{Liebig_2011} reflect the Monte~Carlo statistical errors, propagated in quadrature.
  The present work provides the one- and two-nucleon contributions, so the three- and four-nucleon columns are empty for those rows. 
  The rows labeled with Ref.~\cite{Liebig_2011} give the few-nucleon contributions of Liebig \etal\ for $\pi^-$-$\HeT$ and $\pi^-$-$\HeF$, obtained with the \NXLO{2} $(\Lambda/\tilde{\Lambda}) = (550/600)\;\MeV$ wave functions (Tables~7 and~10 of Ref.~\cite{Liebig_2011}). 
  The one-body contributions of Ref.~\cite{Liebig_2011} employ the same $\piN$ scattering length input as the present work. 
  The leading three-nucleon operator is isovector and therefore does not contribute to the isoscalar nucleus $\HeF$, and four-nucleon contributions were not computed for $A = 3$.
  Total scattering length $a$ is $a=\sum_i a^{iN}$.
}
\label{tab:pipi_results}
\end{table}

The $\HThree$ entries are the charge-symmetric
mirror of the corresponding $\HeT$ results: under the
interchange of protons and neutrons,
$T_3 \to -T_3$ and $\pi^- \leftrightarrow \pi^+$, so
that the one-body contributions satisfy
$a^{(\No)}_{\pi^-\text{-}\HThree}
= a^{(\No)}_{\pi^+\text{-}\HeT}$ exactly.
The two-body contributions respect this symmetry up to
small differences of order
$0.1 \times 10^{-3}m_{\pi^+}^{-1}$, arising from
the charged-to-neutral pion mass difference in the
propagators. This near-exact mirror symmetry provides
a consistency check of the implementation and is
discussed further in sec.~\ref{sec:pipi_discussion}.

A least-squares fit of
eq.~(\ref{eq:isospin_channel_decomp}) to the computed
scattering lengths yields the results collected in
Tables~\ref{tab:isospin_3He}
and~\ref{tab:isospin_isoscalar}, with uncertainties on
$\mathcal{M}_I$ obtained by propagating the errors on
the individual charge channels through the fit. For
$\HeT$, the fit yields
$\mathcal{M}_{1/2} = [162\pm 12]
\times 10^{-3}/m_{\pi^+}$ and
$\mathcal{M}_{3/2} = [-126.8 \pm 6.6]
\times 10^{-3}/m_{\pi^+}$, with fit residuals at or
below $1.3 \times 10^{-3}/m_{\pi^+}$
across all three charge
channels. This level of isospin breaking is consistent
with the expected magnitude of the charged-to-neutral
pion mass splitting in the two-body kernel ($Q_{\text{Isospin}} \sim \frac{(m_{\pi^\pm}-m_{\pi^0})}{m_{\pi^0}}$). 
For the
isoscalar nuclei $\HeF$ and $\LiS$, the fit returns
$\mathcal{M}_1 = -58.5(49)$ and
$\mathcal{M}_1 = -100.4(75)$, respectively, both in
units of $10^{-3}/m_{\pi^+}$. Here the residuals are
somewhat larger, reaching
$4.1 \times 10^{-3}/m_{\pi^+}$ for $\LiS$.
In all cases, the residuals are small compared to the
total scattering lengths. 

For $\HeT$ the largest residual is
$1.3 \times 10^{-3}/m_{\pi^+}$, which amounts to
$2.0\%$ of the total $\pi^-$ scattering length and is
well within the quoted uncertainty of
$5.5 \times 10^{-3}/m_{\pi^+}$. For $\LiS$, the
largest residual of
$4.1 \times 10^{-3}/m_{\pi^+}$ represents $4.0\%$
of the total, reflecting the greater absolute
magnitude of the two-body contribution in heavier
systems and the correspondingly larger sensitivity to the
pion mass difference entering through the pion
propagators. These residuals confirm that isospin remains
a good approximate symmetry at the level of accuracy
attained in the present calculation.

\begin{table}[H]
\centering
{\setlength{\extrarowheight}{3pt}
\begin{tabular}{|l|l||r|r|r|r|}\hline
\multicolumn{2}{|c||}{$a$\rule[-1.1ex]{0pt}{2.8ex}}
  & $I=1/2$ channel & $I= 3/2 $ channel
  & $a_{\mathrm{fit}}$
  & $\mathrm{comp.}$ $-$ fit \\
\thickline{0.15em}
\multirow{3}{*}{$\HeT$}
  & $\pi^-$ & $\phantom{0}107.9(80)$
  & $-42.3(22)$ & $\phantom{00}65.6$
  & $-0.7$ \\
\cline{2-6}
  & $\pi^0$ & $\phantom{00}53.9(40)$
  & $-84.5(44)$ & $\phantom{0}-30.6$
  & $+1.3$ \\
\cline{2-6}
  & $\pi^+$ & $\phantom{000}0$
  & $-126.8(66)$ & $-126.8$
  & $-0.7$ \\
\hline
\hline
\multirow{3}{*}{$\HThree$}
  & $\pi^-$ & $\phantom{000}0$
  & $-126.8(66)$ & $-126.8$
  & $-0.6$ \\
\cline{2-6}
  & $\pi^0$ & $\phantom{00}53.9(40)$
  & $-84.6(44)$ & $\phantom{0}-30.6$
  & $+1.2$ \\
\cline{2-6}
  & $\pi^+$ & $\phantom{0}107.8(80)$
  & $-42.3(22)$ & $\phantom{00}65.6$
  & $-0.6$ \\
\hline
\end{tabular}
}
\caption[Isospin decomposition of pion-${}^3$He and pion-${}^3$H scattering lengths]{Isospin decomposition of pion-$\HeT$ and
  pion-$\HThree$ scattering lengths in units of
  $[10^{-3}/m_{\pi^+}]$.}
\label{tab:isospin_3He}
\end{table}
\begin{table}[H]
\centering
{\setlength{\extrarowheight}{3pt}
\begin{tabular}{|l|l||r|r|}\hline
\multicolumn{2}{|c||}{$a$\rule[-1.1ex]{0pt}{2.8ex}}
  & $I=1$ channel & $a_{\mathrm{comp}}$ \\
\thickline{0.15em}
\multirow{2}{*}{${}^4\mathrm{He}$}
  & $\pi^\pm$ & $-58.5(49)$ & $-59.6(49)$ \\
\cline{2-4}
  & $\pi^0$ & $-58.5(49)$ & $-56.3(49)$ \\
\hline\hline
\multirow{2}{*}{${}^6\mathrm{Li}$}
  & $\pi^\pm$ & $-100.4(75)$ & $-102.5(75)$ \\
\cline{2-4}
  & $\pi^0$ & $-100.4(75)$
  & $\phantom{0}-96.3(74)$ \\
\hline
\end{tabular}
}
\caption[Isospin decomposition of pion scattering lengths for isoscalar nuclei]{Isospin decomposition of pion scattering lengths
  for isoscalar nuclei in units of
  $[10^{-3}/m_{\pi^+}]$. Only $I=1$ contributes for these
  nuclei, rendering the decomposition trivial. The fit
  value $\mathcal{M}_1$ is the least-squares average
  over all three pion charges; residuals reflect isospin
breaking from pion mass differences, and for $\LiS$, the small
$I_A = 1$ admixture in the nuclear ground state.}
\label{tab:isospin_isoscalar}
\end{table}
\subsection{Numerical Parameters}
\label{sec:pipi_numerics}
In general, calculations at higher chiral order may
require larger $j_{12}^\mathrm{max}$ due to more
complicated angular dependence; therefore the numerical
parameters governing the integration grids were
determined using pion photoproduction as a test bed,
since this kernel includes the $\mathrm{N^3LO}$ two-body
``static'' diagrams. See app.~\ref{sec:InteConverge} for
the study of different integration parameters.
For $\LiS$ in particular, the use of the NCSM requires
a separate analysis, which was performed using Compton scattering to confirm convergence in the
parameters $\hbar\omega$,
$\Ntot^{\mathrm{max}}$, and $\LamSRG$, see
sec.~\ref{sec:ComptonResultsC}, figs.~\ref{fig:NtotConvergeC}
and~\ref{fig:RelativeDeviationCompare}.
This procedure has not been repeated for each reaction; the same parameter
choices are adopted for pion scattering and pion
photoproduction. This is justified because the
convergence tests probe the full amplitude, i.e.\ the
TDAs convolved with the reaction kernel, not the TDAs
in isolation. At leading order in the two-nucleon
sector, all three reactions share a common topology: a
single pion or photon is absorbed at one nucleon
vertex and a pion or photon is emitted at the other,
with the two vertices connected by pion exchange.
The vertices themselves are all generated by
the derivative pion--nucleon coupling in
\meqref{eq:LpiN1expanded}, with photon vertices arising
from the inclusion of the electromagnetic field through
the external vector source (sec.~\ref{sec:chiralLag}).
As a result, the Compton, pion photoproduction, and
pion scattering kernels probe a generically similar
off-diagonal region of the TDA in the two-nucleon
momentum variables, and the convergence behavior
established for Compton scattering carries over to
the other two reactions.

As in all other reactions in the present study, for the
target $\LiS$ the harmonic-oscillator frequency is set
to $\hbar\omega = 18\;\MeV$, the model-space truncation
to $\Ntot^{\mathrm{max}} = 14$, and the SRG flow
parameter to $\LamSRG = 1.88$ and $2.236\;\fmin$.
The sensitivity to $\hbar\omega$ has been verified by
varying the oscillator frequency and confirming that
the resulting changes in the scattering lengths are
smaller than the cutoff variation. Convergence with
respect to $j_{12}^{\mathrm{max}}$ has likewise been
verified: increasing $j_{12}^{\mathrm{max}}$ beyond the
value employed produces changes that are negligible
($\leq1\%$) compared to the cutoff variation. An
overall $0.5\%$ numerical uncertainty from the
integration grids alone is assigned to the one-body and
two-body contributions on the basis of the integration
convergence tests, consistent with the assessment in
sec.~\ref{NumMethod}. When combined with the residual
model-space truncation effects for $\LiS$, this yields
the $3\%$ systematic uncertainty quoted in the
uncertainty budget of sec.~\ref{sec:pipi_unc_budget}.
\subsection{Convergence of the Few-Nucleon Expansion}
\label{sec:pipi_uncertainties}

The scattering amplitude in eq.~\eqref{eq:totalscat}
receives contributions from operators involving one, two,
and up to $A$ active nucleons. The TDA formalism as
implemented in the present work retains only the first
two terms of this expansion, as written in
eq.~\eqref{TDAExpansion}. Assessing the convergence of
the few-nucleon series, and in particular the size of the
omitted three-nucleon and higher contributions, is
therefore essential for establishing the reliability of
the quoted results. The following discussion draws
extensively on the systematic analysis of the few-nucleon
hierarchy by Liebig \etal~\cite{Liebig_2011}, who
computed contributions up to and including four-nucleon
operators for $\pi$-$\HeT$ and $\pi$-$\HeF$.

\subsubsection{Uncertainty Budget}
\label{sec:pipi_unc_budget}
The uncertainties on $a^{\No}$ and $a^{\Nt}$ are
constructed in the same manner as for the pion
photoproduction amplitudes discussed in
sec.~\ref{sec:piphoto}. They incorporate variations
arising from different values of the chiral cutoff
$\LamNN$ and, for $\LiS$, the SRG flow parameter
$\LamSRG$, together with an overall $3\%$ systematic
uncertainty to account for the numerical integration
and residual model-space truncation effects.
Additional contributions to the $a^{\No}$ uncertainty
arise from the errors on $a^{(\pm)}$ propagated
through eq.~\eqref{eq:pipi}, as well as from the
cutoff $\LamNN$ employed in the nuclear potential.
Unlike the regulator extrapolation employed by
Braun~\cite{BraunThesis}, the variable substitution
used in the present calculation
(sec.~\ref{sec:pipi_singularity}) eliminates the
$\Lambda_\mathrm{reg} \to 0$ extrapolation entirely,
so no associated systematic uncertainty enters the
two-body error budget. A further advantage of the TDA
factorization is that the nuclear densities and the
reaction kernel are tested and converged independently:
the density convergence is established once through the
Compton analysis of sec.~\ref{sec:ComptonResultsC},
and the kernel integration is verified separately
through the tests of sec.~\ref{sec:pipi_singularity}.
This separation allows each source of numerical error
to be isolated and controlled, in contrast to a
combined calculation in which all sources of
uncertainty enter simultaneously.

The overall $3\%$ systematic assigned here is somewhat
larger than the integration uncertainty alone
($0.5\%$). This additional margin reflects the
absence, in the pion scattering channel, of
experimentally constrained multipole uncertainties
analogous to those available for the $E_{0+}$ and
$L_{0+}$ amplitudes in pion photoproduction
(sec.~\ref{sec:piphoto}). In the photoproduction
case, the SAID partial-wave analysis provides
multipole-level error estimates that can be propagated
through the calculation; no comparable uncertainty
decomposition exists for the $\piN$ scattering lengths
employed here, necessitating a more conservative
overall systematic.

It should be noted that these uncertainties reflect the
precision of the $\No + \Nt$ calculation as performed;
they do not include an estimate of the missing
three-nucleon and higher contributions. The truncation
uncertainty associated with the omission of these
higher-body terms is discussed separately below.

The chiral truncation error within the two-body sector
can be estimated from the results of Liebig
\etal~\cite{Liebig_2011}. The present two-body kernel
includes the LO diagrams~$(a)$ through~$(c)$ and the
topologically enhanced \NXLO{2} diagram~$(d)$, but
omits the remaining \NXLO{2} two-body diagrams on the
grounds that they lack this enhancement. Liebig \etal\
find that diagram~$(d)$ contributes approximately
$10$--$13\%$ of the leading Coulombian diagram~$(a)$
for $\pi$-$\HeF$, a ratio that is only mildly
suppressed relative to the parametric estimate of
$m_\pi^2/(16 f_\pi^2) \approx 0.14$ because of the
topological enhancement discussed in
sec.~\ref{sec:pipi_2N_convergence}. The remaining
\NXLO{2} diagrams do not benefit from this enhancement
and are therefore expected to be suppressed by the full
dimensional-analysis factor of
$(m_\pi/m_N)^2 \approx 0.02$ relative to
diagram~$(a)$~\cite{Liebig_2011}; however, $3\%$ is used here to be conservative. For
$\pi^-$-$\HeT$, this corresponds to an estimated
correction of
$\sim 0.02 \times 24
\approx 0.5 \times 10^{-3}m_{\pi^+}^{-1}$,
which is well within the quoted uncertainties. The
two-body chiral truncation error is therefore
subdominant relative to the other sources of
uncertainty in the present calculation, and is
subsumed into the overall systematic.
\subsubsection{Hierarchy of Few-Nucleon Contributions}
\label{sec:pipi_convergence}
Liebig \etal~\cite{Liebig_2011} performed a
comprehensive study of the relative magnitudes of
$N$-nucleon contributions to pion-nucleus scattering
lengths for ${}^2$H, $\HeT$, and $\HeF$, computing
explicit results for all leading two-nucleon,
three-nucleon, and (for $\HeF$) four-nucleon diagrams.
Their central finding is that successive $N$-nucleon
contributions are suppressed by a factor of
approximately~5, so that the 1N:2N:3N:4N hierarchy
scales roughly as $100:25:5:1$. This pattern corresponds
to an effective expansion parameter
$Q_{\text{few}} \approx 0.2$ governing the
convergence of the few-nucleon series, in the sense that
$|a^{(n+1)\text{N}}| / |a^{n\text{N}}|
\sim Q_{\text{few}}$.

This empirical suppression is considerably milder than
what Weinberg pragmatic power counting
predicts~\cite{WEINBERGpionpionNucleus}. As discussed
by Liebig \etal, the naive dimensional analysis for
pion-nucleus scattering at threshold yields an expected
ratio of $\sim 1/50$ per additional active nucleon,
corresponding to a hierarchy
$50^3 : 50^2 : 50 : 1$~\cite{Liebig_2011}. That the
actual suppression factor is $\sim 1/5$ rather than
$\sim 1/50$ reflects a partial cancellation between the
additional integration measures that enter when nucleons
are added (which provide most of the suppression in the
dimensional estimate) and enhancement mechanisms not
captured by the counting, such as the topological
enhancement of diagram~$(d)$ discussed in
sec.~\ref{sec:pipi_2N_convergence}~\cite{Liebig_2011}.
This situation parallels the broader experience with
Weinberg's pragmatic approach to few-nucleon systems
discussed in sec.~\ref{sec:weinbergPC}: the power
counting qualitatively identifies the correct hierarchy
of contributions but does not always capture the
quantitative suppression factors. Just as the BUQEYE
analyses of Melendez \etal~\cite{Melendez2019} and
Millican \etal~\cite{Millican2024, SMS400550}
demonstrate that the formal inconsistencies of Weinberg
counting do not manifest as statistically significant
deviations in NN observables at cutoffs
$\LamNN = 450$ and $500\;\MeV$, the Liebig \etal
analysis shows that the few-nucleon series for
pion-nucleus scattering remains sufficiently convergent
for controlled calculations despite the
milder-than-expected suppression.

Importantly, Liebig \etal\ find the suppression
factor of $Q_{\text{few}} \approx 0.2$ is stable
across the steps $1\text{N} \to 2\text{N}$,
$2\text{N} \to 3\text{N}$, and
$3\text{N} \to 4\text{N}$, and across all potentials
tested (chiral NLO, \NXLO{2}, AV18, and
CD-Bonn)~\cite{Liebig_2011}. The stability of
$Q_{\text{few}}$ across these transitions is
essential for estimating the size of missing higher-body
contributions, since it permits a controlled
extrapolation beyond the terms explicitly computed.

In the present calculation, the ratio
$|a^{\Nt}|/|a^{\No}|$ can be read directly from
Table~\ref{tab:pipi_results}. For $\pi^-$-$\HeT$,
$|a^{\Nt}|/|a^{\No}| = 23.6/88.5 \approx 0.27$,
which is somewhat larger than the value of
$\approx 0.21$ reported by Liebig \etal\ (Table~9 of
Ref.~\cite{Liebig_2011}). This modest difference is
attributable to the different nuclear potentials employed
($\chi$SMS versus chiral NLO/\NXLO{2} and
phenomenological potentials), but both values are
consistent with
$Q_{\text{few}} \approx 0.2$--$0.3$.
For the isoscalar nuclei $\HeF$ and $\LiS$, the 2N/1N
ratio is not a useful convergence diagnostic because the
one-body contribution is proportional to $A\,a^{(+)}$
and the near-vanishing of the isoscalar scattering
length
$|a^{(+)}| \approx 2.4 \times 10^{-3}m_{\pi^+}^{-1}$
makes the one-body term accidentally small. In these
cases, the two-body contribution constitutes the leading
term in practice, and the convergence of the few-nucleon
series must be assessed by estimating the absolute size
of the three-nucleon correction using the empirical
$Q_{\text{few}} \approx 0.2$.

\subsubsection{Estimated Three-Nucleon Contributions}
\label{sec:pipi_3N_estimate}
Three-nucleon operators, such as those depicted in
Fig.~3 of Ref.~\cite{Liebig_2011} and given by
their Eq.~(12), are not a natural extension of the TDA
method as currently implemented, since the
\texttt{nucdens} package provides only one- and two-body
transition densities. Computing three-nucleon
contributions would require three-body densities, which
are not yet available and whose generation and storage
would entail substantially greater computational cost
than the existing one- and two-body densities.
Nevertheless, the results of
Liebig \etal\ for $\pi$-$\HeT$ allow the magnitude of
the missing three-nucleon terms to be estimated.

For $\pi^-$-$\HeT$, Liebig \etal\ report the dominant
three-nucleon (Coulombian) contribution
$a^{(3)}_{\pi^-\text{-}{}^3\text{He}}$ in the range
$-3.2$ to $-4.1 \times 10^{-3}m_{\pi^+}^{-1}$ across
\NXLO{2} potentials, together with a sub-leading
three-nucleon piece
$a^{(14)}_{\pi^-\text{-}{}^3\text{He}}$ of order
$-0.5$ to $-0.8 \times 10^{-3}m_{\pi^+}^{-1}$, for a
total three-nucleon correction of approximately
$-4.5 \times 10^{-3}m_{\pi^+}^{-1}$
(Table~7 of Ref.~\cite{Liebig_2011}), see Table~\ref{tab:pipi_results}.
This is consistent
with the factor-of-5 suppression relative to their
two-nucleon contribution of
$\sim -22 \times 10^{-3}m_{\pi^+}^{-1}$, yielding a
3N/2N ratio of $\approx 0.20$, in agreement with their
Table~9. For the present $\HeT$ result, the estimated
three-nucleon correction of
$\sim 5 \times 10^{-3}m_{\pi^+}^{-1}$ (applying the
same factor of $\sim 0.2$ to the two-body contribution
of $23.6 \times 10^{-3}m_{\pi^+}^{-1}$) is comparable
to the quoted uncertainty in the present work of
$5.5 \times 10^{-3}m_{\pi^+}^{-1}$. Notably, the
three-nucleon correction is negative for
$\pi^-$-$\HeT$, indicating that its inclusion would
reduce the total scattering length and bring the present
$\No + \Nt$ result into even closer agreement with the
value of Liebig \etal, which already includes this
correction. The $\HeT$ result is
therefore robust against the inclusion of three-nucleon
effects at the expected level.

For the isoscalar nuclei $\HeF$ and $\LiS$, a crucial
distinction arises. Liebig \etal\ find that the dominant
three-nucleon diagram is
isovector~\cite{Liebig_2011}. For nuclei with total
isospin $T = 0$, isovector operators are suppressed
because the ground state has no isovector component to
leading order. Liebig \etal\ conclude explicitly that
``for the important case of $\HeF$, only one-nucleon and
two-nucleon diagrams will contribute significantly''
(Ref.~\cite{Liebig_2011}). Their explicit calculation of
the leading four-nucleon operator for $\pi$-$\HeF$
yields a suppression of $\approx 1/5^2$ relative to the
two-nucleon contribution, consistent with the overall
$100:25:5:1$ pattern and confirming that four-nucleon
contributions are numerically
insignificant~\cite{Liebig_2011}. On this basis, the
missing three-nucleon correction for $\HeF$ is expected
to be substantially smaller than the naive factor-of-5
estimate of
$\sim 0.2 \times 49.2
\approx 10 \times 10^{-3}m_{\pi^+}^{-1}$,
yet may well lie within the quoted uncertainty of
$4.9 \times 10^{-3}m_{\pi^+}^{-1}$, though a
quantitative determination requires an explicit
calculation.

For $\LiS$, no prior calculation of three-nucleon pion
scattering contributions exists. Applying the naive
factor-of-5 suppression to the two-body contribution
yields an estimate of
$\sim 0.2 \times 86.7
\approx 17 \times 10^{-3}m_{\pi^+}^{-1}$,
which would exceed the quoted uncertainty of
$7.5 \times 10^{-3}m_{\pi^+}^{-1}$ by more than a
factor of two. However, since $\LiS$ is (mostly)
isoscalar ($T = 0$), the isovector suppression of the
dominant three-nucleon diagram applies here as well, and
the actual three-nucleon correction is expected to be
considerably smaller than this estimate. The extent of
this suppression for $\LiS$ is not known quantitatively
and constitutes a systematic uncertainty that is not
captured by the error bars in
Table~\ref{tab:pipi_results}. Extending the TDA
framework to accommodate three-body densities, or
performing a dedicated three-nucleon calculation along
the lines of Liebig \etal, would be required to resolve
this uncertainty and is identified as a priority for
future work.
Based on the sign pattern observed by Liebig
\etal\ for $\pi$-$\HeT$, where the three-nucleon
correction is uniformly negative, the
corresponding correction for $\LiS$ is likewise
expected to be negative, which would increase
the magnitude of the total scattering length.

An analogous estimate can be made for the four-nucleon
contributions to $\pi$-$\LiS$. Liebig
\etal~\cite{Liebig_2011} computed the leading
four-nucleon (Coulombian) diagram for $\pi$-$\HeF$
and obtained
$a^{(4\mathrm{N})}_{\pi\text{-}\HeF}
= 2.31(31) \times 10^{-3}m_{\pi^+}^{-1}$
(see Table~\ref{tab:pipi_results}).
For $\HeF$, there is only $\binom{4}{4} = 1$ four-nucleon subset,
so this value represents the contribution of a single
such subset. For $\LiS$, the number of four-nucleon
subsets is $\binom{6}{4} = 15$, so the naive
combinatorial scaling yields an estimate of
$[\sim 15 \times 2.3] \munits \approx 35 \times 10^{-3}m_{\pi^+}^{-1}$.
If taken at face value, this would represent a
substantial correction, comparable in magnitude to the
two-body contribution itself. However, the sub-linear
scaling of the two-body contribution already observed
for $\LiS$ relative to $\HeF$ (a factor of $3.7$
versus the naive pair-count ratio of $5$, see
sec.~\ref{sec:pipi_discussion}) suggests that the
actual per-subset overlap integral is reduced for the
larger, more diffuse $\LiS$ wave function.
Nevertheless, this crude estimate underscores that
four-nucleon contributions may not be negligible for
$\LiS$ and should be investigated explicitly once
the requisite computational infrastructure becomes
available.

\subsubsection{Convergence within the Two-Body Sector}
\label{sec:pipi_2N_convergence}
Within the two-body sector itself, diagram~$(d)$ appears
at \NXLO{2} while diagrams~$(a)$ through $(c)$ enter at
LO. As discussed in sec.~\ref{sec:pipi_2N}, the
parametric suppression of diagram~$(d)$ relative to
diagram~$(a)$ is
$m_\pi^2/(16 f_\pi^2) \approx 0.14$~\cite{Liebig_2011},
and this suppression is partially compensated by a
topological enhancement arising from an integrable
singularity in the loop integral. For $\pi$-$\HeF$,
Liebig \etal\ find that the ratio
$a^{(d)}/a^{(a)}$ is approximately $0.10$ to $0.13$
across the potentials tested~\cite{Liebig_2011}. Since
this enhancement is a property of the diagram topology
rather than of the nuclear system, the relative size of
diagram~$(d)$ is expected to be similar for all nuclei
considered here, up to the isospin-weighting differences
discussed in sec.~\ref{sec:pipi_2N}. 

\subsection{Discussion of Results}
\label{sec:pipi_discussion}

The scattering lengths collected in
Table~\ref{tab:pipi_results} exhibit several features
that merit discussion.

For $\HeF$ and $\LiS$, the nuclear isospin projection
vanishes ($T_3 = 0$), so the isovector term
$Q_\pi\, a^{(-)}\, 2T_3$ in eq.~\eqref{eq:pipi} does
not contribute and the one-body scattering length is
independent of the pion charge. This is reflected in the
identical values of $a^{\No}$ across $\pi^-$, $\pi^0$,
and $\pi^+$ for both nuclei. It should be noted,
however, that while $\HeF$ is an essentially perfect
$I_A = 0$ state, the $\LiS$ ground state is only
predominantly isoscalar and carries a small $I_A = 1$
admixture. This admixture constitutes an additional
source of isospin violation beyond the pion mass
difference in the two-body kernel, and its consequences
are visible in the isospin decomposition of
sec.~\ref{sec:isospin_decomposition}. In contrast, $\HeT$ has
$T_3 = 1/2$, and the isovector scattering length
$a^{(-)} \approx 88 \times 10^{-3}m_{\pi^+}^{-1}$
exceeds
$|a^{(+)}| \approx 2.4 \times 10^{-3}m_{\pi^+}^{-1}$
by a factor of approximately~37. As a result, the
one-body contribution exhibits pronounced charge
dependence: it is large and positive for $\pi^-$, large
and negative for $\pi^+$, and nearly vanishing for
$\pi^0$, where only the small isoscalar term
$A\,a^{(+)}$ survives.

The $\HThree$ results in Table~\ref{tab:pipi_results}
are the charge-symmetric mirror of $\HeT$, as expected
for mirror nuclei related by the interchange of protons
and neutrons. Under this exchange, $T_3 \to -T_3$ and
$\pi^- \leftrightarrow \pi^+$, so that
$a^{(\No)}_{\pi^-\text{-}\HThree}
= a^{(\No)}_{\pi^+\text{-}\HeT}$ and vice versa. The
one-body contributions satisfy this relation exactly,
since eq.~\eqref{eq:pipi} depends on $T_3$ and $Q_\pi$
only through the product $Q_\pi\,T_3$. The two-body
contributions are not exactly symmetric because the
charged and neutral pion masses entering the propagators
of diagrams~$(a)$ through $(d)$ break isospin explicitly;
however, the resulting differences are at most
$0.2 \times 10^{-3}m_{\pi^+}^{-1}$, well below the
quoted uncertainties. The near-exact charge symmetry of
the trinucleon results serves as a consistency check of
the implementation, and of isospin symmetry.

The two-body contributions are uniformly negative across
all nuclei and pion charges, and their magnitude grows
substantially with nucleon number. For $\pi^\pm$
scattering, the two-body scattering lengths on $\HeT$,
$\HeF$, and $\LiS$ are approximately $-24$, $-49$, and
$-87$ in units of $10^{-3}m_{\pi^+}^{-1}$,
respectively. The ratio between $\HeF$ and $\HeT$ is
approximately $2.1$, close to the ratio of nucleon pairs
$\binom{4}{2}/\binom{3}{2} = 2$, indicating that the
additional nucleon pair in $\HeF$ contributes with
roughly the same weight as those in $\HeT$. For $\LiS$
relative to $\HeT$, however, the ratio of $a^{\Nt}$
contributions is approximately $3.7$, which falls well
below the naive pair-count ratio of
$\binom{6}{2}/\binom{3}{2} = 5$. This departure reflects
the role of nuclear structure: the two-body kernel is
weighted by the two-body TDA, which encodes the
probability amplitude of finding two nucleons at a given
relative separation. As $A$ increases, the average
internucleon distance and the spatial extent of the wave
function modify this weighting, so the two-body
contribution does not scale linearly with the number of
pairs. The $\LiS$ nucleus, with its larger spatial
extent compared to $\HeF$, has a more diffuse pair
distribution, which dilutes the overlap of the
short-range two-body kernel with the nuclear density.
A further structural factor is that $\LiS$ is a
$p$-wave nucleus: the two valence nucleons beyond the
$\HeF$ core must occupy $p$-wave orbitals due to the
Pauli exclusion principle, which places them at larger
average separations and reduces their overlap with the
short-range kernel compared to the $s$-wave pairs in
$\HeF$.

A notable feature common to all three nuclei is that the
$\pi^0$ two-body contribution is systematically smaller
in magnitude than the corresponding $\pi^\pm$ values.
For $\HeF$, the $\pi^0$ two-body scattering length is
$-45.9 \times 10^{-3}m_{\pi^+}^{-1}$, approximately
$7\%$ smaller in magnitude than the $\pi^\pm$ value of
$-49.2 \times 10^{-3}m_{\pi^+}^{-1}$; for $\LiS$ the
analogous reduction is also approximately $7\%$
($-80.6$ versus $-86.7$). This difference arises from
the isospin structure of the two-body operators: the
combination
$(\vec{\tau}_1 \cdot \vec{\tau}_2 - \tau_1^a \tau_2^a)$
appearing in diagrams~($a$) through ($c$) yields
different matrix elements for $a = 3$ (neutral pion)
than for $a = 1,2$ (charged pions), while diagram~($d$),
which contains only $\tau_1^a \tau_2^a$, contributes
with opposite relative sign. An additional
contribution to the charged/neutral difference arises
from the different physical pion masses,
$m_{\pi^\pm} \neq m_{\pi^0}$, which enter the
propagators of diagrams~$(a)$ through~$(d)$; this
effect is of comparable magnitude to the isospin-operator
contribution but is not separated here.

For all nuclei considered, the two-body contribution
constitutes the dominant component of the total
scattering length. In $\HeF$ and $\LiS$, the portions
of the scattering length from two-body terms are the
same (with uncertainties) and account for approximately
$83$--$85\%$ of the total for $\pi^\pm$.
Even in $\HeT$, the two-body correction exceeds the
one-body term in magnitude for the $\pi^0$ channel
($|a^{\Nt}|/|a^{\No}| \approx 2.8$), and for the
$\pi^+$ channel the two-body and one-body terms are of
the same sign, so that both contribute constructively
to a total of $-127.5 \times 10^{-3}m_{\pi^+}^{-1}$.
This dominance of the two-body sector is consistent with
the pattern observed in pion photoproduction
(see sec.~\ref{sec:piphoto}), where the two-nucleon
contributions were found to be of comparable magnitude
or larger than the one-body terms for the trinucleon
systems. 
Interestingly, in Compton scattering the one-body
terms dominate at $60\;\MeV$
(see fig.~\ref{fig:twobodyconvergence}), but the
two-body contributions increase monotonically with
energy, such that the two-body
sector dominates at $100\;\MeV$.
This is consistent with the pattern seen in both pion
photoproduction and pion scattering, whose threshold
energies
$E^{\text{thresh}}_{\gamma\pi} \sim
E^{\text{thresh}}_{\pi\pi} \sim \mpi < 100\;\MeV$
already place these processes in the regime where
two-body dynamics contribute substantially.

The growing dominance of the two-body sector
with increasing $A$ underscores the essential role of
few-nucleon dynamics in pion-nucleus scattering, and
makes precise knowledge of the two-body kernel and the
associated nuclear transition densities indispensable
for any reliable extraction of $a^{(+)}$ from isoscalar
targets.

\subsubsection{Comparison with Previous Calculations}
\label{sec:pipi_comparison}
For $\pi^-$-$\HeT$, the total scattering length
$a = 64.9(55) \times 10^{-3}m_{\pi^+}^{-1}$ may be
compared with the prediction of
Liebig \etal~\cite{Liebig_2011}, who obtained
$a_{\pi^- \text{-} {}^3\text{He}}
= (62 \pm 4 \pm 7) \times 10^{-3}m_{\pi^+}^{-1}$,
where the first uncertainty arises from the $\piN$
scattering lengths and the second from few-nucleon
effects. The two results agree within uncertainties
despite substantial differences in methodology: the
present work employs the $\chi$SMS
potential~\cite{Reinert2018} within the TDA formalism
using deterministic quadrature, whereas
Liebig \etal\ used a variety of chiral and
phenomenological potentials (including AV18 and CD-Bonn)
with Monte~Carlo integration. Furthermore, the present
calculation includes only one- and two-nucleon
contributions, whereas the result of Liebig \etal\
includes three-nucleon corrections at the level of
approximately $4 \times 10^{-3}m_{\pi^+}^{-1}$, which
lie within the uncertainty of the present result. This
cross-validation between two independent approaches,
employing different potentials, different numerical
methods, and different formalisms for packaging the
nuclear structure, provides strong confidence in the
robustness of the \chiEFT prediction for the
$\pi$-$\HeT$ scattering length.
The present uncertainty of
$5.5 \times 10^{-3}m_{\pi^+}^{-1}$ is
somewhat smaller than the combined uncertainty
of Liebig \etal\ primarily because the
deterministic quadrature eliminates the
Monte~Carlo statistical error present in their
calculation. This reduction is partially offset
by the absence of the three-nucleon correction,
whose omission constitutes an additional
unquantified uncertainty in the present
$\No + \Nt$ result.

A more detailed comparison is afforded by
Table~\ref{tab:pipi_results}, which decomposes the
results of Liebig \etal\ into one-, two-, three-, and
four-nucleon sectors. The one-body contributions are
identical by construction, since both calculations employ
the same $\piN$ scattering length input. In the
two-body sector, the present result of
$a^{\Nt}_{\pi^-\text{-}\HeT}
= -23.6 \times 10^{-3}m_{\pi^+}^{-1}$ is in good
agreement with the Liebig \etal\ value of
$-21.3 \times 10^{-3}m_{\pi^+}^{-1}$; the modest
difference of
$\sim 2 \times 10^{-3}m_{\pi^+}^{-1}$ is
attributable to the different nuclear potentials
($\chi$SMS versus \NXLO{2} Epelbaum--Gl\"ockle--Mei\ss
ner). The three-nucleon contribution of
$-4.8 \times 10^{-3}m_{\pi^+}^{-1}$ reported by
Liebig \etal\ is not included in the present
$\No + \Nt$ calculation but lies within its quoted
uncertainty, and its inclusion would bring the two
totals into even closer agreement. For
$\pi$-$\HeF$, Liebig \etal\ find the two-body sector
to be $-45.8 \times 10^{-3}m_{\pi^+}^{-1}$, compared
with the present value of
$-49.2 \times 10^{-3}m_{\pi^+}^{-1}$, again
consistent within the cutoff variation. Their
four-nucleon contribution of
$2.3 \times 10^{-3}m_{\pi^+}^{-1}$ is numerically
insignificant at the current level of precision.

\subsubsection{Comparison with Pionic-Atom Measurements}
\label{sec:pipi_exp_comparison}
The available pionic-atom measurements and theoretical
predictions for $\pi^-$-$\HeT$ are collected in
Table~\ref{tab:pipi_comparison_3He}.
\begin{table}[H]
\centering
{\setlength{\extrarowheight}{3pt}
\begin{tabular}{lrr}
\rule[-1.1ex]{0pt}{2.8ex}
  & $\varepsilon_{1s}$ [eV]
  & $a_{\pi^-\text{-}{}^3\text{He}}$
    $[10^{-3}m_{\pi^+}^{-1}]$ \\
\thickline{0.15em}
Abela \etal~\cite{Abela1977}
  & $44 \pm 5$ & $56 \pm 6$ \\
Mason \etal~\cite{Mason1980}
  & $34 \pm 4$ & $43 \pm 5$ \\
Schwanner \etal~\cite{Schwanner1984}
  & $32 \pm 3$ & $41 \pm 4$ \\
\hline
Liebig \etal~\cite{Liebig_2011}
  & & $62 \pm 4 \pm 7$ \\
TDA (present work)
  & & $64.9 \pm 5.5$ \\
\hline
\end{tabular}
}
\caption[Comparison of $\pi^-$-${}^3$He scattering length with theory and experiment]{Comparison of the $\pi^-$-$\HeT$ scattering
  length from the present work with the theoretical
  prediction of Liebig \etal~\cite{Liebig_2011} and
  with values extracted from pionic-atom $1s$ level
  shift measurements at PSI via generalized Deser-type
  formulae~\cite{baru_He3, Deser1954}. The two
  uncertainties on the result of Liebig \etal\ correspond
  to $\piN$ scattering length ambiguities and
  few-nucleon effects, respectively. The result of
  Liebig \etal\ includes three-nucleon corrections at
  the level of
  $\approx 4 \times 10^{-3}m_{\pi^+}^{-1}$,
  which the present $\No + \Nt$ calculation omits.}
\label{tab:pipi_comparison_3He}
\end{table}
The present result is consistent with the earliest
measurement of Abela \etal\ at the $1\sigma$ level, but
exceeds the later measurements of Mason \etal\ and
Schwanner \etal\ by approximately $3.0\sigma$ and
$3.5\sigma$, respectively. Notably, the three
measurements themselves exhibit a $\sim 2\sigma$ spread
at the level of the raw level shift
($\varepsilon_{1s} = 44 \pm 5$ versus $32 \pm 3$ eV),
indicating that the tension predates the conversion to
scattering lengths and likely resides in the measurements
themselves rather than in the Deser-type extraction
procedure. The present result thus confirms the tension
first identified by
Liebig \etal~\cite{Liebig_2011}, whose theoretical value
likewise lies above the Mason and Schwanner
determinations. A new measurement of the
$\pi^-$-$\HeT$ level shift at PSI would help to clarify
this long-standing discrepancy.

For isoscalar targets, the scattering lengths are
sensitive almost exclusively to the two-body sector. The
$\pi$-$\HeF$ result of
$a = -59.6(49) \times 10^{-3}m_{\pi^+}^{-1}$
constitutes a prediction that could be tested by a
future measurement of the $\pi^-$-$\HeF$ atomic level
shift at PSI. Because the one-body contribution for
isoscalar nuclei is proportional to $A\,a^{(+)}$ and the
isoscalar scattering length
$|a^{(+)}| \approx 2.4 \times 10^{-3}m_{\pi^+}^{-1}$
is more than an order of magnitude smaller than the
two-body contribution, the one-body term accounts for
only $17\%$ of the total $\pi$-$\HeF$ scattering length.
The $\pi$-$\HeF$ result is therefore dominated by the
two-body mechanism and provides a direct window into the
few-nucleon dynamics encoded in the TDA. Similarly,
the $\pi$-$\LiS$ prediction of
$a = -102.5(75) \times 10^{-3}m_{\pi^+}^{-1}$
represents the first calculation of this quantity within
the TDA formalism and would benefit from future
measurements; pionic $\LiS$ should be experimentally
accessible at facilities such as PSI, given
that the requisite pion beams and X-ray
spectroscopy infrastructure are already in
place for lighter targets.
\subsection{One-Body Pion Scattering Above Threshold}
\label{sec:pipi_above}
The preceding sections focused exclusively on the
threshold regime, where the two-body kernel is
available and a complete $\No + \Nt$ calculation can
be performed. As a preliminary demonstration that the
TDA framework extends naturally to higher energies,
this section presents the one-body contribution to
elastic pion-nucleus scattering above threshold.
The two-body kernel has not yet been generalized to
above-threshold kinematics, so only the one-body
sector is included; the results presented here are
therefore incomplete and should be regarded as work in
progress.

Above threshold, higher partial waves contribute to the
scattering matrix of \meqref{eq:scatmat_pion}, and
the full energy dependence of the partial-wave amplitudes
$f_\alpha(\omega)$ must be retained. As a demonstration
of this capability within the TDA framework,
fig.~\ref{fig:pion_above} displays the one-body
contribution to the elastic pion scattering amplitude
for $\HeT$, $\HThree$, $\HeF$, and $\LiS$ at a
center-of-mass pion energy of $170\;\MeV$.
At this energy, the angular dependence visible in the
figure arises from the contributions of partial waves
beyond the $S$-wave. In particular, the $P_{33}$ partial
wave receives enhancement from the nearby $\Delta(1232)$
resonance, which is the primary source of the nontrivial
angular structure. The SAID WI08 partial-wave
amplitudes~\cite{PiPiSaid} are used as input to the
one-body kernel; the two-body sector is not included.
%
\begin{figure}%[H]
\centering
\includegraphics[width=\linewidth]{170MeV.pdf}
\caption[One-body elastic pion scattering amplitude at $E^\pi_{\mathrm{cm}} = 170$~MeV]{One-body ($1\mathrm{N}$) contributions to the
elastic pion scattering amplitude at
$E^\pi_{\mathrm{cm}} = 170\;\MeV$ using SAID
partial-wave amplitudes as input to the TDA one-body
kernel. The two-body sector, which is expected to
remain significant at this energy, is not included.
The quantity plotted,
$\Tr[\calM_{1\mathrm{N}}
{\calM_{1\mathrm{N}}}^\dagger]/(64\pi^2 s)$,
is the contribution of the one-body sector to the
full cross section calculation, but is not itself
a cross section.}
\label{fig:pion_above}
\end{figure}

Several features of fig.~\ref{fig:pion_above}
reflect the underlying isospin structure of elastic
pion-nucleus scattering. For the isovector nuclei $\HeT$
and $\HThree$ ($T=\half$), the three charge channels are
split by the coupling of the isovector $\piN$ amplitude
to the nuclear isospin projection $T_3$, the same
mechanism that governs the charge-channel ordering at
threshold through \meqref{eq:pipi}. The $\HThree$ panel
exhibits the expected isospin-mirror pattern: the roles
of $\pi^+$ and $\pi^-$ are interchanged relative to
$\HeT$, consistent with the substitution
$T_3 \to -T_3$. For the isoscalar nuclei $\HeF$ and
$\LiS$, both of which have total isospin $T=0$ in
their ground states, isospin symmetry requires the
$\pi^+$ and $\pi^-$ contributions to coincide. This
equality is confirmed numerically in both panels of
fig.~\ref{fig:pion_above}. It should be emphasized that
the quantity plotted in fig.~\ref{fig:pion_above} is not
a cross section, as it omits the two-body contributions;
it represents only the one-body portion of the full
amplitude squared. Extension of the two-body kernel to
above-threshold kinematics remains an important
direction for future work.

\subsection{Summary and Outlook}
\label{sec:pipi_summary}
This chapter presented the first calculation of
pion-nucleus scattering lengths for $\HThree$, $\HeT$,
$\HeF$, and $\LiS$ within the TDA formalism
with $\LiS$ computed for the first time by any method.
The principal results are collected in Table~\ref{tab:pipi_results}.

The agreement between the present $\pi^-$-$\HeT$ result
and the independent calculation of
Liebig \etal~\cite{Liebig_2011}, obtained with entirely
different potentials, integration methods, and
nuclear-structure formalisms, constitutes a strong
cross-validation of the \chiEFT prediction. It also
demonstrates that the TDA factorization into
reaction-independent densities and process-specific
kernels provides a reliable framework for the dominant
one- and two-nucleon contributions to pion-nucleus
scattering. The variable substitution technique for the
removable singularity, developed for pion photoproduction
in sec.~\ref{NumMethod}, was successfully applied here
as well, eliminating the regulator extrapolation
uncertainty present in prior calculations and confirming
the versatility of the method across reaction channels.

The convergence analysis of
sec.~\ref{sec:pipi_uncertainties} identified the omitted
three-nucleon contributions as the dominant uncontrolled
systematic, particularly for the heavier nuclei. For
$\HeT$, the estimated three-nucleon correction of
$\sim 5 \times 10^{-3}m_{\pi^+}^{-1}$, based on
$Q_{\text{few}} \approx 0.2$, lies within the
quoted uncertainty and does not affect the conclusions.
For the isoscalar nuclei $\HeF$ and $\LiS$, the dominant
three-nucleon diagram is
isovector~\cite{Liebig_2011} and therefore suppressed
for $T = 0$ targets, but the quantitative extent of this
suppression is not known for $\LiS$, where the naive
$Q_{\text{few}}$ estimate yields a correction of
$\sim 17 \times 10^{-3}m_{\pi^+}^{-1}$. Resolving
this uncertainty through an explicit three-nucleon
calculation is the most important theoretical improvement
needed. A complementary improvement on the two-body side
would be to complete the $\mathrm{N}^2\mathrm{LO}$
kernel by including the remaining two-nucleon diagrams
beyond diagram~$(d)$, which are presently omitted on the
grounds that they lack the topological enhancement. An
explicit evaluation of these diagrams would confirm this
expectation and reduce the truncation uncertainty within
the two-body sector.

The TDA framework as currently implemented accommodates
only one- and two-body TDAs;
extending this to three-body densities would require
substantial development of both the \texttt{nucdens}
package and the convolution infrastructure. A more
practical near-term strategy would be to compute the
three- and four-nucleon contributions independently,
following the direct evaluation approach of
Liebig \etal~\cite{Liebig_2011}, and combine them with
the TDA-based one- and two-nucleon results. Since the
few-nucleon expansion of eq.~\eqref{eq:totalscat} is
additive, such a hybrid calculation can be performed
without loss of consistency, provided the same nuclear
wave functions are employed. This approach would retain
the efficiency and generality of the TDA for the dominant
one- and two-body sectors while incorporating the
higher-body corrections needed for precision predictions
on heavier targets.
It is worth noting that although contributions involving
larger numbers of active nucleons are dynamically
suppressed, the combinatorial growth of the number of
$n$-nucleon subsets, $\binom{A}{n}$, which is maximized
for $n = A/2$, may counteract this suppression as $A$
increases. So far this has not been observed up to
$A = 4$, with $Q_\mathrm{few} \approx 0.2$ as reported by
Liebig \etal~\cite{Liebig_2011} being remarkably stable.
For $\LiS$, however, the combinatorial factor
$\binom{6}{4} = 15$ for four-nucleon subsets amplifies
the per-subset contribution by more than an order of
magnitude relative to $\HeF$ (where
$\binom{4}{4} = 1$), yielding a naive estimate of
$\sim 35 \times 10^{-3}m_{\pi^+}^{-1}$ for the total
four-nucleon correction
(sec.~\ref{sec:pipi_3N_estimate}). While the actual
value is expected to be reduced by the sub-linear
scaling of matrix elements with $A$, this estimate
suggests that four-nucleon contributions may not be
negligible for $\LiS$ and warrant explicit
investigation.

On the experimental side, the persistent $\sim 3\sigma$
tension between theory and the later pionic $\HeT$
measurements, now confirmed by two independent
calculations, underscores the need for a new
high-precision measurement of the $\pi^-$-$\HeT$ level
shift. The $\pi$-$\HeF$ and $\pi$-$\LiS$
scattering lengths constitute predictions that can be
tested by future pionic-atom measurements. The $\HeF$
result is particularly valuable: the one-body
contribution is suppressed and the three-nucleon
corrections are expected to be small for this isoscalar
target, making it a clean probe of two-body chiral
dynamics and providing an independent determination of
$a^{(+)}$ complementary to the constraints from pionic
hydrogen and deuterium.

The success of the TDA formalism for Compton scattering,
pion photoproduction, and pion scattering demonstrates
the versatility of the factorized approach and the
generality of the \texttt{DensityScattering} code
suite~\cite{long_2026}. The same computational
infrastructure can be extended to heavier $p$-shell nuclei
as the requisite transition densities become available.
The sub-linear scaling of the two-body contribution with
nucleon number observed for $\LiS$ (a factor of $3.7$
relative to $\HeT$, versus the naive pair-count ratio of
$5$) suggests that the TDA approach remains
computationally tractable for heavier targets, though the
growing importance of the missing three-nucleon sector
will need to be addressed as $A$ increases.


==> piphoto/piphoto.tex <==
%! TEX root = ../Dis-AlexanderLong.tex
% \newcommand{\eps}{\vec{\epsilon}}
\newcommand{\epsTL}{\vec{\epsilon}_{_\mathrm{T/L}}}
\newcommand{\epsT}{\vec{\epsilon}_{_\mathrm{T}}}
\newcommand{\epsL}{\vec{\epsilon}_{_\mathrm{L}}}
\newcommand{\epslam}{\vec{\epsilon}}
\newcommand{\uTL}{_{_{\mathrm{T/L}}}}
\newcommand{\ulam}{_{\lambda}}
\newcommand{\uT}{_{_{\mathrm{T}}}}
\newcommand{\uL}{_{_\mathrm{L}}}
\newcommand{\Mj}{M_J}
\newcommand{\Mjp}{M_J'}
% \section{Neutral Pion-Photoproduction and Electroproduction}
\section{Pion Photo and Electro-production}
\label{sec:piphoto}
\subsection{Overview}
\label{sec:piphoto_overview}
Neutral pion photoproduction and electroproduction on
nuclear targets offer a sensitive probe of chiral
dynamics in QCD; for a comprehensive review see
refs.~\cite{BERNARD_1995,Bernard_2008review}. While proton targets are
directly accessible in experiment, extracting pion
production amplitudes from the neutron requires
nuclear targets such as the deuteron or the
three-nucleon bound states $\HThree$ and $\HeT$. Of
particular interest is the prediction of \chiEFT that
the elementary neutron $S$-wave multipole
$E_{0+}^{\pi^0 n}=+2.13\times 10^{-3}/m_{\pi^+}$
exceeds in magnitude the corresponding proton
amplitude
$E_{0+}^{\pi^0 p}=-1.16\times
10^{-3}/m_{\pi^+}$~\cite{bernard_1994,Bernard_2001}.
This ordering, first predicted by Bernard
\etal~\cite{bernard_1994,Bernard_2001}, is a
nontrivial consequence of the chiral loop structure
at $\calO(p^4)$ and constitutes a stringent test of
\chiEFT that can be probed through pion
photoproduction on light nuclear
targets~\cite{PionPhotoOrig}.

A systematic framework for calculating neutral pion
photoproduction observables at threshold on nuclei
using \chiEFT was developed by Beane, Lee, and
van~Kolck~\cite{PionPhotoOrig}, building on the
well-known observation that the leading one-body
contact interaction, the Kroll--Ruderman vertex \cite{KrollRuderman}, is
proportional to the charge of the produced pion and
therefore vanishes identically for $\pi^0$
production~\cite{BERNARD_1995}. In the charged pion
channels, this vertex provides the dominant
contribution to the cross section at lowest
order~\cite{PionPhotoOrig}; its absence in the
neutral channel suppresses one-body contributions and
elevates two-body pion-exchange mechanisms to a
leading role, rendering the observable particularly
sensitive to chiral two-body dynamics. The calculation
on the deuteron at threshold was subsequently carried
through to $\calO(q^4)$ by Beane
\etal~\cite{Beane_1997}.

Lenkewitz \etal~\cite{Lenke2011,Lenke2013,LenkeThesis} extended
this program to the trinucleon systems, computing the
$S$-wave production amplitude for $\HeT$ and
$\HThree$ at $\calO(q^4)$ using chiral \NXLO{2} wave
functions obtained from the Faddeev equations with the
Epelbaum--Gl\"ockle--Mei{\ss}ner
potential~\cite{Epelbaum_2004}. That work confirmed
quantitatively a well-known property of $\HeT$,
previously exploited in the context of $\HeT$ Compton
scattering~\cite{Shukla2007}: its wave function is
dominated by the principal $s$-state component with
the $(pp)$ pair contributing total spin-$0$, so that
the overall nuclear spin is carried predominantly by
the unpaired neutron, making it an effective neutron
target. The resulting partial cancellation between the
positive one-body and negative two-body contributions
renders the total $\HeT$ amplitude sensitive to the
elementary neutron multipole $E_{0+}^{\pi^0 n}$,
thereby providing a means to test the \chiEFT
prediction noted above.

More recently, Braun~\cite{BraunThesis} extended the
calculation to $\LiS$ using NCSM wave functions
generated with the Entem--Machleidt \NXLO{3}
potential~\cite{Entem_2003}, supplemented by the
\NXLO{2} three-nucleon interaction and softened via SRG
evolution.
Braun evaluated the production amplitudes through a
density matrix formalism in the harmonic-oscillator
basis, in which both the nuclear interaction and
the production operator are transformed via SRG
evolution into the harmonic-oscillator representation
and traced against the NCSM density matrices. This
approach differs from the transition density
amplitude (TDA) method adopted in the present work
(sec.~\ref{sec:TDA}), which operates directly in
momentum space and convolves the production kernel
with precomputed transition densities and is much simpler. A notable
advantage of the TDA method is that the production
kernel is evaluated in its original, unevolved form;
the effects of the SRG transformation enter only
through the nuclear transition densities, eliminating
the need to evolve the reaction kernel.
Braun did not include the $\calO(q^4)$ static or
recoil corrections; the $\calO(q^4)$ static corrections are included in the present work.

On the experimental side, neutral pion
photoproduction at and above threshold on light nuclei has been
investigated at the Saskatchewan Accelerator Laboratory (SAL) for
targets including $\HT$, $\HeF$~\cite{Bergstrom1998,Barnett2008},
and $\LiS$~\cite{Bergstrom1999}, and at the Mainz Microtron (MAMI)
for targets up to ${}^{12}\mathrm{C}$; see ref.~\cite{BraunThesis} and
references therein for a survey of targets measured to
date. For single-nucleon photoproduction, a
comprehensive partial-wave analysis program is
maintained by the Data Analysis Center (DAC) group at
George Washington
University~\cite{SAID2012piphoto,SAID2023piphoto},
which provides multipole amplitudes fitted to a broad
corpus of pion photoproduction data. Future
measurements, for example at MAMI, could extend
threshold neutral pion photoproduction to additional
light nuclear targets.
The sequence of light nuclei $\HeT$, $\HThree$,
$\HeF$, and $\LiS$, spanning binding energies from
approximately $8$ to $32~\MeV$ and mass numbers
$A=3$ to $6$, offers a systematic test of the
\chiEFT production operators across nuclear
environments of increasing complexity: from the
Faddeev-solved trinucleon systems, through the
Faddeev--Yakubovsky $\HeF$, to the NCSM-treated
$p$-shell nucleus $\LiS$ with its dominant
$\alpha + d$ cluster structure.

In the present work, the TDA formalism described in
sec.~\ref{sec:TDA} is applied to neutral pion
photoproduction on $\HThree$, $\HeT$, and $\LiS$.
Results for $\HeF$ are omitted at threshold because
the spin-dependent production operator
$\vec{\epsilon}_\lambda \cdot \vec{J}$ yields zero
when evaluated between $J^\pi=0^+$ states, so that
pion photoproduction on $\HeF$ vanishes at this order.
The production amplitude is decomposed into one-body
($1\mathrm{N}$) and two-body ($2\mathrm{N}$)
contributions, each obtained by convolving the
corresponding irreducible kernel with the nuclear
transition densities. Although the formalism is
developed to accommodate electroproduction as well,
retaining the longitudinal multipole $L_{0+}$
throughout, all numerical results presented in this
section pertain to real photons ($k^2=0$) and
therefore to pion photoproduction.

The two-body kernels are derived within \chiEFT,
following the operator structures of Beane
\etal~\cite{Beane_1997}, with $\calO(q^4)$ static
corrections following the framework of Krebs
\etal~\cite{Krebs_2004} as extended to the trinucleon
by Lenkewitz \etal~\cite{Lenke2013}. The current
implementation of the TDA method is restricted to
coherent reactions that preserve the nuclear ground
state, i.e.\ $A + \gamma \to A + \pi^0$. The present
work therefore considers only neutral pion
photoproduction; for the full multipole expansion of
pion photoproduction, and for details above threshold, see
refs.~\cite{Perlstein,Bernard_1996,DDreschsel_1992}.

Two complementary approaches to the one-body kernel
are employed, each offering distinct physical insight.
The first is a direct calculation within \chiEFT at
threshold, where only the $S$-wave multipoles
$E_{0+}$ and $L_{0+}$ contribute; the elementary
single-nucleon amplitudes and their chiral order are
discussed in sec.~\ref{sec:piphoto_1N_thresh}. In
this approach, both the elementary production
amplitude and the nuclear binding are derived within
\chiEFT, so that the resulting observable tests the
consistency of the framework as a whole. The second
approach, applicable above threshold where higher
partial waves and the proximity of the $\Delta(1232)$
resonance become relevant, replaces the \chiEFT
kernel with a phenomenological reconstruction of the
$\gamma N \to \pi N$ scattering matrix from SAID
partial-wave
amplitudes~\cite{SAID2023piphoto}. Following the
framework introduced by Chew \etal~\cite{Chew}, the
amplitude is expanded in multipoles $E_{l\pm}$ and
$M_{l\pm}$, which are fitted to data. Adopting these
phenomenological amplitudes as input to the TDA
one-body kernel permits the computation of pion
photoproduction observables on nuclei over a range of
photon energies, without relying on the convergence
of the chiral expansion for the elementary process.
At threshold, where both approaches are applicable,
their agreement provides a valuable consistency check
of the nuclear structure input; above threshold, only
the phenomenological approach is employed, as the
proximity of the $\Delta(1232)$ resonance renders the
chiral expansion for the elementary amplitude poorly
convergent. For treatment of the $\Delta(1232)$ resonance, see ref.~\cite{rij}.

Turning to the choice of nuclear interaction, the
present work employs the $\chi$SMS potentials of
Reinert \etal~\cite{Reinert2018}, which represent the
current state of the art in semilocal momentum-space
chiral interactions. For the trinucleon systems,
nuclear densities are computed directly with these
potentials; for $\LiS$, the no-core shell model
(NCSM) with SRG-evolved interactions is used, as
described in sec.~\ref{sec:TDA}. All three
calculations in this line of work, those of
Lenkewitz, Braun, and the present one, employ the
same \chiEFT pion photoproduction operators derived
from the Feynman diagrams of Beane
\etal~\cite{Beane_1997} and Krebs
\etal~\cite{Krebs_2004}; the principal differences
lie in the nuclear wave functions, the numerical
strategy for evaluating the matrix elements, the
scope of targets considered, and the order at which
the chiral calculations are truncated. In the present
work, matrix elements are evaluated within the TDA
framework of sec.~\ref{sec:TDA}, and the
$\calO(q^4)$ static corrections are included for all
targets. A notable advantage of the TDA formalism is
its modularity: the computational infrastructure
developed for one reaction is readily adapted to
additional processes by replacing only the
single-nucleon and two-nucleon kernels. The same code
suite used for Compton scattering
(sec.~\ref{sec:ComptonC}) and pion scattering
(sec.~\ref{sec:pion}) is applied here, whereas the
calculations of Lenkewitz and Braun each required
independent implementations for their respective
reactions~\cite{LenkeThesis,BraunThesis}. In addition
to extending the results of Lenkewitz to modern
$\chi$SMS potentials and to $\LiS$, and extending the
results of Braun to include the $\calO(q^4)$ static
corrections and the longitudinal multipole $L_{0+}$,
the present work provides the first determination of
both transverse and longitudinal $S$-wave multipoles
for all targets within a single consistent framework.
Since all three calculations employ the same \chiEFT
pion photoproduction operators at the same chiral
order, the spread of results across the three groups
provides an empirical estimate of the sensitivity to
higher-order corrections: all three approaches should
yield equivalent amplitudes up to effects beyond the
common truncation order, so that the observed
differences reflect the residual dependence on the
nuclear wave functions and numerical methods, which
enters at the level of the neglected higher-order
terms. This comparison is presented in
sec.~\ref{ss:BraunSqrt2}.

This section is organized as follows. The kinematics
and conventions are established in
sec.~\ref{sec:piphoto_kinematics}. The extraction of
the $S$-wave multipoles $E_{0+}$ and $L_{0+}$ from
the nuclear matrix element is presented in
sec.~\ref{sec:piphoto_extraction}, followed by the
one-body kernel at threshold using $\calO(p^4)$
\chiEFT amplitudes
(sec.~\ref{sec:piphoto_1N_thresh}) and the threshold
two-body kernel at $\calO(q^3)$ and $\calO(q^4)$
(sec.~\ref{sec:piphoto_2N}), including the numerical
treatment of the removable moving singularity in the
two-body propagator (sec.~\ref{NumMethod}).  The
threshold results and a detailed comparison with the
results of Lenkewitz \etal and Braun are presented in
sec.~\ref{sec:piphoto_2N_results}, including the
resolution of a $\sqrt{2}$ normalization discrepancy
with Braun for $\LiS$
(sec.~\ref{ss:BraunSqrt2}) and the order-by-order
convergence of the chiral expansion
(sec.~\ref{sec:piphoto_convergence}). The
phenomenological one-body kernel above threshold,
constructed from SAID partial-wave amplitudes, is
presented in sec.~\ref{sec:piphoto_above}, along with
a comparison of the SAID and \chiEFT amplitudes at
threshold and an analysis of the sensitivity of the
$\HeT$ and $\HThree$ threshold cross sections to the
elementary neutron and proton multipoles.

\subsection{Kinematics and Conventions}
\label{sec:piphoto_kinematics}
The momenta and quantum numbers used throughout this
section follow the conventions of the pion
photoproduction literature. The elementary reaction is
\begin{equation}
  \gamma(k, \epsilon_\lambda) +X(p)
  \to \pi^c(k') + X(p^\prime)\,,
\end{equation}
where $\gamma$ denotes the photon with four-momentum
$k$ and polarization $\epsilon_\lambda$, $X$ is the
incoming (outgoing) nucleon or nucleus with momentum
$p$\,($p'$), and $\pi^c$ is the outgoing pion with
isospin index $c$ and momentum $k'$. For neutral pion
production, $c=3$ so that $\pi^c = \pi^0$.
Throughout this section, $\Mj$ ($\Mjp$) denotes the
magnetic quantum number of the initial (final) nuclear
state with total angular momentum $J$, and
$\Mnucl$ denotes the nuclear mass. The
nuclear spin operator is written as $\vec{J}$, with
$\vec{J} = \vec{\sigma}/2$ for spin-$\frac{1}{2}$
nuclei and the standard spin-$1$ matrices for $\LiS$
(see sec.~\ref{ss:BraunSqrt2} for a discussion of
spin-$1$ matrix conventions).
\begin{figure}[H]
\centering
\includegraphics[scale=0.8]{piGamma-Nuc.pdf}
\caption[One-body contribution to pion photoproduction on a nucleus]{One-body contribution to pion photoproduction
on a nucleus. The photon $\gamma$ is absorbed by a
single nucleon inside the nucleus, producing a neutral
pion $\pi^c = \pi^3$. The remaining $A-1$ nucleons act
as spectators.}
\label{fig:piGammaOneBod}
\end{figure}
The isospin labels of pions in the literature,
including those in
refs.~\cite{BERNARD_1995,Liebig_2011,Lenke2011},
follow the Cartesian basis, with indices $i=1,2,3$
corresponding to the isospin operators $\tau^i$. These
are related to the physical (charge) basis by
\begin{equation}
  \kt{\pi^\pm} = \frac{1}{\sqrt{2}}
  \left( \kt{\pi^1} \pm \kt{\pi^2} \right),
  \qquad \kt{\pi^3} = \kt{\pi^0}.
\end{equation}
The quantities calculated in this section also give
rise to electroproduction observables, in which the
real photon is replaced by a virtual photon exchanged
between the electron and the nucleus:
\begin{equation}
  e(k_e) + X(p) \to e'(p_{e'}) + \pi^c(k') + X(p')
  \qquad\text{with}\quad k = p_e - p_{e'}\,.
\end{equation}
Here $k$ is the four-momentum of the virtual photon;
the kinematic consequences of $k^2\ne0$ are 
discussed in the following section.
\subsection{\texorpdfstring{Extraction of $S$-Wave
Multipoles at Threshold}{Extraction of S-Wave
Multipoles at Threshold}}
\label{sec:piphoto_extraction}
The framework for extracting one- and two-body pion
photoproduction amplitudes at threshold was
established by Beane
\etal~\cite{PionPhotoOrig,Beane_1997} for the
deuteron and subsequently extended to the trinucleon
systems by Lenkewitz
\etal~\cite{Lenke2011,Lenke2013} and to $\LiS$ by
Braun~\cite{BraunThesis}. The two-body kernel
derived for $\HT$ requires only a generalization of
the nuclear spin and active-nucleon isospin
dependence to be applicable within the TDA framework.
The present work considers primarily $S$-wave
contributions, which dominate at threshold; for the
full multipole expansion see
refs.~\cite{Perlstein,Bernard_1996,DDreschsel_1992}.
The following presentation closely follows the
formalism of Lenkewitz
\etal~\cite{Lenke2011,LenkeThesis}, adapted to the
TDA framework of sec.~\ref{sec:TDA}. The $S$-wave
amplitudes for neutral pion photoproduction are
extracted by matching the computed nuclear matrix
element to the standard decomposition in terms of
transverse and longitudinal multipoles. Defining, as
in sec.~\ref{sec:TDA},
\meqref{TDAExpansion}
\begin{equation}
  \begin{split}
  \calM&= 2i E_{0+} (\epsT \cdot \vec{J})
  + 2i L_{0+} ( \epsL\cdot \vec{J} )\\
       &= \langle M_J^{\prime}|\bigg[
  \binom{A}{1} \hat{O}_{1 \mathrm{N}}(\bv{k},
  \kvp)
  + \binom{A}{2} \hat{O}_{2 \mathrm{N}}(\bv{k},
  \kvp)
  \bigg]|M_J \rangle_\psi\;,
  \end{split}
\end{equation}
where $\vec{J}$ is the nucleus spin operator, and
$\epsT=\epslam-\left(\epslam \cdot
\hat{k}\right) \hat{k}$
and
$\epsL=\left(\epslam \cdot \hat{k}\right) \hat{k}$
are the transverse and longitudinal polarization
vectors, and $\epslam$ is the photon polarization. The
quantities $E_{0+}$ and $L_{0+}$ are the transverse
and longitudinal $S$-wave multipoles, respectively.
For real photons, only the transverse polarization is
physical, so the multipole $E_{0+}$ governs pion
photoproduction. The longitudinal multipole $L_{0+}$
contributes only when the photon is virtual, i.e.\ in
pion electroproduction; it is retained here for
generality.

At threshold the outgoing pion is at rest
($\kvp=\vec{0}$), so the only kinematic vector
available is the photon polarization
$\epslam$. To form a scalar matrix element, this vector must be combined with
another vector; the nuclear spin operator $\vec{J}$
provides that partner. The decomposition into $E_{0+}$
and $L_{0+}$ is therefore the most general
parametrization of the production amplitude at
threshold. The spin operator $\vec{J}$ arises from
this angular momentum structure rather than from the
kernel operator itself; in particular, $\vec{J}$ does
not enter in the convolution with the TDAs.

The unpolarized pion photoproduction cross section in
the center-of-mass frame is given by
\begin{equation}
  \frac{\mathrm{d}\sigma}
  {\mathrm{d}\Omega} = \frac{1}{64 \pi^2 s}
  \frac{1}{2(2J+1)}\frac{|\kvp|} {|\kv|}
  \sum_{\lambda=\pm1} \sum_{\Mj,\Mjp}
  \left| \calM_\lambda\right|^2\;,
  \label{GeneralCS}
\end{equation}
where $J$ is the total angular momentum of the target
nucleus, and the sum runs over initial photon
helicities and nuclear spin projections. Because
$|\vec{q}\,|\to 0$ at threshold, the differential
cross section of \meqref{GeneralCS} vanishes there. It
is therefore conventional to characterize the
threshold behavior by a generalized scattering
length $a_0$, defined for both pion photoproduction and electroproduction as~\cite{BERNARD_1995}
\begin{equation}
  a_0 = \lim_{q_\pi\to 0}
  \frac{|\kv|}{|\kvp|}
  \frac{\dd \sigma}{\dd \Omega}
  =\frac{4}{3} J(J+1) \left(|E_{0+}|^2
    - \varepsilon \frac{k^2}{k_{0}^2}
  |L_{0+}|^2 \right)\;.
  \label{Generala0}
\end{equation}
Here $k_{0}=(s-\Mnucl^2 +k^2)/2 \sqrt{s}$ is the CM
energy of the virtual photon, $s$ is the Mandelstam
variable, and $\varepsilon$ is the virtual photon
polarization parameter characterizing the degree of
transverse linear polarization, see ref.~\cite{BERNARD_1995} section 4.4 and ref.~\cite{LenkeThesis} appendix A for 
further details. $\varepsilon$ is given by
\begin{equation}
  \varepsilon = \left(1 + \frac{2|\vec{k}|^2}{-k^2} \tan^2\frac{\theta_e}{2}\right)^{-1},\quad \varepsilon \in [0,1]
\end{equation}
where $\theta_e$ is electron scattering angle in the \textit{lab} frame.
For pion electroproduction, the virtual photon four-momentum squared
$k^2$ may be inferred from the scattering angle of the
outgoing particles. For pion photoproduction the
photons are real and on-shell, so that $k^2=0$, giving
\begin{equation}
  a_0=\begin{cases}
    \,\;\;0& \quad\text{spin\;} 0 \quad   \HeF \\
    \,\;\;|E_{0+}|^2& \quad\text{spin\;}
      \frac{1}{2}\quad   \HeT,\HThree, p,n \\
    \,\frac{8}{3}|E_{0+}|^2& \quad\text{spin\;}
      1\quad  \LiS.\\
  \end{cases}
\end{equation}
Despite the nomenclature, $a_0$ is not a scattering
length in the sense of the effective range expansion.
It is proportional to the threshold cross section
with units $[\fm^2]$, rather than the typical units
$[\fm]$ of a true scattering length. The present work
adopts the definition of \meqref{Generala0} in
accordance with
refs.~\cite{Lenke2011,LenkeThesis,BraunThesis,BERNARD_1995}.
Future researchers are advised to pick better variable names.
This observable provides a direct test of \chiEFT
predictions and is sensitive to the interplay between
one-body and two-body contributions to the production
amplitude. The multipoles decompose into one-body
($1 \mathrm{N}$) and two-body ($2 \mathrm{N}$) parts,
\begin{equation}
\begin{split}
E_{0+} & =E_{0+}^{1 \mathrm{N}}
  +E_{0+}^{2 \mathrm{N}}, \\
L_{0+} & =L_{0+}^{1 \mathrm{N}}
  +L_{0+}^{2 \mathrm{N}} .
\end{split}
\label{EL_decomp}
\end{equation}
\subsubsection{One-body Form Factors}
\label{sec:piphoto_1N_thresh}
The one-body transition operator for pion photoproduction
on a nucleus with mass number $A$ is obtained by summing
the single-nucleon production amplitudes over all
nucleons, weighted by the appropriate isospin projections.
Following the treatment of Lenkewitz
\etal~\cite{Lenke2011}, the one-body matrix element takes the form
\begin{equation}
  \label{oneBodpiphoto}
  \begin{split}
 \left\langle M_J^{\prime}\right| \hat{O}_\mathrm{1 \mathrm{N}}\left|M_J\right\rangle_\psi 
&=i \epsT \cdot \vec{J}_{M_J^{\prime} M_J}\left(E_{0+}^{\pi^0 p} F_T^{S+V}+E_{0+}^{\pi^0 n} F_T^{S-V}\right)\\
&+i \epsL \cdot \vec{J}_{M_J^{\prime} M_J}\left(L_{0+}^{\pi^0 p} F_L^{S+V}+L_{0+}^{\pi^0 n} F_L^{S-V}\right)\;.
  \end{split}
\end{equation}

The factors $E_{0+}^{\pi^0 p}$, $E_{0+}^{\pi^0 n}$,
$L_{0+}^{\pi^0 p}$, and $L_{0+}^{\pi^0 n}$ are the
results for single-nucleon
multipoles. They are calculated here in \chiEFT and receive contributions
starting at $\calO(p^3)$;
at $\mathcal{O}(p^4)$ their values
are~\cite{bernard_1994,Bernard_1996}
\begin{equation}
\begin{split}
E_{0+}^{\pi^0 p} & =[-1.16 \pm 0.06] \times 10^{-3} / m_{\pi^{+}} \quad
E_{0+}^{\pi^0 n}  =[+2.13 \pm 0.11] \times 10^{-3} / m_{\pi^{+}} \\
L_{0+}^{\pi^0 p} & =[-1.35 \pm 0.07] \times 10^{-3} / m_{\pi^{+}} \quad
L_{0+}^{\pi^0 n} =[-2.41 \pm 0.12] \times 10^{-3} / m_{\pi^{+}}\;.
\end{split}
\label{ChiMultipoles}
\end{equation}
The uncertainties quoted above correspond to an
estimated $5\%$ truncation error on each multipole.
It is worth noting that the chiral expansion for
the proton multipole $E_{0+}^{\pi^0 p}$ converges
slowly: the $\calO(p^3)$ prediction differs
substantially from the $\calO(p^4)$ value quoted
above, owing to large one-loop corrections that
first enter at $\calO(p^3)$ and significant
counterterm contributions at
$\calO(p^4)$~\cite{BERNARD_1995,bernard_1994,Bernard_2001};
this motivates the $5\%$ uncertainty assignment.

At threshold, the $\No$ amplitudes are parameterized by
\begin{equation}
\begin{split}
& F_{T / L}^S\,
\vec{\epsilon}_{\mathrm{T} / \mathrm{L}} \cdot \vec{J}_{M_J^{\prime} M_J}=\frac{A}{2} \left\langle M_J^{\prime}\right| \vec{\epsilon}_{ \mathrm{T} / \mathrm{L}} \cdot \vec{\sigma}\left|M_J\right\rangle_\psi \\
& F_{T / L}^V \,\vec{\epsilon}_{\mathrm{T} / \mathrm{L}} \cdot \vec{J}_{M_J^{\prime} M_J}=\frac{A}{2} \left\langle M_J^{\prime}\right| \vec{\epsilon}_{ \mathrm{T} / \mathrm{L}} \cdot \vec{\sigma} \tau^z\left|M_J\right\rangle_\psi\;,
\end{split}
\end{equation}
where $F_{T / L}^{S \pm V} = F_{T / L}^S \pm F_{T / L}^V$
and where $A=\binom{A}{1}$ is the nucleon number, and
$\vec{\sigma}/2$ is the nucleon spin vector.
Inspection of \meqref{oneBodpiphoto} shows that the
combination $F^{S+V}_{T/L}$ multiplies the proton
amplitude and $F^{S-V}_{T/L}$ the neutron amplitude,
so that these form factors directly quantify the
contribution of each nucleon species to the one-body
multipole.
This may also be written in terms of the isoscalar
and isovector parts as
\begin{equation}
  \begin{split}
 \left\langle M_J^{\prime}\right| \hat{O}_\mathrm{1 \mathrm{N}}\left|M_J\right\rangle_\psi 
 &= \left\langle\Mjp\left| i\left(E_{0+}^{\pi^0 S}+\tau_i^z E_{0+}^{\pi^0 V}\right)\epsT \cdot \vec{\sigma}\right|\Mj\right\rangle_\psi\\
  &+\left\langle\Mjp\left|i \left( L_{0+}^{\pi^0 S}+\tau_i^z L_{0+}^{\pi^0 V}\right) \epsL \cdot \vec{\sigma}\right|\Mj\right\rangle_\psi\;.
  \end{split}
\end{equation}
Note that $\Mj$ and $\Mjp$ are the magnetic quantum
numbers of the nucleus, whereas the Pauli vector
$\vec{\sigma}$ acts on the spin indices $m_s,m_s'$ of the
active nucleon in the convolution with the transition
densities.
Likewise, the isoscalar and isovector single-nucleon multipoles are

\begin{equation}
\begin{split}
E_{0+}^{\pi^0 S} & =\frac{E_{0+}^{\pi^0 p}+E_{0+}^{\pi^0 n}}{2}\qquad L_{0+}^{\pi^0 S} =\frac{L_{0+}^{\pi^0 p}+L_{0+}^{\pi^0 n}}{2}\\
E_{0+}^{\pi^0 V} & =\frac{E_{0+}^{\pi^0 p}-E_{0+}^{\pi^0 n}}{2} \qquad L_{0+}^{\pi^0 V} =\frac{L_{0+}^{\pi^0 p}-L_{0+}^{\pi^0 n}}{2}\;.
\end{split}
\label{SVMultipoles}
\end{equation}
That is, $E_{0+}^{\pi^0 S}$ and $L_{0+}^{\pi^0 S}$
are the arithmetic means of the proton and neutron
amplitudes, while $E_{0+}^{\pi^0 V}$ and
$L_{0+}^{\pi^0 V}$ are their half-differences.
As in eq.~\eqref{TDAExpansion}, the subscript
$\psi$ denotes a summation over the internal nucleon
quantum numbers that arises in the convolution of the
kernel with the transition densities.
In the language of the TDA framework, the one-body matrix
element and kernel in operator form are given by
\begin{equation}
  \begin{split}
    \calM_{1\mathrm{N}}&=A\left\langle M_J^{\prime}\right| \hat{O}_\mathrm{1 \mathrm{N}}\left|M_J\right\rangle_\psi\\
                       =&iA K_{1\mathrm{N}}\, 
  \br{M_J'} 
E^{\pi^0 p}_{0+}\epsT \cdot(\vec{\sigma}+\vec{\sigma} \tau^z) 
  +E^{\pi^0 n}_{0+}\epsT(\vec{\sigma}-\vec{\sigma} \tau^z) \\
  &+L^{\pi^0 p}_{0+}\,\epsL\cdot(\vec{\sigma}+\vec{\sigma} \tau^z) 
  +L^{\pi^0 n}_{0+}\,\epsL\cdot(\vec{\sigma}-\vec{\sigma} \tau^z)
  \kt{M_J}_\psi\;.
  \end{split}
\end{equation}
The multipoles are then given by
\begin{equation}
\begin{aligned}
E_{0+}^{1 \mathrm{N}} & =\frac{K_{1 \mathrm{N}}}{2}\left(E_{0+}^{\pi^0 p} F_T^{S+V}+E_{0+}^{\pi^0 n} F_T^{S-V}\right) \\
L_{0+}^{1 \mathrm{N}} & =\frac{K_{1 \mathrm{N}}}{2}\left(L_{0+}^{\pi^0 p} F_L^{S+V}+L_{0+}^{\pi^0 n} F_L^{S-V}\right)\;,
\end{aligned}
\end{equation}
and $K_{1 \mathrm{N}}$ is a kinematic prefactor that
accounts for the difference in phase space between the
single-nucleon and nuclear systems.
It is given by~\cite{LenkeThesis}
\begin{equation}
  K_{1 \mathrm{N}}= \frac{m_N+m_\pi}{\Mnucl+m_\pi} \frac{\Mnucl}{m_N}\;,
\end{equation}
where $m_N$ is the nucleon mass and $\Mnucl$
is the nuclear mass. For the trinucleon systems considered
here, $K_{1\mathrm{N}} \approx 1.092$, and for $\LiS,\; K_{1 \mathrm{N}}\approx1.119$.

The $\chi$SMS potential is employed, as in Compton scattering (sec. \ref{sec:ComptonC}), with cutoffs of
$\LamNN=450~\MeV$ and $500~\MeV$, consistent with the
discussion in sec.~\ref{sec:SRG}. In some cases, the
parametrization of the three-nucleon interaction has also been
varied, subject to the availability of the corresponding
TDAs. Where present, these variations include small
changes to the low-energy constants $c_1,c_3,c_4$ in the
two-pion--one-nucleon sector of the interaction, together
with corresponding adjustments to the three-nucleon interaction
parameters $c_d$ and $c_e$. This procedure generates a set of
values $\{x_i\}$ from which the reported central value is
obtained as
$\overline{x}=\mathrm{mean}(\{x_i\})$, with the
potential-variation uncertainty given by
$\sigma_\mathrm{pot}=\frac{1}{2}
\left[\mathrm{max}(\{x_i\})
-\mathrm{min}(\{x_i\})\right]$.
A $3\%$ numerical uncertainty
$\sigma_\mathrm{num}=0.03\,|\overline{x}|$ is assigned
to account for the numerical integration over the
spectator-nucleon momenta and for the angular momentum
truncation in the creation of the TDAs, in accordance with the
convergence study in sec.~\ref{sec:InteConverge}.
These two sources of uncertainty are reported separately
throughout this section. For the form factors, the first
uncertainty quoted is $\sigma_\mathrm{pot}$ and the
second is $\sigma_\mathrm{num}$:
\begin{equation}
  \sigma_\mathrm{pot}=\tfrac{1}{2}
  \bigl[\max(\{x_i\})-\min(\{x_i\})\bigr]\;,
  \quad
  \sigma_\mathrm{num}=0.03\,|\overline{x}|\;.
  \label{tot_uncer}
\end{equation}
For the one-body multipole amplitudes
$E_{0+}^{1\mathrm{N}}$ and $L_{0+}^{1\mathrm{N}}$,
an additional source of uncertainty enters through
the $\calO(p^4)$ \chiEFT{} single-nucleon
amplitudes. Following the estimate of
Lenkewitz~\etal~\cite{LenkeThesis}, a $\sim 5\%$
uncertainty is assigned to the elementary multipoles
$E_{0+}^{\pi^0 p}$, $E_{0+}^{\pi^0 n}$,
$L_{0+}^{\pi^0 p}$, and $L_{0+}^{\pi^0 n}$.
Because the one-body multipoles are bilinear in the
elementary amplitudes and the form factors, the
multipole uncertainty from the elementary amplitudes is
obtained by evaluating the multipole at the corners of
the joint uncertainty region spanned by the elementary
amplitude variations, and taking the maximum deviation
from the central value.
For $E_{0+}^{1\mathrm{N}}$ and $L_{0+}^{1\mathrm{N}}$,
the two uncertainties quoted are: first, the combined
nuclear-structure uncertainty
$\sqrt{\sigma_\mathrm{pot}^2+\sigma_\mathrm{num}^2}$
(from the form factors), and second, the uncertainty
from the elementary single-nucleon amplitudes. This
separation permits the reader to assess independently
the contributions of the nuclear wave functions and of
the chiral single-nucleon input.
Tables~\ref{tab:1N_3H}--\ref{tab:1N_6Li} present the
one-body form factors and the corresponding $S$-wave
multipole amplitudes for $\HThree$, $\HeT$, and $\LiS$,
along with a comparison to the results of
Lenkewitz~\etal~\cite{Lenke2011,LenkeThesis}
and Braun~\cite{BraunThesis}.
\begin{table}[H]
\centering
{\setlength{\extrarowheight}{3pt}
\setlength{\tabcolsep}{4pt}
\small
\begin{tabular}{@{}|l||l|l|l||l|l|l|@{}}\hline
${}^3\mathrm{H}$ \rule[-1.1ex]{0pt}{2.8ex} & $F_T^{S+V}$ & $F_T^{S-V}$ & $E_{0+}^{1\mathrm{N}}$ & $F_L^{S+V}$ & $F_L^{S-V}$ & $L_{0+}^{1\mathrm{N}}$ \\
\noalign{\hrule height 0.15em}
TDA & $1.48(1)(4)$ & $-0.047(5)(1)$ & $-0.99(3)(5)$ & $1.48(1)(4)$ & $-0.035(5)(1)$ & $-1.04(3)(6)$ \\
\hline
Lenkewitz & $1.493(25)$ & $0.012(13)$ & $-0.93(3)(5)$ & $1.487(27)(8)$ & $-0.083(14)(8)$ & $-0.99(4)(5)$ \\
\hline
Braun & $1.551(78)$ & $0.039(2)$ & $-0.94(5)(5)$ & -- & -- & -- \\
\hline
\end{tabular}
}
\caption[One-body pion photoproduction results for ${}^3\mathrm{H}$]{One-body results for ${}^3\mathrm{H}$. Form factors $F_{T/L}$ are unitless. $E_{0+}^{1\mathrm{N}}$ and $L_{0+}^{1\mathrm{N}}$ in units of $[10^{-3}/m_{\pi^+}]$. For TDA form factors, the first (second) uncertainty is from the potential variation (numerical precision). For $E_{0+}^{1\mathrm{N}}$ and $L_{0+}^{1\mathrm{N}}$, the first (second) uncertainty is from the nuclear structure (elementary single-nucleon amplitudes).}
\label{tab:1N_3H}
\end{table}


\begin{table}[H]
\centering
{\setlength{\extrarowheight}{3pt}
\setlength{\tabcolsep}{4pt}
\small
\begin{tabular}{@{}|l||l|l|l||l|l|l|}\hline
${}^3\mathrm{He}$ \rule[-1.1ex]{0pt}{2.8ex} & $F_T^{S+V}$ & $F_T^{S-V}$ & $E_{0+}^{1\mathrm{N}}$ & $F_L^{S+V}$ & $F_L^{S-V}$ & $L_{0+}^{1\mathrm{N}}$ \\
\thickline{0.15em}
TDA & $-0.044(5)(1)$ & $1.47(1)(4)$ & $1.74(5)(9)$ & $-0.032(5)(1)$ & $1.47(1)(4)$ & $-1.92(6)(10)$ \\
\hline
Lenkewitz & $0.017(13)$ & $1.480(26)$ & $1.71(4)(9)$ & $-0.079(14)(8)$ & $1.479(26)(8)$ & $-1.89(4)(9)$ \\
\hline
Braun & $0.041(2)$ & $1.544(77)$ & $1.77(9)(9)$ & -- & -- & -- \\
\hline
\end{tabular}
}
\caption[One-body pion photoproduction results for ${}^3$He]{One-body results for ${}^3\mathrm{He}$. Form factors $F_{T/L}$ are unitless. $E_{0+}^{1\mathrm{N}}$ and $L_{0+}^{1\mathrm{N}}$ in units of $[10^{-3}/m_{\pi^+}]$. For TDA form factors, the first (second) uncertainty is from the potential variation (numerical precision). For $E_{0+}^{1\mathrm{N}}$ and $L_{0+}^{1\mathrm{N}}$, the first (second) uncertainty is from the nuclear structure (elementary single-nucleon amplitudes).}
\label{tab:1N_3He}
\end{table}

\begin{table}[H]
\centering
{\setlength{\extrarowheight}{3pt}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{|l||l|l|l||l|l|l|}\hline
${}^6\mathrm{Li}$ \rule[-1.1ex]{0pt}{2.8ex} & $F_T^{S+V}$ & $F_T^{S-V}$ & $E_{0+}^{1\mathrm{N}}$ & $F_L^{S+V}$ & $F_L^{S-V}$ & $L_{0+}^{1\mathrm{N}}$ \\
\thickline{0.15em}
TDA & $0.47(0)(1)$ & $0.47(0)(1)$ & $0.25(1)(4)$ & $0.47(0)(1)$ & $0.47(0)(1)$ & $-0.99(3)(5)$ \\
\hline
Braun & $0.476(24)$ & $0.479(24)$ & $0.26(3)(3)$ & -- & -- & -- \\
\hline
\end{tabular}
}
\caption[One-body pion photoproduction results for ${}^6$Li]{One-body results for ${}^6\mathrm{Li}$. Form factors $F_{T/L}$ are unitless. $E_{0+}^{1\mathrm{N}}$ and $L_{0+}^{1\mathrm{N}}$ in units of $[10^{-3}/m_{\pi^+}]$. For TDA form factors, the first (second) uncertainty is from the potential variation (numerical precision). For $E_{0+}^{1\mathrm{N}}$ and $L_{0+}^{1\mathrm{N}}$, the first (second) uncertainty is from the nuclear structure (elementary single-nucleon amplitudes).}
\label{tab:1N_6Li}
\end{table}

For $\LiS$, the approximate equality
$F_T^{S+V}\approx F_T^{S-V}\approx 0.47$ reflects
the near-symmetric proton-neutron structure of $\LiS$,
which has equal numbers of protons and neutrons ($Z=N=3$).
The small one-body multipole
$E_{0+}^{1\mathrm{N}}(\LiS)=0.25\times
10^{-3}/m_{\pi^+}$ arises because the product
$E_{0+}^{\pi^0 p} F_T^{S+V}$ is negative while
$E_{0+}^{\pi^0 n} F_T^{S-V}$ is positive, and the two
terms nearly cancel.
This cancellation is a direct consequence of the
opposing signs of the proton and neutron
single-nucleon multipoles combined with the
near-equality of the isoscalar and isovector form
factors. The smallness of the $\LiS$ one-body
amplitude is consistent with the cluster
decomposition $\LiS \approx \HeF + \HT$: since the
production amplitude for the spin-$0$ $\HeF$ core
vanishes at threshold, the one-body contribution to
$\LiS$ is governed primarily by the loosely bound
deuteron-like pair, and the resulting amplitude is
comparable in magnitude to that of the
deuteron~\cite{BraunThesis}.

The near-equality of the transverse and longitudinal
form factors, $F_T^{S\pm V}\approx F_L^{S\pm V}$,
visible in all three one-body tables, follows from
the Wigner--Eckart theorem: the one-body operator at
threshold is proportional to
$\vec{\epsilon}\cdot\vec{\sigma}$, a rank-1 spherical
tensor whose reduced matrix element is independent
of the polarization direction. At threshold
the equality $F_T^{S\pm V}= F_L^{S\pm V}$ is therefore
exact; any residual differences visible in the tables
are numerical artifacts of the momentum-space
integration. For the dominant form factors
($|F|\approx 1.5$), the transverse and longitudinal
values agree to better than $0.03\%$. For the
subdominant form factors ($|F|\lesssim 0.05$), which
arise from a near-complete cancellation between proton
and neutron contributions, the absolute T/L splitting
of $\sim 0.01$ is comparable in size to the form
factors themselves. This splitting provides an internal
consistency check: it reflects the true numerical
precision of these cancellation-sensitive quantities
and indicates that the assigned $3\%$ uncertainty,
while appropriate for the dominant form factors, 
underestimates the absolute numerical error for the
subdominant ones. The subdominant form factors
contribute negligibly to the physical observables
$E_{0+}^{1\mathrm{N}}$ and $L_{0+}^{1\mathrm{N}}$,
so this enhanced numerical noise does not affect the
reported multipole amplitudes.
At next chiral order, the so-called ``boost'' $\No$ corrections break this symmetry
with expansion parameter $Q\sim |\kv|/\Mnucl$, see ref.~\cite{LenkeThesis}.

The one-body form factors and multipole amplitudes
reported in Tables~\ref{tab:1N_3H}--\ref{tab:1N_6Li}
demonstrate that the TDA method yields results broadly
consistent with the literature across all three nuclei.
The dominant form factors
$F_{T/L}^{S\pm V}$ agree with
Lenkewitz~\etal~\cite{Lenke2011} at the few-percent
level. This agreement constitutes an independent
confirmation of the Lenkewitz results, obtained here with
a different numerical method and different nuclear
potentials. Since all three calculations employ the same
\chiEFT production operators at the same chiral order,
the spread of results across groups provides an
empirical estimate of the sensitivity to higher-order
corrections: the observed differences reflect the
residual dependence on the nuclear wave functions and
numerical methods, which enters at the level of the
neglected higher-order terms.

For the subdominant form factors, such as $F_T^{S+V}$
for $\HeT$ and $F_T^{S-V}$ for $\HThree$, the TDA and
Lenkewitz values differ in sign, placing them in clear
tension. These form factors arise from near-complete
cancellations between proton and neutron contributions,
rendering them sensitive to details of the wave
function that differ between the two calculations. The
discrepancies exceed the quoted uncertainties, which
capture only the parameter variation within each
calculation and not the systematic offset from the
choice of nuclear interaction.

Although the subdominant form factors are small in
magnitude, they are weighted by the larger of the two
elementary amplitudes in the expression for the
one-body multipole. For $\HThree$, the subdominant
$F_T^{S-V}$ is multiplied by
$E_{0+}^{\pi^0 n}=+2.13\times 10^{-3}/m_{\pi^+}$, so
that its discrepancy drives most of the offset in
$E_{0+}^{1\mathrm{N}}$ between the TDA and Lenkewitz
results. When both the nuclear-structure and
elementary-amplitude uncertainties are included, the
one-body multipole amplitudes $E_{0+}^{1\mathrm{N}}$
and $L_{0+}^{1\mathrm{N}}$ are consistent across
calculations; the $5\%$ uncertainty on the
single-nucleon amplitudes dominates the error budget
and absorbs the inter-calculation offsets.

The values utilized in this work for $E_{0+}^{\pi^0 p}$, $E_{0+}^{\pi^0 n}$,
$L_{0+}^{\pi^0 p}$, and $L_{0+}^{\pi^0 n}$ of \meqref{ChiMultipoles} can be considered as input parameters; their direct calculation is beyond
the scope of the present work. 
The form factors $F_{\mathrm{T}/\mathrm{L}}^{S\pm V}$ reported in
Tables~\ref{tab:1N_3H}--\ref{tab:1N_6Li} are independent
of the choice of single-nucleon multipoles; the one-body
amplitudes $E^{1\mathrm{N}}_{0+}$ and
$L^{1\mathrm{N}}_{0+}$ may therefore be reconstructed
from these form factors using any set of single-nucleon
multipole values, including potential future values calculated with greater accuracy.

\subsection{Threshold Two-Body Pion Photoproduction}
\label{sec:piphoto_2N}
\subsubsection{Leading Order Contributions}
The two-body contribution to the $S$-wave multipoles
$E_{0+}^{2\mathrm{N}}$ and $L_{0+}^{2\mathrm{N}}$ is
evaluated at threshold. At leading order in the chiral
expansion, $\calO(q^3)$, only two Feynman diagrams
contribute in Coulomb gauge, with all remaining diagrams
vanishing at
threshold~\cite{PionPhotoOrig,Beane_1997}. These diagrams
have been verified and are shown in figs.~\ref{DiagramA} and~\ref{DiagramB}.
\begin{figure}[H]
 \centering
 \includegraphics[scale=0.85]{Pphoto-2b-a.pdf}
 \caption[Leading-order two-body diagram $(a)$ for neutral pion photoproduction]{Leading order two-body diagram $(a)$ for neutral pion photoproduction}
 \label{DiagramA}
\end{figure}

\begin{figure}[H]
\centering
 \includegraphics[scale=0.8]{Pphoto-2b-b.pdf}
 \caption[Leading-order two-body diagram $(b)$ for neutral pion photoproduction]{Leading order two-body diagram $(b)$ for neutral pion photoproduction}
 \label{DiagramB}
\end{figure}
The following momentum definitions are used:
\begin{equation}
\begin{split}
  \qv&=\vec{p}-\pvp+(\vec{k}+\vec{k}^\prime)/2\\
  \qvp&=\vec{p}-\pvp+(\vec{k}-\vec{k}^\prime)/2\;.
\end{split}
\end{equation}
At threshold, $\kvp=0$.
The contribution of these diagrams to the scattering
matrix is given by
\begin{align}
E_{0+}^{2 \mathrm{N}} & =K_{2\mathrm{N}}\left(F_T^{(a)}-F_T^{(b)}\right) \\
L_{0+}^{2 \mathrm{N}} & =K_{2\mathrm{N}}\left(F_L^{(a)}-F_L^{(b)}\right)\;,
\end{align}
where $K_{2\mathrm{N}}$ is a kinematic prefactor given
by~\cite{LenkeThesis}. Analogous to $K_{1\mathrm{N}}$,
it accounts for the difference in phase space between the
single-nucleon and nuclear systems.

\begin{equation}
  K_{2\mathrm{N}}=\frac{\mpi e g_A \Mnucl }{16 \pi\left(\Mnucl+\mpi\right)(2 \pi)^3 f_\pi^3}\approx
\begin{cases}
&0.135\; \fm \times 10 ^{-3} /m_{\pi^+}\quad \text{for}\; \HeT, \HThree\\
&0.137\; \fm \times 10 ^{-3} /m_{\pi^+}\quad \text{for}\; \LiS\;,
\end{cases}
\end{equation}
where $e\approx0.3029$ is the electron charge,
$\Mnucl$ is the nuclear mass, $f_\pi=92.42 \MeV$, and $g_A=1.26$.
The quantities $F^{(a/b)}_{T/L}$ correspond to the
transverse and longitudinal contributions from diagrams
$a$ and $b$, respectively.
In the following discussion, the ${T}$ and
${L}$ indices are suppressed and the polarization is indicated by $\lambda$.
The two-body kernel is 
\begin{equation}
  \begin{split}
    \left\langle{M_J'}\right|\hat{O}^{\lambda}_{2 \mathrm{N}}\left|M_J\right\rangle_\psi&=
  \br{M_J'}K_{2\mathrm{N}}\,\left(\widehat{F}^{(a)}_{\lambda}-\widehat{F}^{(b)}_{\lambda}\right)\kt{M_J}_\psi\\
                                                                          &=\epslam \cdot \vec{J}_{M'_J,M_J}\; K_{2\mathrm{N}} \left(F^{(a)}_\lambda - F^{(b)}_\lambda\right)\;.
  \end{split}
  \label{2bdodpiphoto}
\end{equation}
For comparison to the literature, the negative sign in the
combination $F^{(a)}_\lambda - F^{(b)}_\lambda$ is
retained.
Eq.~\eqref{2bdodpiphoto} 
has utilized the following relation
\begin{equation}
  F^{(a/b)}_\lambda\; \epslam\cdot \vec{J}_{M'_J,M_J}=\br{M_J'} \hat{F}^{(a/b)}\ulam \kt{M_J}_\psi,
  \label{operdef}
\end{equation}
where on the left-hand side of eq.~\eqref{operdef}
$F^{(a/b)}\ulam$ is a scalar, whereas on the right-hand
side $\hat{F}^{(a/b)}\ulam$ is an operator.
Note that the combinatorial factor $\binom{A}{2}$ is
absorbed into the TDA convolution and is not included in
the form factor definitions; readers comparing directly
with Lenkewitz~\etal~\cite{Lenke2011} should account for
this difference for $A=3$.
The contribution from diagram $(a)$ is \cite{Lenke2011}
\begin{equation}
  \begin{split}
    F^{(a)}\ulam\epslam \cdot \vec{J}_{M'_J,M_J}&=
  \left\langle{\Mjp}\left|
    \ddfrac{ \epslam \cdot\left(\vec{\sigma}_1+\vec{\sigma}_2\right)\left(\vec{\tau}_1 \cdot \vec{\tau}_2-\tau_1^z \tau_2^z\right)}
  {2\vec{q}^{\, 2}}
\right|\Mj\right\rangle_\psi\\
                                                                       &=\br{\Mjp}\hat{F}^{a}\ulam\kt{\Mj}_\psi\;,
  \end{split}
\label{pp2b-a}
\end{equation}
and the contribution from diagram $(b)$ is \cite{Lenke2011}
\begin{equation}
  \begin{split}
  F^{(b)}\ulam \epslam \cdot \vec{J}_{M'_J,M_J}&=
  \left\langle{\Mjp}\left|
  \frac{\left(\vec{\tau}_1 \cdot \vec{\tau}_2-\tau_1^z \tau_2^z\right)\left[\left(\vec{q}^{\,\prime}-\vec{k}\right) \cdot\left(\vec{\sigma}_1+\vec{\sigma}_2\right)\right]\left[\epslam \cdot\left(\vec{q}^{\,\prime}-\vec{k} / 2\right)\right]}
  {\left[\left(\qpv-\vec{k}\right)^2+M_{\pi^{+}}^2\right] \vec{q}^{\,2}}
\right|\Mj\right\rangle_\psi\\
                                               &=\br{\Mjp}\hat{F}^{b}\ulam\kt{\Mj}_\psi\;,
\end{split}
\label{pp2b-b}
\end{equation}
where the above relations define the operator form of
the diagram $a$ and $b$ contributions $\hat{F}^{(a/b)}$.
Note that at threshold, $\vec{q}^{\,\prime} = \vec{q}$,
so that the polarization factor
in diagram $(b)$ reduces to
$\epslam \cdot (\vec{p} - \pvp)$.
\subsubsection{Treatment of the Removable Singularity}
\label{NumMethod}
Diagrams $(a)$ and $(b)$ contain a
removable singularity of the form
$1/\qvs$ from the pion propagator, where
$\vec{q}=\vec{p}-\pvp+\vec{k}/2$. It is integrable but must be handled with care to ensure
numerical stability in the convolution with the transition
densities. Its key feature is that it is
a \emph{moving} singularity: its position in the
integration domain depends on the relative Jacobi momenta
$\vec{p}_{12}$ and $\vec{p}_{12}^{\,\prime}$ as well as
the photon momentum $\vec{k}$. As one integrates over the
remaining momenta, the singular surface shifts
continuously, so that no fixed set of quadrature points
can avoid the singular region throughout the entire
integration domain. This renders the singularity
difficult to treat with standard quadrature methods. An advantage of the
TDA formalism is that the convolution with the transition
densities reduces the problem to two three-dimensional
integrations over $\vec{p}_{12}$ and
$\vec{p}_{12}^{\,\prime}$, with all remaining momentum
integrations already performed in the construction of the
densities. The moving singularity is therefore more
constrained than in a direct evaluation of the full
$A$-body matrix element, as the singular surface depends
only on $\vec{p}_{12}$,
$\vec{p}_{12}^{\,\prime}$, and $\vec{k}$.

Summation over quantum numbers may be factored out of the
integration; this detail is therefore suppressed in the
following discussion.
Let the momentum dependence in the numerator be given by
$f(\pv,\pvp)$ and note that
$\vec{q}=\vec{p}-\pvp+\vec{k}/2$.
The singularity can be removed by the following
variable substitution
\begin{equation}
  \begin{split}
  \int \dd^3 p\, \dd^3 p^\prime 
  \frac{ f(\pv,\pvp)}{
  \left(\vec{p}-\pvp+\vec{k}/2\right)^2
  }
  &=\int \dd^3 p \,\dd^3 q \ddfrac{ f(\pv,\pv-\qv+\kv/2) }{\qv\sq}\\
  &=\int \dd^3 p \int \dd q \,\dd\theta_q \,\dd\varphi_q \sin{\theta_q}\;
  f(\pv,\pv-\qv+\kv/2)\;,
  \end{split}
\end{equation}
where the transformation to spherical coordinates has been
employed, with the corresponding Jacobian
$\dd^3 x = r_x^2 \sin\theta_x \,\dd r_x \dd\theta_x \dd\varphi_x$
yielding a cancellation with the denominator.
A similar transformation was also adopted by Lenkewitz \cite{LenkeThesis}.
In principle, the function $f$ must be expressed in
spherical coordinates. In practice, however, the user provides the kernel in Cartesian coordinates. The subsequent conversion to spherical coordinates is handled internally by the code suite.
The angular integration of the kernel is performed using a
Lebedev-Laikov grid, while the radial integration employs
Gauss-Legendre quadrature; both methods are discussed in
sec.~\ref{sec:Inte}.
This approach is readily generalizable and is employed
also in the evaluation of the pion scattering kernel
in sec.~\ref{sec:pion}, where an analogous singularity
arises.

Several cross-checks have been performed to verify success of this procedure. The extracted form factors
are consistent across different combinations of initial
and final nuclear spin projections $M_J$, $M_J'$ and
photon polarizations $\lambda$, as required by rotational
invariance. Both tests provide strong evidence that the
variable substitution solves the present issue.
Prior to adopting this variable substitution, a number of
alternative approaches were investigated. An
$i\varepsilon$ prescription of the form
$\qvs \to \qvs+i \varepsilon$, for small $\varepsilon>0$ was attempted,
but this modification did not produce convergent values as
$\varepsilon\to 0$.
A rotation of the angular integration axis was explored
as well, with the aim of ensuring that no grid point
coincides with the singular surface; however, the results
proved sensitive to the rotation angle, with changes of
approximately $2^\circ$ in the angular grid orientation
producing variations of order $10\%$ in the final result.
This level of instability indicates that the quadrature
grid was not adequately resolving the integrand in the
vicinity of the singularity. None of these approaches
yielded reliable results; only the variable substitution
described above produced numerically stable form factors.
An alternative treatment of the same singularity was
employed by Braun~\cite{BraunThesis}, who introduced
a mass regulator $\Lambda$ and replaced the singular
propagator according to
\begin{equation}
  \frac{1}{\qvs}  \to \frac{1}{\qvs +\Lambda^2}.
\end{equation}
Observables are then calculated for a range of values of
$\Lambda$, and a fit is performed to extrapolate
$\Lambda \to 0$. The variable substitution employed in the
present work avoids this extrapolation entirely and
requires only a single evaluation of the integral,
thereby also eliminating the systematic uncertainties
associated with the extrapolation procedure.

The variable substitution used here to handle the
removable singularity could in principle also be applied
to Compton scattering at the pion production
threshold, where a similar propagator singularity arises.
Whether the same variable transformation suffices above threshold remains to be investigated.

Above threshold, in pion photoproduction the singularity
becomes more involved because the nonzero pion momentum
$|\vec{q}\,|>0$ modifies the singular surface. A suitable
variable substitution that removes the singularity may
exist but has not yet been identified; the difficulty is
compounded by the moving character of the singularity
in the multi-dimensional integration domain, as the
position of the singular surface depends simultaneously on
the integration variables and the nonzero outgoing pion
momentum. Nevertheless, the TDA framework offers a
structural advantage: the two-body kernel involves only
two relative momenta, $\vec{p}_{12}$ and
$\vec{p}_{12}^{\;\prime}$, so that the singularity must
be resolved in a two-dimensional integration rather than
in the $N$-dimensional space encountered in a general
$N$-body treatment. This observation applies equally to
the analogous singularity in pion and Compton scattering.
Identifying a suitable variable substitution in this
reduced space is therefore a tractable problem and is
left for future work.

The calculations presented in this work employ a radial
Gauss-Legendre grid with $n_1=14$ points in the first
region and $n_2=2$ in the second, a Lebedev-Laikov angular
grid of order $N=50$, and a maximum two-body angular
momentum of $j_{12\,\mathrm{max}}=1$ in the TDA
convolution. The selection of these parameters is
justified by the numerical convergence study presented in
sec.~\ref{sec:InteConverge} and Table~\ref{HeTConvTable}.
Increasing the integration grid to $n_1=16$, $n_2=4$,
$N=72$ changes the $\HeT$ form factors by $0.16\%$, while
increasing the angular momentum truncation to
$j_{12\,\mathrm{max}}=2$ changes the result by $0.33\%$.
Both variations are well below the theoretical
uncertainties from the truncation of the \chiEFT
expansion (see sec.~\ref{sec:truncation}), confirming that the numerical integration is
well converged. Similar patterns ($\leq 1 \%$ change) were found for $\LiS$. 
In accordance with the results of the convergence study in sec.~\ref{sec:InteConverge} $3\%$ numerical uncertainty is
assigned, see \meqref{tot_uncer}.

For the target $\LiS$, NCSM parameters $\omega_H$ and $\Ntot$ that control
the quality of the nuclear wave functions and transition
densities have been optimized in the Compton scattering
analysis of sec.~\ref{sec:ComptonC}, where an extensive
convergence study was performed as a function of
$\omega_H$, $\Ntot$, $\LamSRG$, and $\LamNN$. 

The present pion photoproduction calculations employ
the same density sets. For $\LiS$, the
potential-variation uncertainty $\sigma_\mathrm{pot}$
is obtained from $8$ density-set variants defined by
the combinations
$\Ntot = 14$;\;
$\LamNN = 450,\,500~\MeV$;\;
$\omega_H = 16,\,18~\MeV$;\;
$\LamSRG = 1.88,\,2.236~\fmin$,
as in the Compton scattering analysis of
sec.~\ref{sec:ComptonC},
with $j_{12\,\mathrm{max}} = 1$.
For the trinucleon systems $\HeT$ and $\HThree$, the
SRG transformation is not employed; the
potential-variation uncertainty is determined from
$2$ density sets corresponding to
$\LamNN = 450$ and $500~\MeV$.
A dedicated convergence study
for the pion photoproduction form factors as a
function of $\omega_H$ and $\Ntot$, analogous to that
presented for Compton scattering in
sec.~\ref{sec:ComptonC}, would further constrain the
NCSM truncation uncertainty but is not expected to
reveal qualitatively different behavior given the
comparable momentum scales involved.

\subsubsection[Static contributions]{$\calO(q^4)$
Static Contributions}
The $\calO(q^4)$ corrections to the two-body contribution
contain two parts: a so-called static contribution and a
recoil correction, each first described by Krebs
\etal~\cite{Krebs_2004}.
The recoil corrections are, within their error bars,
compatible with zero~\cite{LenkeThesis},
and are not considered here.
The static contributions give corrections to diagrams
$a/b$, which are written as
$\hat{O}_{12}^{(a/b)_i}$
and have been implemented in the TDA kernel for pion
photoproduction. In each two-body diagram, the
subscript $12$ denotes the assignment of roles: nucleon
$1$ absorbs the photon and emits the pion while
nucleon $2$ exchanges the mediating pion. The permuted
contribution $\hat{O}_{21}^{(a/b)_i}$, in which the
roles of the two nucleons are interchanged, must also
be included; this symmetrization is sometimes denoted
$+ (1 \leftrightarrow 2)$ in the literature. The total
contribution from each static diagram is therefore
\begin{equation}
  K_{2\mathrm{N}}^{(4)}\left( \hat{O}_{12}^{(j)} + \hat{O}_{21}^{(j)}\right) = K_{2\mathrm{N}}^{(4)}\; \hat{O}^{(j)}\;.
\end{equation}
The prefactor arises from phase space considerations and
normalization,
\begin{equation}
   K_{2\mathrm{N}}^{(4)} = K_{2\mathrm{N}}^{(3)} \left( \frac{-1}{4 m_N m_\pi}  \right).
\end{equation}
The $\calO(q^4)$ static corrections exhibit the same
removable $1/\qvs$ singularity as the leading-order
diagrams and are treated by the same variable
substitution described in sec.~\ref{NumMethod}.
The individual corrections to diagram $(a)$ from
fig.~\ref{DiagramA} are given
below:
\begin{equation}
\begin{split}
  \hat{O}^{a_1}_{12}&=(1-2g_A^2)\frac{
    \epslam \cdot
\vec{\sigma}_{1}
}{\qvs}(\vec{\tau}_1\cdot\vec{\tau}_2-\tau_1^z\tau_2^z)
\,\left(\qvs+2\vec{q}\cdot\vec{p}\,\right)~,\\
~
    \hat{O}^{a_2}_{12}&=\frac{2\;
      \epslam
      \cdot\left(
(\vec{q}+2\vec{p}_{12}^{\;\prime}-\vec{k})\,\vec{\sigma}_{1}\cdot\vec{q}
+i[\vec{q}\times\vec{k}](1+\kappa_V)\right)
}{\qvs}
(\vec{\tau}_1\cdot\vec{\tau}_2-\tau_1^z\tau_2^z)~,\\
~
        \hat{O}^{a_3}_{12}&=\frac{2\;
          \epslam \cdot\left(\vec{q}
+2\vec{p}_{12}^{\;\prime}-\vec{k}+i[\vec{\sigma}_1\times\vec{k}](1+\kappa_V)\right)
\vec{\sigma}_{2}\cdot\vec{q}
}{\qvs+M^2_{\pi^+}}
(\vec{\tau}_1\cdot\vec{\tau}_2-\tau_1^z\tau_2^z)~,\\
~
            \hat{O}^{a_4}_{12}&=2g_A^2\frac{
              \epslam
              \cdot
\left(-(\vec{q}+2\vec{p}_{12}^{\;\prime}-\vec{k})+i[\vec{\sigma}_1\times
(\vec{q}-\vec{k})]\right)\vec{\sigma}_{2}\cdot\vec{q}}{\qvs+M^2_{\pi^+}}
(\vec{\tau}_1\cdot\vec{\tau}_2-\tau_1^z\tau_2^z)~.
\end{split}
\end{equation}
The corrections to diagram $(b)$, from
fig.~\ref{DiagramB}, are
\begin{equation}
  \label{eq:T2Nb1}
  \hat{O}^{b_1}_{12} =-\left(1-2g_A^2\right)
  \frac{\vec{\sigma}_1 \cdot \vec{q}^{\,\prime}\;
  \epslam
\cdot(\vec{q}^{\,\prime}+\vec{q})}
  {
   \left( \qvps+M^2_{\pi^+}\right)
   \qvs
}
(\vec{\tau}_1\cdot\vec{\tau}_2-\tau_1^z\tau_2^z)\,
\left(\qvs+2\vec{q}\cdot\vec{p}^{\,\prime}\right).
\end{equation}



\begin{figure}[H]
\centering
%\includegraphics[width=\linewidth]{file_path}
\includegraphics[width=0.6\linewidth]{static5-eps-converted-to.pdf}
\caption[$\calO(q^4)$ static contributions to the two-body pion photoproduction kernel]{$\calO(q^4)$ static contributions to the
two-body pion photoproduction kernel. Figure from
ref.~\cite{Lenke2013}.}
\label{fig:StaticDiags}
\end{figure}

\subsubsection{Two-Body Threshold and Combined Results}
\label{sec:piphoto_2N_results}
The two-body contribution dominates the total pion
production amplitude at threshold, as first established
by Beane \etal~\cite{Beane_1997} for the deuteron. This
dominance arises because the leading one-body contact
interaction, the Kroll--Ruderman vertex \cite{KrollRuderman}, is proportional
to the charge of the produced pion and therefore vanishes
identically for neutral pion production, leaving the
two-body pion-exchange mechanisms as the primary
contribution at this chiral order.

Tables~\ref{tab:2N_3H}--\ref{tab:2N_6Li} present the
results for the two-body form factors
$F^a_T - F^b_T$ and $F^a_L - F^b_L$, along with the
corresponding multipole amplitudes
$E^{2\mathrm{N}}_{0+}$ and $L^{2\mathrm{N}}_{0+}$.
Results are shown at both $\calO(q^3)$ (leading order) and
$\calO(q^4)$ (including static corrections).
The uncertainty values presented in
Tables~\ref{tab:2N_3H}--\ref{tab:2N_6Li} follow the same
convention as in \meqref{tot_uncer}: for the TDA form factors,
the first uncertainty is the potential variation
$\sigma_\mathrm{pot}$ and the second is the numerical
uncertainty $\sigma_\mathrm{num}=0.03\,|\overline{x}|$.
For the two-body multipole amplitudes
$E_{0+}^{2\mathrm{N}}$ and $L_{0+}^{2\mathrm{N}}$,
which do not depend on the elementary single-nucleon
amplitudes, a single combined uncertainty
$\sqrt{\sigma_\mathrm{pot}^2+\sigma_\mathrm{num}^2}$
is reported.
\begin{table}[H]
\centering
{\setlength{\extrarowheight}{3pt}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{|l|l||l|l|l|l|}\hline
\multicolumn{2}{|c||}{\rule[-1.1ex]{0pt}{2.8ex}
  $\calO(q^4)$ correction}
  & $\Delta(F_T^{(a)}-F_T^{(b)})$
  & $\Delta(F_L^{(a)}-F_L^{(b)})$
  & $\Delta E_{0+}^{2\mathrm{N}}$
  & $\Delta L_{0+}^{2\mathrm{N}}$ \\
\thickline{0.15em}
\multirow{2}{*}{$\HThree$}
  & TDA  & $0.63(0)(1)$ & $-0.11(0)(0)$
  & $0.08(0)(0)$ & $-0.01(0)(0)$ \\
\cline{2-6}
  & Lenkewitz & $-0.15(5)(8)$ & $-0.49(4)(10)$
  & $-0.02(1)(1)$ & $-0.07(1)$ \\
\hline\hline
\multirow{2}{*}{$\HeT$}
  & TDA  & $0.61(0)(1)$ & $-0.11(0)(0)$
  & $0.08(0)(0)$ & $-0.01(0)(0)$ \\
\cline{2-6}
  & Lenkewitz & $-0.13(1)(7)$ & $-0.54(6)(11)$
  & $-0.02(1)$ & $-0.07(1)(1)$ \\
\hline\hline
\multirow{1}{*}{$\LiS$}
  & TDA  & $0.30(0)(0)$ & $0.01(0)(0)$
  & $0.04(0)(0)$ & $0.00(0)(0)$ \\
\hline
\end{tabular}
}
\caption[Shift from $\calO(q^3)$ to $\calO(q^4)$ in two-body photoproduction]{Shift from $\calO(q^3)$ to $\calO(q^4)$
in the two-body contributions due to the static
corrections. $\Delta(F_{T/L}^{(a)}-F_{T/L}^{(b)})$
in units of $[\fmin]$.
$\Delta E_{0+}^{2\mathrm{N}}$ and
$\Delta L_{0+}^{2\mathrm{N}}$ in units of
$[10^{-3}/m_{\pi^+}]$.
Where two uncertainties are
given, the first (second) is the potential-variation
(numerical) uncertainty. For the TDA
multipole amplitudes, the quoted uncertainty is the
combined numerical and potential-variation
contribution added in quadrature. The corrections are
uniformly small relative to the leading $\calO(q^3)$
values (Tables~\ref{tab:2N_3H}--\ref{tab:2N_6Li}),
confirming good convergence of the chiral expansion
for the two-body sector. Recoil corrections are
omitted.}
\label{tab:static_shift}
\end{table}
\begin{table}[H]
\centering
{\setlength{\extrarowheight}{3pt}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{|l|l||l|l|l|l|}\hline
\multicolumn{2}{|c||}{${}^3\mathrm{H}$ \rule[-1.1ex]{0pt}{2.8ex}} & $F_T^{(a)}-F_T^{(b)}$ & $F_L^{(a)}-F_L^{(b)}$ & $E_{0+}^{2\mathrm{N}}$ & $L_{0+}^{2\mathrm{N}}$ \\
\thickline{0.15em}
\multirow{3}{*}{$\mathcal{O}(q^3)$} & TDA Method & $-30.89(27)(93)$ & $-24.40(20)(73)$ & $-4.12(13)(0)$ & $-3.25(10)(0)$ \\
\cline{2-6}
 & Lenkewitz & $-29.7(3)$ & $-23.2(1)(1)$ & $-4.01(3)$ & $-3.13(1)$ \\
\cline{2-6}
 & Braun & $-27.2(33)$ & -- & $-3.55(43)$ & -- \\
\hline\hline
\multirow{2}{*}{$\mathcal{O}(q^4)$} & TDA Method & $-30.25(36)(91)$ & $-24.50(22)(74)$ & $-4.03(13)(0)$ & $-3.27(10)(0)$ \\
\cline{2-6}
 & Lenkewitz & $-29.8(3)(1)$ & $-23.69(11)(14)$ & $-4.030(32)(10)$ & $-3.20(1)(1)$ \\
\hline
\end{tabular}
}
\caption[Two-body pion photoproduction results for ${}^3$H]{Two-body results for ${}^3\mathrm{H}$. $F_{T/L}^{(a)}-F_{T/L}^{(b)}$ in units of $[\mathrm{fm}^{-1}]$. $E_{0+}^{2\mathrm{N}}$ and $L_{0+}^{2\mathrm{N}}$ in units of $[10^{-3}/m_{\pi^+}]$. $\mathcal{O}(q^4)$ results omit recoil contributions. For TDA form factors, the first (second) uncertainty is from the potential variation (numerical precision).}
\label{tab:2N_3H}
\end{table}

\begin{table}[H]
\centering
{\setlength{\extrarowheight}{3pt}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{|l|l||l|l|l|l|}\hline
\multicolumn{2}{|c||}{${}^3\mathrm{He}$ \rule[-1.1ex]{0pt}{2.8ex}} & $F_T^{(a)}-F_T^{(b)}$ & $F_L^{(a)}-F_L^{(b)}$ & $E_{0+}^{2\mathrm{N}}$ & $L_{0+}^{2\mathrm{N}}$ \\
\thickline{0.15em}
\multirow{3}{*}{$\mathcal{O}(q^3)$} & TDA Method & $-30.65(27)(92)$ & $-24.19(19)(73)$ & $-4.09(13)(0)$ & $-3.22(10)(0)$ \\
\cline{2-6}
 & Lenkewitz & $-29.3(3)$ & $-22.9(2)(1)$ & $-3.95(3)$ & $-3.09(2)$ \\
\cline{2-6}
 & Braun & $-27.1(33)$ & -- & $-3.53(42)$ & -- \\
\hline\hline
\multirow{2}{*}{$\mathcal{O}(q^4)$} & TDA Method & $-30.04(35)(90)$ & $-24.30(22)(73)$ & $-4.01(13)(0)$ & $-3.24(10)(0)$ \\
\cline{2-6}
 & Lenkewitz & $-29.4(3)(1)$ & $-23.44(21)(15)$ & $-3.97(3)(1)$ & $-3.160(22)(10)$ \\
\hline
\end{tabular}
}
\caption[Two-body pion photoproduction results for ${}^3$He]{Two-body results for ${}^3\mathrm{He}$. $F_{T/L}^{(a)}-F_{T/L}^{(b)}$ in units of $[\mathrm{fm}^{-1}]$. $E_{0+}^{2\mathrm{N}}$ and $L_{0+}^{2\mathrm{N}}$ in units of $[10^{-3}/m_{\pi^+}]$. $\mathcal{O}(q^4)$ results omit recoil contributions. For TDA form factors, the first (second) uncertainty is from the potential variation (numerical precision).}
\label{tab:2N_3He}
\end{table}

\begin{table}[H]
\centering
{\setlength{\extrarowheight}{3pt}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{|l|l||l|l|l|l|}\hline
\multicolumn{2}{|c||}{${}^6\mathrm{Li}$ \rule[-1.1ex]{0pt}{2.8ex}} & $F_T^{(a)}-F_T^{(b)}$ & $F_L^{(a)}-F_L^{(b)}$ & $E_{0+}^{2\mathrm{N}}$ & $L_{0+}^{2\mathrm{N}}$ \\
\thickline{0.15em}
\multirow{2}{*}{$\mathcal{O}(q^3)$} & TDA Method & $-16.84(9)(51)$ & $-13.11(6)(39)$ & $-2.30(7)(0)$ & $-1.79(5)(0)$ \\
\cline{2-6}
 & Braun$\times\sqrt{2}$ & $-16.1(20)$ & -- & $-2.15(25)$ & -- \\
\hline\hline
\multirow{1}{*}{$\mathcal{O}(q^4)$} & TDA Method & $-16.54(16)(50)$ & $-13.10(11)(39)$ & $-2.26(7)(0)$ & $-1.79(6)(0)$ \\
\hline
\end{tabular}
}
\caption[Two-body pion photoproduction results for ${}^6$Li]{Two-body results for ${}^6\mathrm{Li}$. $F_{T/L}^{(a)}-F_{T/L}^{(b)}$ in units of $[\mathrm{fm}^{-1}]$. $E_{0+}^{2\mathrm{N}}$ and $L_{0+}^{2\mathrm{N}}$ in units of $[10^{-3}/m_{\pi^+}]$. $\mathcal{O}(q^4)$ results omit recoil contributions. For TDA form factors, the first (second) uncertainty is from the potential variation (numerical precision). Values from Braun multiplied by $\sqrt{2}$ in accordance with discussion in sec.~\ref{ss:BraunSqrt2}.}
\label{tab:2N_6Li}
\end{table}

\begin{table}[H]
\centering
{\setlength{\extrarowheight}{3pt}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{|l|l||l|l|l|l|l|l|l|}\hline
\multicolumn{2}{|c||}{\rule[-1.1ex]{0pt}{2.8ex}} & $E_{0+}^{1\mathrm{N}}$ & $E_{0+}^{2\mathrm{N}}$ & $E_{0+}$ & $L_{0+}^{1\mathrm{N}}$ & $L_{0+}^{2\mathrm{N}}$ & $L_{0+}$ & $a_0\;(\gamma \pi^0)$ \\
\thickline{0.15em}
\multirow{3}{*}{${}^3\mathrm{H}$} & TDA & $-0.99$ & $-4.03$ & $-5.03(14)$ & $-1.04$ & $-3.27$ & $-4.31(12)$ & $25.25(143)$ \\
\cline{2-9}
 & Lenkewitz & $-0.93$ & $-4.03$ & $-4.96(7)$ & $-0.99$ & $-3.20$ & $-4.19(7)$ & $24.60(67)$ \\
\cline{2-9}
 & Braun & $-0.94$ & $-3.55$ & $-4.49(44)$ & -- & -- & -- & $20.16(391)$ \\
\hline\hline
\multirow{3}{*}{${}^3\mathrm{He}$} & TDA & $1.74$ & $-4.01$ & $-2.26(17)$ & $-1.92$ & $-3.24$ & $-5.16(15)$ & $5.12(74)$ \\
\cline{2-9}
 & Lenkewitz & $1.71$ & $-3.97$ & $-2.26(10)$ & $-1.89$ & $-3.16$ & $-5.05(10)$ & $5.11(47)$ \\
\cline{2-9}
 & Braun & $1.77$ & $-3.53$ & $-1.76(44)$ & -- & -- & -- & $3.10(154)$ \\
\hline\hline
\multirow{2}{*}{${}^6\mathrm{Li}$} & TDA & $0.25$ & $-2.26$ & $-2.00(8)$ & $-0.99$ & $-1.79$ & $-2.77(8)$ & $10.69(89)$ \\
\cline{2-9}
 & Braun* & $0.26$ & $-2.15$ & $-1.89(25)$ & -- & -- & -- & $9.52(260)$ \\
\hline
\end{tabular}
}
\caption[Summary of pion photoproduction results]{
Summary of photoproduction results. $E_{0+}$ and $L_{0+}$ in units of $[10^{-3}/m_{\pi^+}]$. $a_0$ in units of $[10^{-6}/m_{\pi^+}^2]$. $E_{0+} = E_{0+}^{1\mathrm{N}} + E_{0+}^{2\mathrm{N}}$, $L_{0+} = L_{0+}^{1\mathrm{N}} + L_{0+}^{2\mathrm{N}}$. All $1\mathrm{N}$ values at $\mathcal{O}(q^4)$. TDA and Lenkewitz $2\mathrm{N}$ results at $\mathcal{O}(q^4)$; Braun at $\mathcal{O}(q^3)$. ${}^*$The ${}^6\mathrm{Li}$ results of Braun have been multiplied by $\sqrt{2}$ to correct for the spin-1 matrix normalization error identified in sec.~\ref{ss:BraunSqrt2}. 
Uncertainties on $E_{0+}$, $L_{0+}$, and $a_0$ combine the one-body
and two-body uncertainties in quadrature;
See Tables~\ref{tab:1N_3H}--\ref{tab:2N_6Li} for uncertainty breakdowns.
}
\label{piphoto_summary}
\end{table}
Several features of these results merit discussion.
First, the two-body form factors for $\HeT$ and $\HThree$
are nearly identical in magnitude, differing only at the
sub-percent level. This near-equality reflects the isospin
structure of the two-body operators in
eqs.~\eqref{pp2b-a} and \eqref{pp2b-b}, which depend on
the combination
$(\vec{\tau}_1 \cdot \vec{\tau}_2 - \tau_1^z \tau_2^z)$.
Since $\HeT$ and $\HThree$ are isospin mirror nuclei,
they yield equivalent matrix elements up to small
isospin-breaking corrections.

Second, the $\LiS$ two-body form factors are
approximately half the magnitude of the $A=3$ results.
This reduction can be understood from the dominant
$\alpha + d$ cluster structure of $\LiS$, in which the
tightly bound $\HeF$ core contributes negligibly to pion
production. The $\HeF$ nucleus has $J^\pi = 0^+$ and thus
yields vanishing matrix elements of the spin-dependent
production operator. The active contribution arises
primarily from the deuteron-like $pn$ pair, which accounts
for the observed similarity between the $\LiS$ and $\HT$
production amplitudes, a correspondence also noted by
Braun~\cite{BraunThesis}.

\subsubsection{Combined Results and Sensitivity}
\label{sec:piphoto_combined}
Turning to the total amplitude
$E_{0+} = E_{0+}^{1\mathrm{N}} +
E_{0+}^{2\mathrm{N}}$, the two-body piece dominates
for all nuclei considered. For $\HThree$, both
$E_{0+}^{1\mathrm{N}} = -0.99$ and
$E_{0+}^{2\mathrm{N}} = -4.03$ are negative, so that the
total amplitude is the largest in magnitude
($E_{0+} = -5.03$). For $\HeT$, the positive one-body
contribution ($E_{0+}^{1\mathrm{N}} = +1.74$) partially
offsets the negative two-body contribution
($E_{0+}^{2\mathrm{N}} = -4.01$), yielding a reduced
total ($E_{0+} = -2.26$). The ratio of two-body to
one-body contributions is approximately $4{:}1$ for
$\HThree$ and $2.3{:}1$ for $\HeT$, confirming that the
two-body mechanism is dominant in both cases. For $\LiS$,
the ratio is approximately $9{:}1$, reflecting the
suppression of the one-body contribution in this
nucleus, as anticipated from the near-cancellation
between proton and neutron one-body amplitudes
already observed in Compton scattering
(sec.~\ref{sec:ComptonC}). These ratios are comparable
to the two-body to one-body ratios found in Compton
scattering at similar momentum transfer, where the
two-body contributions likewise dominate for all
nuclei considered.
The combined uncertainties on the threshold scattering
length $a_0$ (Table~\ref{piphoto_summary}) average
approximately $9\%$ across the three nuclei, with the
$\HeT$ uncertainty being the largest ($\sim 14\%$) due
to the partial cancellation between one-body and
two-body contributions that suppresses the central value.

The partial cancellation in $\HeT$ renders it
particularly sensitive to the input values of the
elementary neutron multipole and thus provides an
opportunity to extract neutron multipoles, which
cannot be measured from free neutrons. This
selectivity arises because the $\HeT$ wave function is
dominated by its principal $s$-state component in
which the $(pp)$ pair contributes total spin-$0$, so
that the nuclear spin is carried predominantly by the
unpaired neutron. The same $np$-pair structure was
exploited in the context of $\HeT$ Compton scattering
(sec.~\ref{sec:ComptonC}), where it renders $\HeT$
an effective neutron target for the extraction of
neutron polarizabilities. The importance of two-body
contributions at threshold, though most dramatic here
due to the vanishing of the
Kroll--Ruderman vertex~\cite{KrollRuderman}, is a
recurring theme in nuclear reactions computed within
the TDA framework; in Compton scattering, the
two-body contributions likewise provide significant
corrections that must be included for a quantitative
description.
\subsubsection{Comparison with Experiment}
\label{sec:piphoto_exp_comparison}
A direct comparison with experiment is possible for $\LiS$. The
threshold $\LiS(\gamma,\pi^0)$ cross section was measured at SAL by
Bergstrom \etal~\cite{Bergstrom1999}, who extracted a threshold
dipole amplitude
$E_{0+}^{\mathrm{exp}}(\LiS)=(-1.63\pm0.12)\times10^{-3}/m_{\pi^+}$.
The present result,
$E_{0+}(\LiS)=(-2.00\pm0.08)\times10^{-3}/m_{\pi^+}$
(Table~\ref{piphoto_summary}), exceeds the measured magnitude by
approximately $23\%$. Adding the theoretical and experimental
uncertainties linearly (the more conservative convention) shows that the two differ at the $1.8\sigma$ level.

This level of agreement mirrors that found in the deuteron channel.
The \chiEFT prediction for the deuteron threshold amplitude,
$E_d=(-1.8\pm0.2)\times10^{-3}/m_{\pi^+}$ at
$\calO(q^4)$~\cite{Beane_1997}, exceeds the SAL measurement
$E_d^{\mathrm{exp}}=(-1.45\pm0.09)\times10^{-3}/m_{\pi^+}$
\cite{Bergstrom1998} by approximately $24\%$. The
theory-to-experiment ratio is therefore nearly identical in the two
systems: $1.24$ for the deuteron and $1.23$ for $\LiS$. That the
same fractional offset appears at $A=2$ and $A=6$ suggests that the
discrepancy is governed by the elementary single-nucleon input and
by the one-body boost corrections omitted here
(sec.~\ref{sec:piphoto_convergence}), rather than by a
target-dependent failure of the few-nucleon description.
The significance of this correspondence is best appreciated in its
historical context. The deuteron amplitude furnished one of the
earliest quantitative validations of the chiral two-body mechanism
in neutral pion photoproduction. The counterintuitive ordering
$|E_{0+}^{\pi^0 n}| > |E_{0+}^{\pi^0 p}|$ originates in the
$\calO(q^3)$ pion-loop (pion-cloud) contribution~\cite{bernard_1994,
Bernard_2001}, a quantum effect absent from the phenomenological
production models in use at the time. Setting the neutron multipole
to zero, as those models effectively did, yields
$E_d \approx -2.6\times10^{-3}/m_{\pi^+}$ and a threshold cross
section roughly twice the \chiEFT value~\cite{Beane_1997}; the
subsequent SAL measurement confirmed the chiral prediction and
excluded the model expectation. That the present $\LiS$ result
reproduces the deuteron offset to within one percent therefore
extends this validation of the chiral two-body dynamics from the
$A=2$ system to a $p$-shell nucleus, with the same normalization
factor relating theory and data in both targets.


A caveat applies to the comparison: the value extracted by
Bergstrom \etal\ includes pion final-state distortion through the
DWIA factor $R_d=1.09$, whereas the present calculation contains no
such distortion. The comparison above therefore uses the physical
(distorted) amplitude, consistent with the treatment of the
deuteron channel. The distortion-removed equivalent,
$E_{0+}^{\mathrm{exp}}/\sqrt{R_d}
=(-1.56\pm0.11)\times10^{-3}/m_{\pi^+}$, would widen the deviation
to approximately $2.3\sigma$.

\subsubsection{Comparison with Lenkewitz and Braun}
\label{ss:BraunSqrt2}
The comparison with Braun reveals a systematic
discrepancy for $\LiS$. While the present $\HeT$ and
$\HThree$ two-body form factors differ from those of
Braun by approximately $13\%$, consistent within the
combined uncertainties at the $1.1\sigma$ level owing
to Braun's larger error bars, the $\LiS$ results
differ by a factor of approximately $\sqrt{2}$.
Specifically:
\begin{equation}
  \frac{(F^a_T - F^b_T)_{\text{TDA}}}
  {(F^a_T - F^b_T)_{\text{Braun}}}
  \approx \frac{-16.84}{-11.4}
  \approx 1.48 \approx \sqrt{2}\;.
\end{equation}
This discrepancy originates from an error in the
normalization of the spin-1 matrices used by Braun to
calculate the form factors. The pion production
amplitude is extracted by matching the computed matrix
element to the form
$\vec{\epsilon}_{\lambda,T} \cdot \vec{J}$, where
$\vec{J}$ denotes the nuclear spin operator. For
spin-$1/2$ systems, $\vec{J} = \vec{\sigma}/2$. For
spin-1 systems such as $\LiS$ and $\HT$, the standard
angular momentum matrices take the form used in the
present TDA approach

\begin{equation}
  S_x = \frac{1}{\sqrt{2}}
  \begin{pmatrix} 0 & 1 & 0 \\
  1 & 0 & 1 \\
  0 & 1 & 0 \end{pmatrix},
  \quad
  S_y = \frac{1}{\sqrt{2}}
  \begin{pmatrix} 0 & -i & 0 \\
  i & 0 & -i \\
  0 & i & 0 \end{pmatrix},
  \quad
  S_z = \begin{pmatrix} 1 & 0 & 0 \\
  0 & 0 & 0 \\
  0 & 0 & -1 \end{pmatrix}\;.
\end{equation}
The factors of $1/\sqrt{2}$ appearing in $S_x$ and $S_y$
arise from the angular momentum ladder operator relations
$\langle J, M_J \pm 1 | J_\pm | J, M_J
\rangle = \sqrt{(J \mp M_J)(J \pm M_J + 1)}$,
which for $J=1$ yields $\sqrt{2}$.

If these $1/\sqrt{2}$ factors are omitted in the spin
matrices used to extract the form factors, the matrix
elements of $(\vec{\epsilon} \cdot \vec{J})$ are
larger by a factor of $\sqrt{2}$, causing the extracted
form factors $F$ to be smaller by the same factor. This is
precisely the pattern observed: the $\LiS$ form factors
reported by Braun are smaller than those of the present
work by approximately $\sqrt{2}$, while the spin-$1/2$
results exhibit only the $\sim 13\%$ systematic offset
attributable to differences in wave functions. The
discrepancy is therefore not a matter of differing
conventions but an error in the spin-1 matrix
normalization employed by Braun~\cite{BraunThesis}. 

Once the Braun results are corrected, as indicated in Table~\ref{tab:2N_6Li},
the $\LiS$ form factors agree to within $0.4\sigma$,
or approximately $5\%$, consistent with the
$\sim 13\%$ offset observed for the trinucleon systems
and attributable to the different nuclear wave
functions employed.

\subsubsection{Order-by-Order Convergence}
\label{sec:piphoto_convergence}
The convergence of the chiral expansion can be
assessed by comparing the results at successive
chiral orders for each contribution separately and
for the total amplitude.
For the one-body contribution, the values reported in
Tables~\ref{tab:1N_3H} to~\ref{tab:1N_6Li} are
evaluated using the $\calO(p^4)$ single-nucleon
multipoles of Bernard
\etal~\cite{bernard_1994,Bernard_2001}. Next leading
order ($\mathrm{NLO}$) corrections to the $\No$
contribution arise from boost effects, which account
for the relative motion of the struck nucleon with
respect to the nuclear center of mass. Boost
corrections are not included in the present results
but they were computed by Lenkewitz
\etal~\cite{LenkeThesis,Lenke2013}. For the
trinucleon systems, Lenkewitz found boost corrections
to be modest: the effect on $E_{0+}$ amounts to
$13\%$ and $38\%$ of the leading $\No$ value for
$\HeT$ and $\HThree$, respectively, while the
$L_{0+}$ corrections are negligible, at $0\%$ and
$2\%$. However, the $\No$ contribution is
substantially smaller than the dominant $\Nt$ sector
for all nuclei considered here, so even the $38\%$
shift of $E^{\No}_{0+}$ for $\HThree$ translates to
a correction of only $\sim 7\%$ of the total $E_{0+}$
amplitude, and $\sim 9\%$ for $\HeT$. The effect on
$L_{0+}$ is smaller still. A comparable relative
shift is expected in the present calculation, since
the boost corrections depend primarily on the nuclear
kinematics rather than on the choice of potential.
These shifts represent the leading omission in the
one-body sector; the remaining sources of uncertainty,
in particular the numerical convergence of the TDA
convolution and the absence of explicit three-nucleon
contributions to the production operator, are expected
to be at least as significant as the chiral
order-by-order convergence of the one-body kernel for
the overall error budget.

For the two-body contribution, the $\calO(q^4)$
static corrections produce small shifts relative to
the leading $\calO(q^3)$ values in all cases, as
summarized in Table~\ref{tab:static_shift}. In the
transverse channel, the shift from $\calO(q^3)$ to
$\calO(q^4)$ is uniformly approximately $2\%$ across
all three nuclei: $E_{0+}^{2\mathrm{N}}$ shifts from
$-4.12$ to $-4.03$ for $\HThree$, from $-4.09$ to
$-4.01$ for $\HeT$, and from $-2.30$ to $-2.26$ for
$\LiS$ (all in units of $10^{-3}/m_{\pi^+}$). In the
longitudinal channel, the corrections are smaller
still, at or below the $1\%$ level, while the $\LiS$
longitudinal multipole is unchanged within the quoted
precision. This pattern is consistent with the
findings of Lenkewitz
\etal~\cite{LenkeThesis}, who observed that the
$\calO(q^4)$ static and recoil corrections to the
longitudinal amplitude nearly cancel. The naive
expectation for the relative size of the $\calO(q^4)$
correction to the leading $\calO(q^3)$ two-body
contribution is $Q \sim \mpi/\Lambda_\chi$, which for
a breakdown scale $\Lambda_\chi \sim 600~\MeV$ gives
$Q \approx 0.23$. The observed $\sim 2\%$ transverse
shift is well below this estimate, a suppression
attributable to the partial cancellation between the
static and recoil contributions identified by
Lenkewitz \etal~\cite{LenkeThesis}. The two-body
contribution is therefore well described at leading
order, with the $\calO(q^4)$ corrections representing
a perturbation smaller than the uncertainties
introduced by variation in $\LamNN$, $\LamSRG$, and
$\omega_H$.

As shown in Table~\ref{tab:static_shift}, the sign of
the static correction to the transverse form factors
differs between the present work and Lenkewitz
\etal~\cite{LenkeThesis}. This is not unexpected: the
$\calO(q^4)$ static contribution is a sum of five
diagram topologies (fig.~\ref{fig:StaticDiags}) with
individually larger but partially canceling
contributions. The sign of the small residual is
sensitive to the nuclear wave function, so that
different potential models can yield corrections of
opposite sign. In both calculations, the magnitude of
the correction is at or below the $2\%$ level,
confirming that the two-body amplitude is well
described at leading order.

\subsection{One-Body Pion-Photoproduction Above Threshold}
\label{sec:piphoto_above}
This section uses momentum labeling consistent with the single-nucleon pion and electroproduction
literature, rather than the labeling used elsewhere in the TDA framework. In particular, the outgoing 
pion momentum is now labeled $q$.
The one-body contribution to pion photoproduction can be
calculated from Feynman diagrams, but above threshold
this approach becomes increasingly involved. The
proximity of the $\Delta(1232)$ resonance necessitates
the inclusion of many partial waves and higher-order terms
to achieve even moderate precision~\cite{rij}.
An alternative approach is to employ a phenomenological
reconstruction. As pioneered by Chew
\etal~\cite{Chew}, the $\gamma N\to\pi N$ amplitude is
expanded in partial waves, and the multipole amplitudes
$E_{l\pm}$ and $M_{l\pm}$ are fitted to data. The present
work uses the fits provided by the SAID partial-wave
analysis facility at George Washington
University~\cite{SAID2012piphoto,SAID2023piphoto}.
The Mandelstam variables (expressed in
terms of four-vectors) are
\begin{equation}
  s=(p+k)^2=\left(p^{\prime}+q\right)^2,
  \quad t=\left(p-p^{\prime}\right)^2
  =(k-q)^2,
  \quad u=(p-q)^2
  =\left(k-p^{\prime}\right)^2\,.
\end{equation}
For pion photoproduction on the nucleon in the center-of-mass frame, the photon energy
$\omega$ and pion energy $E_\pi$ are
\begin{equation}
  \omega=\frac{s-m_N^2}{2 \sqrt{s}},
  \quad E_\pi=\frac{s+m_\pi^2-m_N^2}
  {2 \sqrt{s}}\,,
\end{equation}
where $m_N$ is the nucleon mass; in practice, the average of the proton and neutron masses is employed.
When generalizing to the TDA framework, of course the mass of the nucleus is employed in kinematics 
rather than that of the nucleon. The relationship between the scattering angle $\theta$
and the Mandelstam variable $t$ is
\begin{equation}
  t=m_\pi^2-2\left(\omega E_\pi
  -|\vec{k}||\vec{q}\,|
  \cos (\theta)\right)\,.
\end{equation}
As noted above, the present implementation of the TDA
method is restricted to coherent reactions preserving the
nuclear ground state,
i.e.\ $ \gamma + X \to  \pi^0 + X$; charged pion channels,
which involve nuclear charge exchange, are not yet
accessible.
The four physical reaction channels may be reconstructed from the following multipole decomposition. They are given by
\begin{equation}
  \gamma p \rightarrow \pi^0 p,
  \quad \gamma p \rightarrow \pi^{+} n,
  \quad \gamma n \rightarrow \pi^0 n,
  \quad \gamma n \rightarrow \pi^{-} p\,.
  \label{eq:piphoto_channels}
\end{equation}
In isospin space, the matrix elements are
conventionally parameterized
by~\cite{Chew,BERNARD_1995}
\begin{equation}
  T_{\gamma N \rightarrow \pi N}^c
  =\delta_{c 3} T_{\gamma N}^{(+)}
  +\tau_c T_{\gamma N}^{(0)}
  +\mathrm{i} \varepsilon_{c 3 a}
  \tau_a T_{\gamma N}^{(-)}\,,
\end{equation}
where $c$ is the isospin of the outgoing pion and
$\varepsilon$ is the Levi-Civita tensor. The three
amplitudes correspond to isospin change
$\Delta I = 0,\,1,\,2$, respectively:
$T_{\gamma N}^{(+)}$ is the isoscalar (iso-singlet)
amplitude, $T_{\gamma N}^{(0)}$ is the isovector
amplitude, and $T_{\gamma N}^{(-)}$ is the
isotensor amplitude. The superscript convention
$(+,\,0,\,-)$ is standard in the pion photoproduction
literature but does not directly reflect the isospin
transfer; the correspondence
$T^{(+)} \leftrightarrow \Delta I = 0$,\;
$T^{(0)} \leftrightarrow \Delta I = 1$,\;
$T^{(-)} \leftrightarrow \Delta I = 2$
should be kept in mind.
Writing this out explicitly for the four physical
channels yields
\begin{equation}
  \begin{array}{ll}
T_{\gamma p \rightarrow \pi^0 p}
=T_{\gamma N}^{(+)}+T_{\gamma N}^{(0)},
&\qquad T_{\gamma p \rightarrow \pi^{+} n}
=\sqrt{2}\left(T_{\gamma N}^{(0)}
+T_{\gamma N}^{(-)}\right) \\
T_{\gamma n \rightarrow \pi^0 n}
=T_{\gamma N}^{(+)}-T_{\gamma N}^{(0)},
&\qquad T_{\gamma n \rightarrow \pi^{-} p}
=\sqrt{2}\left(T_{\gamma N}^{(0)}
-T_{\gamma N}^{(-)}\right)\,.
\end{array}
\end{equation}
These are further decomposed into isospin-$3/2$,
proton isospin-$1/2$, and neutron isospin-$1/2$
amplitudes. The isospin-$3/2$ amplitude is common to
proton and neutron targets and is dominated by the
$\Delta(1232)$ resonance, while the isospin-$1/2$
amplitudes encode the non-resonant background and
differ for proton and neutron:
\begin{equation}
  \begin{aligned}
T_{\gamma N}^{\left(\frac{3}{2}\right)}
& =T_{\gamma p}^{\left(\frac{3}{2}
\right)}=T_{\gamma n}^{\left(
\frac{3}{2}\right)}
=T_{\gamma N}^{(+)}-T_{\gamma N}^{(-)}\\
T_{\gamma p}^{\left(\frac{1}{2}\right)}
& =T_{\gamma N}^{(0)}
+\frac{1}{3} T_{\gamma N}^{(+)}
+\frac{2}{3} T_{\gamma N}^{(-)},
\quad T_{\gamma n}^{\left(\frac{1}{2}
\right)}=T_{\gamma N}^{(0)}
-\frac{1}{3} T_{\gamma N}^{(+)}
-\frac{2}{3} T_{\gamma N}^{(-)}\,.
\end{aligned}
\end{equation}
Solving for the physical reaction channels
in terms of the isospin amplitudes yields
\begin{equation}
\begin{split}
  &T_{\gamma p \to \pi^0 p}
  = T_{\gamma p}^{\left(\frac{1}{2}
  \right)} + \frac{2}{3}
  T_{\gamma N}^{\left(\frac{3}{2}
  \right)}\qquad\qquad\;\;
  T_{\gamma n \to \pi^0 n}
  = -T_{\gamma n}^{\left(\frac{1}{2}
  \right)} + \frac{2}{3}
  T_{\gamma N}^{\left(\frac{3}{2}
  \right)}\\
  &T_{\gamma p \to \pi^+ n}
  =\sqrt{2}\left(
  T_{\gamma p}^{\left(\frac{1}{2}
  \right)} - \frac{1}{3}
  T_{\gamma N}^{\left(\frac{3}{2}
  \right)}\right)\quad
  T_{\gamma n \to \pi^- p}
  = \sqrt{2}\left(
  T_{\gamma n}^{\left(\frac{1}{2}
  \right)} + \frac{1}{3}
  T_{\gamma N}^{\left(\frac{3}{2}
  \right)}\right)\,.
\end{split}
\label{Channels}
\end{equation}
In practice, the multipole amplitudes corresponding to
$\gamma p$, $\gamma n$, and $\gamma N$ channels are
tabulated in the SAID database.
In the CM frame with real photons
($k^2=0$) and the gauge choice
$\epsilon^0=0$,
the amplitude $\mathcal{F}$ can be
expressed in terms of the Chew,
Goldberger, Low, and Nambu (CGLN)
amplitudes~\cite{Chew}.
For a given isospin channel $I$, the CGLN decomposition
reads

\begin{equation}
  \mathcal{F}_I =\mathrm{i} \vec{\sigma}
  \cdot \vec{\epsilon}\, \mathcal{F}_1
  +\frac{(\vec{\sigma} \cdot \vec{q})\,
    \vec{\sigma} \cdot(\vec{k}
  \times \vec{\epsilon})}
  {|\vec{q}\,||\vec{k}|} \mathcal{F}_2
  +i \frac{(\vec{\sigma}
  \cdot \vec{k})\,( \vec{q}
  \cdot \vec{\epsilon}\,)}
  {|\vec{q}\,||\vec{k}|} \mathcal{F}_3
  +i \frac{(\vec{\sigma}
  \cdot \vec{q}\,)\,(\vec{q}
  \cdot \vec{\epsilon})}
  {|\vec{q}\,|^2} \mathcal{F}_4\,.
  \label{CGLN}
\end{equation}
The functions $\mathcal{F}_j$ are given
by~\cite{Chew, Ball}

\begin{equation}
  \begin{split}
\mathcal{F}_1 & =\sum_{l=0}^{\infty} \left\{\left[l M_{l+}+E_{l+}\right] P_{l+1}^{\prime}(x) +\left[(l+1) M_{l-}+E_{l-}\right] P_{l-1}^{\prime}(x)\right\}, \\
\mathcal{F}_2 & =\sum_{l=1}^{\infty} \left[(l+1) M_{l+} +l M_{l-}\right] P_l^{\prime}(x), \\
\mathcal{F}_3 & =\sum_{l=1}^{\infty} \left\{\left[E_{l+}-M_{l+}\right] P_{l+1}^{\prime \prime}(x) +\left[E_{l-}+M_{l-}\right] P_{l-1}^{\prime \prime}(x)\right\},\\
\mathcal{F}_4 & =\sum_{l=2}^{\infty} \left[ M_{l+} - E_{l+} - M_{l-}-E_{l-} \right] P_l^{\prime \prime}(x)\,,
\end{split}
\label{AmpList}
\end{equation}
where the isospin index $I$ has been suppressed,
$x=\cos\theta$, $P_l(x)$ denotes the Legendre
polynomials, and $P_l'(x)$, $P_l''(x)$ denote their
first and second derivatives with respect to $x$.
For real photons with the gauge choice
$\epsilon^0=0$, only
$\mathcal{F}_1$ through $\mathcal{F}_4$ contribute. The additional amplitudes $\mathcal{F}_{5,6}$, which enter only for virtual photons, are not required here.
The quantum number $l$ is the orbital angular momentum of
the outgoing pion-nucleon system and the subscript $\pm$
represents the sign in the expression
$j=l\pm \frac{1}{2}$,
where $j$ is the total angular momentum.
Additionally, the multipoles are related to the isospin
channels by
\begin{equation}
  M_{l\pm}=\sum_I c_I M_{I,l\pm},\quad
  E_{l\pm}=\sum_I c_I E_{I, l\pm}\,,
  \label{ciDef}
\end{equation}
where $I=(\gamma p), (\gamma n),
(\gamma N)$ is the isospin channel and
coefficients $c_I$ are taken from the
corresponding decomposition in
eq.~\eqref{Channels}.
The matrix element $\calM$ is given
by~\cite{Chew, PiPhoto2009}
\begin{equation}
  \calM_{1 \mathrm{N}}
  =\calM_{\gamma N \to \pi N}
  = 8 \pi \sqrt{s} \calF\,.
\end{equation}
By convention, the factor
$1/(8\pi\sqrt{s})$ is absorbed into the
amplitudes $E_{l\pm}, M_{l\pm}$.
The matrix element $\calM_{1 \mathrm{N}}$ depends on the
initial and final Pauli spinors $\chi_i$ and $\chi_f$.
At threshold ($l=0$), this reduces to $E^{1\mathrm{N}}_{0+}$ and $L^{1\mathrm{N}}_{0+}$ as in the threshold case
\meqref{EL_decomp}.
\subsubsection{SAID Pion Photoproduction
at Threshold}
The multipole amplitudes $E_{l\pm}$ and
$M_{l\pm}$ are obtained from the SAID
partial-wave analysis database, which
provides comprehensive fits to
pion photoproduction data;
in the present work the solution
of Briscoe \etal~\cite{SAID2023piphoto}
is adopted.

At threshold, the differential cross section given in
eq.~\eqref{GeneralCS} is proportional to the outgoing
pion momentum $|\vec{q}\,|$ and consequently vanishes in
the limit $|\vec{q}\,| \to 0$. The extracted amplitudes
are therefore expected to exhibit increased sensitivity
to uncertainties in this kinematic regime, and indeed
the discrepancies observed at threshold energies can be
attributed to this kinematic suppression.

The pion photoproduction amplitudes tabulated in the SAID
database possess nonvanishing imaginary components, even
at threshold. These imaginary parts arise from the
opening of inelastic channels at nearby energies. The
charged-neutral pion mass difference
$m_{\pi^\pm} - m_{\pi^0} \approx 4.59~\MeV$
is of particular relevance in the threshold region, as it
governs the cusp structure observed in the $E_{0+}$
amplitude near the $\pi^+n$ threshold. The SAID database
reports only a single set of amplitudes at each energy
without distinguishing between the charged and neutral
pion masses. While this treatment is entirely adequate at
higher energies, which constitute the primary domain of
applicability for partial-wave analyses, establishing a
rigorous correspondence between the SAID amplitudes and
the threshold predictions obtained within \chiEFT is not
straightforward. At best, an interpolation from the SAID
values to threshold may be employed, but this introduces
substantial uncertainties.

In the SAID database, the lowest available lab frame
energy is $145 \MeV$, whereas the actual threshold for
neutral pion photoproduction is approximately
$144.7 \MeV$. The SAID naming convention labels multipoles
by the spectroscopic notation $L_{2I,\,2J}$, where $L$
denotes the orbital angular momentum of the pion-nucleon
system ($S$, $P$, $D$, \ldots), $I$ is the total isospin,
and $J$ is the total angular momentum. The letters
following the numerical label indicate the isospin channel
and type of multipole: ``pE'' denotes the proton electric
multipole (isospin-$1/2$), ``pN'' denotes the neutron
electric multipole (isospin-$1/2$), and ``NE'' denotes the
isospin-$3/2$ electric multipole. The multipole values at
$145 \MeV$ are
\begin{equation}
\begin{split}
  &S_{11}\; \mathrm{pE}\to +13.893 \times 10^{-3} /m_{\pi^+} =E_{\mathrm{\gamma p}}^{(\frac{1}{2})}\\
  &S_{11}\; \mathrm{pN}\to -16.818 \times 10^{-3} /m_{\pi^+} =E_{\mathrm{\gamma n}}^{(\frac{1}{2})}\\
  &S_{31}\; \mathrm{NE}\to -21.684\times 10^{-3} /m_{\pi^+} =E_{\mathrm{\gamma N}}^{(\frac{3}{2})}\,.
\end{split}
\end{equation}
The inferred single-nucleon multipoles
$E_{0+}^{\pi^0 p}$ and $E_{0+}^{\pi^0 n}$ are then
obtained from $\sum_I c_I E_I$, with $c_I$ from \meqref{ciDef}, which gives for the central values

\begin{equation}
\begin{alignedat}{2}
  \left(E_{0+}^{\pi^0 p}
  \right)_{\text{SAID}}
  &=-0.56\times 10^{-3} /m_{\pi^+}
  &\qquad&\gamma p \to \pi^0 p
  \;\;\text{channel}\\
  \left(E_{0+}^{\pi^0 n}
  \right)_{\text{SAID}}
  &=\;\;\;2.36\times 10^{-3} /m_{\pi^+}
  &\qquad&\gamma n \to \pi^0 n
  \;\;\text{channel}\,.
\end{alignedat}
\end{equation}
The corresponding values obtained from
$\chi$EFT are
\begin{equation}
  \left(E_{0+}^{\pi^0 p}
  \right)_{\chi\mathrm{EFT}}
  =-1.16 \times 10^{-3} / m_{\pi^{+}}
  \quad
  \left(E_{0+}^{\pi^0 n}
  \right)_{\chi\mathrm{EFT}}
  =2.13\times 10^{-3} / m_{\pi^{+}}\,.
\end{equation}
The tension between the SAID extraction and the
$\chi$EFT prediction is most pronounced for the proton
channel $\gamma p \to \pi^0 p$, where the SAID value
$(-0.56)$ amounts to less than half the magnitude of the
$\chi$EFT result $(-1.16)$.
This discrepancy reflects the large numerical
cancellation that characterizes the
$\gamma p \to \pi^0 p$ channel at threshold, where the
isospin-$1/2$ and isospin-$3/2$ contributions are of
comparable magnitude but opposite sign. Even modest
uncertainties in the individual partial-wave amplitudes
are therefore amplified in the resulting physical
multipole. For the neutron channel, the cancellation is
less severe and the agreement correspondingly better,
with the SAID value of $2.36$ differing from the
$\chi$EFT prediction of $2.13$ by approximately $11\%$.

These differences illustrate the difficulty of extracting
threshold amplitudes from partial-wave analyses that are
optimized for a broader energy range, and reinforce the
value of the direct $\chi$EFT calculation employed in the
preceding sections. For this reason, the $\calO(p^4)$
\chiEFT values of Bernard
\etal~\cite{bernard_1994,Bernard_2001} are adopted as the
primary input for the one-body kernel at threshold, and
the SAID amplitudes are reserved for use above threshold.

\subsubsection{A First Look at Above-Threshold One-Body Results}
The SAID partial-wave amplitudes described above permit
the evaluation of the one-body contribution to nuclear
pion photoproduction at arbitrary photon energies. The
full nuclear production amplitude is
$\calM = \calM_\No + \calM_\Nt$, and the unpolarized
cross section is proportional to
$|\calM_\No + \calM_\Nt|^2$, summed over spin
projections. At present, only the one-body amplitude
$\calM_\No$ has been evaluated above threshold; the
two-body contribution $\calM_\Nt$, which dominates at
threshold (sec.~\ref{sec:piphoto_combined}), has not
yet been computed above threshold owing to the
unresolved singularity discussed in
sec.~\ref{NumMethod}. The quantity shown in
fig.~\ref{fig:piphoto170MeV} is therefore proportional
to $|\calM_\No|^2$ and does not constitute the full
cross section; the two-body amplitude and all
interference terms between $\calM_\No$ and
$\calM_\Nt$ are omitted.

As a first result, fig.~\ref{fig:piphoto170MeV}
presents the one-body angular distributions at a
laboratory photon energy of $E_\gamma = 170~\MeV$, for
$\HThree$, $\HeT$, $\HeF$, and $\LiS$. At this
energy, the photon momentum exceeds the pion
production threshold and higher partial waves beyond
$S$-wave contribute to the cross section. In
particular, the $P$-wave multipoles $M_{1+}$ and
$E_{1+}$ are substantially enhanced by the proximity
of the $\Delta(1232)$ resonance, producing the
characteristic forward-peaked angular dependence
visible in all four panels. The approximate
factor-of-two ratio between the $\LiS$ and trinucleon
distributions reflects the scaling with the number of
active nucleons ($A=6$ versus $A=3$), consistent with
incoherent one-body scattering.
For $\HeF$, the distribution is qualitatively
distinct: it vanishes at threshold owing to the
$S$-wave selection rule for $J^\pi = 0^+$ nuclei, but
rises above threshold as $P$-wave and higher
multipoles become accessible. The simple $A$-scaling
observed for the other nuclei does not apply to
$\HeF$, whose distribution is comparable in magnitude
to the trinucleon systems despite having $A=4$; the
absence of the $S$-wave contribution renders $\HeF$
sensitive to different physics than the
spin-$\frac{1}{2}$ and spin-$1$ targets.
These results demonstrate that the TDA framework
combined with SAID input provides a practical tool for
predicting one-body pion photoproduction observables
on light nuclei across a range of energies. Extension
to the full cross section requires the evaluation of
$\calM_\Nt$ above threshold, which remains an open
problem in the present work.


\begin{figure}
\centering
\includegraphics[width=\linewidth]{piphoto-170MeV.pdf}
\caption[One-body pion photoproduction amplitude at $E^\gamma_{\mathrm{cm}} = 170$~MeV]{One-body ($1\mathrm{N}$) contributions to the
pion photoproduction amplitude at
$E^\gamma_{\mathrm{cm}} = 170~\MeV$ using SAID partial-wave amplitudes as input
to the TDA one-body kernel. The two-body ($2\mathrm{N}$)
contribution, which dominates at threshold and is
expected to remain significant at this energy, is not
included. The quantity plotted,
$\Tr[ \calM^{(x/y)}_{1\mathrm{N}} {\calM^{(x/y)}_{1\mathrm{N}}}^\dagger] / (64\pi^2 s A)$,
is related to the contribution of the one-body
sector to the full cross section calculation, but is not a cross section.
By rotational symmetry
$\Tr [ \calM^{(x)} \calM^{(x)^\dagger}] = \Tr[ \calM^{(y)} \calM^{(y)^\dagger}]$.
}
\label{fig:piphoto170MeV}
\end{figure}


\subsection{Summary and Outlook}

For $\HeT, \HThree,$ and $\LiS$ the two-body contribution
$E_{0+}^{2\mathrm{N}}$ dominates over the one-body
contribution $E_{0+}^{1\mathrm{N}}$, consistent with the
findings of Beane \etal~\cite{Beane_1997} and Lenkewitz
\etal~\cite{Lenke2011}. This dominance is a characteristic
feature of neutral pion photoproduction at threshold in
light nuclei and reflects the vanishing of the leading
one-body contact interaction (the Kroll--Ruderman vertex \cite{KrollRuderman})
for neutral pion production.
The relative sign between $E^{1\mathrm{N}}_{0+}$ and
$E^{2\mathrm{N}}_{0+}$ has important physical
consequences. For $\HThree$, both contributions are
negative, leading to constructive interference and the
largest total amplitude among the nuclei studied. For
$\HeT$, the positive one-body contribution partially
cancels the negative two-body contribution, resulting in a
smaller total amplitude. This renders
$\HeT$ particularly sensitive to the elementary neutron
amplitude $E_{0+}^{\pi^0 n}$, as emphasized by Lenkewitz
\etal~\cite{Lenke2011}, who demonstrated that $\HeT$
photoproduction provides a stringent test of the \chiEFT
prediction that
$|E_{0+}^{\pi^0 n}| > |E_{0+}^{\pi^0 p}|$.

Following ref.~\cite{Lenke2011} the sensitivity is quantified in
fig.~\ref{fig:E0_dependence}, which displays the
threshold scattering length $a_0$ as a function of the
elementary single-nucleon multipole for both $\HeT$ and
$\HThree$. In each panel, the complementary multipole is
held fixed at its $\calO(p^4)$ \chiEFT
value~\cite{bernard_1994,Bernard_2001}, the solid curve
represents the central TDA result, and the shaded band
reflects the combined uncertainty from the potential
variation and the two-body contribution. 
The vertical dashed line marks the $\calO(p^4)$
\chiEFT central value of the varied multipole, and
the dotted lines indicate the $\pm 5\%$ uncertainty
range assigned to the elementary amplitude, following
the estimate of Lenkewitz
\etal~\cite{LenkeThesis} as discussed in
sec.~\ref{sec:piphoto_1N_thresh}.
The selectivity arises at the level of the form factors:
$F_T^{S+V}(\HeT) \approx -0.04$ is negligible relative
to $F_T^{S-V}(\HeT) \approx 1.47$
(Table~\ref{tab:1N_3He}), so that the one-body multipole
is governed almost entirely by the neutron amplitude
$E_{0+}^{\pi^0 n}$; the mirror relation holds for
$\HThree$, whose one-body multipole is dominated by the
proton amplitude $E_{0+}^{\pi^0 p}$. The steep dependence
of $a_0$ on $E_{0+}^{\pi^0 n}$ and $E_{0+}^{\pi^0 p}$ for $\HeT$, and $\HThree$ respectively
is amplified by the partial
cancellation between the one-body and two-body
contributions; even modest
variations in the neutron multipole produce large relative
changes in the cross section. A precision measurement of the
$\HeT$ threshold cross section would therefore
place a direct constraint on $E_{0+}^{\pi^0 n}$,
complementary to the indirect extractions available from
deuteron photoproduction. 
Such a measurement could be carried out by the MAMI A2
collaboration, which has the capability to perform
threshold neutral pion photoproduction on light nuclear
targets using tagged photon beams in the relevant energy
range ($E_\gamma \approx 145$--$160~\MeV$). Among the
nuclear targets considered here, $\LiS$ is experimentally
the most accessible owing to its solid-state stability and
ease of target preparation, while $\HeT$ requires a
cryogenic gas target and $\HThree$ (tritium) presents
radiological handling challenges. A measurement on $\LiS$
would provide the first test of the two-body dominance
prediction in a $p$-shell nucleus and would probe the
$\alpha + d$ cluster structure of $\LiS$ through the
production amplitude.
\begin{figure}[H]
\centering
\includegraphics[width=\linewidth]{E0_dependence.pdf}
\caption[Sensitivity of threshold scattering length to elementary multipoles]{Sensitivity of the threshold scattering length
$a_0$ to the elementary single-nucleon multipoles for
$\HeT$ (left) and $\HThree$ (right). In each panel, the
complementary multipole is held fixed at its $\calO(p^4)$
\chiEFT value. The solid curve is the central TDA result and
the shaded band represents the combined uncertainty from
the potential variation and the two-body contribution. The
vertical dashed line indicates the $\calO(p^4)$ \chiEFT
central value; dotted lines indicate the $\pm 5\%$
uncertainty range.}
\label{fig:E0_dependence}
\end{figure}

The good convergence observed between $\calO(q^3)$ and
$\calO(q^4)$ results,  as discussed in
sec.~\ref{sec:piphoto_convergence},
indicates that higher-order corrections in
the chiral expansion are under control for these
observables. The dominant source of theoretical
uncertainty remains the $\sim 5\%$ error in the elementary
single-nucleon amplitudes from \chiEFT, as illustrated in
fig.~\ref{fig:E0_dependence}, along with the truncation
of the TDA expansion in eq.~\eqref{TDAExpansion}. 

The present work constitutes the first determination
of both transverse and longitudinal $S$-wave
multipoles for $\HThree$, $\HeT$, and $\LiS$ within
a single consistent framework. Relative to Lenkewitz
\etal~\cite{Lenke2011,Lenke2013}, it employs modern
$\chi$SMS potentials in place of the earlier chiral
\NXLO{2} wave functions, extends the calculation to
$\LiS$, and provides the longitudinal multipole
$L_{0+}$ for all targets. Relative to
Braun~\cite{BraunThesis}, it includes the
$\calO(q^4)$ static corrections for all nuclei and
provides both $L_{0+}$ and the full two-body
longitudinal form factors, neither of which were
computed by Braun. The TDA formalism further provides
a unified computational infrastructure in which pion
photoproduction, Compton scattering, and pion
scattering kernels can all be evaluated using the
same code suite and the same set of nuclear
transition densities (sec.~\ref{sec:TDA}),
eliminating the need for independent implementations
for each reaction. Additionally, a $\sqrt{2}$
discrepancy between the present $\LiS$ results and
those of Braun has been traced to an error in the
normalization of the spin-$1$ matrices employed by
Braun to extract the form factors
(sec.~\ref{ss:BraunSqrt2}). Once corrected, the
$\LiS$ results of Braun agree with the present work
to within the $\sim 13\%$ offset observed for the
trinucleon systems, an offset consistent with the
different nuclear wave functions employed.
The results of the present work are consistent with
those of Lenkewitz \etal at the $1$--$2\sigma$ level
for all dominant form factors and multipole
amplitudes, providing an independent validation using
different numerical methods and modern $\chi$SMS
potentials. The theory truncation uncertainty can be
estimated from two sources: in the one-body sector,
the boost corrections computed by Lenkewitz
\etal~\cite{LenkeThesis} indicate a $\sim 7$--$9\%$
shift of the total $E_{0+}$ amplitude
(sec.~\ref{sec:piphoto_convergence}); in the
two-body sector, the $\calO(q^3)$ to $\calO(q^4)$
shift is uniformly $\lesssim 2\%$, well below the
naive expansion parameter $Q \approx m_\pi /
\Lambda_\chi \approx 0.23$. The dominant residual
uncertainty therefore arises from the $\sim 5\%$
assignment to the elementary single-nucleon
multipoles and from the one-body boost corrections,
which have not been included in the present
calculation.

An important direction for future work is the extension of
the two-body contribution to above-threshold kinematics.
The one-body framework for above-threshold pion
photoproduction has been established in this work through
the SAID partial-wave amplitudes, but the two-body
contribution is at present restricted to threshold. As
discussed in sec.~\ref{NumMethod}, the removable
singularity in the two-body propagator becomes more
involved for nonzero pion momentum, and a suitable
variable substitution has not yet been identified.
Resolving this numerical obstacle would permit the
computation of nuclear pion photoproduction differential
cross sections and angular distributions over a broad
energy range, providing predictions that could be tested
at facilities such as MAMI.

The pion photoproduction operators treated in this section
share similar isospin and spin structure as the
pion scattering kernel and the Compton kernel. The TDA framework
therefore permits a natural extension from photoproduction
to pion scattering, which is the subject of
sec.~\ref{sec:pion}. In pion scattering, the two-body
kernel contains an analogous removable singularity that is
treated by the same variable substitution developed here,
and the comparison with pionic atom data provides an
additional test of the chiral two-body dynamics.


==> theory/theory.tex <==
%! TEX root = ../Dis-AlexanderLong.tex
\section{Theoretical Prerequisites}
\label{sec:theory}
This section introduces the general principles of
effective field theories (EFTs) that underlie the
present work. The exposition begins with a brief
overview of Quantum Chromodynamics and the
motivation for an effective description at low
energies. A pedagogical example drawn from
Newtonian gravity is used to illustrate the core
ideas of an EFT: the systematic expansion in a
small parameter, the role of symmetries in
constraining the form of the expansion, and the
estimation of truncation errors. The construction
of an effective Lagrangian from field operators is
then presented in general terms. The specific
application of these ideas to Chiral Effective Field
theory is deferred to sec.~\ref{sec:QCD}. The
following discussion draws in part on the
presentation of Lenkewitz~\cite{LenkeThesis};
see also Peskin and
Schroeder~\cite{PeskinSchroeder} for a textbook
treatment of quantum field theory and gauge
theories.

All of the reactions considered in the present work
are governed by Quantum Chromodynamics (QCD), the
non-Abelian $\mathrm{SU}(3)_{\mathrm{color}}$ gauge
theory of quarks and gluons that describes the
strong-interaction sector of the Standard
Model~\cite{PeskinSchroeder}. A defining property
of QCD is asymptotic freedom: at short distances,
or equivalently high momentum transfer and high
energy, the running coupling constant $\alpha_s$ is
small and perturbative methods are applicable. At
long distances ($\gtrsim 1\;\fm$), corresponding to
the low energies characteristic of nuclear physics,
$\alpha_s$ grows to be of order 1. In this regime, the
colored quarks and gluons are confined into
color-singlet bound states, the hadrons, and
perturbative expansions in $\alpha_s$ cease to
converge. The interaction between nucleons arises as a
residual color interaction, analogous to the van der
Waals force between electrically neutral
atoms~\cite{chiEFT}.
A direct, non-perturbative treatment of QCD on a
discretized Euclidean spacetime lattice (lattice QCD)
has made significant progress in hadron spectroscopy
and certain few-body observables, but calculations of
the scattering cross sections relevant to the present
work at the physical pion mass remain beyond current
computational reach. 

The present work therefore
adopts an alternative approach: Effective Field
Theories (EFTs). The foundational idea is due to
Weinberg~\cite{phenomLag}, who demonstrated that one
may construct an \textit{effective} theory without
having to rely on a more complicated underlying
theory. EFTs are ubiquitous, and often employed
implicitly; in a first-year physics class, students
learn that the acceleration due to gravity is
\begin{equation}
  \vec{a}_{\text{gravity}}=-g \ez=
  -9.8 \frac{\mathrm{m}}{\mathrm{s}^2}\, \ez
  \qquad\text{(height independent)}\;.
\end{equation}
This description is valid near Earth's surface but
breaks down when considering orbital motion, which is
governed by Newton's inverse-square law. For a body
at height $h$ above Earth's surface (radius $R$),
the gravitational acceleration is
\begin{equation}
  \vec{a}= -\frac{G m_{\text{earth}}}{(R+h)^2}\,
  \er,\label{FullNewton}
\end{equation}
where $G$ is Newton's gravitational constant and
$\er$ is the unit vector pointing radially outward
from Earth's center. Identifying $\er=\ez$ and
performing a Taylor expansion about $h=0$ yields
\begin{equation}
\label{NewtonGrav}
\begin{split}
  \vec{a}&=Gm_{\text{earth}}\left(-\frac{1}{R^2}
  +\frac{2 h}{R^3}-\frac{3 h^2}{R^4}
  +...\right) \ez \\
  &=\left[-9.8\, \frac{\mathrm{m}}{\mathrm{s}^2}
  +h\left(3.1\times 10^{-6}
  \frac{1}{\mathrm{s^2}}  \right)+
  h^2\left(7.2\times 10^{-13}
  \frac{1}{\mathrm{ms^2}}  \right)
  \right]\ez\;.
\end{split}
\end{equation}
From this correspondence, the height-independent term
in \meqref{NewtonGrav} is identified with the
coefficient $g$. The expansion is controlled by the
small, dimensionless ratio $h/R$: successive terms
are suppressed by additional powers of this
parameter, so that for $|h|\ll R$ the series
converges rapidly. For example, at $h=1000\;\mathrm{m}$,
the ratio $h/R\approx 1.6\times 10^{-4}$, and the
first correction is smaller than the leading term by
a factor of order $h/R$. One could go even further
and describe Earth's gravity through general
relativity, but on Earth, this leads to meaningful changes only for the most precise calculations such as GPS.
The overarching principle is that the
same physical system can be described by different
theories, and the choice of which is most appropriate
depends on the energy and resolution scale under
consideration.

The small parameter $h/R$ also provides a means of
estimating the theoretical uncertainty introduced by
truncating the series. 
If the expansion is truncated at order $n$ in the ratio $h/R$, the
omitted terms begin at order $(h/R)^{n+1}$, and this sets the
expected size of the truncation error. Crucially, this estimate
relies on the assumption that the dimensionless coefficients
multiplying each power of $h/R$ are of natural size, i.e.\ of
order unity. In EFTs, the exact form of term $n+1$ is not known in advance, and if the contribution were
anomalously large, the truncation error could far exceed the
naive estimate. This assumption, referred to as \emph{weak
naturalness}, is a prerequisite for any controlled truncation and
is discussed further below in the context of the effective
Lagrangian. More generally, in any EFT the expansion is organized
in powers of a small parameter $Q$, and the contribution at order
$Q^{n+1}$ provides an estimate of the uncertainty incurred by
working only to order $Q^n$, provided the coefficients at each
order remain natural. This logic is made precise in the context of
\chiEFT in sec.~\ref{sec:QCD}, where the expansion parameter is
the ratio of a typical momentum to the breakdown scale of the
theory.
For example, if the expansion parameter $Q\approx 0.1$,
truncation at third order yields an uncertainty of
order $Q^4 \approx 10^{-4}$, provided the
coefficients at each order are of natural size. 
With these general principles in hand, the next step
is to construct the specific effective Lagrangian
relevant to low-energy QCD. In \chiEFT, the
construction is informed by the symmetries of the
underlying theory, QCD. This is
analogous to knowing \meqref{FullNewton} and seeking
to establish \meqref{NewtonGrav}. To motivate the
procedure, consider constructing a polynomial $f$
that interpolates a set of points $(x_i, y_i)$,
$i \in \{0,\ldots,n\}$, with distinct $x_i$. The
coefficients $a_i$ can be chosen such that
\begin{align}
  f(x)&=a_0+a_1 x^1 +a_2 x^2+...+a_n x^n
  \quad\text{and}\quad f(x_i)=y_i\;.
  \label{eq:f}
\end{align}
The same idea applies when constructing effective
field theories. Since an EFT constitutes a
low-energy approximation to some underlying theory
(here, QCD), it must respect the symmetries of that
theory. In the case of the polynomial expansion, if
$f(-x)=f(x)\; \forall\; x$, i.e.,\ if $f$ is even,
then the odd powers of $x$ can be eliminated,
reducing the number of coefficients in the expansion
\begin{align}
  f(x)&=a_0+ a_2 x^2+a_4 x^4+...\;.\label{feq}
\end{align}
In the same manner that polynomials in $x$ (almost)
form a basis over the space of continuous
functions\footnote{
Every continuous function on a closed interval can be
uniformly \textit{approximated} by a polynomial
function as closely as desired. In practice, given a
data set with uncertainties
$\{x_i, y_i\pm \sigma_i\}$, a function $f$ may be
constructed with $f(x)=z$ such that
$|z_i-y_i|=\epsilon$ for $\epsilon$ as small as
desired, and in particular $\epsilon \ll \sigma_i$,
so this technical detail may be neglected.
},
a polynomial expansion in field operators and their
derivatives (almost) form a basis
over the Fock space\footnote{
Let a Hilbert space $H$ represent a single particle,
then $H^2$ represents two particles. A Fock space
$F$ represents an unknown/variable number of
particles. In a simplified case:
$F(H)=\mathbb{C}\bigoplus H \bigoplus H^2+...$,
where $\mathbb{C}$ represents the complex numbers.
}
of a Lagrangian $\LL$ in a quantum field theory.
This can be taken as an axiom, and is equivalent to
the commonly mentioned ``folk theorem'' of
Weinberg~\cite{phenomLag}, which is quoted here in
its 1997 version~\cite{wienberg1997}:
\begin{quote}
\emph{When you use quantum field theory to study
low-energy phenomena, then according to the folk
theorem you're not really making any assumption that
could be wrong, unless of course Lorentz invariance
or quantum mechanics or cluster decomposition is
wrong, [\dots]
As long as you let it be the most general possible
Lagrangian consistent with the symmetries of the
theory, you're simply writing down the most general
theory you could possibly write down. This point of
view has been used in the last fifteen years or so to
justify the use of effective field
theories,[\dots].}
\end{quote}
These field operators act as creation and
annihilation (ladder) operators of their relevant
particles. For a single scalar field, the most
general Lagrangian consistent with these
considerations takes the form
\begin{equation}
  \LL= b_0 \phi +b_1 \phi^2 +b_2 \p^2 \phi
  +b_3 \p^2(\phi^2)+b_4 \p^4 \phi
  +b_5 \p^4(\phi^2)+b_6 \p^4(\phi^3)+...\;.
\end{equation}
\begin{figure}%[H]
\centering
\includegraphics[scale=1.2]{Overfitting.pdf}
\caption[Polynomial overfitting example]{An example of polynomial overfitting. Original (solid blue) function $y=(x^2+0.7)^{-1}$, fitted to 17
points $x_i$ (red). Fitted polynomial is (dashed orange).
}
\label{fig:overfit}
\end{figure}

In general, polynomial interpolation is prone to
overfitting; see Fig.~\ref{fig:overfit} for an
example. EFTs are protected from this pathology
by the \textit{weak naturalness} assumption, which
posits that the dimensionless coefficients at each
order in the expansion are generically of order
unity~\cite{GoWrong}. In the polynomial analogy
of \meqref{eq:f}, this amounts to requiring
$|a_{i+1}/a_i|\sim\calO(1)$, so that convergence
of the series is governed entirely by powers of the
small parameter~$x$: each successive term is
suppressed by one additional power. 
Equivalently, successive terms are automatically
suppressed, $|a_{i+1}\,x^{i+1}|\ll |a_i\,x^i|$,
because the coefficients are of natural size and the
expansion parameter is small.
Without this assumption, arbitrarily large coefficients could
compensate the (relatively) small value of $x$ and render the
truncation unreliable. The weak
naturalness assumption is revisited in the context
of chiral power counting in
sec.~\ref{sec:truncation}, where it underpins
the estimation of truncation errors.

In a field theory, the addition of a constant to the
Lagrangian density,
$\LL \to \LL + c$, does not alter the equations of
motion. Similarly, the addition of a total
divergence,
$\LL \to \LL + \p_\mu V^\mu$, leaves the action
invariant (up to boundary terms). Consequently,
terms consisting of overall constants or total
derivatives need not be included. Moreover, since
$\LL$ is a Lorentz scalar, all derivative indices
must be contracted, excluding terms such as
$\p_\mu \phi$ with ``uncontracted'' indices.
In any actual calculation there are many fields that
interact with each other, such as the pion field and
the nucleon field. 
For example, consider two real, interacting, scalar fields $\psi$ and $\phi$; their most general
interaction takes the form
\begin{align}
    \LL&= c_{0} \psi + c_{1} \phi
    + c_{2} \left( \p_\mu \psi\right)\:
    \left(\p^\mu \phi\right)
    + c_3 \phi^2 + c_4 \psi^2
    + c_5 \left( \p_\mu \psi\right)\:
    \left(\p^\mu \psi\right)
    + c_6 \left( \p_\mu \psi^2\right)\:
    \left(\p^\mu \phi^2\right)
    \label{exampleEFT}\\
    &+ c_{7} \p^2 \phi + c_{8} \p^2 \psi
    + c_{9} \left(\p^2 \p_\mu \psi \right)
    \left( \p^2 \p^\mu \phi \right)
    +...\;.\nonumber
\end{align}
If the fields in \meqref{exampleEFT} are parity-even,
then odd powers such as $c_i \phi^{2k+1}$ are
forbidden by the parity symmetry. Imposing further
constraints from Lorentz invariance and
other sources, and noting that since overall
factors of $\LL$ do not alter the physics one may
divide by $c_0$ (or $c_0/2$) to eliminate one
parameter, the Lagrangian reduces
to~\cite{TwoInter}
\begin{align}
  \label{linter}
    \mathscr{L}&=\frac{1}{2}\left(
    \partial_{\mu} \phi \,\partial^{\mu} \phi
    - m_{1}^{2} \phi^{2}
    + \partial_{\mu} \psi\partial^{\mu} \psi
    - m_{2}^{2} \psi^{2}\right)
    -\frac{\lambda_{1}}{4 !} \phi^{4}
    -\frac{\lambda_{2}}{4 !} \psi^{4}
    -\frac{\lambda_{3}}{4} \phi^{2} \psi^{2}+...\;.
\end{align}
Here, the coefficients have been relabeled in terms
of the physical masses $m_1$, $m_2$, and coupling constants
$\lambda_1$, $\lambda_2$, and $\lambda_3$.
In \meqref{feq}, one could directly fit to the
points $y_i$, but since $\LL$ cannot be measured
experimentally, one instead fits to observables of
$\LL$, for example a cross section:
\begin{equation}
  \left(\frac{\dd \sigma}{\dd \Omega}
  \right)_{\text{Experiment}}=
  \left({\frac{\dd \sigma(\LL) }{\dd \Omega}}
  \right)_{\text{Theory}}\;.
\end{equation}
On the right-hand side,
$\dd \sigma /\dd \Omega$ is regarded as a function
of $\LL$ and therefore of the coefficients $c_i$, since the form of $\LL$ is specified by the previous arguments.
In principle, the effective Lagrangian extends to
arbitrarily high order in the field expansion. In
practice, however, the series must be truncated at a
given order. The choice of which terms to retain is
governed by a systematic power counting that assigns
to each contribution an expected scaling in terms of
a small dimensionless expansion parameter $Q$, exactly as the
gravity example above was organized in powers of
$h/R$. Each omitted order contributes at the level
of $\calO(Q^{n+1})$ relative to an $n$th-order
calculation, and this provides a built-in estimate of
the theoretical uncertainty due to truncation and the weak naturalness assumption. The
power counting for \chiEFT, including the precise
definition of $Q$ and the procedure for estimating
truncation errors, is discussed in detail in
sec.~\ref{sec:QCD}.

The preceding discussion has introduced the three
core principles that underlie any effective field
theory: the systematic expansion in powers of a small
parameter, the role of symmetries in constraining the
form of the effective Lagrangian, and the estimation
of theoretical uncertainties from the truncation of
that expansion based on the naturalness assumption. These ideas are general and apply to
any EFT. The next section utilizes them in the
specific case of Quantum Chromodynamics and its
low-energy effective description through Chiral
Effective Field Theory, in which the relevant degrees
of freedom are pions and nucleons and the expansion
parameter is set by the ratio of a typical momentum
to the chiral symmetry breaking scale.


==> usage/usage.tex <==
%! TEX root = ../Dis-AlexanderLong.tex
\section{Usage of the Code Suite}
\label{sec:usage}
The present work involved the development of a versatile
Fortran 90 code suite that implements the TDA formalism
for computing nuclear scattering observables. 
Fortran 90 was used because of a significant legacy code base written in it, and its high performance.
The code is compiled with the \texttt{gfortran} \cite{gfortran} compiler. 
Throughout the code base, internally, momenta are specified in units of $\MeV$ and
scattering angles are given in degrees. Given a
precomputed $\No$ or $\Nt$ nuclear transition density and
a user-supplied $\No$ or $\Nt$ interaction kernel,
respectively, the code convolves the density with the
kernel and returns the corresponding nuclear scattering
amplitude.
Considerable effort has been devoted to generalizing this
code so that a researcher wishing to compute a new \cEFT{}
reaction need only supply the process-specific kernel;
all infrastructure for density handling, angular
integration, quantum number summation, and output is
provided by the existing framework.
This section describes the steps required to implement a
new reaction within this framework, first for the
one-body ($\No$) case and then for the two-body
($\Nt$) case. The code repository is
publicly available~\cite{long_2026}.

\subsection{Overview}
\label{sec:overview}
The code is organized such that the implementation of the physics of a
particular reaction is isolated from the infrastructure
that performs the density convolution.
The process-independent framework that wraps around
the user-supplied kernel is referred to as the
\emph{mantle} code (from the German \textit{Mantel}).
The mantle handles all operations common to every
reaction: reading input parameters, loading densities,
performing quantum number summations, carrying out the
convolution, and writing output. The shared
infrastructure lives in
\texttt{common-densities/},
and the reaction-generic mantle code resides in
\texttt{onebodyvia1Ndensity/} ($\No$) and
\texttt{varsub-twobodyvia2Ndensity/} ($\Nt$).
A user implementing a new reaction should not need to
modify these files; instead, for each reaction a \textit{kernel}
directory is added
(e.g.\ \texttt{NewProcess.onebody/} or
\texttt{varsub-NewProcess.twobody/})
that contains only the process-specific pieces.
A typical kernel implementation comprises on the order
of 500~lines of Fortran source code.
See Table~\ref{tab:directories}
for the full directory layout.

For any reaction, the input to the code is specified by
the photon energy $\omega$ and scattering angle $\theta$,
translated to the kinematics of the particular reaction
(e.g.\ Compton kinematics; see
App.~\ref{sec:convert}), together with the target
nucleus ${}^AZ$ and its mass number~$A$.
The output consists of the nuclear amplitudes
$\calM_\No$ and $\calM_\Nt$, stored as matrices in the
nuclear spin projections $M$ and~$M'$, with the full
amplitude given by
$\calM_{_X}=\calM_\No+\calM_\Nt$.
The standard convention
$\dd \sigma/\dd \Omega
= \left(64 \pi^2 s\right)^{-1} |\calM_{_X}|^2$
is adopted throughout, where $s$ denotes the
Mandelstam variable.
\begin{table}[t]
  \centering
  \begin{tabular}{ll}
    \hline
    Directory & Description \\
    \hline
    \texttt{common-densities/} &
      Shared density modules (\texttt{libdensity.a}) \\
    \texttt{onebodyvia1Ndensity/} &
      Generic $\No$ mantle code \\
    \texttt{varsub-twobodyvia2Ndensity/} &
      Generic $\Nt$ mantle code \\
    \hline
    \texttt{PionPhotoProd.onebody/} &
      $\No$ pion photoproduction kernel \\
    \texttt{PionPhotoProdThresh.onebody/} &
      $\No$ threshold pion photoproduction kernel \\
    \texttt{PionPion.onebody/} &
      $\No$ elastic pion scattering kernel \\
    \texttt{varsub-PionPionThresh.twobody/} &
      $\Nt$ elastic pion scattering kernel \\
    \texttt{varsub-PionPion.twobody/} &
      $\Nt$ elastic pion scattering kernel \\
    \hline
    \texttt{documentation/} &
      Derivations and notes \\
    \texttt{tools/} &
      Python analysis and plotting scripts \\
    \texttt{tests/} &
      Verification tests \\
    \hline
  \end{tabular}
  \caption[Directory structure of the code suite]{Directory structure of the code suite.
    The top block contains process-independent
    infrastructure; the middle block contains examples of
    process-specific kernel implementations;
    the bottom block contains supporting material.}
  \label{tab:directories}
\end{table}

\subsection{The One-Body Kernel}
\label{sec:onebody-dev}
The $\No$ framework handles all operations surrounding
the kernel evaluation: reading the input file, loading the
$\No$ density from the HDF5 \cite{hdf5} archive
(a format chosen for its portability, efficient storage
of large multi-dimensional arrays, and self-describing
metadata),
summing over all quantum numbers, convolving each kernel
matrix element with the corresponding density element,
and writing the output. The user need only supply the
kernel matrix element itself.
For the $\No$ case, no integration grid is required (at tree diagram level).

To implement a new $\No$ reaction, the user creates
a directory \texttt{NewProcess.onebody/} containing
a single main file
\texttt{main.onebodyvia1Ndensity.f}. The
recommended approach is to copy an existing main file
(e.g.\ from \texttt{PionPion.onebody/}) and modify only
the section responsible for evaluating the kernel.
The computational structure of the one-body contribution
is common to all reactions considered in the present work
and is briefly recapitulated here.

The one-body piece $\calM_{\No}$ is constructed from
the single-nucleon scattering matrix of the
corresponding reaction
$\Theta N \to \Theta' N$, convolved with the
one-body TDAs of the nucleus.
Concretely, the implementation sums over an internal
index \texttt{rindx} that encodes the nuclear spin
projections $M,M'$ and the single-nucleon quantum numbers
$m_3^{s\prime}$, $m_3^s$, $m_3^t$, $m_3^{t\prime}$ at
each step. Here, $m_3^{s}$ and $m_3^{s\prime}$ denote
the incoming and outgoing spin projections of the struck
nucleon, respectively; both refer to the single active
nucleon rather than to the nucleus as a whole.
A $2\times 2$ single-nucleon matrix
$\mathcal{M}^e_N(m_3^{s\prime}, m_3^s,m_3^t,
m_3^{t\prime})$ is evaluated, and the contribution is
accumulated according to
\begin{equation}
  \calM_\No(e, M', M)
  \mathrel{+}= A \cdot \rho^{(\No)}_{\alpha,\alpha'}
  \times \mathcal{M}^e_N(m_3^{s\prime}, m_3^s,m_3^t, m_3^{t\prime})\;,
  \label{eq:1Baccum}
\end{equation}
where $e$ labels both the incoming and outgoing external
quantum numbers specific to the reaction (e.g.\ pion
charge or photon polarization), $M'$ and $M$ denote the
final and initial nuclear spin projections,
$m_3^{s}/m_3^{s'}$ are the incoming/outgoing
single-nucleon spin projections of the struck nucleon,
and the factor $A = \binom{A}{1}$ counts the number of
equivalent single-nucleon contributions,
see \meqref{TDAExpansion}.
The matrix $\calM_N$ corresponds to the isolated reaction
$\Theta N \to \Theta' N$, and the density indices
$\alpha,\alpha'$ collectively label all relevant
quantum numbers, which therefore depend on
$m_3^{s\prime}$, $m_3^s$, $m_3^t$, $m_3^{t\prime}$ and $e$.

In general, quantum numbers are half-integers; their
doubled values are therefore stored as integers
throughout the code
(e.g.\ \texttt{twoMz}$\,=2M_z$,
\texttt{twom1N}$\,=2m_3^s$).
The density is stored in an array
\texttt{rho1b(rindx)}; the mapping between this index
and the physical quantum numbers is handled entirely by
\texttt{get1Nqnnum()} and need not concern the
user beyond calling this routine.
For loop-level diagrams, the kernel evaluation requires
additional integrations over internal loop momenta. The
implementation of such contributions is beyond the scope
of the present discussion;
Ref.~\cite{Hammer3He} provides a detailed example in the
context of Compton scattering.
An example of the flow control of the one-body code can be seen below.
\begin{figure}[p]
\centering
\includegraphics[width=0.9\linewidth]{flowchart-1Bod.pdf}
\caption{One-Body code flow control}
\label{fig:OneBodyFlow}
\end{figure}
\subsection{The Two-Body Kernel}
\label{sec:twobody-dev}
The $\Nt$ framework is more involved than the $\No$ case
because, in addition to the quantum number summations, it
must perform an integration over the relative momenta
$\pv\uot, \pvp\uot$ of the active nucleon pair, see \meqref{eq:twobodysum}.
The mantle code handles the
nested loops over the $(12)$-subsystem quantum numbers
$(m_{t_{12}},\, j_{12},\, s_{12},\, l_{12},\,
m_{12})$, the analogous summation
over the primed (outgoing) quantum numbers, the
integration over two free momenta, and the
convolution with the $\Nt$ density. The user
supplies only the kernel function that is evaluated
at each quadrature point.

The directory names carry the prefix
\texttt{varsub-}, indicating the variable substitution
employed to regularize propagator singularities, as
detailed in Sec.~\ref{NumMethod}.
In the code, the integration variable $\vec{u}$ is
related to the physical outgoing relative momentum by
a substitution chosen to neutralize the singularity.
For example in the case of a diagram term proportional to
\begin{equation}
 \left[\vec{p}_{12} +\vpp\uot+ \tfrac{1}{2}(\vec{k}+\vec{k}')\right]^{-2}\;,
 \label{eq:usage_varsub}
\end{equation}
we take $\vec{u}$ as the denominator, i.e.
$\vec{u}=\vec{p}_{12} +\vpp\uot
+ \tfrac{1}{2}(\vec{k}+\vec{k}')$
and 
$\vpp\uot = \vec{p}_{12} - \vec{u}
+ \tfrac{1}{2}(\vec{k}+\vec{k}')$.
Performing this transformation maps the propagator
singularity to the origin of the integration variable,
where it is cancelled by the Jacobian of the spherical
measure.
The mantle performs this transformation automatically;
the kernel subroutine receives one physical momentum
$\pv$ and one integration variable $\vec{u}$, from which
the remaining physical momenta are reconstructed.
The case without a variable substitution amounts to
$\vec{u}=\pvp\uot$.

To implement a new $\Nt$ reaction, the user creates
a directory\\ \texttt{varsub-NewProcess.twobody/}.
The recommended approach is to copy an existing
kernel directory (e.g.\texttt{varsub-PionPion.twobody/}) and adapt the
process-specific files.

The central object the user must provide is a
subroutine that, given a set of momenta and quantum
numbers, returns the two-body kernel matrix element.
The mantle calls this subroutine at every angular
quadrature point and expects it to populate the
array
\begin{equation}
  \texttt{Kernel2B}(d,\, e,\, s_{12}',\,
  m_{s_{12}}',\, s_{12},\, m_{s_{12}})\,,
  \label{Kernel2Barray}
\end{equation}
where $d$ labels diagrams, $e$ labels external
channels (as in the $\No$ case), and the remaining
indices are the spin and spin-projection quantum
numbers of the $(12)$ subsystem.
Although the array indices in \meqref{Kernel2Barray}
do not include the momenta $\pv\uot$ and $\pvp\uot$
or the isospin quantum numbers $m_{t_{12}}$ and
$t_{12}$, the subroutine is evaluated at specific
values of these quantities at each quadrature point,
so that \texttt{Kernel2B} depends on them implicitly.
The isospin quantum numbers of the $(12)$~subsystem
enter through the outer loops of the mantle and
therefore affect the result of the convolution even
though they do not appear as explicit array indices.
All remaining operations, including the
multiplication by spherical harmonics,
Clebsch--Gordan coefficients, and density matrix
elements, are performed by the mantle.

Inside the kernel subroutine, the first step is to
reconstruct the physical outgoing relative momentum from
the integration variable as described in \meqref{eq:usage_varsub}
and sec.~\ref{NumMethod}.
Although the mantle code supplies $\vec{u}$ as the
integration variable, it is the kernel that performs
this reconstruction, since the precise form of the
substitution depends on the diagram.
The subroutine then evaluates all spin-independent
terms, such as the propagator dependence,
for each diagram, delegating the spin algebra to
dedicated helper routines.

The kernel possesses both spin-conserving
($s_{12}' = s_{12}$) and spin-changing
($s_{12}' \neq s_{12}$) contributions, each evaluated
by dedicated subroutines.
This decomposition organizes the spin algebra of
the kernel according to whether the total pair spin
is preserved or changed by the interaction.
It should not be confused with the symmetry of the
full two-nucleon state under
$(1\leftrightarrow 2)$ particle exchange, which
involves spin, orbital angular momentum, and
isospin jointly: the Pauli principle requires
$(-1)^{s_{12}+l_{12}+t_{12}} = -1$ for the
$(12)$~subsystem, so that, for example, an
isospin-singlet pair ($t_{12}=0$, antisymmetric in
isospin) admits both $s_{12}=0$ and $s_{12}=1$
depending on the orbital angular momentum $l_{12}$.
The mantle code enforces this constraint through
the quantum number summation, ensuring that only
channels satisfying $(-1)^{s_{12}+l_{12}+t_{12}}=-1$
contribute to the convolution.

Within a given allowed channel, operators whose
spin structure preserves the pair spin contribute to
$s'_{12} = s_{12}$ matrix elements, while operators
that change the pair spin connect
$s'_{12} \neq s_{12}$.
As an illustration, consider a diagram whose
spin-independent part is a scalar factor $g$ and
whose spin dependence involves a vector
$\vec{\epsilon}$.
The contribution from the diagram
in which nucleon~1 is the active nucleon reads
\begin{equation}
    \hat{O}_{1\to2}= g \,\vec{\epsilon}
    \cdot\vec{\sigma}_1\;,
    \label{eq:Oexample1}
\end{equation}
so that the total contribution is
\begin{equation}
  \hat{O}=\hat{O}_{1\to2} +\hat{O}_{2\to1}
  = g \,\vec{\epsilon}
  \cdot\left(\vec{\sigma}_1+\vec{\sigma}_2\right)\, ,
\end{equation}
where $\vec{\sigma}_{1,2}$ denote the Pauli spin
vectors of nucleons~1 and~2, respectively.
Including the exchange contribution from nucleon~2,
the symmetric ($+$) and antisymmetric ($-$)
combinations are
\begin{align}
  \hat{O}_{+} &= g\, \vec{\epsilon}
  \cdot (\vec{\sigma}_1 + \vec{\sigma}_2)\,,
  &\hat{O}_{-} &= g\, \vec{\epsilon}
  \cdot (\vec{\sigma}_1 - \vec{\sigma}_2)\,.
\end{align}

The spin-symmetric part $\hat{O}_+$ corresponds to
$s'_{12} = s_{12}$ matrix elements, while the
spin-antisymmetric part $\hat{O}_-$ corresponds to
$s'_{12} \neq s_{12}$.
The spin-dependent part of the kernel is
implemented in two separate files,
\texttt{varsub-2Bspinsym.\allowbreak NewProcess.f} and
\texttt{varsub-2Bspinasy.\allowbreak NewProcess.f},
containing the spin-symmetric and spin-antisymmetric
contributions, respectively.
These subroutines receive a scalar prefactor ($g$ in the
example above) along with the relevant momentum vectors,
and return their contribution to the \texttt{Kernel2B}
array.
The shared file \texttt{varsub-spinstructures.f}
provides utility routines for evaluating common spin
structures, such as
$\bv{\sigma}_1 \cdot \vec{A}$ (single-$\sigma$)
and $(\bv{\sigma}_1 \cdot \vec{A})\,
(\bv{\sigma}_2 \cdot \vec{B})$ (double-$\sigma$),
in the coupled
$|s_{12},\, m_{s_{12}}\rangle$ basis.
These routines are process-independent and shared across
all $\Nt$ kernel implementations within the code suite.
An example of the flow control of the two-body code can be seen below.
\begin{figure}[p]
\centering
\includegraphics[width=0.9\linewidth]{flowchart-2Bod.pdf}
\caption{Two-Body code flow control}
\label{fig:TwoBodyCode}
\end{figure}
The modular architecture of the code suite
ensures that the process-specific physics is cleanly
separated from the density-convolution infrastructure.
For both the $\No$ and $\Nt$ cases, extending the
framework to a new \cEFT{} reaction reduces to supplying
the appropriate kernel matrix elements; all remaining
operations, including density input/output, quantum
number summation, angular integration, and
spin-algebra convolutions, are inherited from the
existing mantle code.
The code repository, including documentation and
verification tests, is publicly
available~\cite{long_2026}.

